An Exploration of Multicalibration Uniform Convergence Bounds

Recent works have investigated the sample complexity necessary for fair machine learning. The most advanced of such sample complexity bounds are developed by analyzing multicalibration uniform convergence for a given predictor class. We present a framework which yields multicalibration error uniform convergence bounds by reparametrizing sample complexities for Empirical Risk Minimization (ERM) learning. From this framework, we demonstrate that multicalibration error exhibits dependence on the classifier architecture as well as the underlying data distribution. We perform an experimental evaluation to investigate the behavior of multicalibration error for different families of classifiers. We compare the results of this evaluation to multicalibration error concentration bounds. Our investigation provides additional perspective on both algorithmic fairness and multicalibration error convergence bounds. Given the prevalence of ERM sample complexity bounds, our proposed framework enables machine learning practitioners to easily understand the convergence behavior of multicalibration error for a myriad of classifier architectures.

==> Arxiv/src/0_abstract.tex <==
\begin{abstract}
{\color{black} Recent works have investigated the sample complexity necessary for
fair machine learning.  The most advanced of such sample complexity
bounds are developed by analyzing multicalibration uniform convergence
for a given predictor class.  We present a framework which yields
multicalibration error uniform convergence bounds by reparametrizing sample complexities for Empirical Risk Minimization (ERM) learning. From this framework, we demonstrate that
multicalibration error exhibits dependence on the classifier architecture as well as
the underlying data distribution.  We perform an experimental
evaluation to investigate the behavior of multicalibration error for
different families of classifiers.  We compare the results of this
evaluation to multicalibration error concentration bounds.  Our
investigation provides additional perspective on both algorithmic
fairness and multicalibration error convergence bounds.  Given the prevalence of ERM sample complexity bounds, our proposed framework enables machine learning practitioners to easily understand the convergence behavior of multicalibration error for a myriad of classifier architectures.
}\end{abstract}



==> Arxiv/src/300_SVMCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our Rademacher complexity based multicalibration uniform convergence sample-complexity bounds for the kernel SVM. As indicated earlier, an advantage of this formulation is that it yields a sample-complexity of learning for nearly any classifier, even those with infinite VC-dimension.  This Rademacher complexity approach also has the added benefit of capturing the effect of the underlying data distribution on multicalibration uniform convergence.




First, we take our description of kernels from Cortes et al. \shortcite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.  Since we are operating in the binary classification setting, we consider the set of kernel SVMs trained using hinge loss.


We prescribe notation for the thresholded hypothesis class. For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernel}$:

\begin{dmath}\label{eq:kernelHypothesisClass}
   \hypothesisClass_{\kernel} \definedAs \left\{\sample \mapsto \sgn\left(\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right) \right\}
\end{dmath}

We also prescribe notation for the non-thresholded hypothesis class.  For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernelFunction}'$:

\begin{equation}
   \hypothesisClass_{\kernelFunction}' \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\:\bf{:}\:\lvert \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) \rvert \geq 1}
\end{equation}

Cortes et al. \shortcite{cortes2010generalization} developed several generalization bounds for such kernelized predictors.  We will utilize one such bound, \cref{thm:cortesRademacher}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Simplified version of Theorem 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\kernelFunction$ be a kernel function and that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ .  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis class $\hypothesisClass_{\kernelFunction}'$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}') \leq \sqrt{\frac{23e\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

The simplification taken to yield this bound is discussed in the appendix.

We will also need a two-sided Rademacher complexity generalization bound.




\begin{theorem}[Two-sided Rademacher complexity based Generalization Bound]\label{thm:shalevRademacherImproved}
   Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $\vec{\placeholder} \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp,\vec{\placeholder})\right| \leq c$. Then
   with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
   \begin{dgroup}
   \begin{dmath}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\placeholderCount}}
   \end{dmath}
   \begin{dmath}\label{eq:RademacherEmpiricalTwoSided}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass)\\ + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
   \end{dmath}
\end{dgroup}
\end{theorem}
\Cref{thm:shalevRademacherImproved} represents a modification of Theorem 26.5 from Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding} as it establishes a two-sided Rademacher complexity bound for generalization. Ou proof of this theorem largely follows that of Shalev-Shwartz and Ben-David, and is deferred to the appendix.

The last piece of the puzzle to yield Rademacher complexity based sample-complexity bounds for multicalibration uniform convergence is to draw analogues of two  graph dimension based lemmas from Shabat et al.  We arrive at our analogues of Shabat's lemmas by upon invocation of \cref{thm:shalevRademacherImproved}.  

Before stating these lemmas, we must state the contraction lemma, which bounds the Rademacher complexity of a  function of known Lipschitz constant composed with a set of known Rademacher complexity:

\begin{lemma}[Contraction Lemma, Theorem 7 from Meir and Zhang \shortcite{meir2003generalization}]\label{lem:contraction}
  Let $\trainingData = \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ $\left\{\placeholderFunction\right\}_{i=1}^{\numSamples}$ be functions with Lipschitz constants $\placeholderScalar_i$, then
   \begin{equation}
      \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\rademacherRV_i\placeholderFunction_i(\hyp(\sample_i)) \right\} \leq \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\placeholderScalar_i\rademacherRV_i\hyp(\sample_i) \right\} 
   \end{equation} where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$.
\end{lemma} 

We use the contraction lemma to determine a bound on the Rademacher complexity of $\hypothesisClass_{\kernel}$ when given both the Rademacher complexity of $\hypothesisClass_{\kernel}'$ and the value of $\min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$: 

\begin{lemma}\label{lem:kernelHypothesisContraction}
   Let $\hypothesisClass_{\kernel} : \sampleSpace \to \left\{\pm 1\right\}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and assume $\lambda > 0$, then we have

   \begin{equation}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}) \leq \max\left\{\frac{1}{\lambda},1\right\}\rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}')
   \end{equation}
\end{lemma}

\begin{proof}
   Because $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$, exactly one of the following cases holds:

   \begin{enumerate}
      \item Case $\lambda \geq 1$:
      
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $1$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$

       \item Case $0 < \lambda < 1$:
  
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $\frac{1}{\lambda}$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$


   \end{enumerate}

   
   Taking the $\max$ over both cases and applying the contraction lemma (\cref{lem:contraction}) yields the bound.
\end{proof}
   

The core theory underpinning our main result lies in \cref{lem:shabat24analogue,lem:shabat25analogue}.  Even though neither lemma on its own represents a bound on the sample complexity of multicalibration uniform convergence, when the statements in both \eqref{eq:statement24} and \eqref{eq:statement25}  are combined, we are able to provide the sample complexity bound on multicalibration uniform convergence, which is our main result.  Shabat et al. remark upon the difficulty of directly computing a bound on the sample complexity of multicalibration uniform convergence: uniform convergence guarantees over the infinite collection of distributions induced by the infinite hypothesis class $\hypothesisClass$ and the set of interesting categories $(\group,\interval)$ is challenging \shortcite{shabat2020sample}.



\begin{lemma}[Analogue of Lemma 24 from \shortcite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \subseteq \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement24}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke our two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$ in terms of Rademacher complexity.  We accomplish this by setting $\errorTolerance$ to be less than or equal to the right side of \eqref{eq:RademacherEmpiricalTwoSided}.  Let $\numSamples_{\group}$ be the minimum number of samples necessary to satisfy the following inequality:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
      \end{dmath}
      \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




      % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

      \begin{dmath}
         \errorTolerance  \leq 23\max\left\{1,\frac{1}{\lambda^2}\right\} \frac{\scalarBound^2}{\numSamples_\group} + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
      \end{dmath}


      \intertext{Which gives us, after algebraic manipulation}

      \begin{dmath}
         \numSamples_{\group} < \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
      \end{dmath}

   \end{dgroup}
      
Lastly, we know that if $\left|\trainingData_{\group}\right| > \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$, then $\left|\trainingData_{\group}\right| > \numSamples_{\group}$ which completes the proof.
\end{proof}

The proof technique for \cref{lem:shabat25analogue} is identical to that of \cref{lem:shabat24analogue}.

\begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}'} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement25}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

Now that we have the necessary lemmas stated, we may state our main result: a sample complexity bound for multicalibration uniform convergence, defined in~\eqref{eq:multicalibrationUniformConvergence}, which depends on the Rademacher complexity of hypothesis class $\hypothesisClass_{\kernel}$ with respect to sample $\trainingData$:

\begin{theorem}[Main Result]\label{thm:OurBoundSVM}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$,  $\hypothesisClass_{\kernel}$ has the multicalibration uniform convergence property with 

{\small
\begin{dmath}
   \sampleComplexity_{\hypothesisClass_{\kernel}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2 + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}
}
\end{theorem}

This bound on the sample complexity exhibits a similar form as that of Shabat et al.:

\begin{dmath}\label{eq:shabatVCBound}
   \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

where $\graphDimension$ is the graph dimension\footnote{The graph dimension is a multi-class generalization of the VC-dimension} of hypothesis class $\hypothesisClass$.

The main difference, however, is that Rademacher complexity based bound has a direct dependence on the test-set margin and the kernel's sensitivity. Our bound has no explicit dependence on the VC dimension of the chosen hypothesis class, as we show in \cref{fig:adult_nn_bounds,fig:compas_nn_bounds}. These differences imply classifier-agnostic bounds for multi-calibration uniform convergence are unlikely to be effective in practice as notions of fairness are themselves data-dependent. Take for example the RBF kernel; this kernel has an infinite VC dimension, yet for all $\sample \in \sampleSpace$ we know $\kernelFunction(\sample,\sample) \leq \scalarBound^2 = 1$. Hence, our bound can provide a more meaningful sample complexity bound for group fairness. 

While \cref{thm:OurBoundSVM} is fairly specific to the kernel SVM, it is possible to derive sample complexity bounds for multicalibration uniform convergence on other architectures by composing the relevant analogues to \cref{lem:shabat24analogue,lem:shabat25analogue} and replacing the Rademacher complexity of the kernel SVM with a (preferably tight) Rademacher complexity bound suitable for the choice of architecture. For instance,  one such family of classifiers is the feedforward ReLU network. An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al. \shortcite{bartlett2017spectrally}. This bound has a dependence on the number of samples, the norm of the input, and a couple varieties of matrix norm computed on the weight matrices.

% Let us now illustrate the utility of our bound on the RBF kernel SVM.
% \begin{example}[Example Instantiation of Bounds]. Consider the RBF kernel SVM, i.e. $\kernel_{\eta}(\sample,\sample')  = \exp\left(-\eta\norm{\sample'- \sample}_2^2\right)$ where $\eta$ is a positive real number and let $\gamma,\psi,\epsilon,\delta \in (0,1]$.  It is easy to see that $\scalarBound = 1=\max_{\sample} \kernel_{\eta}(\sample,\sample)$. which grants us a finite upper-bound on sample complexity by \cref{thm:OurBoundSVM}.  

% Compare this to the bound of Shabat et al. (\eqref{eq:shabatVCBound}):  The RBF kernel SVM is known to have an infinite VC dimension. Hence the bound presents an upper bound of infinity on the sample complexity.

% \end{example}







% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 






% \begin{theorem}[Corollary 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:CortesGeneralization}
%    Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
%    \begin{equation}
%       \risk_\hyp \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
%    \end{equation}
%    where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
% \end{theorem}






% With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

% \begin{theorem}
% \label{thm:OurBoundSVM}
% Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
% \small{
%   \begin{dmath}
%       \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
%   \end{dmath}
%   }
% \end{theorem}  
% \begin{proof}[Proof Sketch]
% The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
% \end{proof}

% Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  








==> Arxiv/src/A100_proofs.tex <==
%!TeX root = ../note.tex
\section{Existing Lemmas and Definitions}

In this section we re-state, for completeness, several lemmas which appear in the paper by Shabat et al.  In our main paper, for the lemmas stated here which have a dependence on VC dimension and/or graph dimension of an underlying hypothesis class, we developed analogues with dependence on the class's Rademacher complexity.

\begin{lemma}[Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.   Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 25 from \cite{shabat2020sample}]\label{lem:shabat25}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let ${\group} \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 26 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat26}
   Let $p_1,p_2,\tilde{p}_1,\tilde{p}_2,\epsilon,\psi \in [0,1]$ such that $p_1,\psi \leq p_2$ and $\left|p_1-\tilde{p}_1\right|,\left|p_2-\tilde{p}_2\right| \leq \psi\epsilon/3$.  Then,

   \begin{equation}
      \left|\frac{p_1}{p_2} - \frac{\tilde{p}_1}{\tilde{p}_2}\right| \leq \epsilon
   \end{equation}

\end{lemma}

\begin{lemma}[Lemma 27 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat27}
   Let $\gamma \in (0,1)$ and let $\Gamma_\gamma = \left\{\group \in \Gamma \given \Pr_{\sample \drawnFrom \sampleDist}\left[\sample \in \group\right] \geq \gamma\right\}$ be the collection of subpopulations from $\Gamma$ that has probability at least $\gamma$ according to $\sampleDist$.  Let $\errorConfidence \in (0,1)$ and let $\trainingData$ be a random sample of $\numSamples$ drawn i.i.d. from $\sampleDist$.  Then with probability at least $1-\errorConfidence$, if $\numSamples \geq \frac{8\log\left(\frac{\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$,

   \begin{dmath}
      \forall \group \in \Gamma_{\gamma} \hiderel{:} \left|\trainingData \intersection \group\right| \hiderel{>} \frac{\gamma \numSamples}{2}
   \end{dmath}

\end{lemma}

\begin{remark}[Remark on Theorem 1]
Firstly, we expand on the simplification from Theorem 2 by Cortes et al. taken to yield \cref{thm:cortesRademacher}.  Our \cref{thm:cortesRademacher}, which is a simplification of theorem 2 as by given Cortes et al. \cite{cortes2010generalization}, is a bound on the hypothesis class consisting of a non-negative combinations of at least two kernels. Given a set $\placeholderCount \geq 2$,  The authors' theorem 2 applies to the hypothesis class denoted $\hypothesisClass_{\placeholderCount}^1$ where

\begin{dmath}
\hypothesisClass_{\placeholderCount}^1 \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^{\placeholderCount}\alpha_i\kernelFunction_i, \norm{\weights} \leq 1, \vec{\alpha} \geq 0, 1= \sum_{i=1}^{\placeholderCount}\alpha_i \right\}
\end{dmath}

Our non-thresholded hypothesis class $\hypothesisClass_{\kernel}'$, on the other hand, consists of only one kernel:

\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :   \norm{\weights} \leq 1\right\}
\end{dmath}

 



Hence, when invoking the bounds from Cortes et al., we implicitly consider our hypothesis class to be non-negative combinations of our kernel and a dummy kernel $\kernelFunction_{\mathrm{dummy}}$.  The dummy kernel is assumed to always have weight $0$.  We accomplish this by re-writing $\hypothesisClass_{\kernel}'$ as
\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :  \kernelFunction = 1\cdot \kernelFunction + 0\cdot\kernelFunction_{\mathrm{dummy}}, \norm{\weights} \leq 1\right\}
\end{dmath}


\end{remark}



==> Arxiv/src/A300_proof_thm_3.tex <==
\section{Proof of \Cref{thm:OurBoundSVM}}

Our proof of \cref{thm:OurBoundSVM} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize Rademacher complexity instead of VC dimension.


\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to subpopulation ${\group}$. Let $\hypothesisClass_{\kernel}$ denote the hypothesis class defined in \eqref{eq:kernelHypothesisClass}. Let $\Gamma_\gamma$ denote the set of all subpopulations $\group \in \Gamma$ which have probability at least $\gamma$:
   \begin{dmath}
      \Gamma_{\gamma} \definedAs \left\{{\group} \in \Gamma \given \Pr_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
   \end{dmath}

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
   \begin{dmath}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{dmath}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\interval)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
   \end{align}

   By \cref{lem:shabat24analogue}, we know  for any $\predictionValue \in \labelSpace$ and any ${\group} \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{dgroup}
   \begin{dmath}
      \numSamples_1 \geq \frac{64\log\left(\frac{4}{\errorConfidence'}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{(\epsilon')^2}
   \end{dmath}
   \begin{dmath}
      = \frac{64\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{\left(\frac{\psi\errorTolerance}{3}\right)^2}
   \end{dmath}
   \begin{dmath}
      = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
   \end{dmath}
\end{dgroup}
   then we have

   
\begin{dmath}
   \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{dmath}
By \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any subpopulation ${\group} \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \left\{-1,1\right\}$, where

\begin{dmath} 
   \numSamples_2 \geq\frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
\end{dmath}

then we also have 

   \begin{dmath}
         \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{dmath}
   Set $\numSamples^\marker$ such that 
   \begin{dmath}
    \numSamples^\marker = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
   \end{dmath}
   Then, if for all subpopulations ${\group} \in \Gamma_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

   \begin{dgroup}
      \begin{dmath}\label{eq:calibrationClosenessA}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}\label{eq:calibrationClosenessB}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  = \frac{1152\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 414\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\gamma\errorTolerance^2\psi^2} 
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \Gamma_\gamma$. Recall there are at most $\left|\Gamma \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \Gamma_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{dgroup}
      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{dgroup}
   \begin{dmath}
      p_1(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      p_2(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_1(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_2(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
   \end{dmath}
\end{dgroup}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$:

\begin{dmath}
   {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \Pr\left[\sample \in {\group}\right] \hiderel{\geq} \gamma,  \Pr\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi \implies
   \left|\calibrationError(\hyp,{\group},\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
\end{dmath}

which completes the proof.


\end{proof}




% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to subpopulation $U$.  Let $\Gamma_\gamma$ denote the set of all subpopulations $U \in \Gamma$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \Gamma_{\gamma} \definedAs \left\{U \in \Gamma \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all subpopulations $U \in \Gamma_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \Gamma_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\Gamma}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\Gamma}} = \frac{1}{2\abs{\hypothesisClass}\abs{\Gamma}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.


==> Arxiv/src/A400_proof_NN.tex <==
\section{Proof of \Cref{thm:OurBoundSVM}}


Let us consider multicalibration uniform convergence bounds on depth $\depth$ ReLU networks.  Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$ Hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\weightMatrix = (\weightMatrix_1,\dotsc,\weightMatrix_\depth)$, where $\weightMatrix_{i} \in \realNumbers^{\dimension_{i}\times\dimension_{i-1}}$ where $\dimension = \dimension_0$. In the binary classification setting, we have $\dimension_{\depth} = 1$, and in the multi-class setting, we have $\dimension_{\depth} = \abs{\labelSpace}$.  Let $\nonlinearity(\cdot)$ be the ReLU function.  $\nonlinearity(\vec{\placeholder})$ applies the ReLU to each coordinate in $\vec{\placeholder}$. Such networks are of the form
\begin{equation*}
    \weightMatrix_{\depth}\nonlinearity\left(\weightMatrix_{\depth-1}\nonlinearity\left(\cdots\nonlinearity\left(\weightMatrix_{1}\sample\right)\cdots\right)\right)
\end{equation*}
\begin{theorem}[\cite{bartlett2017spectrally}]
Consider the neural network hypothesis class
\begin{equation}\label{eq:neuralNetworkHypothesisClass}
    \hypothesisClass_{\neuralNetwork} = \left\{\hyp_{\weightMatrix}(\sample) : \weightMatrix : \left(\weightMatrix_1,\dotsc,\weightMatrix_\depth\right), \norm{\weightMatrix_i}_2 \leq \placeholder_i, \norm{\weightMatrix_i^{\transpose}}_{2,1} \leq \placeholder'_{i}, i \in \left\{1,\dotsc,\depth\right\}\right\}
\end{equation}
Then we have 
\begin{equation*}
    \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{\sfrac{3}{2}}} + \frac{26\log(\numSamples)\log(2\dimension_{\max})}{\numSamples}\norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}
\end{equation*}
where $\vec{X}$ are the unlabeled training data $\trainingData$, i.e. $\vec{X} = \left[\sample_1,\dotsc,\sample_N\right]$
\end{theorem}
Our proof of \cref{thm:OurBoundSVM} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize Rademacher complexity instead of VC dimension.


% \left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}

Let us begin by proving a lemma that will be helpful for proving a multicalibration uniform convergence bound.

\begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
   Let $\hypothesisClass_{\neuralNetwork}$ be a ReLU neural network predictor class. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \groups$ be a population group, and assume 
   
   \begin{equation*}1 \leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \end{equation*}  
   
   Furthermore, let   Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is $\sampleDist$ conditioned on examples being members of group $\group$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of 
   
   \begin{equation*}
       \left|\trainingData_\group\right| \geq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}
   \end{equation*} 
   examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
  \begin{dmath}
      \forall \hyp \hiderel{\in} \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]\right| \hiderel{\leq} \errorTolerance
  \end{dmath}
\end{lemma}

\begin{proof} Our proof strategy is to invoke a two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$:
     \begin{dgroup}
      \begin{dmath}
         \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
      \end{dmath}
      \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




      % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

      \begin{dmath}
         \errorTolerance  \hiderel{\leq} \frac{8}{\numSamples_\group^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples_{\group})\log(2\dimension_{\max})}{\numSamples_{\group}}\norm{\vec{X}}_{\Frobenius}\hiderel{\cdot}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \hiderel{+} 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}
            \begin{dmath}
         \leq \frac{8}{\numSamples_\group^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples_{\group})\log(2\dimension_{\max})}{\numSamples_{\group}^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}
      
      \intertext{Let us now assume that }
         \begin{dmath*}1 \leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \end{dmath*}  
    \intertext{Which gives us}
       \begin{dmath}
         \errorTolerance \leq  \frac{60 \log(2\dimension_{\max})}{\numSamples_{\group}^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}


      \intertext{Which gives us, after algebraic manipulation}

      \begin{dmath}
 \numSamples_{\group} \leq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}      
 \end{dmath}

   \end{dgroup}
   
\end{proof}


\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to group ${\group}$. Let $\hypothesisClass_{\neuralNetwork}$ denote the hypothesis class defined in \eqref{eq:neuralNetworkHypothesisClass}.  Recall that $\gamma$ is the lowest frequency amongst groups $\group \in \groups$ present in the training data $\trainingData$:
   

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups$:
   \begin{dmath}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{dmath}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\interval)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
   \end{align}

   By \cref{lem:shabat24analogue}, we know  for any $\predictionValue \in \labelSpace$ and any ${\group} \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{dgroup}
   \begin{dmath}
      \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence'}\right)}{(\errorTolerance')^2} 
   \end{dmath}
   \begin{dmath}
      =       \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\frac{4}{\frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}}\right)}{(\frac{\psi\errorTolerance}{3})^2} 
   \end{dmath}
   \begin{dmath}
      =       \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2} 
   \end{dmath}
\end{dgroup}
   then we have

   
\begin{dmath}
   \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{dmath}
By \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any group ${\group} \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \labelSpace$, where

\begin{dmath} 
     \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2} 
\end{dmath}

then we also have 

   \begin{dmath}
         \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{dmath}
   Set $\numSamples^\marker$ such that 
   \begin{dmath}
    \numSamples^\marker = \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2}  \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
   \end{dmath}
   Then, if for all groups ${\group} \in \groups_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

   \begin{dgroup}
      \begin{dmath}\label{eq:calibrationClosenessA}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}\label{eq:calibrationClosenessB}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs   \frac{129600\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 1152\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\gamma\psi^2\errorTolerance^2} 
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \groups_\gamma$. Recall there are at most $\left|\groups \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \groups_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{dgroup}
      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{dgroup}
   \begin{dmath}
      p_1(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      p_2(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_1(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_2(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
   \end{dmath}
\end{dgroup}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$:

\begin{dmath}
   {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\  \Pr\left[\sample \in {\group}\right] \hiderel{\geq} \gamma,  \Pr\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi \implies
   \left|\calibrationError(\hyp,{\group},\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
\end{dmath}

which completes the proof.


\end{proof}

% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to group $U$.  Let $\groups_\gamma$ denote the set of all groups $U \in \groups$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \groups_{\gamma} \definedAs \left\{U \in \groups \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all groups $U \in \groups_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \groups_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\groups}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\groups}} = \frac{1}{2\abs{\hypothesisClass}\abs{\groups}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.


==> Arxiv/src/B1_Inequalities_and_facts.tex <==
% !TeX root = ../note.tex

\section{Important Inequalities and Facts}

We begin by stating facts and inequalities necessary for our proofs:

\begin{lemma}[From \url{https://math.stackexchange.com/questions/171241/approximations-for-the-partial-sums-of-exponential-series}]\label{lem:expPartialSum}

    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}

\end{lemma}

\begin{lemma}[Frech\'et Inequality]\label{lem:frechet}
    Let $\event_1,\dotsc,\event_{\placeholderCount}$ be probabilistic events.  The following is true:
    
    \begin{equation}
        \Pr{\bigIntersection_{i=1}^{\placeholderCount} \event_i} \leq \min_{i} \Pr{\event_i}
    \end{equation}
    
    \end{lemma}



    \begin{theorem}[Hoeffding's Inequality \cite{hoeffding1963probability}]\label{\hoeffding}. Let $\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_{\placeholderCount}$ independent random variables strictly bounded by the intervals $\bracket{a_i,b_i}$, then

        \begin{equation}
            \Pr{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i - \sum_{i=1}^{\placeholderCount}\E{\placeholderRandomVariable_i}} \geq \placeholder} \leq \exp\paren*{-\frac{2\placeholderCount^2\placeholder^2}{\sum_{i=1}^{\placeholderCount}\paren*{b_i-a_i}^2}}
        \end{equation}
        
        \end{theorem}

        \begin{definition}
            The $\ell_1$ distance between any two distributions $\placeholderDist_1,\placeholderDist_2$ is defined as 
            \begin{equation}
                \norm{\placeholderDist_1-\placeholderDist_2}_1 \definedAs \sum_{\placeholder \in \support\paren*{\placeholderDist_1} \union \support\paren*{\placeholderDist_2}} \abs{\placeholderDist_1(\placeholder)-\placeholderDist_2(\placeholder)}
            \end{equation}
            \end{definition}

            \begin{lemma}[Lemma from Thomas and Cover \cite{coverthomas1991elements}]\label{lem:pinsker}
                \begin{equation}
                \infdiv{\placeholderDist_1}{\placeholderDist_2} \geq \frac{1}{2 \ln 2}\norm{\placeholderDist_1-\placeholderDist_2}_1^2
                \end{equation}
                \end{lemma}

                \begin{theorem}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{thm:chernoffNice}
                    Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
                    \begin{align}
                        \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
                             \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
                    \end{align}
                    \end{theorem}
                    
                    \begin{corollary}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{cor:chernoffNice}
                        Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\errorConfidence > 0$ then
                        \begin{align}
                            \Pr{\paren*{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}} && 0 \leq \frac{\errorTolerance}{\E{\randomVariable}}\leq 1
                        \end{align} 
                        \end{corollary}
                    
                        \begin{proof}
                            \begin{align}
                            \Pr{{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} + \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\errorTolerance} \\
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \placeholderCount\errorTolerance} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\placeholderCount\errorTolerance}
                            \intertext{Putting $\errorTolerance$ in terms of the parameters in \cref{thm:chernoffNice}, we see that $\errorTolerance = \relativeErrorTolerance \E{\randomVariable}$}
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} \\
                            &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}}
                            \end{align}
                        \end{proof}


\begin{lemma}\label{lem:multinomialDistributionBound}
    Let $\vec{\placeholder} \in \realNumbers^{\dimension}$ be a vector of probabilities.  That is, for $i \in \set{1,\dotsc,\dimension}$, we have $0 \leq \placeholder_i \leq 1$ and $1=\sum_{i=1}^{\dimension}\placeholder_{i}$.  Furthermore, the entries of $\vec{\placeholder}$ are ordered such that $\placeholder_1 \geq \placeholder_2 \geq \dotsc \geq \placeholder_{\dimension}$.  Then for all $i \in \set{1,\dotsc,\dimension}$, we have
    
    \begin{equation}
        \placeholder_i \leq \frac{1}{i}
    \end{equation}
    \end{lemma}
    \begin{proof}
        todo
    \end{proof}
    
                    

==> Arxiv/src/img/tex/binsForLearner.tex <==
%!TeX root = ../../../note.tex
 

\begin{tikzpicture}
\foreach \x in {0,...,5}{
\draw (\x*2,0) rectangle (\x*2+1, 1);};
\node  at (6*2+0.5,0.5) {$\ldots$}  ;
\draw (7*2,0) rectangle (7*2+1, 1);
\draw[black,fill=black] (0.5, 0.5) circle (0.1);
\end{tikzpicture}

==> Arxiv/src/old_stuff/2_related_work.tex <==
\section{Background}



% As machine learning systems have exhibited exemplary performance across a wide variety of tasks, the scope of their use has broadened.  Impactful life decisions which in the past have been rendered exclusively by humans, such as college admission and mortgage approval, are now using machine learning systems to supplement, or even outright replace, humans in the decision making process.  This shift in how such important decisions are made has sparked a new field of machine learning research: \emph{fairness}. 

% Much of modern ML fairness literature is concerned with the implications of learning classifiers via empirical risk minimization (ERM), or some variant thereof, subject to what is known as a fairness constraint.  A fairness constraint is typically formulated as a constraint on the optimization objective which is dependent on the value of a so-called \emph{protected attribute} (also referred to as a \emph{sensitive attribute}). Examples include the fairness constraints known as \emph{statsitical parity} (also referred to as \emph{demographic parity}) introduced by Dwork et al. \citep{dwork2012fairness} and \emph{equality of opportunity} introduced by Hardt et al. \citep{hardt2016equality}.  Most importantly, these works assume access to a fairness constraint which can be enforced during ERM, which is to say, it is known precisely which constraints are required to make the resulting trained classifier fair.  We refer to the setting in which the protected attribute is available to the learner as \emph{learner assessable fairness}.

% When the protected attribute is not available to the learner, the learner is unable to evaluate the fairness of classifier.  In such situations, fairness of the learned classifier is assessed by a meta-learner which \emph{does} have access to the protected attribute.  This setting we refer to as \emph{learner remitted fairness}. In learner remitted fairness, a learner only has access to information about the underlying data distribution.  Examples of such information include, but are not limited to the number of protected groups, and the frequency of each protected group.  The exact information to which a learner has access is often context dependent.

% Multicalibration is a well studied quantity which captures the fairness of a classifier in the learner remitted fairness setting: Hebert-Johnson et al. were the first to develop and study the notion of multicalibration \cite{hebert2017calibration}.  In particular, the authors develop algorithms for learning multicalibrated predictors 
 

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.





==> Arxiv/src/old_stuff/3_5_calibration_concentration.tex <==
%!TeX root = ../note.tex
\section{Concentration Inequalities for Multi-calibration}

We begin this section by stating a sample-complexity bound for multi-calibration uniform convergence from Shabat et al. \cite{shabat2020sample}

\begin{theorem}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Furthermore assume that groups $\set{U_1,\dotsc,U_{\abs{\Gamma}}}$ may overlap.Then $\hypothesisClass$ has the uniform multicalibration convergence property with
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\gamma,\psi} = \bigOh\paren*{\frac{\log\paren*{\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}}{\errorTolerance^2\gamma\psi}}
    \end{equation}

\end{theorem}

We will improve upon this bound by utilizing the structure which the assumption of mutually exclusive groups provides:

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    The ``bad'' event $B^{\trainingData}$ is the event in which denotes the existence of an interesting category for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$:

    \begin{equation}
        B^{\trainingData} \definedAs \set*{\trainingData : \exists \hyp \in \hypothesisClass, \exists (U,I) \in C_{\hyp} : \abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance}
    \end{equation}

    We also define the ``good'' event $G^{\trainingData,\placeholder}$, which is the event that each interesting category in $\trainingData$  contains at least $\placeholder$ samples:

    \begin{equation}
        G^{\trainingData,\placeholder} \definedAs \set*{\trainingData : \forall \hyp \in \hypothesisClass, \forall (U,I) \in C_{\hyp} : \abs{(U_{\trainingData},I)} \geq \placeholder }
    \end{equation}

    Note that the ``bad'' event and the ``good'' event are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    \begin{equation}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}
    \end{equation}

    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Now, we upper-bound this quantity:

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\
        &\leq  \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C_{\hyp}} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}\\
        &\leq 4\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\lambda}\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}



   \begin{equation}
    \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}  \iff \placeholder \geq \frac{2}{\errorTolerance^2}\log\paren*{\frac{8\abs*{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}
   \end{equation}

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   
   \begin{align}
    \Pr{\abs{\paren*{U_\trainingData,I}} \leq \placeholder} &\leq Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
    &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
    &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
   \end{align}
\end{proof}



With only lower bounds on the frequency of an ``interesting'' category, our bounds are remarkably similar to those
Let's now analyze the case of the finite hypothesis class but in the leave $k$ out setting.  That is, given $k$, a non-negative integer less than $\abs{\Gamma}$, what is the sample complexity necessary for at least $\abs{\listInterestingCategories_{\hyp}} -k$ groups to satisfy the fairness criteria?


\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  

 

    We also define the ``good'' event $G^{\trainingData,\placeholder,m}$, which is the event that at least $\abs{C}-m$ interesting categories in $\trainingData$  contain at least $\placeholder$ samples.

    Note again the ``bad'' events and the ``good'' events are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    We now define a new ``bad'' event, distinct from the event defined in the previous proof.  Let $B^{\trainingData,\listInterestingCategories}$ be the event which denotes the existence of at least $1$ interesting category in set $\listInterestingCategories$ for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$.  Suppose we have a function $\goodGroups$ which takes in, as an argument, the event $G^{\trainingData,\placeholder,m}$ and returns the powerset of exactly $\numInterestingCategories-k$ distinct categories $(U,I)$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$ holds true. That is to say, for any integer $k$, $\goodGroups\paren*{G^{\trainingData,\placeholder,k}}$ $\numInterestingCategories - m$ categories which satisfy this condition.

    WE further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\listInterestingCategories} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.
    
    Event $B^{\trainingData,l,\listInterestingCategories}$ occurs when at least $l$ categories $(U,I)$ in list $\listInterestingCategories$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$

    Let $\listInterestingCategories^k$ denote the list of all possible combinations of $k$ interesting categories.  In order to have leave-$k$-out fairness, we bound 
    
    \begin{align}\Pr{\bigIntersection_{i=1}^{\abs{\listInterestingCategories}} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \sum_{\listInterestingCategories' \in \listInterestingCategories^k}\prod_{i=1}^k \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder} \given \bigIntersection_{j=1}^{i-1}\curlyBrace*{B_{\interestingCategory_j}^{\trainingData} \union \lnot G_{\interestingCategory_j}^{\trainingData,\placeholder}} }\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k} \subseteq \listInterestingCategories} \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k}} \errorConfidence\\
    &= \errorConfidence^{k}
    \end{align}



 
    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Suppose we wish to have leave-$k$-out fairness.  Then must we have $l+m\geq k$
    
    Then the event we are interested upper-bounding is:

    
    \begin{align}
        \Pr{B^{\trainingData,\listInterestingCategories_\hyp^{\marker},l} \given G^{\trainingData,\placeholder,m}} &\leq \sum_{\hyp \in \hypothesisClass} \Pr{B_{\interestingCategory_1}^{\trainingData,\listInterestingCategories_\hyp^{\marker} \setminus \set*{}} \intersection B_{\interestingCategory_2}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_1}} \intersection \hdots \intersection  B_{\interestingCategory_l}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_i}_{i=1}^{l-1}}} \\
        &\leq \sum_{\hyp \in \hypothesisClass} \binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}\\
        &\leq \abs{\hypothesisClass}\binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}
    \end{align}

    where $\listInterestingCategories_{\hyp}^{\marker}\definedAs \goodGroups\paren*{G^{\trainingData,\placeholder,m}}$

    which suggests

    \begin{equation}
        \frac{\errorConfidence}{2} \geq \abs{\hypothesisClass}\binom{\listInterestingCategories_{\hyp}-m}{l}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^l \iff \placeholder \geq \frac{2}{\errorTolerance^2}\ln\paren*{4\sqrt[l]{\binom{\abs{\listInterestingCategories_{\hyp}}-m}{l}\frac{2\abs*{\hypothesisClass}}{\errorConfidence}}}
    \end{equation}

    Let us now bound $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}}$ 

    In order to compute this bound, we further decompose the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    We upper-bound the complement of the good event, $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,m}}}$, by translating it into the language of category-wise good events,$G^{\trainingData,\placeholder,\listInterestingCategories}_{\interestingCategory}$ , into it's category-wise good events:

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{}}_{\interestingCategory_1} \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_1}}_{\interestingCategory_2} \intersection \hdots \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_i}_{i=1}^{m-1}}_{\interestingCategory_m}}\\
        &\prod_{i=1}^m
    \end{align}



    In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$, hence we have

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
        &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
        &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
       \end{align}


    % \Pr{\set*{\bigcup_{\listInterestingCategories \in \goodGroups\paren*{G^{\trainingData,\placeholder,k}}}\trainingData \in B^{\trainingData,l,\listInterestingCategories}} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{B^{\trainingData,k} \in \powerSet_{\trainingData,k}}\sum_{(U,I)\in C_{\hyp}\setminus \badGroups\paren*{B^{\trainingData,k}}}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData,l,\listInterestingCategories} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq 4\binom{\abs{\listInterestingCategories}}{l}\abs{\hypothesisClass} \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}

The bad event is not so simple.  If we are considering leave 

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   

\end{proof}

==> Arxiv/src/old_stuff/3_7_calibration_concentration.tex <==
%!TeX root = ../note.tex

\subsection{Multi-calibration uniform convergence in the Poisson Model.}

\begin{theorem}  Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then, for the Poisson model, we have the following sample-complexity for leave $k$ out fairness:
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\poissonRate_{\interestingCategory},k} = \bigOh\paren*{\frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\poissonRate_\interestingCategory\errorTolerance^2}}
    \end{equation}
\end{theorem}

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  
    We further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\hyp} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder,\hyp} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.

    In order to have leave-$k$-out fairness, there must be at least $k$ distinct categories $\interestingCategory$ for which at least one of the following is true:

    \begin{enumerate}
        \item Good event $G_{\interestingCategory}^{\trainingData,\placeholder}$ does \emph{not} occur
        \item Bad event $B_{\interestingCategory}^{\trainingData,\listInterestingCategories}$ does occur
    \end{enumerate}

    \begin{align}
        \Pr{\lnot G_{\interestingCategory}^{\trainingData,\placeholder}} &= \Pr{\abs{\interestingCategory} \leq \placeholder} \\
        &\leq \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}
        % &= \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}
    \end{align}

    where $\regularizedGammaFunction$ is the regularized gamma function:

    \begin{equation}
        \regularizedGammaFunction(\placeholder_1,\placeholder_2) \definedAs \frac{\GammaFunction\paren*{\placeholder_1,\placeholder_2}}{\GammaFunction\paren*{\placeholder_1}} = \frac{\int_{\placeholder_2}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}{\int_{0}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}
    \end{equation}

    Let us now bound $\Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}}$:

    \begin{align}
        \Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}} &\leq \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}}  \\
        &\leq 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}


    Let $\listInterestingCategories^{k}$ denote the set of all combinations of $k$ categories in $\listInterestingCategories$.  All together, we have:

    \begin{align}
\Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} +\exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}}^k\\
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\placeholder_{\interestingCategory}}^2}{2\poissonRate_{\interestingCategory}}}}}^k 
            \intertext{assume $\placeholder \leq \poissonRate_{\interestingCategory}/2$}
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}}}^k  \label{eq:PoissonUnionBound}\\
    \end{align}

    % \begin{align}
    %     \Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}^k\\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}}^k \\
    %                 &= \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\sum_{i=0}^{\placeholder}\frac{\poissonRate_{\interestingCategory}^i}{i!}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\paren*{e^{\poissonRate_{\interestingCategory}}-\frac{\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate}\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &< \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate_{\interestingCategory}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}\exp\paren*{-\paren*{\placeholder+1}+\frac{1}{12\placeholder + 13}}}}}}^k \\
    %                 &=\paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{\exp\paren*{-\poissonRate_{\interestingCategory}+\placeholder+1-\frac{1}{12\placeholder+13}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}}}}}^k \label{eq:PoissonUnionBound}\\
    %         \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the left-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}} & \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}& \leq \frac{k\errorConfidence^{\frac{1}{k}}}{8 e \abs{\listInterestingCategories}} \\ 
        \placeholder &\geq \frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\errorTolerance^2}
    \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the right-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\exp\paren*{-\frac{\paren*{\placeholder}^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{ k\errorConfidence^{\frac{1}{k}}}{2e\abs{\listInterestingCategories}} \\
       \placeholder& \geq \sqrt{2\poissonRate_{\interestingCategory}\ln\paren*{\frac{2e\abs{\listInterestingCategories}}{ k\errorConfidence^{\frac{1}{k}}}}} \\
    \end{align}

\end{proof}



    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}




\begin{lemma}
    \begin{align}
      \binom{\abs{\listInterestingCategories}}{k}^{\frac{1}{k}} < \paren*{\frac{1}{\sqrt{2\pi}}\frac{\abs{\listInterestingCategories}^{\paren*{\abs*{\listInterestingCategories}+\frac{1}{2} }}}{\paren*{\abs*{\listInterestingCategories}-k}^{\abs*{\listInterestingCategories}-k + \frac{1}{2}}k^{k+\frac{1}{2}} }}^{\frac{1}{k}}
    \end{align}

\end{lemma}

\begin{lemma} Let $a,b$ be integers such that $a \geq b \geq 1$ (from wiki)
    THe following are true:
    \begin{equation}
        \frac{a^b}{b^b} \leq \binom{a}{b} \leq \frac{a^b}{b!} \leq \paren*{\frac{e\cdot a}{b}}^{b}
    \end{equation}
\end{lemma}

==> Arxiv/src/old_stuff/3_RevisitingResidualHypothesisBoosting.tex <==
\section{Revisiting Residual Hypothesis Boosting}
% In this note we present a boosting framework for any sequential composition of functions.
% For the rest of note let $T \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $T$ feature transformations:
% $$F(\sample) = (G_T \circ G_{T-1} \circ \cdots \circ G_1)(\sample),$$
% where $G_t$ ($t \in [T]$) is some function. Note that $G_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $G_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically say a CNN.
% The final binary classifier is determined by another weight vector $\weights_T$ of appropriate shape,
% where the classification is determined as
% $$\sign(\weights_T^{\transpose}F(\sample))$$
% We will use the notation $G_{1:t}$ to mean the composition $G_t \circ G_{t-1} \circ \cdots \circ G_1$.
% We further use the notation $g_t \definedAs G_{1:t}$ to mean the composition of the first $t$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
The weight vectors $\weights_1, \dots, \weights_{T-1}$ will not appear in the final classifier, but they are used to
guide training. Specifically, the following proposition is straightforward:
\begin{proposition}[Final hypothesis is sum of residuals]
  The final hypothesis is the \emph{sum of residual hypotheses} scaled by $1/\alpha_T$:
  \begin{align*}
    \weights_T^{\transpose}F(\sample) = \frac{1}{\alpha_T}\sum_{t=0}^{T-1}h_t(\sample)
  \end{align*}
\end{proposition}
Therefore we can focus on training $\sum_{t=1}^Th_t$, and we can do it simply by AdaBoost.
In fact, let us see what is going on there: Let $K \in [T]$, and suppose that $h_1, \dots, h_{K-1}$
have been trained (when $K=1$, we have $0$ to start with), and our goal is to train a hypothesis
$\sum_{t=1}^Kh_t$ to minimize the training error. That is
\begin{align}
  \minimize_{h_0,\dots,h_{K-1}} \sum_{i=1}^\numSamples \exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right)
\end{align}
where we have been using exponential loss. We note that:
\begin{align}
  &\exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right) \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right) + (-y_ih_{K-1}(\sample_i))\right) && \text{($h_0, \dotsc, h_{K-2}$ have been trained)} \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right)\right) \exp(-y_ih_{K-1}(\sample_i)) \\
  = &\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))\exp(-y_ih_{K-1}(\sample_i)) \\
\end{align}
Here the term $\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i)$ is viewed as a ``weight'' we assigned to each training point.
In AdaBoost there is a specific iterative weighting procedure to turn these weights into a proper probability distribution.
That probability distribution will be important for the theory, so we repeat that derivation here:
\begin{itemize}
\item The end goal is to turn these terms into
  \begin{align}
    D_{K}(i) = \frac{\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))}{\sum_{j=1}^\numSamples\exp(-y_j\alpha_{K-1}o_{K-1}(\sample_j))}
  \end{align}
\item Note that we know that
  \begin{align}
    \alpha_{K-1}o_{K-1} \definedAs \sum_{t=1}^{K-1}h_t
  \end{align}
  It turns out that such a distribution can be constructed recursively as follows:
  \begin{enumerate}
  \item Start with a uniform distribution on all the training points: $D_0(i) = \frac{1}{N}$.
  \item Then for $t = 1, 2, \dots$,
    \begin{align}
      \label{def:recursive-weighting}
      D_t(i) = \frac{D_{t-1}(i)\exp(-y_ih_t(\sample_i))}{\sum_{j=1}^\numSamples D_{t-1}(j)\exp(-y_jh_t(\sample_j))}.
    \end{align}
  \end{enumerate}
\end{itemize}
Therefore at the stage $K$ of AdaBoost, the minimization problem is equivalent to:
\begin{align}
  \label{def:stage-K-objective}
  \minimize_{h_K}\sum_{i=1}^\numSamples D_{K-1}(i)\exp(-y_ih_K(\sample_i))
\end{align}
Let us now open $h_K$ a little, by definition
\begin{align*}
  h_{K-1}(\sample) &= \alpha_Ko_K(\sample) - \alpha_{K-1}o_{K-1}(\sample) \\
         &= \alpha_K\weights_K^{\transpose}G_K(g_{K-1}(\sample)) - \alpha_{K-1}o_{K-1}(\sample)
\end{align*}
The unknowns here are only $\alpha_K, \weights_K$, and $G_K$ (the feature transformation at step $K$),
and therefore the minimization problem at boosting stage $K$ can be rewritten as:
\begin{align*}
  (\alpha_K, \weights_K, G_K) = \argmin_{\alpha, w, G} \sum_{i=1}^\numSamples D_{K-1}(\sample_i)\exp\left(
  -y_i \left(\alpha \cdot w^{\transpose} \cdot G(g_{K-1}(\sample_i)) - \alpha_{K-1}o_{K-1}(\sample_i)\right)\right)
\end{align*}
\begin{remark}
  If one plugs in the ResNet where $G_K(g_{K-1}(\sample_i)) = f_K(g_{K-1}(\sample_i)) + g_{K-1}(\sample_i)$,
  then the goal is to identify $f_K$. This recovers BoostResNet!
\end{remark}

\section{On proving that training error will vanish}

We now give a key observation of why this general residual hypothesis boosting can quickly make
the training error vanish. The argument here is really already in the proof of AdaBoost.
We want to repeat it here because it demonstrates again that there is nothing special in BoostResNet about ResNet!
Here is the key argument: In binary classification we eventually want to bound the following:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\exp\left(-y_i\left(\sum_{t=0}^{T-1}h_t(\sample_i)\right)\right)
\end{align}
This can be turned into a sum of product:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp\left(-y_ih_t(\sample_i)\right)
\end{align}
Basically, this recursive nature of $D_K$ allows us to turn this \emph{sum of product} into \emph{product of sum}.
That is:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i))
  &= \sum_{i=1}^{\numSamples}\Big\{D_0(i)\exp(-y_ih_0(\sample_i))\Big\}\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples} \left\{D_1(i)\left(\sum_{j=1}^mD_0(j)\exp(-y_jh_0(\sample_j))\right)\right\} \prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples}D_1(i)Z_1\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i))
\end{align}
where we define $Z_1 \definedAs \sum_{j=1}^mD_0(j)\exp(-y_jh_1(\sample_j))$,
which measures the quality of residual hypothesis $h_1$. Continue doing this we have:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i)) = \prod_{t=0}^{T-1}Z_t
\end{align}
where
$$Z_t \definedAs \sum_{j=1}^\numSamples D_{t}(j)\exp(-y_jh_t(\sample_j)).$$
This is the key why we can bound training error!

==> Arxiv/src/old_stuff/4_NNCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Neural Networks and Fairness}

Our technique for deriving sample complexity bounds is not just limited to the kernelized classifier, but we are able to compute multicalibration uniform convergence bounds any hypothesis class for which the Rademacher complexity is defined.  One such family of classifiers is the feedforward neural network:

Each hypothesis $\hyp_{\neuralNetwork}$ in the hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\mat{W} \definedAs \left(\mat{W}_1,\mat{W}_2,\dotsc,\mat{W}_\depth\right)$.  For $i \in \left\{1,\dotsc,\depth\right\}$, we assume $\mat{W}_i \in \realNumbers^{\dimension_i \times \dimension_{i-1}}$ where $\dimension_0$ is the dimension of the input vector $\sample$ and $\dimension_{\depth} = 1$.  We let $\nonlinearity(\cdot)$ denote the rectified linear unit (ReLU), i.e. for $\vec{\placeholder} \in \realNumbers^{\dimension}$, $\nonlinearity(\vec{\placeholder}) \definedAs \max\left\{\vec{\placeholder},\vec{0}_\dimension\right\}$ and is applied element-wise to $\vec{\placeholder}$. The neural network is formulated as:



\begin{dmath}
    \hyp_{\mat{W}}'(\sample) \definedAs \mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))
\end{dmath}

and the decision version of the neural network is formulated as:

\begin{dmath}\label{eq:NNHypothesisClass}
        \hyp_{\mat{W}}(\sample) \definedAs \sgn\left(\mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))\right)
\end{dmath}
An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al \cite{bartlett2017spectrally}.  We use the ``nice'' formulation of the bound from Yin et al. \cite{yin2019rademacher}.

\begin{theorem}[Theorem 5 from Yin et al.]
    Consider the neural network hypothesis class \begin{dmath}\hypothesisClass_{\neuralNetwork} \definedAs \left\{\hyp_{\neuralNetwork} : \mat{W} = (\mat{W}_1,\dotsc,\mat{W}), \\ \forall i \in \left\{1,\dotsc,\depth\right\}: \norm{\mat{W}_i}_{\sigma} \leq \spectralBound_i, \norm{\mat{W}_i}_{2,1} \leq \normBound_i\right\} \end{dmath}

    Then we have 

    \begin{dmath}
        \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{3/2}} + \frac{26\log\left(\numSamples\right)\log\left(2\dimension_{\max}\right)}{\numSamples}A
    \end{dmath}
    where $A=\norm{\mat{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\spectralBound_i \right)\left(\sum_{j=1}^{\depth} \left(\frac{\normBound_j}{\spectralBound_j}\right)^{2/3}\right)^{3/2}$
\end{theorem}

Using techniques similar to those of the previous section, we are able to determine sample complexity bounds for multicalibration uniform convergence in feedforward ReLU networks.  In particular, we develop lemmas similar to \cref{lem:shabat24analogue,lem:shabat25analogue}, but for feedforward ReLU networks:

\begin{lemma} Let $\hypothesisClass_{\neuralNetwork}$ be as defined in \cref{eq:NNHypothesisClass}.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a subpopulation.  Furthermore, let $\lambda = \min_{\hyp'\in \hypothesisClass_{\neuralNetwork}',\sample \in \sampleSpace}\left\{\hyp'(\sample)\right\}$

\end{lemma}
Scratch:
\begin{dgroup}
    \begin{dmath}
        \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\neuralNetwork}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{4}{\numSamples_{\group}^{3/2}} + \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Assume for some $\alpha \in \realNumbers_+$, $\frac{4}{\numSamples_{\group}^{3/2}} \leq \alpha \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A $}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\frac{\sqrt{\numSamples_\group-1}}{\numSamples_\group}\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(2\dimension_{\max}\right)}{\sqrt{\numSamples_{\group}}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation:}
        \begin{dmath}
                \errorTolerance^2 \leq 8\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{26^2(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
            \begin{dmath}
                = 5408\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
        \intertext{Algebraic Manipulation}
        \begin{dmath}
                \numSamples_{\group} \leq \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2} + \frac{64{\log\left(4/\errorConfidence\right)}}{\errorTolerance^2}
        \end{dmath}
\end{dgroup}
 

==> Arxiv/src/old_stuff/4_ballsandbins.tex <==
%!TeX root = ../note.tex

\section{Balls and Bins}\label{sec:ballsAndBins}


Before investigating the behavior of our fairness on general loss function, we seek to develop intuition via a ``balls-and-bins'' perspective: We imagine the learner, blind to protected feature $\sampleProtected$, must classify each sample (the ball) in $\trainingData$ with exactly one of $\abs{\labelSpace}$  labels (the bins).  After all examples in $\trainingData$ have been classified, a meta-learner which has access to all features of any sample, including the protected feature $\sampleProtected$.

\begin{figure}
    \input{src/img/tex/binsForLearner.tex}
\end{figure}


We may view fairness with a balls and bins perspective.  Within the two group setting in which the elements of $\labelSpace$ are discrete, we examine $\numSamples_+$ and $\numSamples_-$ impact an empirical fairness metric.  We again consider the setting in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$, however the protected groups are not always balanced: $\Pr{\sampleProtected = \groupA}$ is not necessarily equal to $\Pr{\sampleProtected = \groupB}$.

We now share our first bound on our fairness metric, which arises from two invokations of the union bound.  We utilize the following fact in our to construct our bounds: we utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$.  Note the dependence on number of labels $\abs{\labelSpace}$ appears both inside and outside the exponential. 

\begin{theorem}\label{\thmOne}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}
\end{equation}

\end{theorem}





\begin{proof}
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
    &\leq \sum_{\labelElement \in \labelSpace}\exp\paren*{-\frac{\numSamples_{+,\labelElement}\placeholder^2}{\abs*{\labelSpace}}} + \exp\paren*{-\frac{\numSamples_{-,\labelElement}\placeholder^2}{\abs*{\labelSpace}^2}}\label{eq:applyHoeffdingInequality}\\
        &\leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}\label{eq:applySimplification}
\end{align}
\end{proof}

\Cref{\thmOne} does gives us some intuition about our machine learning fairness. Namely, our fairness metric has no explicit dependence on the accuracy of our classifier.  Furthermore, this bound is broadly applicable as it is agnostic to underlying classification architecture: The bound has dependence only on the sample distribution $\sampleDist$.  This upper-bound on fairness has a dependence on the number of labels $\abs{\labelSpace}$ and the number of the lowest number of samples assigned to a (label $\labelElement$, group $\sampleProtected$) pair.

The  dependence on $\abs{\labelSpace}$ is in fact suboptimal -- the above bound is na\"vely constructed.  Whereas we only used the fact that probabilities are bounded between $0$ and $1$, we may use knowledge that the sum of all probabalistic events is $1$ to tighten our bound and yield \cref{thm:Two}.  More formally, we know:

\begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i} \end{equation} 




We will show in \cref{\thmTwo} that we can indeed eliminate the dependence on $\abs{\labelSpace}$  outside the exponential by utilizing the fact: \begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i}\end{equation}



The bound presented in $\cref{\thmOne}$ is also loose: We applied a union bound several times to arrive at $\cref{eq:applyUnionBound}$ which is an upper-bound on the left side of $\cref{eq:triangleInequality}$. By using Hoeffding's inequality, we only utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$, hence our bounds implicitly assume that the random variable $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has the maximum variance of a random variable bounded over such an interval, yet it cannot be the case, that when $\abs*{\labelSpace}\neq 2$ $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has maximum variance for each $\placeholder, \marker$ pair, as we know 

\begin{equation}
    1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}
\end{equation}

Lastly, we compare \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification}:  if the number of samples assigned to each label $\labelElement \in \labelSpace$ is balanced, then \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification} evaluate to similar quantities.  On the other hand, if there exists a label $\labelElement$ in label space $\labelSpace$ such that the number of samples assigned to that label is a small, positive rational number, then it is not hard to see  \cref{eq:applySimplification} is a very loose upper bound on \cref{eq:applyHoeffdingInequality}.  Naturally, the question which follows is, can we do better?  Indeed, we can do better, as we prove in \cref{\thmTwo}

\begin{theorem}\label{\thmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \frac{\numSamples_{ \sampleProtected,\labelElement}}{1}$

\end{theorem}


\begin{proof}
    
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
        \shortintertext{Utilizing \cref{cor:chernoffNice} with $\errorTolerance = \frac{\placeholder}{2\abs{\labelSpace}}$:}
    % &\leq \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{+,\labelElement}}{3}} +  \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{-,\labelElement}}{3}}\\
    &\leq\sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{+,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} +  \sum_{\labelElement \in \labelSpace}2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{-,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}\\
    &\leq \sum_{\labelElement \in \labelSpace} 4\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} \\
    \intertext{We invoke \cref{lem:multinomialDistributionBound} to yield the right-hand-sum:}
        &\leq 16\sum_{i=2}^{\abs{\labelSpace}} \exp\paren*{-\frac{ i\placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}} \\
        \intertext{We utilize \cref{fact:geometricSeriesFinite}, which gives a closed-form expression for a finite geometric series}
    % &=  8\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}-8 - 8\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}\\
    &<  16\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}-1} \\
    %  &=  8\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}-1+\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}}\\
          &<  16\paren*{\frac{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}}
          \shortintertext{Assume $\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}} < \sfrac{1}{2}$}
          & <  32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}^2+1}} \\
          &<32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{align}
\end{proof}

Let us now discuss \cref{\thmTwo}.  Much like in \cref{\thmOne}, the bound we present here shows that our choice of fairness metric has no dependence on the accuracy of the underlying classifier.  The bound in $\cref{\thmTwo}$ exhibits a tighter dependence on $\abs{\labelSpace}$. Indeed the discrepancy between the bounds presented in \cref{\thmOne} and \cref{\thmTwo} becomes more significant as the number of labels $\abs{\labelSpace}$ increases.  

While the implications of both \cref{\thmOne,\thmTwo} are similar, the proof of $\cref{\thmTwo}$ is more intricate: we utilize the fact that $1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}$ by invoking lemma \cref{lem:multinomialDistributionBound}.  We also invoke the Chernoff bound, \cref{thm:chernoffNice}, which can be far tighter than Hoeffding's Inequality.

Let us now devise a bound for the case that $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$. The bound follows from \cref{\thmTwo} and \cref{lem:pinsker}

\begin{corollary} \label{\corThmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} + \sqrt{2\ln\paren{2}\infdiv{\sampleDist_a}{\sampleDist_b}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{corollary}

Compared to the bounds presented in \cref{\thmOne} and \cref{\thmTwo}, the bound presented in \cref{\corThmTwo} provides a bound on our fairness metric when the distribution of labels depends on the group.




==> Arxiv/src/old_stuff/5_lowerBounds.tex <==
!TeX root = ../note.tex

\section{Lower Bound}
Let us now develop a lower bound on $    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder}$. 

\begin{theorem}\label{thm:lowerBound}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
\end{theorem}


\begin{proof}  
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
    &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
        &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
        &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
                &\geq 1- \paren*{1-\exp\paren*{-2\placeholder^2\numSamples_{\min}}}\label{eq:postAbsIntersection}\\
                &= \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{align}

Where to relate \cref{eq:preAbsIntersection} to \cref{eq:postAbsIntersection}, we used both Hoeffding's inequality (\cref{\hoeffding}) that for any non-negative $\placeholder$:
\begin{equation}
    \Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}} \leq \min \curlyBrace*{\Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}, \Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}>-\placeholder}}
\end{equation}
\end{proof}
Indeed, this lower bound is similar to that which is presented in \cref{\thmTwo}.  Notably, no $\abs{\labelSpace}$ term appears in the exponent. Note this lower bound is tightest when $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  A sharper bound for the case in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$ has not been developed.

{\color{blue}
CURRENTLY IN PROGRESS
\begin{theorem}\label{thm:lowerBound}
    Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  Furthermore, for all $\labelElement^{\marker} \in \labelSpace$ assume $\Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \labelElement]{\labelElement = \labelElement^{\marker}} \geq \placeholderScalar$ where $0 < \placeholderScalar < \frac{1}{\abs{\labelSpace}}$:
    \begin{equation}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq ??
    \end{equation}
    where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
    \end{theorem}

    \begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
        &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
            &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
            &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
            &\geq 1- \paren*{1-\exp\paren*{-\frac{\numSamples\placeholder^2}{2\paren*{1-\placeholderScalar\paren*{\abs{\labelSpace}-1}}\paren*{\placeholderScalar\paren*{\abs{\labelSpace}-1}} + \frac{2\placeholder}{3}}}}\\
    \end{align}
}

==> Arxiv/src/old_stuff/6_LossFunctions.tex <==
%!TeX root = ../note.tex
\section{Fairness and (Un-)Bounded Loss Functions}

In \cref{sec:ballsAndBins}, we examined fairness in the context of counting.  Let us now compare examine fairness in the context of positive-valued loss functions.  Let $\loss$ be a  positive-valued loss function, that is $\loss : \sampleSpace \times \labelSpace \to (0,\infty)$.

Let $\lossContribution_{\groupA}$ denote the total loss contribution from group $\groupA$

That is
 
\begin{equation}
    \lossContribution_{\evalutationData,\groupA} \definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)
\end{equation}

Similarly, we define the loss contribution from the group $\groupA$, label $\labelElement$ pair:

\begin{equation}
    \lossContribution_{\evalutationData,\groupA,\labelElement} \definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
\end{equation}

% \begin{theorem}\label{\thmOne}
%     Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
%     \begin{equation}
%         \Pr{\sum_{\labelElement \in \labelSpace}\abs{\lossContribution_{\evalutationData,\groupA,\labelElement} -\lossContribution_{\evalutationData,\groupB,\labelElement}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}}}}
%     \end{equation}
    
%     \end{theorem}


Our interest lies in bounding

\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder}
\end{equation}

Note that for all labels $\labelElement \in \labelSpace$, we have $0<\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}<1$. Furthermore, we know $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$
  
% In particular, for any $\labelElement \in \labelSpace$, we have $0 \leq \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} \leq 1$.  Furthermore, we have $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$.  These facts allow us to provide tight bounds on $ \Pr{\sum_{\labelElement \in \labelSpace}\abs{ \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} > \placeholder} $


\begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder}  
\end{align}

\begin{align}
    \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x=\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \cdot e^{tx} \differential x
\end{align}



Let us upper-bound the variance of such a random variable.

\begin{align}
    \variance\bracket*{X} &= \E{X^2} - \E{X}^2 \\
    &\leq  \E{X^2} \\
    &= \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x}} \cdot x^2 \differential x \\
    &\leq \E{X}
\end{align}

\begin{theorem}[Bhatia-Davis Inequality]
    Let $X$ be a random variable.  $X$ is bounded between $0$ and $1$, i.e. $X \in [0,1]$.  Then
    \begin{equation}
        \variance(X) \leq \paren*{1-\E{X}}\paren*{\E{X}}
    \end{equation}
\end{theorem}

\begin{theorem}[Bernstein Inequality]
    Suppose $
\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_\placeholderCount$ are i.i.d. random variables with zero mean.  If for all $i$, $\abs{\placeholderRandomVariable_i} < \scalarBound$, then for all $\placeholderCount > 0$

\begin{equation}
    \Pr{\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i > \placeholder} \leq \exp\paren*{-\frac{\placeholderCount\placeholder^2}{2\variance\paren*{\placeholderRandomVariable} + \frac{2\scalarBound \placeholder}{3} }}
\end{equation}

\end{theorem}

\begin{theorem}\label{thm:UnboundedLossFairnessUB}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
    \end{equation}
    where \begin{align}
        \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
        \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
    \end{align}
    \end{theorem}
\begin{proof}
Without loss of generality, we assume that $i \in \set{1,\dotsc,\abs{\labelSpace}}$, we have $ \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \geq \dotsc \geq  \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_{\abs{\labelSpace}}}}{\lossContribution_{\evalutationData,\groupA}}}$, then we know $\E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \leq \frac{1}{i}$


\begin{align}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder/2} + \Pr{\sum_{i = 1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder/2} \\
    &\leq \sum_{i = 1}^{\abs{\labelSpace}} \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\ 
    % \begin{split}\leq \sum_{\labelElement \in \labelSpace} \brparen*{\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
    %      \qquad \qquad+\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}}}
    % \end{split}\\
   &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}}\label{eq:theoremFollowsFromHere}
   \intertext{We now invoke the Bhatia-Davis Inequality in combination with \cref{lem:multinomialDistributionBound}}
   &\leq \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &< \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} + \frac{1}{6}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}  + \frac{1}{6}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} }}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}} \\
    \begin{split}\leq 2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
+2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
   \end{split}\\
%    \begin{split}\leq 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
%     +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
%        \end{split} \\
%        \begin{split}= 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
%         +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
%            \end{split} \\
           \begin{split}= 2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
            +2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
               \end{split} \\
               \intertext{Assume $\frac{1}{2}\geq\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}$}
              &\leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }\\
    \end{align}
\end{proof}

\begin{corollary}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } +  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
    \end{equation}
\end{corollary}




% On sub-Gaussianity of random variables:

% \begin{definition}
%     Let $\placeholderRandomVariable$ be a random variable with expectation $\E{\placeholderRandomVariable}$.  If $\placeholderRandomVariable \drawnFrom \subGaussian(\proxyStandardDeviation^2)$, then for any $t > 0$
%     \begin{align}
%         \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} > t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}} &\text{and}&& \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} < -   t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}}
%     \end{align}

% \end{definition}

% \subsection{Does the Bhatia-Davis bound on variance also a bound on proxy-variance?}

% Let $X$ be a random variable bounded between $0$ and $1$.

% \begin{align}
%     \Pr{\placeholderRandomVariable = 1} =  \Pr{\placeholderRandomVariable -\E{\placeholderRandomVariable} > 1-\E{\placeholderRandomVariable}} \leq \E{X}
% \end{align}

% Now we compare $\E{\placeholderRandomVariable}$ with $\exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}}$

% \begin{align}
%     \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}} &\leq \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\E{\placeholderRandomVariable}\paren*{1-\E{\placeholderRandomVariable}}}} \\
%     &= \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}}{2\E{\placeholderRandomVariable}}} \\
%     &= \exp\paren*{\frac{\E{\placeholderRandomVariable}-1}{2\E{\placeholderRandomVariable}}} \\
%     &=\exp\paren*{\frac{1}{2}}\exp\paren*{-\frac{1}{2\E{\placeholderRandomVariable}}}\\
% \end{align}     

==> Arxiv/src/old_stuff/7_lossFunctionDifference.tex <==
%!TeX root = ../note.tex
\section{The Weakness of Simple Ratios}

The ratio-type fairness bounds developed in the previous section are informative to fairness, their weakness is demonstrated in the following example:

\begin{example}
     Suppose for each $\labelElement \in \labelSpace$, $\lossContribution_{\evalutationData,\groupA,\labelElement}$ and $\lossContribution_{\evalutationData,\groupB,\labelElement}$ are positive-valued random variables, and $\placeholderScalar \neq 1$ is a positive-valued real number.  Given $\lossContribution_{\evalutationData,\groupA,\labelElement} = \placeholderScalar\lossContribution_{\evalutationData,\groupB,\labelElement}$, we see that $ 0=\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}$.  Our ratio based fairness metric suppresses the fact that when $\placeholderScalar > 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} > \lossContribution_{\evalutationData,\groupB,\labelElement}$, and when $\placeholderScalar < 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} < \lossContribution_{\evalutationData,\groupB,\labelElement}$.  We conclude that while a naive ratio-based fairness metric is informative, it suppresses differences between total loss contributions among groups.
\end{example} 

Hence, it is useful to capture in our fairness metric differences between total loss contributions among groups AND any discrepancy in ratios which the  naive ratio-based fairness metric captures.  Therefore, we consider the following fairness metric:


\begin{theorem}\label{thm:LossFunctionDifference}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
     \end{equation}
     where \begin{align}
         \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
         \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
     \end{align}
     \end{theorem}
\begin{proof}
\begin{align}
     \begin{split}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} 
     &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          & + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split} \\
     \begin{split}
          &\leq \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
          & + \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}}
     \end{split} \\
     \begin{split}
     &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}} \\
     &+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}}}
     \end{split}
\end{align}
Since $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$ and  $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$, the the rest of the proof is identical to the proof of \cref{thm:UnboundedLossFairnessUB} from equation \cref{eq:theoremFollowsFromHere} to end.
\end{proof}

\begin{corollary}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }+  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
     \end{equation}
 \end{corollary}

\hrule

Given the weakness of such naive ratio-based fairness metrics, we analyze a fairness metric which has utility in when loss is unbounded -- and avoids the pitfall of the fairness metric in the above example.  We consider 

\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}


We recognize that the above quantity is bounded by \begin{align}
     \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} &=  \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}} }
\end{align}

It is clear that both $\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}} \leq 1$ and $\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}}  \leq 1$ are true, but what can we say about $     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}}$ and $
\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}}$?

{\color{blue} The above function is not always easily interpretable}


\hrule
\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}

\begin{align}
     \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} &\leq \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }, \frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\lossContribution_{\evalutationData,\groupA} }},\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\lossContribution_{\evalutationData,\groupB} }}}
\end{align}

\begin{align}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} \leq 
     \begin{split}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split}
\end{align}



\hrule


Let us now consider $\max_{\labelElement_1,\labelElement_2 \in \labelSpace} \abs*{\log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupB,\labelElement_1}}} - \log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_2}}{\lossContribution_{\evalutationData,\groupB,\labelElement_2}}} }$

Suppose the distribution of losses is identical for both group $\groupA$ and group $\groupB$




==> Arxiv/src/old_stuff/__latexindent_temp.tex <==
!TeX root = ../note.tex
\section{Boosting and Fairness}

We now consider the multiclass boosting framework from Huang et al \cite{huang2018learning} in the context of fairness.
 

Trivial Bound[Bad]


\begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{theorem}

\begin{proof}
\begin{align}
\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
&\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{align}
\end{proof}

A better bound...

Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


\begin{lemma}
    Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
    \begin{equation}
        \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
    \end{equation}
\end{lemma}

Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  That is, we investigate 
\begin{equation}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\sample \in \unlabeledTrainingData \given \sampleProtected \in \groupA}\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} }{\groupWeight_{\groupA}}-\frac{\numSamples_{-,\labelElement}}{\groupWeight_{\groupB}}} > \placeholder}\end{equation}

where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$


\begin{align}
123
\end{align}
% \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> Arxiv/src/old_stuff/old_background.tex <==
% !TeX root = ../note.tex


\section{Background}


% \subsection{Notation and Definitions}

% Within thI is paper, we adopt the following notational conventions:

We consider a setting where we have an input set $\sampleSpace \subseteq \realNumbers^{\dimension}$ and a label set $\labelSpace$.  A sequence of examples is denoted as $\trainingData{} \subseteq \sampleSpace \times \labelSpace{}$ and contains the $\numSamples$ examples which constitute the population group.

Let $\Gamma_{\trainingData} = \set{\group_1,\dotsc,\group_{\abs{\Gamma}}}$ be a finite collection of subsets of $\trainingData$, heretoforth refered to as \emph{population subgroups}.  We follow the lead of existing multicalibration literature and assume population groups may be overlapping \cite{shabat2020sample,hebert2017calibration}.  $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  Our setting is that of binary classification: $\labelSpace = \left\{\pm 1\right\}$.  Since the labels in $\labelSpace$ are discrete, we also have $\Lambda = \left\{\pm 1\right\}$.


We now discuss our notation population subgroups: Given set of examples $\trainingData$ which will be clear from context, For each group $\group \in \Gamma_\trainingData$, $\left|\trainingData_{\group}\right|$ denotes the number of samples in $\trainingData$ within subgroup $\group$ and $\left|\trainingData_{(\group,\interval)}\right|$ denotes the number of samples in $\trainingData$ within category $(\group,\interval)$

% We now discuss the Poisson Process from which population groups are constructed:

% Samples belonging to each category $\interestingCategory \in \listInterestingCategories$ arrive in the population according to a Poisson Process with rate $\poissonRate_{\interestingCategory}$.  In this paper, we will assume $1 = \sum_{\interestingCategory \in \listInterestingCategories} \poissonRate_{\interestingCategory}$.  We denote by $\poissonRate_{\min}$, the minimum rate over over all categories, that is $\poissonRate_{\min} = \min_{\interestingCategory \in \listInterestingCategories}\poissonRate_{\interestingCategory}$

% We consider two stopping conditions:

% \begin{enumerate}
%     \item The Poisson process stops when there are exactly $\numSamples$ arrivals.
%     \item The Poisson process stops after running for $\period$ time.
% \end{enumerate}



% As necessary, subscripts will be used when enumerating training data; it may be expedient to write $\trainingData{}\definedAs \set{(\sample_1,\labelElement_1), \hdots, (\sample_{\numSamples},\labelElement_{\numSamples})}$. Let $\hypothesisClass$ be a hypothesis class from which a deterministic prediction rule, $\hyp : \sampleSpace \to \labelSpace$ is selected. For example, in a binary classification setting, a hypothesis class $\hypothesisClass$ which appears frequently in literature is the set of non-homogeneous linear classifiers in $\realNumbers^\dimension$, i.e. classifiers of the form $\hyp(\sample) = \sgn\set{\vec{w}^{\transpose}\sample + b}$ where $\vec{w} \in \realNumbers^{\dimension},b\in\realNumbers$. $\positiveIntegers$ denotes the set of positive integers.  

A \emph{protected} feature is defined to be a feature to which our learner is blind, but is of interest to a meta-learner.  Without loss of generality, we assume the population group, $\group$, is determined by the value of that protected feature. 
 
% Let $\Gamma = \set{U_1,\dotsc,U_{\abs{\Gamma}}}$ be a finite collection of population groups.  We break from a portion of multicalibration literature in which population groups may be overlapping \cite{shabat2020sample,hebert2017calibration} and instead follow the convention of Pleiss et al. \cite{pleiss2017fairness,kleinberg2016inherent}: we assume the groups to be mutually exclusive.   $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  The assumption of mutual exclusivity among population groups provides additional structure to the problem which we leverage when constructing our bounds. Namely, we know

% \begin{equation}
%    1 \geq \sum_{U \in \Gamma} \Pr[\sample \drawnFrom \sampleDist]{\sample \in U}
% \end{equation}






% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA}$ and $\numSamples_{\trainingData,\groupB}$ are calculated is clear from context, we instead write $\numSamples_{\groupA}$ and $\numSamples_{\groupB}$.

% Similarly, we denote by $\numSamples_{\trainingData,\groupA,\labelElement_i}$the number of samples in population with feature $\sampleProtected=\groupA$ and ground truth label $y=\labelElement_i \in \labelSpace$.  $\numSamples_{\trainingData,\groupB,\labelElement_i}$ denotes the number of samples in population with feature $\sampleProtected=\groupB$ and ground truth label $y=\labelElement_i$ where $\labelElement_i \in \labelSpace$.  That is, 

% \begin{align}
%     \numSamples_{\trainingData,\groupA,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupA}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}} &  \numSamples_{\trainingData,\groupB,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupB}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}}
% \end{align}

% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA,\labelElement_i}$ and $\numSamples_{\trainingData,\groupB,\labelElement_i}$ are calculated is clear from context, we instead write $\numSamples_{\groupA,\labelElement_i}$ and $\numSamples_{\groupB,\labelElement_i}$.

% % We abuse notation and take $\numSamples_{\marker,\placeholder}$ to mean $\numSamples_{\marker,\placeholder,\depth}$

% To characterize the performance of our classifiers, we will use both the emprical risk and the true risk:

% \begin{definition}
%   Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, training set $\trainingData{}$ and predictor $\hyp$, we denote the empirical risk as \begin{equation}
%       {\risk}_{\trainingData}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}} \loss\paren*{\hyp(\sample),\labelElement}
%   \end{equation}
% \end{definition}

% \begin{definition}
%     Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, sample distribution $\sampleDist$ and predictor $\hyp$, we denote the true risk as \begin{equation}
%         \risk_{\sampleDist}(\hyp) \definedAs \Ex_{(\sample,\labelElement)\drawnFrom \sampleDist}\left[{\loss\paren*{\hyp(\sample),\labelElement}}\right]
%     \end{equation}
%   \end{definition}

%   As true risk has a dependence on the unknown distribution $\sampleDist$, the exact value of the true risk is also unknown.  Hence, our characterization of classifier performance will be probabilistic bounds on the difference between true risk and empirical risk. That is, classifier performance will be characterized in the following manner:  Given a non-negative real number $\placeholder$, $\Pr{\abs{\risk_{\sampleDist}(\hyp)-\risk_{\trainingData}(\hyp)} \geq \placeholder} \leq \errorConfidence$ where $\errorConfidence$ is a real number between $0$ and $1$ which depends on $\placeholder$, the number of samples $\numSamples$ used to calculate the empirical risk, and other context dependent factors.

%   We will see that the the concentration of our fairness metric behaves in a manner similar to the way empirical risk concentrates about the true risk.

  We use several definitions from Shabat et al. \cite{shabat2020sample}, the first of which is the category:

  \begin{definition}[Category]
      A category is a pair $(\group,\interval)$ of a subgroup $\group \in \Gamma$ and an interval $I \in \Lambda$.  A category  $(\group,\interval)$ is interesting according to predictor $\hyp$ and parameters $\gamma, \psi \in (0,1]$ if $\PR_{\sample \drawnFrom \sampleDist}\left[{\sample \in \group} \right]\geq \gamma$ and  $\PR_{\sample \drawnFrom \sampleDist}\left[{\hyp\paren*{\sample} \in \interval \given \sample \in \group}\right] \geq \psi$.
  \end{definition}

%   \begin{remark}
%     Given an arrival occurs at time $t$, the probability it belongs to category $\interestingCategory$ is $\frac{\poissonRate_{\interestingCategory}}{\sum_{\interestingCategory'\in \listInterestingCategories} \poissonRate_{\interestingCategory'}}$
%   \end{remark}


We investigate how the empirical calibration error concentrates about the true multicalibration error:




  \begin{definition}[Calibration Error]
    Let $\sampleDist \subseteq \sampleSpace \times \labelSpace$ be a sample distribution and let  $(\group,\interval)$ be a category.  The calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to a category $(\group,\interval)$ is denoted $\calibrationError\paren*{\hyp,\group,\interval}$:
    \begin{dmath}
        \calibrationError\paren*{\hyp,\group,\interval} \definedAs \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[{\labelElement \given \sample \in \group, \hyp\paren*{\sample}\in \interval}\right] - \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[\hyp\paren*{\sample} \given \sample \in \group, \hyp\paren*{\sample}\in \interval\right]
    \end{dmath}


\end{definition}

Put in words, the calibration error is the difference between the expectations of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.


\begin{definition}[Empirical Calibration Error]
    Let $\trainingData\drawnFrom\sampleDist^{\numSamples}$ be a training set of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist\subseteq \sampleSpace \times \labelSpace$ and let $(\group,\interval)$ be a category.  The empirical calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to category $(\group,\interval)$ and sample $\trainingData$ is denoted $\empiricalCalibrationError\paren*{\hyp,\group,\interval,\trainingData}$
    \begin{dmath}
        \empiricalCalibrationError\paren*{\hyp,U,I,\trainingData} \definedAs \sum_{(\sample,\labelElement) \in \trainingData}\left\{\frac{\indicatorFunction\left[\sample \in \group, \hyp(\sample) \in \interval \right]}{\left|\trainingData_{(\group,\interval)}\right|}\times\left(\labelElement-\hyp(\sample)\right)\right\}
    \end{dmath}


\end{definition}

Intuitively, empirical calibration error captures the difference between the average, taken over samples in $\trainingData$, of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.



Lastly we define the Vapnik-Chervonenkis (VC) dimension \cite{vapnik1971uniform} and the Rademacher complexity \cite{bartlett2002rademacher}, two notions of function class expressiveness which are used in proving bounds multicalibration uniform convergence sample complexity bounds.

Existing state-of-the-art bounds on multicalibration uniform convergence depend on the VC dimension:

\begin{definition}[Vapnik-Chervonenkis (VC) dimension] Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A hypothesis class $\hypothesisClass$ shatters set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ if 
    \begin{dmath}
        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
    \end{dmath}

The VC-dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$
\end{definition}

While the VC-dimension represents a seminal contribution to theoretical machine learning, it does limitations.  Notably, VC-dimension does not capture the generalization properties of the Radial Basis Function (RBF) Kernel.  

The Rademacher complexity is a notion of function class expressiveness.  Our sample complexity bound for multicalibration uniform convergence will depend on the Rademacher complexity and will be applicable to the RBF kernel:



\begin{definition}[Rademacher Complexity]
    The Rademacher complexity of a hypothesis class class $\hypothesisClass$ with respect to a sample $\trainingData$ is
\begin{equation}
    \rademacherComplexity_{\trainingData}\left(\hypothesisClass\right) \definedAs \frac{1}{\numSamples}\Ex_{\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{\hypothesisClass}}\sum_{i=1}^{\numSamples}\rademacherRV_i \hyp(\sample_i)\right]
    \end{equation}
    where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$ and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$
    \end{definition}

    Our goal is to determine a bound on the sample complexity, $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorConfidence,\errorTolerance,\gamma,\psi)$, of uniform convergence guarantees on multicalibration error.  That is, we wish to determine a bound on the number of samples neeeded to yield guarantees of the form:

\begin{dmath}
    \PR\left\{\forall \hyp \hiderel{\in} \hypothesisClass,\forall \group \hiderel{\in} \Gamma, \forall \predictionValue \hiderel{\in} \labelSpace \hiderel{:} \\
    \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{dmath}

The state-of-the-art for such sample-complexity bounds was developed by Shabat et al. \cite{shabat2020sample}.  For a hypothesis class of VC-dimension $\graphDimension$ which we denote $\hypothesisClass_{\graphDimension}$, the authors claim the following multicalibration unfiform-convergence sample complexity bound:

\begin{dmath}
        \sampleComplexity_{\hypothesisClass_{\graphDimension}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

The VC-dimension is a notion of hypothesis class capacity which is independent from data.  As such, sample complexity bounds utilizing the VC dimension do not leverage any knowledge of the underlying data distribution.  On the other hand, Rademacher complexity does leverage information about the underlying data distribution, so we can surmise some sample complexity bounds which utilize Rademacher complexity will be more informative than those which leverage VC dimension.




% \begin{theorem}
%     Let $\placeholderFunction : [-1,\infty)$ be a function defined by $\placeholderFunction(\placeholder) \definedAs 2\frac{\paren*{1+\placeholder}\ln\paren*{1+\placeholder}-\placeholder}{\placeholder^2}$ and let $\placeholderRandomVariable \drawnFrom \PoissonDistribution\paren*{\poissonRate}$ for some parameter $\poissonRate > 0$.  Then for any $\placeholder > 0$, we have

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \geq \poissonRate + \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \leq \poissonRate - \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{-\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     Lastly, for any $\placeholder > 0$, we have 

%     \begin{equation}
%         \Pr{\abs{\placeholderRandomVariable - \poissonRate} \geq  \placeholder} \leq 2\exp^{-\frac{\placeholder^2}{2\paren*{\poissonRate + \placeholder}}}
%     \end{equation}


% \end{theorem}




% \begin{definition}
%   Let $\trainingData_{\marker}$ be a subset of $\trainingData{}$.  Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers^+$ and predictor $\hyp$,
%   We define the empirical risk contribution of $\trainingData_{\marker}$ (denoted by $\empiricalRisk_{\trainingData_{\marker},\trainingData{}}$, as the amount of empirical risk $\trainingData_{\marker}$ contributes to the total empirical risk over the training data:
%   \begin{equation}
%       \empiricalRisk_{\trainingData_{\marker},\trainingData{}}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}}\set*{ \loss\paren*{\hyp(\sample),\labelElement}\cdot\indicatorFunction\bracket*{(\sample,\labelElement) \in \trainingData_{\marker}}}
%   \end{equation}
% % \end{definition}

% We also define notation specially adapted to our use of residual networks:

% For the rest of note let $\depth \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $\depth$ feature transformations:

% \begin{equation}
%     \functionComposition(\sample) = (\function_{\depth} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1)(\sample),
% \end{equation}
% where $\function_t$ ($t \in \set{1,\dotsc,\depth}$) is some function. Note that $\function_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $\function_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically a convolutional neural network (CNN).
% The final binary classifier is determined by a size-conforming weight vector $\weights_T$,
% where the classification is determined as
% \begin{equation}
%     \sign(\weights_T^{\transpose}\functionComposition(\sample))
% \end{equation}
% We will use the notation $\function_{1:\depthIter}$ to mean the composition $\paren*{\function_{\depthIter} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1}(\sample)$.
% We further use the notation $g_\depthIter \definedAs G_{1:\depthIter}$ to mean the composition of the first $\depthIter$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
% Lastly, let $\BoostResNet{\boost}(\trainingData{},\depth)$ denote the $\depth$ residual network trained on training set $\trainingData{}$ as learned by the $\BoostResNet$ procedure given in Huang et al. \cite{huang2018learning}.

% \subsection{Related Results}

% The residual network, introduced in 2015 by He et al., captures the fundamental design principles underlying many of today's state-of-the-art image classifiers.  As is the case with many classes of deep networks, their performance in practice exceeds what theory is able to explain.  Furthermore, decisions made by deep networks are almost never human interpretable.  In an effort to close this gap between theory and practice while providing some degree of interpretability to deep networks, Huang et al. applied the framework of boosting to show that under certain mild conditions, the training error of a residual network exhibits exponential decay that has an explicit dependence on the depth of the network.

% todo: expand


% We begin our discussion of fairness with a motivational example.  Consider a  protected feature which has two possible values.  That is, $\sampleProtected \in \set{\groupA,\groupB}$ .  Assume the protected feature is probabilistically independent from both the label $\labelElement$ and the unprotected features $\sampleUnprotected$.  That is to say $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=+1}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=-1}$.  We do not require each protected group to be equally likely.  Suppose $\numSamples_+$ in training set $\trainingData$ are such that the value of their protected feature $\sampleProtected$  is $+1$. Given a classifier $\classifierPlaceholder \definedAs \BoostResNet(\depth,\protectedTrainingData)$, let us examine a particular choice of fairness metric, $\fairnessMetric\definedAs \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}(\hyp)-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}(\hyp)}$
% Because the protected feature is independent from both the label and the unprotected features, we have

% \begin{align}
%     \fairnessMetric = \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} &\leq \max \curlyBrace*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData},\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} \\ &=\max\curlyBrace*{\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = +1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2},\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}}\\
%     &= \frac{1}{\numSamples}\cdot \abs*{\max\set*{\abs*{\trainingData_{\curlyBrace{\sampleProtected = +1}}},\abs*{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% From this, we see the difference in size of each protected group has a direct impact on which group contributes the most to training error.  This result is entirely unsurprising, but it motivates that simple metrics, such as the difference in loss, may not be the best way to measure fairness.

% We can see, for a given training set $\trainingData$, the value of fairness metric $\fairnessMetric$ has a dependence on the imbalance in population between the protected group and unprotected group, yet the total empirical risk over the training data remains constant, regardless of how individuals are assigned to the protected or unprotected group.


% \begin{theorem}[Theorem 2.8 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffLowerBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a>b\geq 1$ and $\placeholderScalar \geq 2$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} > \frac{1}{\sqrt{2\pi}}\exp\paren*{b-\frac{1}{8\placeholderScalar}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\left(\placeholderScalar-1\right)+1 }}{(a-b)^{\paren*{a-b}\paren*{\placeholderScalar-1}-b+1}b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}


% \begin{theorem}[Theorem 2.6 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffUpperBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a\geq b\geq 1$ and $\placeholderScalar \geq 1$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} < \frac{1}{\sqrt{2\pi}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\placeholderScalar + \frac{1}{2}}}{\paren*{a-b}^{\paren*{a-b}\placeholderScalar + \frac{1}{2}} b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}

==> Arxiv/src/old_stuff/old_proofs_svm.tex <==
\section{Proof of \cref{thm:OurBoundSVM}}
\begin{proof}
\begin{dgroup}
   \begin{dmath}
   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
\begin{dmath}
=\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\begin{dmath}
   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp}\PR\left[ \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Substituting in $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, as per \cref{thm:CortesGeneralization}, we arrive at}:
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp} \errorConfidence'
\end{dmath}
\begin{dmath}
   =2\left|\Gamma\right|\left|\hypothesisClass\right| \errorConfidence'
\end{dmath}
\end{dgroup}




Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence'}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, where $\errorConfidence' = \frac{\errorConfidence}{2\left|\Gamma\right|\left|\hypothesisClass\right|}$ completes the proof.

\end{proof}

==> Arxiv/src/old_stuff/old_svm_study.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our tight multicalibration uniform convergence bounds on kernelized predictors which includes the Kernel SVM, and RELU networks with one hidden layer.



% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 

We take our description of Kernelized  classifiers from Cortes et al \cite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.

We focus on a particular class classifiers, $\hypothesisClass_{\placeholderCount}^{\q}$ the set of non-negative combinations of $\placeholderCount \geq 1$ kernels $\kernelFunction_1,\dotsc,\kernelFunction_{\placeholderCount}$ with the mixture weights obeying an $\ell_{\q}$ constraint:

\begin{equation}
   \hypothesisClass_{\placeholderCount}^{\q} \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^\placeholderCount \placeholderScalar_i\kernelFunction_i : \norm{\vec{\placeholderScalar}}_{\q} = 1, \vec{\placeholderScalar} \geq 0, \norm{\weights} \leq 1,}
\end{equation}

Cortes et al. \cite{cortes2010generalization} developed several generalization bounds for kernelized predictors.  We will utilize one such bound, \cref{thm:CortesGeneralization}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Theorem 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\placeholderCount > 1$ and assume that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and $i \in [1,\placeholderCount]$.  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis set $\hypothesisClass_\placeholderCount^1$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_\placeholderCount^1) \leq \sqrt{\frac{23e\lceil\log\placeholderCount\rceil\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

\begin{theorem}[Corollary 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:CortesGeneralization}
   Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
   \begin{equation}
      \trueRisk(\hyp) \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
   \end{equation}
   where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
\end{theorem}

The above bound requires our kernel be a non-negative combination of a fixed set of $\placeholderCount$ kernels where $\placeholderCount > 1$.  As such, our proofs will leverage a an all-zeros size-conforming `dummy'' kernel.

The last piece of the puzzle, in order to yield Rademacher complexity based sample complexity bounds for multicalibration uniform convergence, is to draw analogues of two  Graph-dimension based lemmas \cref{lem:shabat24,lem:shabat25} from Shabat et al.  We arrive at our analgoues of Shabat's lemmas by upon invokation of \cref{thm:shalevRademacherImproved}:
\begin{lemma}[Analogue of Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke \cref{thm:shalevRademacherImproved} to yield an expression for $\errorTolerance$ in terms of Rademacher complexity.  We perform algebraic manipulation:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance = 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
   
      \begin{dmath}
         \errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) = 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
      \begin{dmath}
         \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 = \frac{32c^2\log\left(4/\errorConfidence\right)}{\placeholderCount}
      \end{dmath}
      \begin{dmath}
         \numSamples_U = \frac{32c^2\ln\left(4/\errorConfidence\right)}{  \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 }
      \end{dmath}
      \intertext{Substituting in for rademacher Complexity of a kernelized classifier \cref{thm:cortesRademacher}, we see that the following inequality implies the previous inequality, we have}
      \begin{dmath}
         \numSamples_U \geq \frac{32\log\left(\frac{4}{\errorConfidence}\right)}{  \left(\epsilon - 2\sqrt{\frac{23e\scalarBound^2}{22\numSamples_U}}\right)^2 }
      \end{dmath}
     \intertext{And now algebra:}
      \begin{dmath}
         \left(\epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2 \geq 32\log\left(\frac{4}{\errorConfidence}\right)
      \end{dmath}
      \begin{dmath}
         \epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}} \geq \sqrt{32\log\left(\frac{4}{\errorConfidence}\right)}
      \end{dmath}
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{\left(\sqrt{32\log\left(\frac{4}{\errorConfidence}\right)} + 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2}{\epsilon^2}
      \end{dmath}
      \intertext{The last step is simplifying \eqref{eq:NUSampleComplexity}.  \Eqref{eq:NUSampleComplexity} holds true when   }
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}
      \end{dmath}
   \end{dgroup}
   which concludes the proof
\end{proof}


\begin{lemma}\label{lem:shabat25analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\dimension_{\graphDimension}(\hypothesisClass) \leq \dimension$ Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}


With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

\begin{theorem}
\label{thm:OurBoundSVM}
Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
\small{
   \begin{dmath}
      \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
   \end{dmath}
   }
\end{theorem}  
\begin{proof}[Proof Sketch]
The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
\end{proof}

Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  

\begin{corollary} The sample-complexity necessary for multicalibration uniform convergence in kernelized predictors is

\begin{dmath}
\numSamples\left({\errorConfidence,\errorTolerance,\gamma,\psi}\right) = \frac{1}{\errorTolerance^2 \gamma \psi}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2}}\right)^2 
=\bigOh\left(\frac{\frac{r\scalarBound^2}{\margin^2} + \log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\errorTolerance^2\gamma\psi}\right)
= \bigOh\left(\frac{{r\scalarBound^2}+ \margin^2\log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\margin^2\errorTolerance^2\gamma\psi}\right)
\end{dmath} 
\end{corollary}



This bound on the sample complexity exhibits a similar form as that of Shabat et al. The main differences, however, is that SVM-specific bound has direct dependency on the test-set margin and the kernel's sensitivity and does not depend on the graph dimension of the classifier. These differences imply that a classifier-agnostic bound for multi-calibration uniform convergence is unlikely to be effective in practice. Take for example the RBF kernel; this kernel has an infinite graph dimension but is bounded between 0 and 1. Our bound can provide a more meaningful sample complexity bound for group fairness.


Using this bound, we can present a bound on the sample complexity of two-layer RELU networks.



% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance' \right] 
% \end{dmath}

% \subsection{Failure of Multi-calibration uniform convergence}

% Inspired by the proof of failure for uniform convergence of Nagarajan et al. (Theorem 3.1 of \cite{nagarajan2019uniform}), we show the failure of multicalibration uniform convergence.   

% \begin{definition} 
%   The \emph{tightest algorithm-dependent multi-calibration uniform convergnce bound} with respect to loss $\loss$ is the smallest value $\errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$ for which there exists a set of sample sets $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ such that $\PR\left[\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}\right] \geq 1-\errorConfidence$ and if we define the space of hypotheses explored by $\learningAlgorithm$ on $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ as $\hypothesisClass_{\errorConfidence} \definedAs \union_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}} \hyp_{\trainingData} \subseteq \hypothesisClass$, the following holds: $\sup_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}}\sup_{\hyp \in \hypothesisClass_{\errorConfidence}} \leq \errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$
% \end{definition}



% \paragraph{Distribution $\placeholderDist$:} Each input $(\placeholder_1,\vec{\placeholder}_2,\vec{\placeholder}_3)$ is a $1+K+D$ dimensional vector where $\placeholder_1 \in \realNumbers$, $\vec{\placeholder}_2 \in \realNumbers^{K}$ and $\vec{\placeholder}_3 \in \realNumbers^{D}$.  $\vec{\mu} \in \realNumbers^{K}$ determines the centers of the classes.  THe label $\labelElement$ is drawn uniformly from $\left\{\pm 1\right\}$ and conditioned on $\labelElement$, we have $\vec{\placeholder}_1 = 2\labelElement\vec{\mu}$ while $\vec{\placeholder}_2$ is sampled independently from $\mathcal{N}(\vec{0}_{D},\frac{32}{D}\vec{I}_D)$


% \begin{theorem}
%   For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \left|\Gamma\right|\ln \sfrac{\numSamples}{\errorConfidence}, \left|\Gamma\right|\numSamples\ln\sfrac{1}{\errorTolerance}\right\}\right)$, there exists a category, $(U,I) \in \listInterestingCategories_{\hyp}$ for which $\errorTolerance_{\textrm{gen}}(\trainingData,U,I,\errorConfidence) \leq \errorTolerance$ while $\errorTolerance_{\unifalg}(\trainingData,U,I,\errorConfidence) \geq 1-\errorTolerance$. 
% \end{theorem}

% \begin{theorem}\label{thm:MansourFinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\gamma\psi}\right)
% \end{dmath}
% \end{theorem}


% \begin{theorem}\label{thm:MansourInfinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be an infinite predictor class from domain $\sampleSpace$ to a discrete prediction set $\labelSpace$ with finite graph-dimension $\dimension_G(\hypothesisClass) \leq \dimension$.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\dimension+ \log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\psi^2\gamma}\right)
% \end{dmath}
% \end{theorem}

% We now compare our bound (\cref{thm:kernelSampleComplexity}) which applies in the binary classification setting, to prior bounds on multicalibration uniform convergence (\cref{thm:MansourFinite,thm:MansourInfinite}) with $\lambda$, a parameter which serves as a proxy for $\left|\labelSpace\right|$, to $2$:

% Whereas 



% \begin{theorem} For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \ln \sfrac{\numSamples}{\errorConfidence}, \numSamples\ln\sfrac{2\abs{\Gamma}{\errorTolerance}}\right\}\right)$, $\greekScalar \in [0,1]$, the multi-calibration uniform convergence satisfies $\errorTolerance$
% \end{theorem}


% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\left|\left(\hat{\mu}_{\hyp}\left(\hyp,U,I,\trainingData \right)-\hat{\mu}_{\labelElement}\left(\hyp,U,I,\trainingData\right)\right)  \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right] =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \left(\hyp(\sample_i)-\labelElement_i  \right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       \leq \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \cdot \min\left(1,\left[1-\frac{\labelElement_i \hyp\left(\sample_i\right)}{\margin}\right]_+\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\hat{\risk}_{\margin,U,I}\left(\hyp\right) \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
% \end{dgroup}

% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\hat{\mu}_{\labelElement}\left(\hyp,U,I\right)-{\mu}_{\labelElement}\left(\hyp,U,I\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2}\right] 
%    \end{dmath}
% \end{dgroup}
% \begin{align}
%    \bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|{\calibrationError\left({\hyp,U,I}\right) - \empiricalCalibrationError\left({\hyp,U,I,\trainingData}\right)\right| \leq \errorTolerance}
% \end{align}

% \section{Boosting and Fairness}

% Let $\sampleInfNormUB \definedAs \E[\evaluationData \drawnFrom \sampleDist]{\max_{i}\norm{\sample_i}_\infty}$.  $\norm{\weights}_1 < \finalLinearClassifierOneNormUB  < \infty$

% \begin{theorem}[Generalization and Margin bound from Huang et al. \cite{huang2018learning}]
%    Given algorithm 1 from \cite{huang2018learning}, the fraction of training examples with margin at most $\margin$ is at most $\paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}$.  And the generalization error $\Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0}$ satisfies
%    \begin{align}
%     \Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0} &\leq \paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}\\ &+ \frac{4\finalLinearClassifierOneNormUB\sampleInfNormUB}{\margin}\sqrt{\frac{\log\paren*{2\dimension}}{2\numSamples}}\sum_{t=0}^{\depth}\weightsOneNormUB_t + \frac{2}{\margin}\sqrt{\frac{\log \depth}{\numSamples}} + \functionPlaceholder\paren*{\margin,\numSamples,\depth,\errorConfidence}
%    \end{align}
%    with probability at least $1-\errorConfidence$ for $\functionPlaceholder(\margin,\numSamples,\depth,\errorConfidence) \definedAs \sqrt{\ceil*{\frac{4}{\margin^2}\log\paren*{\frac{\margin^2 \numSamples}{\log \depth}}}\frac{\log \depth}{\numSamples} + \frac{\log \frac{2}{\errorConfidence}}{2\numSamples}}$
% \end{theorem}

% where $\weightsOneNormUB_t\definedAs \prod_{t'=0}^t2\weightsOneNormUB_{t',t'-1}$ and $\weightsOneNormUB_{t,t-1}$ is the upper bound on the $\ell_1$ norm of the weight vector connecting a neuron at layer $t$ with its preceding layer.

% THe above bound, of course, does not inform loss bounds similar to \cref{thm:LossFunctionDifference}.
 

% Trivial Bound[Bad]


% \begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
% Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
% \begin{equation}
%     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{equation}
% where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

% \end{theorem}

% \begin{proof}
% \begin{align}
% \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
% &\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% \end{proof}

% A better bound...

% Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


% % \begin{lemma}
% %     Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
% %     \begin{equation}
% %         \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
% %     \end{equation}
% % \end{lemma}

% Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  We assume  $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and proceed by bounding
% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}} \end{equation}
 
% where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$,$\indicatorFunctionInstance_{\labelElement}\paren*{\sample} \definedAs\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} $  and $\labelFunction$ is a function which returns some $\labelElement \in \labelSpace$.  

% This quantity is bounded above by

% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}}\end{equation}




% Hoeffding's inequality applies here, and yields a bound similar to the bound derived in \cref{\thmOne}.  Do sharper bounds apply?

% \begin{theorem}[Multiplicative Chernoff-Style Bound Distributions induced by Boosting]\label{thm:chernoffNice}
%     Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
%     \begin{align}
%         \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
%              \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
%     \end{align}
%     \end{theorem}
% % \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> Makefile <==
### Makefile --- 

TARGETS = note

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> aistats/src/0_abstract.tex <==
\begin{abstract}
{\color{black} Recent works have sought the sample complexity necessary for fair machine learning.  The most advanced such sample complexity bounds are developed by analyzing multicalibration uniform convergence of a given hypothesis class.  We put forward a sharper sample-complexity bound for multicalibration uniform convergence when learning a kernel SVM.  Our technique applies to other hypothesis classes.   We perform an experimental evaluation on two datasets to compare our bounds with existing state-of-the-art.  With these findings, we call into question the insights into fair machine learning provided by existing sample complexity bounds.
}\end{abstract}



==> aistats/src/1_introduction.tex <==
% !TeX root = ../note.tex


\section{Introduction}



As machine learning systems have exhibited exemplary performance across a wide variety of tasks, the scope of their use has broadened.  Impactful life decisions which in the past have been rendered exclusively by humans, such as college admission and mortgage approval, are now using machine learning systems to supplement, or even replace, humans in the decision-making process.  This shift in how such important decisions are made has sparked a new field of machine learning research: \emph{fairness}. 

Informally speaking, there are two notions of fairness that appear in the literature.  The first type of fairness is \emph{individual fairness},  which is guided by the philosophy ``similar individuals should be treated similarly.''  The second type of fairness is \emph{group fairness}.  A group is the set of all individuals who share a set of protected attribute(s).  Group fairness is guided by the philosophy ``groups should be treated similarly.''  The focus of this work is on the latter notion of fairness.

% The set of protected attributes used to define a population group is almost always context-dependent.   Furthermore, (un-)fairness criteria are typically subject thorough critique by one or more regulatory body.  
%   Perhaps the most well-known body which provides critique on fairness criteria is the Supreme Court of the United States which has entered landmark decisions on the subject:  The Supreme Court, in a unanimous decision, abolished racial segregation in public schools \shortcite{1954brown} nearly 60 years after declaring the constitutionality of the \emph{separate but equal} doctrine.

In the field of fairness, there is often a tradeoff between a policy's utility as defined by its author (not necessarily aligned with broader societal values) and fairness as defined by the regulatory body. In machine learning, the negative-loss typically takes the role of utility, while fairness appears as a constraint on the optimization objective.
% Context typically influences the correct balance between utility and fairness.

Researchers have proposed different frameworks to formalize fairness notions, one of which is multicalibration -- a comprehensive framework that describes group fairness and is decoupled from specific fairness metrics and prediction error. The notion of multicalibration, when applied in the context of machine learning, is very similar to the colloquial usage of calibration: a classifier is multicalibrated for a population subgroup very much like a scale at the grocery store is calibrated to consistently display the same weight for a given weight placed upon it.  Thus, multicalibration error in the context of machine learning can be thought of as the discrepancy, for a fixed population subgroup, between the predicted label and the average of realized predicted labels of all samples within the subgroup.  Multicalibration is a notion of \emph{precision} and does not necessarily indicate accuracy: an untared scale is still calibrated as long as it consistently displays the gross weight (instead of net weight) of an intended purchase.

In this paper, we provide bounds on sample-complexity necessary to have a uniform convergence guarantee on multicalibration error for the kernel SVM.  Our bounds may be applicable when current state-of-the-art sample-complexity bounds, as introduced by Shabat et al. \shortcite{shabat2020sample}, are not.  For example, our bounds apply to the Radial Basis Function (RBF) Kernel SVM, whereas current state-of-the-art bounds are vacuous for such classifiers. 

\subsection{Related Work}



Much of modern ML fairness literature is concerned with the implications of learning classifiers via empirical risk minimization (ERM), or some variant thereof, subject to what is known as a fairness constraint.  A fairness constraint is often formulated as a constraint on the optimization objective, which is dependent on the value of a so-called \emph{protected attribute} (also referred to as a \emph{sensitive attribute}). Examples include the fairness constraints known as \emph{statistical parity} (also referred to as \emph{demographic parity}) introduced by Dwork et al. \shortcite{dwork2012fairness} and \emph{equality of opportunity} introduced by Hardt et al. \shortcite{hardt2016equality}.  Most importantly, these works assume the fairness constraint(s) can be enforced during training.  Typically, this means the learner has access to the protected attribute itself.  We refer to the setting in which the protected attribute is available to the learner as \emph{learner assessable fairness}.

When the protected attribute is not available to the learner, the learner is typically unable to explicitly enforce a fairness constraint.  In such situations, the fairness of the learned classifier is assessed by a meta-learner, which \emph{does} have access to the protected attribute.  We refer to this setting as \emph{learner remitted fairness}. In this setting, a learner only has access to information about the underlying data distribution.  Examples of such information include, but are not limited to, the number of protected groups and the frequency of each protected group.  The exact information to which a learner has access is often context-dependent.

Multicalibration is a well-studied quantity capturing the fairness of a classifier in the learner remitted fairness setting; Hebert-Johnson et al. were the first to develop and study the notion of multicalibration \shortcite{hebert2017calibration}.  They develop several algorithms for learning multicalibrated predictors and analyze their sample complexity. 

Liu et al. consider a two-protected group binary decision problem. The learner aims to identify the selection policy, which maximizes utility subject to a fairness constraint.  Samples are assumed to have a score that serves as a proxy for the utility of being selected.  The authors relate the multicalibration of a learned selection policy subject to a fairness constraint to the prediction utility \shortcite{liu2018delayed}.

Liu et al. also study the relationship between multicalibration and unconstrained machine learning \shortcite{liu2019implicit}. The authors show that for a large class of loss functions, if a learned classifier has a small excess risk over the Bayes risk when conditioning on protected attribute(s), the learned classifier will also be well-calibrated.  The results apply to both the learner assessable fairness and the learner remitted fairness setting.

Kearns et al. utilized the Vapnik-Chervonenkis dimension \shortcite{vapnik1971uniform} (VC dimension)  in their study of auditing algorithms for learner assessable fairness in an effort to prevent gerrymandering.  \shortcite{kearns2018preventing}.

More recently, Shabat et al. utilize the graph dimension \shortcite{daniely2011multiclass}, a multi-class generalization of the VC dimension, to determine the sample-complexity necessary for uniform convergence guarantees on multicalibration error \shortcite{shabat2020sample}.  Their results have no dependence on the underlying learning algorithm.
% and the results apply to the general setting of calibration of measuring instruments such as pressure gauges and scales.


 \subsection{Contributions}
 We study the sample complexity necessary for a certain level of classifier precision. The tightest bounds on sample complexity in this setting have been achieved by Shabat et al.~\shortcite{shabat2020sample}; these bounds have an explicit dependence on the frequency of a protected group and the graph dimension of a hypothesis class. The dependence on the graph dimension indicates that these bounds are not representative of the multicalibration error in all real-world settings: the graph dimension is infinite for some well-studied hypothesis classes. In this paper, we explore multicalibration uniform convergence guarantees based on Rademacher complexity. This paper makes the following contributions:

\begin{enumerate}
    
    \item We instantiate the bounds of Shabat et al. bounds on the kernel SVM. We find their bounds are sensitive to the choice of the kernel function. The specific case of the RBF kernel SVM shows that Shabat et al.'s bounds are not always explanatory when our bounds are informative. 

    \item We draw insights into factors affecting convergence of multicalibration error as a proxy for studying fairness. We find that there are structural issues in a dataset that induce a baseline of unfairness that cannot be overcome with a training regime. Furthermore, we look into the impact of the classifier architecture on multicalibration error itself. 

    \item We perform empirical evaluation on two representative datasets: Adult from UCI \shortcite{Dua:2019} COMPAS from ProPublica \shortcite{dressel2018accuracy,dieterich2016compas}. We study the tightness of the presented bounds and draw insights about the impact of both the data distribution and classifier regime on fairness. We make available our code for evaluating the sample complexity bounds presented.
\end{enumerate}


==> aistats/src/2_technical_background_and_motivation.tex <==
% !TeX root = ../note.tex


\section{Background}


We consider a setting where we have an input set $\sampleSpace \subseteq \realNumbers^{\dimension}$ and a label set $\labelSpace$.  A sequence of examples is denoted as $\trainingData{} \subseteq \sampleSpace \times \labelSpace{}$ and contains the $\numSamples$ examples which constitute the population group.

Let $\Gamma_{\trainingData} = \set{\group_1,\dotsc,\group_{\abs{\Gamma}}}$ be a finite collection of subsets of $\trainingData$, referred to as \emph{population subgroups}.  We follow the lead of existing multicalibration literature and assume population subgroups may be overlapping \shortcite{shabat2020sample,hebert2017calibration}.  $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  Our setting is that of binary classification: $\labelSpace = \left\{+1,-1\right\}$.  Since the labels in $\labelSpace$ are discrete, we also have $\Lambda = \left\{\left\{+1\right\},\left\{-1\right\}\right\}$. For each group $\group \in \Gamma_\trainingData$, $\left|\trainingData_{\group}\right|$ denotes the number of samples in $\trainingData$ within subgroup $\group$.


% We now discuss our notation for population subgroups: given set of examples $\trainingData$, which will be clear from the context. 



A \emph{protected} feature is defined to be a feature to which our learner is blind but is of interest to a meta-learner.  In this work, the population subgroup $\group$ to which an example $\sample$ belongs is that example's protected feature.  That is to say, given an example $\sample$, the learner is \emph{blind} to which population subgroup $\group$ the example $\sample$ belongs, but the meta-learner is \emph{aware} of the population subgroup to which the example belongs.
 


  We use several definitions from Shabat et al. \shortcite{shabat2020sample}, the first of which is the category.

  \begin{definition}[Category]
      A category is a pair $(\group,\interval)$ of a subgroup $\group \in \Gamma$ and a partition $I \in \Lambda$.  A category  $(\group,\interval)$ is interesting according to predictor $\hyp$ and parameters $\gamma, \psi \in (0,1]$ if $\PR_{\sample \drawnFrom \sampleDist}\left[{\sample \in \group} \right]\geq \gamma$ and  $\PR_{\sample \drawnFrom \sampleDist}\left[{\hyp\paren*{\sample} \in \interval \given \sample \in \group}\right] \geq \psi$.
  \end{definition}


The second definition is the calibration error. We investigate how the empirical calibration error concentrates around the true multicalibration error.


  \begin{definition}[True Calibration Error]
    Let $\sampleDist \subseteq \sampleSpace \times \labelSpace$ be a sample distribution and let  $(\group,\interval)$ be a category.  The calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to a category $(\group,\interval)$ is denoted $\calibrationError\paren*{\hyp,\group,\interval}$:
    \begin{dmath}
        \calibrationError\paren*{\hyp,\group,\interval} \definedAs \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[{\labelElement \given \sample \in \group, \hyp\paren*{\sample}\in \interval}\right] - \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[\hyp\paren*{\sample} \given \sample \in \group, \hyp\paren*{\sample}\in \interval\right]
    \end{dmath}


\end{definition}

The calibration error is the difference between the expectations of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ and the hypothesis $\hyp$ mapping $\sample$ to values in partition $\interval$.  


\begin{definition}[Empirical Calibration Error]
\label{def:emp_cal_error}
    Let $\trainingData\drawnFrom\sampleDist^{\numSamples}$ be a training set of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist\subseteq \sampleSpace \times \labelSpace$ and let $(\group,\interval)$ be a category.  The empirical calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to category $(\group,\interval)$ and sample $\trainingData$ is denoted $\empiricalCalibrationError\paren*{\hyp,\group,\interval,\trainingData}$
    {\small
    \begin{dmath}
        \empiricalCalibrationError\paren*{\hyp,U,I,\trainingData} \definedAs \sum_{(\sample,\labelElement) \in \trainingData}\left\{\frac{\indicatorFunction\left[\sample \in \group, \hyp(\sample) \in \interval \right]}{\left|\trainingData_{(\group,\interval)}\right|}\times\left(\labelElement-\hyp(\sample)\right)\right\}
    \end{dmath}
    }
\end{definition}

Intuitively, the empirical calibration error captures the difference between the average, taken over samples in $\trainingData$, of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ on which hypothesis $\hyp$ maps to values in partition $\interval$.




% Informally, a predictor with group fairness guarantees should exhibit little discrepancy between its average classification error on any subgroup and the error incurred by any example within the same subgroup.  This discrepancy is denoted as the calibration error. The true calibration error establishes this notion over the data distribution $\sampleDist$, while the empirical calibration error establishes a similar notion over the training set $\trainingData$. 

We focus on how empirical calibration error concentrates around the true calibration error for each population subgroup.  Sample-complexity bounds for multicalibration uniform convergence capture how the difference between the true and empirical calibration errors relate to a number of context dependent factors including the size of the training set, the number of categories, and the frequency of the least common population subgroup. Such sample-complexity bounds yield high-probability guarantees that the true calibration error is similar to the empirical calibration error. Our goal is to determine a bound on that sample complexity, denoted as $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorConfidence,\errorTolerance,\gamma,\psi)$.  That is, we wish to determine a bound on the number of samples needed to yield guarantees of the form:

\begin{dmath}\label{eq:multicalibrationUniformConvergence}
    \PR\left\{\forall \hyp \hiderel{\in} \hypothesisClass,\forall \group \hiderel{\in} \Gamma, \forall \predictionValue \hiderel{\in} \labelSpace \hiderel{:} \\
    \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{dmath}

where $\errorTolerance,\errorConfidence,\psi,\gamma \in (0,1].$





Lastly, we define the Vapnik-Chervonenkis (VC) dimension \shortcite{vapnik1971uniform} and the Rademacher complexity \shortcite{bartlett2002rademacher}, two notions of function class expressiveness which are useful in proving bounds for multicalibration uniform convergence sample complexity bounds. Existing state-of-the-art bounds on multicalibration uniform convergence depend on the VC dimension.

\begin{definition}[VC dimension]\label{def:VCdimension} Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ shatters hypothesis class $\hypothesisClass$ if 
    \begin{dmath}
        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
    \end{dmath}

The VC dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$.
\end{definition}

The state-of-the-art for the sample complexity bounds on uniform multicalibration convergence was developed by Shabat et al. \shortcite{shabat2020sample}.  For a hypothesis class of VC dimension $\graphDimension$ which we denote $\hypothesisClass_{\graphDimension}$, the multicalibration uniform-convergence sample complexity bound is given as:

\begin{dmath}
        \sampleComplexity_{\hypothesisClass_{\graphDimension}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}


While the VC dimension represents a seminal contribution to theoretical machine learning, it has some limitations.  Notably, the VC dimension does not capture the generalization properties of kernel SVMs for which the kernel yields an infinite-dimensional feature mapping.  Examples of such kernels include the Laplace kernel and the RBF kernel. The second limitation of the VC dimension is its inability to capture the effect of the underlying data distribution on generalization (we further discuss this in Sec.~\ref{sec:evaluation}). As such, the VC dimension is a notion of hypothesis class capacity, which is independent of the underlying data distribution. 

On the other hand, Rademacher complexity \cite{bartlett2002rademacher} does leverage information about the underlying data distribution. Hence, we can surmise some sample complexity bounds which utilize Rademacher complexity will be more informative than sample complexity bounds which leverage the VC dimension.  Our sample complexity bound for multicalibration uniform convergence depends on the Rademacher complexity and is applicable to SVMs with infinite-dimension kernels.



\begin{definition}[Rademacher Complexity]\label{def:rademacherComplexity}
    The Rademacher complexity of a hypothesis class  $\hypothesisClass$ with respect to a sample $\trainingData$ is
\begin{equation}
    \rademacherComplexity_{\trainingData}\left(\hypothesisClass\right) \definedAs \frac{1}{\numSamples}\Ex_{\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{\hypothesisClass}}\sum_{i=1}^{\numSamples}\rademacherRV_i \hyp(\sample_i)\right]
    \end{equation}
    where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$ and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{+1,-1\right\}$.
    \end{definition}

 


==> aistats/src/3_SVMCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our Rademacher complexity based multicalibration uniform convergence sample-complexity bounds for the kernel SVM. As indicated earlier, an advantage of this formulation is that it yields a sample-complexity for nearly any classifier, even those with infinite VC-dimension.  This Rademacher complexity approach also has the added benefit of capturing the effect of the underlying data distribution on multicalibration uniform convergence.




First, we take our description of kernels from Cortes et al. \shortcite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.  Since we are operating in the binary classification setting, we consider the set of kernel SVMs trained using hinge loss.


We prescribe notation for the thresholded hypothesis class. For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernel}$:

\begin{dmath}\label{eq:kernelHypothesisClass}
   \hypothesisClass_{\kernel} \definedAs \left\{\sample \mapsto \sgn\left(\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right) \right\}
\end{dmath}

We also prescribe notation for the non-thresholded hypothesis class.  For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernelFunction}'$:

\begin{equation}
   \hypothesisClass_{\kernelFunction}' \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)}
\end{equation}

Cortes et al. \shortcite{cortes2010generalization} developed several generalization bounds for such kernelized predictors.  We will utilize one such bound, \cref{thm:cortesRademacher}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Simplified version of Theorem 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\kernelFunction$ be a kernel function and that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ .  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis class $\hypothesisClass_{\kernelFunction}'$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}') \leq \sqrt{\frac{23e\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

The simplification taken to yield this bound is discussed in the appendix.

We will also need a two-sided Rademacher complexity generalization bound.




\begin{theorem}[Two-sided Rademacher complexity based Generalization Bound]\label{thm:shalevRademacherImproved}
   Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $\vec{\placeholder} \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp,\vec{\placeholder})\right| \leq c$. Then
   with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
   \begin{dgroup}
   \begin{dmath}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\Ex_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\placeholderCount}}
   \end{dmath}
   \begin{dmath}\label{eq:RademacherEmpiricalTwoSided}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass)\\ + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
   \end{dmath}
\end{dgroup}
\end{theorem}
\Cref{thm:shalevRademacherImproved} represents a modification to Theorem 26.5 from Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding} as it establishes a two-sided Rademacher complexity bound for generalization. The proof of this theorem largely follows that of Shalev-Shwartz and Ben-David, and is deferred to the appendix.

The last piece of the puzzle to yield Rademacher complexity based sample-complexity bounds for multicalibration uniform convergence is to draw analogues of two  graph dimension based lemmas from Shabat et al.  We arrive at our analogues of Shabat's lemmas by upon invocation of \cref{thm:shalevRademacherImproved}.  

Before stating these lemmas, we must state the contraction lemma, which bounds the Rademacher complexity of a  function of known Lipschitz constant composed with a set of known Rademacher complexity:

\begin{lemma}[Contraction Lemma, Theorem 7 from Meir and Zhang \shortcite{meir2003generalization}]\label{lem:contraction}
  Let $\trainingData = \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ $\left\{\placeholderFunction\right\}_{i=1}^{\numSamples}$ be functions with Lipschitz constants $\placeholderScalar_i$, then
   \begin{equation}
      \Ex_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\rademacherRV_i\placeholderFunction_i(\hyp(\sample_i)) \right\} \leq \Ex_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\placeholderScalar_i\rademacherRV_i\hyp(\sample_i) \right\} 
   \end{equation} where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$.
\end{lemma} 

We use the contraction lemma to determine a bound on the Rademacher complexity of $\hypothesisClass_{\kernel}$ when given both the Rademacher complexity of $\hypothesisClass_{\kernel}'$ and the value of $\min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$: 

\begin{lemma}\label{lem:kernelHypothesisContraction}
   Let $\hypothesisClass_{\kernel} : \sampleSpace \to \left\{\pm 1\right\}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and assume $\lambda > 0$, then we have

   \begin{equation}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}) \leq \max\left\{\frac{1}{\lambda},1\right\}\rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}')
   \end{equation}
\end{lemma}

\begin{proof}
   Because $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$, exactly one of the following cases holds:

   \begin{enumerate}
      \item Case $\lambda \geq 1$:
      
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $1$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$

       \item Case $0 < \lambda < 1$:
  
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $\frac{1}{\lambda}$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$


   \end{enumerate}

   
   Taking the $\max$ over both cases and applying the contraction lemma (\cref{lem:contraction}) yields the bound.
\end{proof}
   

The core theory underpinning our main result lies in \cref{lem:shabat24analogue,lem:shabat25analogue}.  Even though neither lemma on its own represents a bound on the sample complexity of multicalibration uniform convergence, when the statements in both \eqref{eq:statement24} and \eqref{eq:statement25}  are combined, we are able to provide the sample complexity bound on multicalibration uniform convergence, which is our main result.  Shabat et al. remark upon the difficulty of directly computing a bound on the sample complexity of multicalibration uniform convergence: uniform convergence guarantees over the infinite collection of distributions induced by the infinite hypothesis class $\hypothesisClass$ and the set of interesting categories $(\group,\interval)$ is challenging \shortcite{shabat2020sample}.



\begin{lemma}[Analogue of Lemma 24 from \shortcite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \subseteq \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement24}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke our two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$ in terms of Rademacher complexity.  We accomplish this by setting $\errorTolerance$ to be less than or equal to the right side of \eqref{eq:RademacherEmpiricalTwoSided}.  Let $\numSamples_{\group}$ be the minimum number of samples necessary to satisfy the following inequality:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
      \end{dmath}
      \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




      % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

      \begin{dmath}
         \errorTolerance  \leq 23\max\left\{1,\frac{1}{\lambda^2}\right\} \frac{\scalarBound^2}{\numSamples_\group} + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
      \end{dmath}


      \intertext{Which gives us, after algebraic manipulation}

      \begin{dmath}
         \numSamples_{\group} < \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
      \end{dmath}

   \end{dgroup}
      
Lastly, we know that if $\left|\trainingData_{\group}\right| > \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$, then $\left|\trainingData_{\group}\right| > \numSamples_{\group}$ which completes the proof.
\end{proof}

The proof technique for \cref{lem:shabat25analogue} is identical to that of \cref{lem:shabat24analogue}.

\begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}'} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement25}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

Now that we have the necessary lemmas stated, we may state our main result: a sample complexity bound for multicalibration uniform convergence, defined in~\eqref{eq:multicalibrationUniformConvergence}, which depends on the Rademacher complexity of hypothesis class $\hypothesisClass_{\kernel}$ with respect to sample $\trainingData$:

\begin{theorem}[Main Result]\label{thm:OurBoundSVM}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$,  $\hypothesisClass_{\kernel}$ has the multicalibration uniform convergence property with 

{\small
\begin{dmath}
   \sampleComplexity_{\hypothesisClass_{\kernel}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2 + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}
}
\end{theorem}

This bound on the sample complexity exhibits a similar form as that of Shabat et al.:

\begin{dmath}\label{eq:shabatVCBound}
   \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

where $\graphDimension$ is the graph dimension\footnote{The graph dimension is a multi-class generalization of the VC-dimension} of hypothesis class $\hypothesisClass$.

The main difference, however, is that Rademacher complexity based bound has a direct dependence on the test-set margin and the kernel's sensitivity. Our bound has no explicit dependence on the VC dimension of the chosen hypothesis class, as we show in \cref{fig:adult_nn_bounds,fig:compas_nn_bounds}. These differences imply classifier-agnostic bounds for multi-calibration uniform convergence are unlikely to be effective in practice as notions of fairness are themselves data-dependent. Take for example the RBF kernel; this kernel has an infinite VC dimension, yet for all $\sample \in \sampleSpace$ we know $\kernelFunction(\sample,\sample) \leq \scalarBound^2 = 1$. Hence, our bound can provide a more meaningful sample complexity bound for group fairness. 

While \cref{thm:OurBoundSVM} is fairly specific to the kernel SVM, it is possible to derive sample complexity bounds for multicalibration uniform convergence on other architectures by composing the relevant analogues to \cref{lem:shabat24analogue,lem:shabat25analogue} and replacing the Rademacher complexity of the kernel SVM with a (preferably tight) Rademacher complexity bound suitable for the choice of architecture. For instance,  one such family of classifiers is the feedforward ReLU network. An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al. \shortcite{bartlett2017spectrally}. This bound has a dependence on the number of samples, the norm of the input, and a couple varieties of matrix norm computed on the weight matrices.

% Let us now illustrate the utility of our bound on the RBF kernel SVM.
% \begin{example}[Example Instantiation of Bounds]. Consider the RBF kernel SVM, i.e. $\kernel_{\eta}(\sample,\sample')  = \exp\left(-\eta\norm{\sample'- \sample}_2^2\right)$ where $\eta$ is a positive real number and let $\gamma,\psi,\epsilon,\delta \in (0,1]$.  It is easy to see that $\scalarBound = 1=\max_{\sample} \kernel_{\eta}(\sample,\sample)$. which grants us a finite upper-bound on sample complexity by \cref{thm:OurBoundSVM}.  

% Compare this to the bound of Shabat et al. (\eqref{eq:shabatVCBound}):  The RBF kernel SVM is known to have an infinite VC dimension. Hence the bound presents an upper bound of infinity on the sample complexity.

% \end{example}







% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 






% \begin{theorem}[Corollary 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:CortesGeneralization}
%    Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
%    \begin{equation}
%       \risk_\hyp \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
%    \end{equation}
%    where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
% \end{theorem}






% With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

% \begin{theorem}
% \label{thm:OurBoundSVM}
% Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
% \small{
%   \begin{dmath}
%       \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
%   \end{dmath}
%   }
% \end{theorem}  
% \begin{proof}[Proof Sketch]
% The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
% \end{proof}

% Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  








==> aistats/src/5_Experiments.tex <==
\section{Evaluation}
\label{sec:evaluation}

We evaluate the presented bounds using different classification architectures over two datasets: Adult from the UCI Machine Learning Repository~\shortcite{Dua:2019} and COMPAS from ProPublica~\shortcite{dressel2018accuracy,dieterich2016compas}. Furthermore, we draw insights about the impact of the data distribution, group distribution, and classification architecture on the multi-calibration convergence. Our experiments are designed to answer three questions:
\begin{enumerate}
    \item \textit{How does (im-)balance between population subgroups affect fairness, manifesting in group distribution and number of samples per class?}  We highlight the dependence of our sample complexity bounds on the least frequent population subgroup and on the least frequent category.
    \item \textit{How does the choice of classifier architecture affect fairness and generalization?} We demonstrate that multicalibration error is very much related to the idea of generalization.
    \item \textit{How representative are the derived bounds to the underlying fairness?}  We plot, as proxies for the two competing sample complexity bounds, upper bounds on both the VC dimension and the Rademacher complexity for two feedforward ReLU networks.
\end{enumerate}

\subsection{Experiment Setup}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/broward_scatter.pdf}
    \caption{Empirical multicalibration error of Kernel SVMs on the COMPAS dataset}
    \label{fig:compas_svm_scatter}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/adult_scatter.pdf}
    \caption{Empirical multicalibration error of Kernel SVMs on the Adult dataset}
    \label{fig:adult_svm_scatter}
\end{figure}


The Adult dataset from the UCI machine learning repository comprises 14 attributes and 48842 records.  Entries in the dataset are extracted from the 1994 Census database. The label indicates if the income of a person exceeds \$50K. The second dataset is the COMPAS (Correctional Offender Management Profiling for Alternative Sanctions) dataset from ProPublica. This dataset contains the features utilized by the COMPAS algorithm in assigning the risk of reoffending for defendants in Broward County, Florida. The dataset comprises roughly 7200 records and 28 features; the label indicates if a defendant re-offends within two years.  

Our classifiers only predict on a subset of the available features. Classifiers on the COMPAS dataset are trained upon the following seven features: \texttt{sex}, \texttt{age}, \texttt{juv_fel_count}, \texttt{juv_misd_count}, \texttt{priors_count}, \texttt{charge_id}, and \texttt{charge_degree (misd/fel)}.

Classifiers for the Adult dataset are trained on the following features: \texttt{Age}, \texttt{Workclass}, \texttt{fnlwgt}, \texttt{Education-Num}, \texttt{Martial Status},
        \texttt{Occupation}, \texttt{Relationship}, \texttt{Sex}, \texttt{Capital Gain}, \texttt{Capital Loss},
        \texttt{Hours per week}, and \texttt{Country}.  Categorical data are one-hot encoded, and ordinal data are left as-is.

For each dataset, we define race as the protected attribute.  Classifiers do not have access to this attribute. We then induce random training/testing splits for each dataset while ensuring representation from each category of the protected attribute.  We train two types of classifiers for each training/testing split, SVMs and RELU networks. We train four SVM classifiers corresponding to the linear, RBF, sigmoid, and polynomial kernels. We also train two RELU networks corresponding to the following network architectures: a feedforward ReLU network with one hidden layer consisting of $2$ activation units and a feedforward ReLU network with one hidden layer consisting of $16$ activation units. As such, we obtain, for each of the two datasets, six classifiers for each random training/testing split. At test time, we introduce back the sensitive attribute to evaluate the empirical calibration error.

\subsection{Measurement Metrics}
In this evaluation, we first report the empirical calibration error as a proxy for a group fairness metric. In particular, we report the empirical calibration error, from~\cref{def:emp_cal_error}, on the test set of each trained classifier with respect to each category within the population.
% 
To measure the difficulty of achieving fairness on a given classifier architecture, we plot two measures of hypothesis class expressiveness: the VC dimension (\cref{def:VCdimension}) and the Rademacher complexity (\cref{def:rademacherComplexity}) . Plotting both measures of hypothesis class expressiveness allows us to compare current state-of-the-art bounds to the bounds developed in this paper.  

The VC dimension serves as a proxy for existing state-of-the-art bounds, i.e., those of Shabat et al. \shortcite{shabat2020sample}.  For a fixed classifier architecture, the VC dimension is constant and is represented by a line.  Unfortunately, the VC dimension for general feedforward ReLU networks is not known, so we plot a nearly tight upper bound developed by Bartlett et al. \shortcite{bartlett2019nearly}.

The Rademacher complexity serves as a proxy for the bounds presented in this work.  Rademacher complexity is data-dependent, so it is plotted as a scatter, with each point representing the Rademacher complexity of a single classifier with respect to a single category within the population.  Rademacher complexity bounds for feedforward neural networks, as given by Yin et al.~\shortcite{yin2019rademacher}, are relatively loose when compared to the nearly tight VC dimension bounds.

% how did we measure the multicalibration error from the dataset. 



\subsection{Results and Insights}



\paragraph{How does (im-)balance between population subgroups affect fairness, manifesting in group distribution and number of samples per class?} 

Empirically, from \cref{fig:compas_svm_scatter,fig:adult_svm_scatter}, we observe that, for a fixed evaluation set and fixed set of interesting categories, sample complexities for multicalibration uniform convergence depend on the frequency of the least common interesting category.  We observe that, as the number of test examples within a given subpopulation decreases, the statistical dispersion of the empirical calibration error increases.  This implies a relationship between class imbalance and perceived fairness: For an evaluation set of fixed size, as an interesting category decreases in frequency, members of that category are more likely to perceive unfairness.

This observation holds across both the COMPAS and Adult datasets and over each choice of classifier architecture shown in the plots; there is a baseline of unfairness that is induced by the underlying data distribution. 



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/broward_nn.pdf}
    \caption{Empirical multicalibration error of ReLU networks on the COMPAS dataset}
    \label{fig:compas_nn_scatter}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/adult_nn.pdf}
    \caption{Empirical multicalibration error of ReLU networks on the Adult dataset}
    \label{fig:adult_nn_scatter}
\end{figure}


\paragraph{How does the choice of classifier architecture affect fairness and generalization?} 

We observe that generalization and sample complexity of multicalibration uniform convergence are indeed correlated.  As a hypothesis class becomes more complex, the more slowly empirical calibration error concentrates around the true calibration error, just as our bounds indicate.  Notice how, in \cref{fig:compas_nn_scatter,fig:adult_nn_scatter}, as the number of hidden units increases, the rate at which empirical calibration error converges slows.  The convergence behavior of multi-calibration appears similar to the convergence behavior of general bounded loss functions such as hinge loss and $0$-$1$ loss.

Note also how the choice of complexity measure ties into fairness.  In \cref{fig:compas_svm_scatter,fig:adult_svm_scatter} we plot multicalibration error over choice on the kernel SVM for a choice of several kernels.  Even though the RBF kernel has infinite VC dimension, multicalibration error taken on the RBF kernel still exhibits convergence behavior, which suggests the VC dimension does not capture  behavior of the multicalibration error for the RBF kernel.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/broward_nn_vc_rad.pdf}
    \caption{Upper bound for both Rademacher Complexity and VC dimension on COMPAS dataset }
    \label{fig:compas_nn_bounds}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{aistats/src/img/adult_nn_vc_rad.pdf}
    \caption{Upper bound for both Rademacher Complexity and VC dimension on Adult dataset }
    \label{fig:adult_nn_bounds}
\end{figure}




\paragraph{How representative are the derived bounds to the underlying fairness?}
\Cref{fig:adult_nn_bounds,fig:compas_nn_bounds} show the Rademacher complexity upper bounds for RELU networks trained on each of the Adult and COMPAS datasets. We compare these bounds to the VC dimension upper bounds taken over the same networks. The Rademacher complexity represents the dominant term in our sample complexity bounds on multicalibration error, whereas the VC dimension represents the dominant term of sample complexity bound multicalibration error of Shabat et al.~\shortcite{shabat2020sample}. These two figures also display our original insights: the Rademacher complexity bounds are more representative of the underlying trends for group fairness. The VC dimension is fixed for any choice of architecture.  Furthermore, the VC dimension is agnostic of the underlying data distribution.   When compared to the nearly tight feedforward ReLU network VC dimension bounds \cite{bartlett2019nearly}, the Rademacher complexity bounds are indeed loose for feedforward ReLU networks~\shortcite{bartlett2017spectrally,yin2019rademacher}. Even these loose Rademacher complexity bounds, however, appear to be an effective proxy for the sample complexity of multicalibration uniform convergence. 








==> aistats/src/7_conclusion.tex <==
%!TeX root = ../note.tex

\section{Conclusion and Future Work}

This paper explored machine learning fairness from the perspective of sample complexities for multicalibration uniform convergence.  We proved a Rademacher complexity style bound on multicalibration uniform convergence.  We explored our bounds and the overarching concept of multicalibration uniform convergence with experimentation using the feedforward ReLU network and the kernel SVM.  Our results suggest that Rademacher complexity can have utility superior to the VC dimension in the context of machine learning fairness.

We will explore the tradeoffs between generalization and fairness analytically in future work. The idea is to study whether some classification regimes are more amenable for a favorable tradeoff. Further, motivated by the fact that existing datasets are considered not to be i.i.d. draws from an underlying distribution, we also intend to explore Rademacher complexity style bounds for machine learning fairness when data is not sampled i.i.d.

==> aistats/src/A1_proofs.tex <==
%!TeX root = ../note.tex
\section{Existing Lemmas and Definitions}

In this section we re-state, for completeness, several lemmas which appear in the paper by Shabat et al.  In our main paper, for the lemmas stated here which have a dependence on VC dimension and/or graph dimension of an underlying hypothesis class, we developed analogues with dependence on the class's Rademacher complexity.

\begin{lemma}[Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.   Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 25 from \cite{shabat2020sample}]\label{lem:shabat25}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let ${\group} \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 26 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat26}
   Let $p_1,p_2,\tilde{p}_1,\tilde{p}_2,\epsilon,\psi \in [0,1]$ such that $p_1,\psi \leq p_2$ and $\left|p_1-\tilde{p}_1\right|,\left|p_2-\tilde{p}_2\right| \leq \psi\epsilon/3$.  Then,

   \begin{equation}
      \left|\frac{p_1}{p_2} - \frac{\tilde{p}_1}{\tilde{p}_2}\right| \leq \epsilon
   \end{equation}

\end{lemma}

\begin{lemma}[Lemma 27 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat27}
   Let $\gamma \in (0,1)$ and let $\Gamma_\gamma = \left\{\group \in \Gamma \given \PR_{\sample \drawnFrom \sampleDist}\left[\sample \in \group\right] \geq \gamma\right\}$ be the collection of subpopulations from $\Gamma$ that has probability at least $\gamma$ according to $\sampleDist$.  Let $\errorConfidence \in (0,1)$ and let $\trainingData$ be a random sample of $\numSamples$ drawn i.i.d. from $\sampleDist$.  Then with probability at least $1-\errorConfidence$, if $\numSamples \geq \frac{8\log\left(\frac{\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$,

   \begin{dmath}
      \forall \group \in \Gamma_{\gamma} \hiderel{:} \left|\trainingData \intersection \group\right| \hiderel{>} \frac{\gamma \numSamples}{2}
   \end{dmath}

\end{lemma}

\begin{remark}[Remark on Theorem 1]
Firstly, we expand on the simplification from Theorem 2 by Cortes et al. taken to yield \cref{thm:cortesRademacher}.  Our \cref{thm:cortesRademacher}, which is a simplification of theorem 2 as by given Cortes et al. \cite{cortes2010generalization}, is a bound on the hypothesis class consisting of a non-negative combinations of at least two kernels. Given a set $\placeholderCount \geq 2$,  The authors' theorem 2 applies to the hypothesis class denoted $\hypothesisClass_{\placeholderCount}^1$ where

\begin{dmath}
\hypothesisClass_{\placeholderCount}^1 \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^{\placeholderCount}\alpha_i\kernelFunction_i, \norm{\weights} \leq 1, \vec{\alpha} \geq 0, 1= \sum_{i=1}^{\placeholderCount}\alpha_i \right\}
\end{dmath}

Our non-thresholded hypothesis class $\hypothesisClass_{\kernel}'$, on the other hand, consists of only one kernel:

\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :   \norm{\weights} \leq 1\right\}
\end{dmath}

 



Hence, when invoking the bounds from Cortes et al., we implicitly consider our hypothesis class to be non-negative combinations of our kernel and a dummy kernel $\kernelFunction_{\mathrm{dummy}}$.  The dummy kernel is assumed to always have weight $0$.  We accomplish this by re-writing $\hypothesisClass_{\kernel}'$ as
\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :  \kernelFunction = 1\cdot \kernelFunction + 0\cdot\kernelFunction_{\mathrm{dummy}}, \norm{\weights} \leq 1\right\}
\end{dmath}


\end{remark}



==> aistats/src/A2_rademacher_two_sided.tex <==
%!TeX root = ../note.tex


\section{Two-sided Rademacher Complexity Bounds}



In this section, we discuss the motivation behind the one-sided Rademacher complexity based generalization bounds of Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding}, and we show how to transform these bounds into two-sided generalization bounds.  Notation and proof techniques in this section largely follow that of Shalev-Shwartz and Ben-David.  Furthermore, the notation is also largely consistent with notation of Shabat et al \cite{shabat2020sample}. 

\begin{definition}Given a loss function $\ell : \labelSpace \times \labelSpace \to \realNumbers_+$, we denote the true risk of a hypothesis $\hyp$ with respect to $\sampleDist$ as $L_{\sampleDist}(\hyp)$:
\begin{dmath}
    L_{\sampleDist}(\hyp) \definedAs \Ex_{(\sample,\labelElement) \drawnFrom \sampleDist}\left[\loss(\hyp(\sample),\labelElement)\right] 
\end{dmath}

\end{definition}

\begin{definition}Given a loss function $\ell : \labelSpace \times \labelSpace \to \realNumbers_+$, we denote the empirical risk of a hypothesis $\hyp$ with respect to a sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ as $L_{\trainingData}(\hyp)$:
\begin{dmath}
    L_{\trainingData}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement)\in \trainingData} \loss(\hyp(\sample),\labelElement)
\end{dmath}

\end{definition}
% Using the Rademacher random variable, Bartlett et al. \cite{bartlett2002rademacher} were able to develop a notion of expressiveness for a given function class.  This measure of expressiveness is known as the Rademacher Complexity:

% \begin{definition}[Rademacher Complexity]
% The Rademacher complexity of a function class $\mathcal{H}$ with respect to a sample $\trainingData$ is
% \begin{dmath}
% \rademacherComplexity\left(\mathcal{H} \circ \trainingData \right) \definedAs \frac{1}{\numSamples}\Ex_{\vec{\rademacherRV}\drawnFrom\left\{\pm 1\right\}}\left[\sup_{f \in \mathcal{H}}\sum_{i=1}^{\numSamples}\rademacherRV_i f(\vec{\placeholder}_i)\right]
% \end{dmath}
% where sample $\trainingData \definedAs \left\{\vec{\placeholder}_1,\dotsc,\vec{\placeholder}_\numSamples \right\}$ is a set of of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$.
% and $\mathcal{H} \circ \trainingData$ denotes the set of all possible evaluations a function $f \in \mathcal{H}$ can achieve on a sample $\trainingData$, i.e.
% \begin{equation}
%     \mathcal{H} \circ \trainingData \definedAs \left\{(f(\vec{\placeholder}_1),\dotsc,f(\vec{\placeholder}_\numSamples)) : f \in \mathcal{H}\right\}
% \end{equation}
% \end{definition}

The Rademacher complexity (\cref{def:rademacherComplexity}) is a useful notion of function class expressiveness because it can be used to bound the \emph{representativeness} of a sample $\trainingData$ with respect to $\loss \circ \mathcal{H}$ as the largest gap between the true risk of a function $\hyp$ and its empirical risk.



\begin{definition}
    The \emph{representativeness} of $\trainingData$, a sample drawn from distribution $\sampleDist$, with respect to $\mathcal{H}$, denoted $\Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData)$, is the largest gap between the true risk of a hypothesis $\hyp$ in hypothesis class $\hypothesisClass$ and its empirical risk.
\begin{dmath}
    \Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData) \definedAs \sup_{\hyp \in \mathcal{H}} \left(L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right)
\end{dmath}
\end{definition}

The following lemma, from Shalev-Shwartz and Ben-David  describes the relationship between expected representativeness and expected Rademacher complexity:

\begin{lemma}[Lemma 26.2 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{lem:representativeness}
    \begin{dmath}
\Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples}} \Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData) \leq 2 \Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData}\left(\loss\circ\mathcal{H} \right) 
    \end{dmath}
\end{lemma}

Inspired by this bound, it is possible to construct generalization bounds based on empirical Rademacher complexity:

\begin{theorem}[Theorem 26.5 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{thm:shalevRademacher}
    Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be an i.i.d. sample of size $\numSamples$. Assume that for all $(\sample,\labelElement) \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp(\sample),\labelElement)\right| \leq c$. Then
    with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
    \begin{dgroup}
    \begin{dmath}
        L_\sampleDist(\hyp) - L_{\trainingData}(\hyp) \leq 2\Ex_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
    \begin{dmath}
        L_\sampleDist(\hyp) - L_{\trainingData}(\hyp) \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
\end{dgroup}
\end{theorem}



Note that \cref{thm:shalevRademacher} contains only one-sided bounds on $L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)$, yet we would like two-sided bounds, i.e. bounds on the probability $\left|L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right|$ is small.  Let us now pursue such bounds $\left|L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp)\right|$ using the Rademacher complexity.  Our proof follows the style of the proof of lemma 26.2 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}.  

\begin{lemma}[Two-sided version of \cref{lem:representativeness}]\label{lem:improvedRepresentativeness}
    \begin{dmath}
    \Ex_{\trainingData \drawnFrom \sampleDist^\numSamples} \sup_{\hyp \in \mathcal{H}} \left|L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2 \Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData}\left(\loss \circ \mathcal{H} \right) 
    \end{dmath}
\end{lemma}
\begin{proof}
Let us now provide a proof of  \cref{lem:improvedRepresentativeness}:
\begin{dgroup}
    \begin{dmath}
    \sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right| = \sup_{\hyp \in \mathcal{H}} \Ex_{\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right|
    \end{dmath}
    \intertext{Because expectation of supremum is larger than supremum of expectation, we have:}
    \begin{dmath}
        \sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right| \leq \Ex_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \sup_{\hyp \in \mathcal{H}} \left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right|
    \end{dmath}
    \intertext{Taking expectation over $\trainingData$ on both sides, we have}
    \begin{dmath}
        \Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right|\right] \leq \Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}} \left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right|\right]
        \end{dmath}
        \begin{dmath}
            =\frac{1}{\numSamples} \Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left| \sum_{i=1}^\numSamples \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]
        \end{dmath}
        \intertext{For each $j$, $(\sample_j',\labelElement_j')$ and $(\sample_j,\labelElement_j)$ are i.i.d. variables, which allows us to make the following statement:}
        {\small
        \begin{dmath}[label={eq:rademacherSplit}]
            \underbrace{\frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_j'),\labelElement_j') - \loss(\hyp(\sample_j),\labelElement_j) +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]}_{A}\\ = \underbrace{\frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_j),\labelElement_j) - \loss(\hyp(\sample_j'),\labelElement_j') +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]}_{B}
        \end{dmath}}
        \intertext{Let $\rademacherRV_j$ be a Rademacher random variable (i.e. a draw from the uniform distribution over $\left\{+1,-1\right\}$).  \Eqref{eq:rademacherSplit} then informs us:}
        \begin{dmath}
            \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\rademacherRV_j(\loss(\hyp(\sample_j'),\labelElement_j') - \loss(\hyp(\sample_j),\labelElement_j)) +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] = \frac{1}{2}\left(A + B\right)
        \end{dmath}
        \begin{dmath}
            = \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]
        \end{dmath}
        \intertext{Let $\vec{\rademacherRV} = \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^{\transpose}$ be a vector consisting of $\numSamples$ i.i.d. samples from the Rademacher distribution.  Repeating this procedure for all $j$, we have}
        {\small
        \begin{dmath}
            \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\sum_{i=1}^{\numSamples} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] =  \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\sum_{i=1}^{\numSamples} \rademacherRV_i(\loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]
        \end{dmath}
        \begin{dmath}
            = \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i'),\labelElement_i') \right) - \inf_{\hyp \in \mathcal{H}}\left(\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right)\right]
        \end{dmath}
        }
        \intertext{We know the distribution of $\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i)$ to be symmetric, hence}
        \begin{dmath}
            = \frac{1}{\numSamples}\Ex_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i'),\labelElement_i') \right) + \sup_{\hyp \in \mathcal{H}}\left(\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right)\right]
        \end{dmath}
        \begin{dmath}
            =\frac{2}{\numSamples}\Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{f \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right) \right]
        \end{dmath}
        \begin{dmath}
            =2\Ex_{\trainingData \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\rademacherComplexity_{\trainingData}(\loss \circ \mathcal{H})\right]
        \end{dmath}
\end{dgroup}
\end{proof}

Upon replacing \cref{lem:representativeness} with \Cref{lem:improvedRepresentativeness}, \cref{thm:ShalevImproved} naturally follows from the proof of \cref{thm:shalevRademacher}.  Hence, we arrive at the following two-sided bound:

\begin{theorem}[Two-sided version of Theorem 26.5 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{thm:ShalevImproved}
    Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $(\sample,\labelElement) \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp(\sample),\labelElement)\right| \leq c$. Then
    with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
    \begin{dgroup}
    \begin{dmath}
        \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\Ex_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
    \begin{dmath}\label{eq:rademacherEmpiricalTwoSided}
        \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass \circ \trainingData) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
\end{dgroup}
\end{theorem}


==> aistats/src/A3_proof_thm_3.tex <==
\section{Proof of \Cref{thm:OurBoundSVM}}

Our proof of \cref{thm:OurBoundSVM} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize Rademacher complexity instead of VC dimension.


\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to subpopulation ${\group}$. Let $\hypothesisClass_{\kernel}$ denote the hypothesis class defined in \eqref{eq:kernelHypothesisClass}. Let $\Gamma_\gamma$ denote the set of all subpopulations $\group \in \Gamma$ which have probability at least $\gamma$:
   \begin{dmath}
      \Gamma_{\gamma} \definedAs \left\{{\group} \in \Gamma \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
   \end{dmath}

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
   \begin{dmath}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{dmath}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\interval)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
   \end{align}

   By \cref{lem:shabat24analogue}, we know  for any $\predictionValue \in \labelSpace$ and any ${\group} \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{dgroup}
   \begin{dmath}
      \numSamples_1 \geq \frac{64\log\left(\frac{4}{\errorConfidence'}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{(\epsilon')^2}
   \end{dmath}
   \begin{dmath}
      = \frac{64\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{\left(\frac{\psi\errorTolerance}{3}\right)^2}
   \end{dmath}
   \begin{dmath}
      = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
   \end{dmath}
\end{dgroup}
   then we have

   
\begin{dmath}
   \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{dmath}
By \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any subpopulation ${\group} \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \left\{-1,1\right\}$, where

\begin{dmath} 
   \numSamples_2 \geq\frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
\end{dmath}

then we also have 

   \begin{dmath}
         \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{dmath}
   Set $\numSamples^\marker$ such that 
   \begin{dmath}
    \numSamples^\marker = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
   \end{dmath}
   Then, if for all subpopulations ${\group} \in \Gamma_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

   \begin{dgroup}
      \begin{dmath}\label{eq:calibrationClosenessA}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}\label{eq:calibrationClosenessB}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  = \frac{1152\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 414\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\gamma\errorTolerance^2\psi^2} 
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \Gamma_\gamma$. Recall there are at most $\left|\Gamma \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \Gamma_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{dgroup}
      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{dgroup}
   \begin{dmath}
      p_1(\hyp,{\group},\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      p_2(\hyp,{\group},\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_1(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_2(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
   \end{dmath}
\end{dgroup}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$:

\begin{dmath}
   {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in {\group}\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi \implies
   \left|\calibrationError(\hyp,{\group},\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
\end{dmath}

which completes the proof.


\end{proof}

% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to subpopulation $U$.  Let $\Gamma_\gamma$ denote the set of all subpopulations $U \in \Gamma$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \Gamma_{\gamma} \definedAs \left\{U \in \Gamma \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all subpopulations $U \in \Gamma_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \Gamma_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\Gamma}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\Gamma}} = \frac{1}{2\abs{\hypothesisClass}\abs{\Gamma}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.


==> aistats/src/B1_Inequalities_and_facts.tex <==
% !TeX root = ../note.tex

\section{Important Inequalities and Facts}

We begin by stating facts and inequalities necessary for our proofs:

\begin{lemma}[From \url{https://math.stackexchange.com/questions/171241/approximations-for-the-partial-sums-of-exponential-series}]\label{lem:expPartialSum}

    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}

\end{lemma}

\begin{lemma}[Frech\'et Inequality]\label{lem:frechet}
    Let $\event_1,\dotsc,\event_{\placeholderCount}$ be probabilistic events.  The following is true:
    
    \begin{equation}
        \Pr{\bigIntersection_{i=1}^{\placeholderCount} \event_i} \leq \min_{i} \Pr{\event_i}
    \end{equation}
    
    \end{lemma}



    \begin{theorem}[Hoeffding's Inequality \cite{hoeffding1963probability}]\label{\hoeffding}. Let $\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_{\placeholderCount}$ independent random variables strictly bounded by the intervals $\bracket{a_i,b_i}$, then

        \begin{equation}
            \Pr{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i - \sum_{i=1}^{\placeholderCount}\E{\placeholderRandomVariable_i}} \geq \placeholder} \leq \exp\paren*{-\frac{2\placeholderCount^2\placeholder^2}{\sum_{i=1}^{\placeholderCount}\paren*{b_i-a_i}^2}}
        \end{equation}
        
        \end{theorem}

        \begin{definition}
            The $\ell_1$ distance between any two distributions $\placeholderDist_1,\placeholderDist_2$ is defined as 
            \begin{equation}
                \norm{\placeholderDist_1-\placeholderDist_2}_1 \definedAs \sum_{\placeholder \in \support\paren*{\placeholderDist_1} \union \support\paren*{\placeholderDist_2}} \abs{\placeholderDist_1(\placeholder)-\placeholderDist_2(\placeholder)}
            \end{equation}
            \end{definition}

            \begin{lemma}[Lemma from Thomas and Cover \cite{coverthomas1991elements}]\label{lem:pinsker}
                \begin{equation}
                \infdiv{\placeholderDist_1}{\placeholderDist_2} \geq \frac{1}{2 \ln 2}\norm{\placeholderDist_1-\placeholderDist_2}_1^2
                \end{equation}
                \end{lemma}

                \begin{theorem}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{thm:chernoffNice}
                    Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
                    \begin{align}
                        \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
                             \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
                    \end{align}
                    \end{theorem}
                    
                    \begin{corollary}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{cor:chernoffNice}
                        Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\errorConfidence > 0$ then
                        \begin{align}
                            \Pr{\paren*{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}} && 0 \leq \frac{\errorTolerance}{\E{\randomVariable}}\leq 1
                        \end{align} 
                        \end{corollary}
                    
                        \begin{proof}
                            \begin{align}
                            \Pr{{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} + \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\errorTolerance} \\
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \placeholderCount\errorTolerance} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\placeholderCount\errorTolerance}
                            \intertext{Putting $\errorTolerance$ in terms of the parameters in \cref{thm:chernoffNice}, we see that $\errorTolerance = \relativeErrorTolerance \E{\randomVariable}$}
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} \\
                            &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}}
                            \end{align}
                        \end{proof}


\begin{lemma}\label{lem:multinomialDistributionBound}
    Let $\vec{\placeholder} \in \realNumbers^{\dimension}$ be a vector of probabilities.  That is, for $i \in \set{1,\dotsc,\dimension}$, we have $0 \leq \placeholder_i \leq 1$ and $1=\sum_{i=1}^{\dimension}\placeholder_{i}$.  Furthermore, the entries of $\vec{\placeholder}$ are ordered such that $\placeholder_1 \geq \placeholder_2 \geq \dotsc \geq \placeholder_{\dimension}$.  Then for all $i \in \set{1,\dotsc,\dimension}$, we have
    
    \begin{equation}
        \placeholder_i \leq \frac{1}{i}
    \end{equation}
    \end{lemma}
    \begin{proof}
        todo
    \end{proof}
    
                    

==> aistats/src/essential/macros.tex <==
\usepackage{bm}
\usepackage{mathtools}
\usepackage{xfrac}
\usepackage{bbm}
\usepackage{cleveref}
\usepackage{tikz}
\usepackage{breqn}

\renewcommand{\vec}{\bm}
\newcommand{\randomVariable}{X}
\newcommand{\randomVariableInstance}{x}
\newcommand{\bernoulliParameter}{p}
\newcommand{\placeholderCount}{m}
\newcommand{\errorTolerance}{\epsilon}
\newcommand{\relativeErrorTolerance}{\eta}
\newcommand{\errorConfidence}{\delta}
\newcommand{\martingaleDifference}{c}
\newcommand{\BernoulliDistribution}{\mathrm{Bernoulli}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2
}
\newcommand{\infdiv}{D\infdivx}
\newcommand{\scratchVariable}{q}
\newcommand{\event}{A}
\newcommand{\decisionFunction}{\sigma}
\newcommand{\hoeffding}{thm:hoeffding}
\newcommand{\placeholderSample}{Q}
\newcommand{\sampleElement}{x}
\newcommand{\labelElement}{y}
\newcommand{\weightsElement}{w}

\newcommand*\rect[1]{
    \tikz[baseline=(char.base)]{
        \node[inner sep=8pt, minimum size=1cm] (char) {#1};
        \draw (char.north west) -- (char.south west) -| (char.north east);
        }
}
\newcommand{\poissonRate}{\lambda}
\newcommand{\PoissonDistribution}{\mathrm{Poisson}}
\newcommand{\bigOh}{O}
\newcommand{\bigOmega}{\Omega}

\newcommand{\unifalg}{\mathrm{unif-alg}}

\newcommand{\loss}{\ell}
\newcommand{\regularizedGammaFunction}{Q}
\newcommand{\GammaFunction}{\Gamma}
\newcommand{\lossContribution}{L}

\newcommand{\labelFunction}{\hat{\sigma}}
\newcommand{\indicatorFunctionInstance}{\zeta}
\newcommand{\period}{T}

\newcommand{\sampleSpace}{\mathcal{X}}
\newcommand{\labelSpace}{\mathcal{Y}}
\newcommand{\sampleDist}{\mathcal{D}}
\newcommand{\drawnFrom}{\sim}
\newcommand{\fairnessMetric}{\mathcal{F}}
\newcommand{\multicalibration}{\mathrm{mc}}

\newcommand{\calibrationError}{\mathrm{c}}
\newcommand{\empiricalCalibrationError}{\hat{\mathrm{c}}}
\newcommand{\Frobenius}{F}

\newcommand{\moduleClassifier}{h}
\newcommand{\hypothesisModule}{\moduleClassifier}
\newcommand{\classifierPlaceholder}{\psi}
\newcommand{\scalarBound}{B}
\newcommand{\spectralBound}{s}
\newcommand{\normBound}{b}

\newcommand{\opt}{*}
\newcommand{\svm}{\mathrm{SVM}}

\newcommand{\moduleScalar}{\alpha}
\newcommand{\blockScalar}{\moduleScalar}
\newcommand{\convexHullOperator}{\mathrm{conv}}
\newcommand{\composeOperator}{\circ}
\newcommand{\greekScalar}{\lambda}
\newcommand{\placeholderScalar}{\alpha}
\newcommand{\metricEntropy}{\Phi}

\newcommand{\zeroVector}{\vec{0}}
\newcommand{\sampleComplexity}{m}
\newcommand{\metric}{\rho}
\newcommand{\setVar}{Y}
\newcommand{\setVarElement}{y}
\newcommand{\protectedTrainingData}{\trainingData_{\mathrm{pro}}}
\newcommand{\rademacherRV}{\sigma}
\newcommand{\variance}{\mathrm{Var}}
\newcommand{\openBall}{B}

\newcommand{\learningAlgorithm}{\mathcal{A}}
\newcommand{\boost}{\textrm{boost}}

\newcommand{\probabilityDensityFunction}{f}
\newcommand{\differential}{\mathrm{d}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\probabilityVar}{q}
\newcommand{\badGroups}{\mathtt{badGroups}}
\newcommand{\goodGroups}{\mathtt{goodGroups}}

\newcommand{\powerSet}{{P}}

\newcommand{\Ex}{\mathop{\mathbb{E}}}
\newcommand{\E}[2][]{\ifthenelse{\equal{#1}{}}{{\mathbb{E}}\left[#2 \right]}{\underset{#1}{ {\mathbb{E}}}\left[#2 \right]}}
\renewcommand{\Pr}[2][]{\ifthenelse{\equal{#1}{}}{\mathbb{P}\left[#2 \right]}{\underset{#1}{\mathbb{P}}\left[#2 \right]}}
\newcommand{\PrEmpirical}[2][]{\ifthenelse{\equal{#1}{}}{\hat{\mathbb{P}}\left[#2 \right]}{\underset{#1}{\hat{\mathbb{P}}}\left[#2 \right]}}
\newcommand{\PR}{\mathop{\mathbb{P}}}
\newcommand{\thmOne}{thm:one}
\newcommand{\thmTwo}{thm:Two}
\newcommand{\corThmTwo}{cor:two}
\newcommand{\intersection}{\cap}

\newcommand{\functionPlaceholder}{\beta}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\numInterestingCategories}{C}
\newcommand{\interestingCategory}{c}
\newcommand{\listInterestingCategories}{\mathcal{C}}

\newcommand{\given}{\mid}

\newcommand{\metricEntropyRadius}{\epsilon}
\newcommand{\q}{q}
\newcommand{\qDual}{r}
\newcommand{\functionComposition}{F}
\newcommand{\function}{G}
\newcommand{\sampleInfNormUB}{r_{\infty}}
\newcommand{\weightsOneNormUB}{\Lambda}
\newcommand{\finalLinearClassifierOneNormUB}{C_{0}}
\newcommand{\rademacherComplexity}{\mathcal{R}}

\newcommand{\blockOutput}{o}
\newcommand{\blockIter}{t}
\newcommand{\blockFunction}{f}
\newcommand{\moduleIter}{\blockIter}
\newcommand{\placeholderInt}{n}
\newcommand{\depth}{T}
\newcommand{\depthIter}{t}
\newcommand{\indicatorFunction}{\mathbbm{1}}
\newcommand{\entropy}{H}
\newcommand{\kernel}{\kernelFunction}
\newcommand{\threshold}{\tau}
\newcommand{\blockError}{\gamma}
\newcommand{\learningCondition}{\eta}
\crefname{fact}{fact}{facts}

\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\curlyBrace}{\{}{\}}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\innerProduct}{\langle}{\rangle}

\newcommand{\BoostResNet}{\mathrm{BoostResNet}}
\newcommand{\groupDist}{\vec{\pi}}
\newcommand{\minNumSamples}[1]{N_{\min,#1}}
\newcommand{\sample}{\vec{\sampleElement}}

\newcommand{\sampleProtected}{\sampleElement_{\protectedIndex}}
\newcommand{\sampleUnprotected}{\sample_{\unprotectedIndices}}
\newcommand{\hypothesisModuleSum}[2]{s_{#1:#2}}

\newcommand{\bigTheta}{\Theta}
\newcommand{\costMatrix}{\vec{C}}
\newcommand{\fairnessCostMatrix}{\vec{F}}

\newcommand{\weights}{\vec{\weightsElement}}
\newcommand{\sumHypothesisModules}{H}

\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\positiveIntegers}{\mathbb{Z}^+}

\newcommand{\dimension}{n}
\newcommand{\trainingData}{S}
\newcommand{\evalutationData}{\evaluationData}
\newcommand{\evaluationData}{T}
\newcommand{\margin}{\theta}
\newcommand{\placeholderConstant}{\alpha}
\newcommand{\Representativeness}{\mathrm{Rep}}

\newcommand{\unlabeledTrainingData}{Q}
\newcommand{\marker}{\dagger}
\newcommand{\bigIntersection}{\bigcap}
\newcommand{\bigUnion}{\bigcup}
%\newcommand{\risk}{R}
\newcommand{\numSamples}{N}
\newcommand{\numSamplesComplement}{N^c}
\newcommand{\placeholderSet}{\mathcal{V}}
\newcommand{\placeholderDist}{\mathcal{Q}}
\newcommand{\placeholderRandomVariable}{X}
\newcommand{\placeholderRandomVariableInstance}{x}
\newcommand{\boostDist}{D}
\newcommand{\placeholder}{z}
\newcommand{\protectedIndex}{1}
\newcommand{\unprotectedIndices}{2:\dimension}
\newcommand{\dimensionUnprotected}{\dimension-1}
\newcommand{\risk}{\mathcal{L}}
\newcommand{\hyp}{\mathrm{h}}
\newcommand{\hypMultiClass}{H}
\newcommand{\hypothesisClass}{\mathcal{H}}
\newcommand{\definedAs}{\triangleq}
\newcommand{\placeholderFunction}{f}
\newcommand{\kernelFunction}{K}
\newcommand{\kernelMapping}{\Phi}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\union}{\cup}
\newcommand{\support}{\mathrm{supp}}
\newcommand{\hilbertSpace}{\mathbb{H}}
\newcommand{\graphDimension}{\mathrm{d}}
\newcommand{\groupA}{a}
\newcommand{\groupB}{b}
\newcommand{\predictionValue}{v}
\newcommand{\groupWeight}{\alpha}
\newcommand{\group}{\mathrm{U}}
\newcommand{\interval}{\mathrm{I}}
\newcommand{\mat}{\bm}
\newcommand{\neuralNetwork}{\mathrm{NN}}
\newcommand{\nonlinearity}{\sigma}

\newcommand{\subGaussian}{\mathsf{subG}}
\newcommand{\proxyStandardDeviation}{\sigma}
\newcommand\MTkillspecial[1]{% helper macro
\bgroup
\catcode`\&=9
\let\\\relax%
\scantokens{#1}%
\egroup
}
\DeclarePairedDelimiter\brparen
\lparen\rparen
\reDeclarePairedDelimiterInnerWrapper\brparen{star}{
\mathopen{#1\vphantom{\MTkillspecial{#2}}\kern-\nulldelimiterspace\right.}
#2
\mathclose{\left.\kern-\nulldelimiterspace\vphantom{\MTkillspecial{#2}}#3}}
\DeclarePairedDelimiter{\angleBracket}{\langle}{\rangle}
\newcommand{\dotProduct}[2]{\angleBracket{#1,#2}}



==> aistats/src/essential/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
%\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> aistats/src/img/tex/binsForLearner.tex <==
%!TeX root = ../../../note.tex
 

\begin{tikzpicture}
\foreach \x in {0,...,5}{
\draw (\x*2,0) rectangle (\x*2+1, 1);};
\node  at (6*2+0.5,0.5) {$\ldots$}  ;
\draw (7*2,0) rectangle (7*2+1, 1);
\draw[black,fill=black] (0.5, 0.5) circle (0.1);
\end{tikzpicture}

==> aistats/src/old_stuff/2_related_work.tex <==
\section{Background}



% As machine learning systems have exhibited exemplary performance across a wide variety of tasks, the scope of their use has broadened.  Impactful life decisions which in the past have been rendered exclusively by humans, such as college admission and mortgage approval, are now using machine learning systems to supplement, or even outright replace, humans in the decision making process.  This shift in how such important decisions are made has sparked a new field of machine learning research: \emph{fairness}. 

% Much of modern ML fairness literature is concerned with the implications of learning classifiers via empirical risk minimization (ERM), or some variant thereof, subject to what is known as a fairness constraint.  A fairness constraint is typically formulated as a constraint on the optimization objective which is dependent on the value of a so-called \emph{protected attribute} (also referred to as a \emph{sensitive attribute}). Examples include the fairness constraints known as \emph{statsitical parity} (also referred to as \emph{demographic parity}) introduced by Dwork et al. \citep{dwork2012fairness} and \emph{equality of opportunity} introduced by Hardt et al. \citep{hardt2016equality}.  Most importantly, these works assume access to a fairness constraint which can be enforced during ERM, which is to say, it is known precisely which constraints are required to make the resulting trained classifier fair.  We refer to the setting in which the protected attribute is available to the learner as \emph{learner assessable fairness}.

% When the protected attribute is not available to the learner, the learner is unable to evaluate the fairness of classifier.  In such situations, fairness of the learned classifier is assessed by a meta-learner which \emph{does} have access to the protected attribute.  This setting we refer to as \emph{learner remitted fairness}. In learner remitted fairness, a learner only has access to information about the underlying data distribution.  Examples of such information include, but are not limited to the number of protected groups, and the frequency of each protected group.  The exact information to which a learner has access is often context dependent.

% Multicalibration is a well studied quantity which captures the fairness of a classifier in the learner remitted fairness setting: Hebert-Johnson et al. were the first to develop and study the notion of multicalibration \cite{hebert2017calibration}.  In particular, the authors develop algorithms for learning multicalibrated predictors 
 

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.





==> aistats/src/old_stuff/3_5_calibration_concentration.tex <==
%!TeX root = ../note.tex
\section{Concentration Inequalities for Multi-calibration}

We begin this section by stating a sample-complexity bound for multi-calibration uniform convergence from Shabat et al. \cite{shabat2020sample}

\begin{theorem}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Furthermore assume that groups $\set{U_1,\dotsc,U_{\abs{\Gamma}}}$ may overlap.Then $\hypothesisClass$ has the uniform multicalibration convergence property with
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\gamma,\psi} = \bigOh\paren*{\frac{\log\paren*{\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}}{\errorTolerance^2\gamma\psi}}
    \end{equation}

\end{theorem}

We will improve upon this bound by utilizing the structure which the assumption of mutually exclusive groups provides:

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    The ``bad'' event $B^{\trainingData}$ is the event in which denotes the existence of an interesting category for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$:

    \begin{equation}
        B^{\trainingData} \definedAs \set*{\trainingData : \exists \hyp \in \hypothesisClass, \exists (U,I) \in C_{\hyp} : \abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance}
    \end{equation}

    We also define the ``good'' event $G^{\trainingData,\placeholder}$, which is the event that each interesting category in $\trainingData$  contains at least $\placeholder$ samples:

    \begin{equation}
        G^{\trainingData,\placeholder} \definedAs \set*{\trainingData : \forall \hyp \in \hypothesisClass, \forall (U,I) \in C_{\hyp} : \abs{(U_{\trainingData},I)} \geq \placeholder }
    \end{equation}

    Note that the ``bad'' event and the ``good'' event are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    \begin{equation}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}
    \end{equation}

    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Now, we upper-bound this quantity:

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\
        &\leq  \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C_{\hyp}} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}\\
        &\leq 4\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\lambda}\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}



   \begin{equation}
    \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}  \iff \placeholder \geq \frac{2}{\errorTolerance^2}\log\paren*{\frac{8\abs*{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}
   \end{equation}

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   
   \begin{align}
    \Pr{\abs{\paren*{U_\trainingData,I}} \leq \placeholder} &\leq Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
    &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
    &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
   \end{align}
\end{proof}



With only lower bounds on the frequency of an ``interesting'' category, our bounds are remarkably similar to those
Let's now analyze the case of the finite hypothesis class but in the leave $k$ out setting.  That is, given $k$, a non-negative integer less than $\abs{\Gamma}$, what is the sample complexity necessary for at least $\abs{\listInterestingCategories_{\hyp}} -k$ groups to satisfy the fairness criteria?


\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  

 

    We also define the ``good'' event $G^{\trainingData,\placeholder,m}$, which is the event that at least $\abs{C}-m$ interesting categories in $\trainingData$  contain at least $\placeholder$ samples.

    Note again the ``bad'' events and the ``good'' events are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    We now define a new ``bad'' event, distinct from the event defined in the previous proof.  Let $B^{\trainingData,\listInterestingCategories}$ be the event which denotes the existence of at least $1$ interesting category in set $\listInterestingCategories$ for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$.  Suppose we have a function $\goodGroups$ which takes in, as an argument, the event $G^{\trainingData,\placeholder,m}$ and returns the powerset of exactly $\numInterestingCategories-k$ distinct categories $(U,I)$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$ holds true. That is to say, for any integer $k$, $\goodGroups\paren*{G^{\trainingData,\placeholder,k}}$ $\numInterestingCategories - m$ categories which satisfy this condition.

    WE further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\listInterestingCategories} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.
    
    Event $B^{\trainingData,l,\listInterestingCategories}$ occurs when at least $l$ categories $(U,I)$ in list $\listInterestingCategories$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$

    Let $\listInterestingCategories^k$ denote the list of all possible combinations of $k$ interesting categories.  In order to have leave-$k$-out fairness, we bound 
    
    \begin{align}\Pr{\bigIntersection_{i=1}^{\abs{\listInterestingCategories}} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \sum_{\listInterestingCategories' \in \listInterestingCategories^k}\prod_{i=1}^k \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder} \given \bigIntersection_{j=1}^{i-1}\curlyBrace*{B_{\interestingCategory_j}^{\trainingData} \union \lnot G_{\interestingCategory_j}^{\trainingData,\placeholder}} }\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k} \subseteq \listInterestingCategories} \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k}} \errorConfidence\\
    &= \errorConfidence^{k}
    \end{align}



 
    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Suppose we wish to have leave-$k$-out fairness.  Then must we have $l+m\geq k$
    
    Then the event we are interested upper-bounding is:

    
    \begin{align}
        \Pr{B^{\trainingData,\listInterestingCategories_\hyp^{\marker},l} \given G^{\trainingData,\placeholder,m}} &\leq \sum_{\hyp \in \hypothesisClass} \Pr{B_{\interestingCategory_1}^{\trainingData,\listInterestingCategories_\hyp^{\marker} \setminus \set*{}} \intersection B_{\interestingCategory_2}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_1}} \intersection \hdots \intersection  B_{\interestingCategory_l}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_i}_{i=1}^{l-1}}} \\
        &\leq \sum_{\hyp \in \hypothesisClass} \binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}\\
        &\leq \abs{\hypothesisClass}\binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}
    \end{align}

    where $\listInterestingCategories_{\hyp}^{\marker}\definedAs \goodGroups\paren*{G^{\trainingData,\placeholder,m}}$

    which suggests

    \begin{equation}
        \frac{\errorConfidence}{2} \geq \abs{\hypothesisClass}\binom{\listInterestingCategories_{\hyp}-m}{l}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^l \iff \placeholder \geq \frac{2}{\errorTolerance^2}\ln\paren*{4\sqrt[l]{\binom{\abs{\listInterestingCategories_{\hyp}}-m}{l}\frac{2\abs*{\hypothesisClass}}{\errorConfidence}}}
    \end{equation}

    Let us now bound $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}}$ 

    In order to compute this bound, we further decompose the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    We upper-bound the complement of the good event, $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,m}}}$, by translating it into the language of category-wise good events,$G^{\trainingData,\placeholder,\listInterestingCategories}_{\interestingCategory}$ , into it's category-wise good events:

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{}}_{\interestingCategory_1} \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_1}}_{\interestingCategory_2} \intersection \hdots \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_i}_{i=1}^{m-1}}_{\interestingCategory_m}}\\
        &\prod_{i=1}^m
    \end{align}



    In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$, hence we have

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
        &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
        &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
       \end{align}


    % \Pr{\set*{\bigcup_{\listInterestingCategories \in \goodGroups\paren*{G^{\trainingData,\placeholder,k}}}\trainingData \in B^{\trainingData,l,\listInterestingCategories}} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{B^{\trainingData,k} \in \powerSet_{\trainingData,k}}\sum_{(U,I)\in C_{\hyp}\setminus \badGroups\paren*{B^{\trainingData,k}}}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData,l,\listInterestingCategories} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq 4\binom{\abs{\listInterestingCategories}}{l}\abs{\hypothesisClass} \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}

The bad event is not so simple.  If we are considering leave 

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   

\end{proof}

==> aistats/src/old_stuff/3_7_calibration_concentration.tex <==
%!TeX root = ../note.tex

\subsection{Multi-calibration uniform convergence in the Poisson Model.}

\begin{theorem}  Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then, for the Poisson model, we have the following sample-complexity for leave $k$ out fairness:
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\poissonRate_{\interestingCategory},k} = \bigOh\paren*{\frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\poissonRate_\interestingCategory\errorTolerance^2}}
    \end{equation}
\end{theorem}

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  
    We further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\hyp} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder,\hyp} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.

    In order to have leave-$k$-out fairness, there must be at least $k$ distinct categories $\interestingCategory$ for which at least one of the following is true:

    \begin{enumerate}
        \item Good event $G_{\interestingCategory}^{\trainingData,\placeholder}$ does \emph{not} occur
        \item Bad event $B_{\interestingCategory}^{\trainingData,\listInterestingCategories}$ does occur
    \end{enumerate}

    \begin{align}
        \Pr{\lnot G_{\interestingCategory}^{\trainingData,\placeholder}} &= \Pr{\abs{\interestingCategory} \leq \placeholder} \\
        &\leq \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}
        % &= \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}
    \end{align}

    where $\regularizedGammaFunction$ is the regularized gamma function:

    \begin{equation}
        \regularizedGammaFunction(\placeholder_1,\placeholder_2) \definedAs \frac{\GammaFunction\paren*{\placeholder_1,\placeholder_2}}{\GammaFunction\paren*{\placeholder_1}} = \frac{\int_{\placeholder_2}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}{\int_{0}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}
    \end{equation}

    Let us now bound $\Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}}$:

    \begin{align}
        \Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}} &\leq \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}}  \\
        &\leq 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}


    Let $\listInterestingCategories^{k}$ denote the set of all combinations of $k$ categories in $\listInterestingCategories$.  All together, we have:

    \begin{align}
\Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} +\exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}}^k\\
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\placeholder_{\interestingCategory}}^2}{2\poissonRate_{\interestingCategory}}}}}^k 
            \intertext{assume $\placeholder \leq \poissonRate_{\interestingCategory}/2$}
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}}}^k  \label{eq:PoissonUnionBound}\\
    \end{align}

    % \begin{align}
    %     \Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}^k\\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}}^k \\
    %                 &= \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\sum_{i=0}^{\placeholder}\frac{\poissonRate_{\interestingCategory}^i}{i!}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\paren*{e^{\poissonRate_{\interestingCategory}}-\frac{\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate}\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &< \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate_{\interestingCategory}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}\exp\paren*{-\paren*{\placeholder+1}+\frac{1}{12\placeholder + 13}}}}}}^k \\
    %                 &=\paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{\exp\paren*{-\poissonRate_{\interestingCategory}+\placeholder+1-\frac{1}{12\placeholder+13}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}}}}}^k \label{eq:PoissonUnionBound}\\
    %         \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the left-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}} & \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}& \leq \frac{k\errorConfidence^{\frac{1}{k}}}{8 e \abs{\listInterestingCategories}} \\ 
        \placeholder &\geq \frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\errorTolerance^2}
    \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the right-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\exp\paren*{-\frac{\paren*{\placeholder}^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{ k\errorConfidence^{\frac{1}{k}}}{2e\abs{\listInterestingCategories}} \\
       \placeholder& \geq \sqrt{2\poissonRate_{\interestingCategory}\ln\paren*{\frac{2e\abs{\listInterestingCategories}}{ k\errorConfidence^{\frac{1}{k}}}}} \\
    \end{align}

\end{proof}



    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}




\begin{lemma}
    \begin{align}
      \binom{\abs{\listInterestingCategories}}{k}^{\frac{1}{k}} < \paren*{\frac{1}{\sqrt{2\pi}}\frac{\abs{\listInterestingCategories}^{\paren*{\abs*{\listInterestingCategories}+\frac{1}{2} }}}{\paren*{\abs*{\listInterestingCategories}-k}^{\abs*{\listInterestingCategories}-k + \frac{1}{2}}k^{k+\frac{1}{2}} }}^{\frac{1}{k}}
    \end{align}

\end{lemma}

\begin{lemma} Let $a,b$ be integers such that $a \geq b \geq 1$ (from wiki)
    THe following are true:
    \begin{equation}
        \frac{a^b}{b^b} \leq \binom{a}{b} \leq \frac{a^b}{b!} \leq \paren*{\frac{e\cdot a}{b}}^{b}
    \end{equation}
\end{lemma}

==> aistats/src/old_stuff/3_RevisitingResidualHypothesisBoosting.tex <==
\section{Revisiting Residual Hypothesis Boosting}
% In this note we present a boosting framework for any sequential composition of functions.
% For the rest of note let $T \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $T$ feature transformations:
% $$F(\sample) = (G_T \circ G_{T-1} \circ \cdots \circ G_1)(\sample),$$
% where $G_t$ ($t \in [T]$) is some function. Note that $G_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $G_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically say a CNN.
% The final binary classifier is determined by another weight vector $\weights_T$ of appropriate shape,
% where the classification is determined as
% $$\sign(\weights_T^{\transpose}F(\sample))$$
% We will use the notation $G_{1:t}$ to mean the composition $G_t \circ G_{t-1} \circ \cdots \circ G_1$.
% We further use the notation $g_t \definedAs G_{1:t}$ to mean the composition of the first $t$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
The weight vectors $\weights_1, \dots, \weights_{T-1}$ will not appear in the final classifier, but they are used to
guide training. Specifically, the following proposition is straightforward:
\begin{proposition}[Final hypothesis is sum of residuals]
  The final hypothesis is the \emph{sum of residual hypotheses} scaled by $1/\alpha_T$:
  \begin{align*}
    \weights_T^{\transpose}F(\sample) = \frac{1}{\alpha_T}\sum_{t=0}^{T-1}h_t(\sample)
  \end{align*}
\end{proposition}
Therefore we can focus on training $\sum_{t=1}^Th_t$, and we can do it simply by AdaBoost.
In fact, let us see what is going on there: Let $K \in [T]$, and suppose that $h_1, \dots, h_{K-1}$
have been trained (when $K=1$, we have $0$ to start with), and our goal is to train a hypothesis
$\sum_{t=1}^Kh_t$ to minimize the training error. That is
\begin{align}
  \minimize_{h_0,\dots,h_{K-1}} \sum_{i=1}^\numSamples \exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right)
\end{align}
where we have been using exponential loss. We note that:
\begin{align}
  &\exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right) \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right) + (-y_ih_{K-1}(\sample_i))\right) && \text{($h_0, \dotsc, h_{K-2}$ have been trained)} \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right)\right) \exp(-y_ih_{K-1}(\sample_i)) \\
  = &\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))\exp(-y_ih_{K-1}(\sample_i)) \\
\end{align}
Here the term $\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i)$ is viewed as a ``weight'' we assigned to each training point.
In AdaBoost there is a specific iterative weighting procedure to turn these weights into a proper probability distribution.
That probability distribution will be important for the theory, so we repeat that derivation here:
\begin{itemize}
\item The end goal is to turn these terms into
  \begin{align}
    D_{K}(i) = \frac{\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))}{\sum_{j=1}^\numSamples\exp(-y_j\alpha_{K-1}o_{K-1}(\sample_j))}
  \end{align}
\item Note that we know that
  \begin{align}
    \alpha_{K-1}o_{K-1} \definedAs \sum_{t=1}^{K-1}h_t
  \end{align}
  It turns out that such a distribution can be constructed recursively as follows:
  \begin{enumerate}
  \item Start with a uniform distribution on all the training points: $D_0(i) = \frac{1}{N}$.
  \item Then for $t = 1, 2, \dots$,
    \begin{align}
      \label{def:recursive-weighting}
      D_t(i) = \frac{D_{t-1}(i)\exp(-y_ih_t(\sample_i))}{\sum_{j=1}^\numSamples D_{t-1}(j)\exp(-y_jh_t(\sample_j))}.
    \end{align}
  \end{enumerate}
\end{itemize}
Therefore at the stage $K$ of AdaBoost, the minimization problem is equivalent to:
\begin{align}
  \label{def:stage-K-objective}
  \minimize_{h_K}\sum_{i=1}^\numSamples D_{K-1}(i)\exp(-y_ih_K(\sample_i))
\end{align}
Let us now open $h_K$ a little, by definition
\begin{align*}
  h_{K-1}(\sample) &= \alpha_Ko_K(\sample) - \alpha_{K-1}o_{K-1}(\sample) \\
         &= \alpha_K\weights_K^{\transpose}G_K(g_{K-1}(\sample)) - \alpha_{K-1}o_{K-1}(\sample)
\end{align*}
The unknowns here are only $\alpha_K, \weights_K$, and $G_K$ (the feature transformation at step $K$),
and therefore the minimization problem at boosting stage $K$ can be rewritten as:
\begin{align*}
  (\alpha_K, \weights_K, G_K) = \argmin_{\alpha, w, G} \sum_{i=1}^\numSamples D_{K-1}(\sample_i)\exp\left(
  -y_i \left(\alpha \cdot w^{\transpose} \cdot G(g_{K-1}(\sample_i)) - \alpha_{K-1}o_{K-1}(\sample_i)\right)\right)
\end{align*}
\begin{remark}
  If one plugs in the ResNet where $G_K(g_{K-1}(\sample_i)) = f_K(g_{K-1}(\sample_i)) + g_{K-1}(\sample_i)$,
  then the goal is to identify $f_K$. This recovers BoostResNet!
\end{remark}

\section{On proving that training error will vanish}

We now give a key observation of why this general residual hypothesis boosting can quickly make
the training error vanish. The argument here is really already in the proof of AdaBoost.
We want to repeat it here because it demonstrates again that there is nothing special in BoostResNet about ResNet!
Here is the key argument: In binary classification we eventually want to bound the following:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\exp\left(-y_i\left(\sum_{t=0}^{T-1}h_t(\sample_i)\right)\right)
\end{align}
This can be turned into a sum of product:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp\left(-y_ih_t(\sample_i)\right)
\end{align}
Basically, this recursive nature of $D_K$ allows us to turn this \emph{sum of product} into \emph{product of sum}.
That is:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i))
  &= \sum_{i=1}^{\numSamples}\Big\{D_0(i)\exp(-y_ih_0(\sample_i))\Big\}\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples} \left\{D_1(i)\left(\sum_{j=1}^mD_0(j)\exp(-y_jh_0(\sample_j))\right)\right\} \prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples}D_1(i)Z_1\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i))
\end{align}
where we define $Z_1 \definedAs \sum_{j=1}^mD_0(j)\exp(-y_jh_1(\sample_j))$,
which measures the quality of residual hypothesis $h_1$. Continue doing this we have:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i)) = \prod_{t=0}^{T-1}Z_t
\end{align}
where
$$Z_t \definedAs \sum_{j=1}^\numSamples D_{t}(j)\exp(-y_jh_t(\sample_j)).$$
This is the key why we can bound training error!

==> aistats/src/old_stuff/4_NNCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Neural Networks and Fairness}

Our technique for deriving sample complexity bounds is not just limited to the kernelized classifier, but we are able to compute multicalibration uniform convergence bounds any hypothesis class for which the Rademacher complexity is defined.  One such family of classifiers is the feedforward neural network:

Each hypothesis $\hyp_{\neuralNetwork}$ in the hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\mat{W} \definedAs \left(\mat{W}_1,\mat{W}_2,\dotsc,\mat{W}_\depth\right)$.  For $i \in \left\{1,\dotsc,\depth\right\}$, we assume $\mat{W}_i \in \realNumbers^{\dimension_i \times \dimension_{i-1}}$ where $\dimension_0$ is the dimension of the input vector $\sample$ and $\dimension_{\depth} = 1$.  We let $\nonlinearity(\cdot)$ denote the rectified linear unit (ReLU), i.e. for $\vec{\placeholder} \in \realNumbers^{\dimension}$, $\nonlinearity(\vec{\placeholder}) \definedAs \max\left\{\vec{\placeholder},\vec{0}_\dimension\right\}$ and is applied element-wise to $\vec{\placeholder}$. The neural network is formulated as:



\begin{dmath}
    \hyp_{\mat{W}}'(\sample) \definedAs \mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))
\end{dmath}

and the decision version of the neural network is formulated as:

\begin{dmath}\label{eq:NNHypothesisClass}
        \hyp_{\mat{W}}(\sample) \definedAs \sgn\left(\mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))\right)
\end{dmath}
An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al \cite{bartlett2017spectrally}.  We use the ``nice'' formulation of the bound from Yin et al. \cite{yin2019rademacher}.

\begin{theorem}[Theorem 5 from Yin et al.]
    Consider the neural network hypothesis class \begin{dmath}\hypothesisClass_{\neuralNetwork} \definedAs \left\{\hyp_{\neuralNetwork} : \mat{W} = (\mat{W}_1,\dotsc,\mat{W}), \\ \forall i \in \left\{1,\dotsc,\depth\right\}: \norm{\mat{W}_i}_{\sigma} \leq \spectralBound_i, \norm{\mat{W}_i}_{2,1} \leq \normBound_i\right\} \end{dmath}

    Then we have 

    \begin{dmath}
        \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{3/2}} + \frac{26\log\left(\numSamples\right)\log\left(2\dimension_{\max}\right)}{\numSamples}A
    \end{dmath}
    where $A=\norm{\mat{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\spectralBound_i \right)\left(\sum_{j=1}^{\depth} \left(\frac{\normBound_j}{\spectralBound_j}\right)^{2/3}\right)^{3/2}$
\end{theorem}

Using techniques similar to those of the previous section, we are able to determine sample complexity bounds for multicalibration uniform convergence in feedforward ReLU networks.  In particular, we develop lemmas similar to \cref{lem:shabat24analogue,lem:shabat25analogue}, but for feedforward ReLU networks:

\begin{lemma} Let $\hypothesisClass_{\neuralNetwork}$ be as defined in \cref{eq:NNHypothesisClass}.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a subpopulation.  Furthermore, let $\lambda = \min_{\hyp'\in \hypothesisClass_{\neuralNetwork}',\sample \in \sampleSpace}\left\{\hyp'(\sample)\right\}$

\end{lemma}
Scratch:
\begin{dgroup}
    \begin{dmath}
        \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\neuralNetwork}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{4}{\numSamples_{\group}^{3/2}} + \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Assume for some $\alpha \in \realNumbers_+$, $\frac{4}{\numSamples_{\group}^{3/2}} \leq \alpha \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A $}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\frac{\sqrt{\numSamples_\group-1}}{\numSamples_\group}\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(2\dimension_{\max}\right)}{\sqrt{\numSamples_{\group}}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation:}
        \begin{dmath}
                \errorTolerance^2 \leq 8\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{26^2(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
            \begin{dmath}
                = 5408\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
        \intertext{Algebraic Manipulation}
        \begin{dmath}
                \numSamples_{\group} \leq \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2} + \frac{64{\log\left(4/\errorConfidence\right)}}{\errorTolerance^2}
        \end{dmath}
\end{dgroup}
 

==> aistats/src/old_stuff/4_ballsandbins.tex <==
%!TeX root = ../note.tex

\section{Balls and Bins}\label{sec:ballsAndBins}


Before investigating the behavior of our fairness on general loss function, we seek to develop intuition via a ``balls-and-bins'' perspective: We imagine the learner, blind to protected feature $\sampleProtected$, must classify each sample (the ball) in $\trainingData$ with exactly one of $\abs{\labelSpace}$  labels (the bins).  After all examples in $\trainingData$ have been classified, a meta-learner which has access to all features of any sample, including the protected feature $\sampleProtected$.

\begin{figure}
    \input{src/img/tex/binsForLearner.tex}
\end{figure}


We may view fairness with a balls and bins perspective.  Within the two group setting in which the elements of $\labelSpace$ are discrete, we examine $\numSamples_+$ and $\numSamples_-$ impact an empirical fairness metric.  We again consider the setting in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$, however the protected groups are not always balanced: $\Pr{\sampleProtected = \groupA}$ is not necessarily equal to $\Pr{\sampleProtected = \groupB}$.

We now share our first bound on our fairness metric, which arises from two invokations of the union bound.  We utilize the following fact in our to construct our bounds: we utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$.  Note the dependence on number of labels $\abs{\labelSpace}$ appears both inside and outside the exponential. 

\begin{theorem}\label{\thmOne}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}
\end{equation}

\end{theorem}





\begin{proof}
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
    &\leq \sum_{\labelElement \in \labelSpace}\exp\paren*{-\frac{\numSamples_{+,\labelElement}\placeholder^2}{\abs*{\labelSpace}}} + \exp\paren*{-\frac{\numSamples_{-,\labelElement}\placeholder^2}{\abs*{\labelSpace}^2}}\label{eq:applyHoeffdingInequality}\\
        &\leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}\label{eq:applySimplification}
\end{align}
\end{proof}

\Cref{\thmOne} does gives us some intuition about our machine learning fairness. Namely, our fairness metric has no explicit dependence on the accuracy of our classifier.  Furthermore, this bound is broadly applicable as it is agnostic to underlying classification architecture: The bound has dependence only on the sample distribution $\sampleDist$.  This upper-bound on fairness has a dependence on the number of labels $\abs{\labelSpace}$ and the number of the lowest number of samples assigned to a (label $\labelElement$, group $\sampleProtected$) pair.

The  dependence on $\abs{\labelSpace}$ is in fact suboptimal -- the above bound is na\"vely constructed.  Whereas we only used the fact that probabilities are bounded between $0$ and $1$, we may use knowledge that the sum of all probabalistic events is $1$ to tighten our bound and yield \cref{thm:Two}.  More formally, we know:

\begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i} \end{equation} 




We will show in \cref{\thmTwo} that we can indeed eliminate the dependence on $\abs{\labelSpace}$  outside the exponential by utilizing the fact: \begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i}\end{equation}



The bound presented in $\cref{\thmOne}$ is also loose: We applied a union bound several times to arrive at $\cref{eq:applyUnionBound}$ which is an upper-bound on the left side of $\cref{eq:triangleInequality}$. By using Hoeffding's inequality, we only utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$, hence our bounds implicitly assume that the random variable $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has the maximum variance of a random variable bounded over such an interval, yet it cannot be the case, that when $\abs*{\labelSpace}\neq 2$ $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has maximum variance for each $\placeholder, \marker$ pair, as we know 

\begin{equation}
    1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}
\end{equation}

Lastly, we compare \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification}:  if the number of samples assigned to each label $\labelElement \in \labelSpace$ is balanced, then \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification} evaluate to similar quantities.  On the other hand, if there exists a label $\labelElement$ in label space $\labelSpace$ such that the number of samples assigned to that label is a small, positive rational number, then it is not hard to see  \cref{eq:applySimplification} is a very loose upper bound on \cref{eq:applyHoeffdingInequality}.  Naturally, the question which follows is, can we do better?  Indeed, we can do better, as we prove in \cref{\thmTwo}

\begin{theorem}\label{\thmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \frac{\numSamples_{ \sampleProtected,\labelElement}}{1}$

\end{theorem}


\begin{proof}
    
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
        \shortintertext{Utilizing \cref{cor:chernoffNice} with $\errorTolerance = \frac{\placeholder}{2\abs{\labelSpace}}$:}
    % &\leq \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{+,\labelElement}}{3}} +  \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{-,\labelElement}}{3}}\\
    &\leq\sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{+,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} +  \sum_{\labelElement \in \labelSpace}2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{-,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}\\
    &\leq \sum_{\labelElement \in \labelSpace} 4\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} \\
    \intertext{We invoke \cref{lem:multinomialDistributionBound} to yield the right-hand-sum:}
        &\leq 16\sum_{i=2}^{\abs{\labelSpace}} \exp\paren*{-\frac{ i\placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}} \\
        \intertext{We utilize \cref{fact:geometricSeriesFinite}, which gives a closed-form expression for a finite geometric series}
    % &=  8\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}-8 - 8\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}\\
    &<  16\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}-1} \\
    %  &=  8\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}-1+\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}}\\
          &<  16\paren*{\frac{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}}
          \shortintertext{Assume $\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}} < \sfrac{1}{2}$}
          & <  32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}^2+1}} \\
          &<32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{align}
\end{proof}

Let us now discuss \cref{\thmTwo}.  Much like in \cref{\thmOne}, the bound we present here shows that our choice of fairness metric has no dependence on the accuracy of the underlying classifier.  The bound in $\cref{\thmTwo}$ exhibits a tighter dependence on $\abs{\labelSpace}$. Indeed the discrepancy between the bounds presented in \cref{\thmOne} and \cref{\thmTwo} becomes more significant as the number of labels $\abs{\labelSpace}$ increases.  

While the implications of both \cref{\thmOne,\thmTwo} are similar, the proof of $\cref{\thmTwo}$ is more intricate: we utilize the fact that $1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}$ by invoking lemma \cref{lem:multinomialDistributionBound}.  We also invoke the Chernoff bound, \cref{thm:chernoffNice}, which can be far tighter than Hoeffding's Inequality.

Let us now devise a bound for the case that $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$. The bound follows from \cref{\thmTwo} and \cref{lem:pinsker}

\begin{corollary} \label{\corThmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} + \sqrt{2\ln\paren{2}\infdiv{\sampleDist_a}{\sampleDist_b}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{corollary}

Compared to the bounds presented in \cref{\thmOne} and \cref{\thmTwo}, the bound presented in \cref{\corThmTwo} provides a bound on our fairness metric when the distribution of labels depends on the group.




==> aistats/src/old_stuff/5_lowerBounds.tex <==
!TeX root = ../note.tex

\section{Lower Bound}
Let us now develop a lower bound on $    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder}$. 

\begin{theorem}\label{thm:lowerBound}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
\end{theorem}


\begin{proof}  
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
    &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
        &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
        &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
                &\geq 1- \paren*{1-\exp\paren*{-2\placeholder^2\numSamples_{\min}}}\label{eq:postAbsIntersection}\\
                &= \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{align}

Where to relate \cref{eq:preAbsIntersection} to \cref{eq:postAbsIntersection}, we used both Hoeffding's inequality (\cref{\hoeffding}) that for any non-negative $\placeholder$:
\begin{equation}
    \Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}} \leq \min \curlyBrace*{\Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}, \Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}>-\placeholder}}
\end{equation}
\end{proof}
Indeed, this lower bound is similar to that which is presented in \cref{\thmTwo}.  Notably, no $\abs{\labelSpace}$ term appears in the exponent. Note this lower bound is tightest when $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  A sharper bound for the case in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$ has not been developed.

{\color{blue}
CURRENTLY IN PROGRESS
\begin{theorem}\label{thm:lowerBound}
    Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  Furthermore, for all $\labelElement^{\marker} \in \labelSpace$ assume $\Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \labelElement]{\labelElement = \labelElement^{\marker}} \geq \placeholderScalar$ where $0 < \placeholderScalar < \frac{1}{\abs{\labelSpace}}$:
    \begin{equation}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq ??
    \end{equation}
    where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
    \end{theorem}

    \begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
        &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
            &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
            &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
            &\geq 1- \paren*{1-\exp\paren*{-\frac{\numSamples\placeholder^2}{2\paren*{1-\placeholderScalar\paren*{\abs{\labelSpace}-1}}\paren*{\placeholderScalar\paren*{\abs{\labelSpace}-1}} + \frac{2\placeholder}{3}}}}\\
    \end{align}
}

==> aistats/src/old_stuff/6_LossFunctions.tex <==
%!TeX root = ../note.tex
\section{Fairness and (Un-)Bounded Loss Functions}

In \cref{sec:ballsAndBins}, we examined fairness in the context of counting.  Let us now compare examine fairness in the context of positive-valued loss functions.  Let $\loss$ be a  positive-valued loss function, that is $\loss : \sampleSpace \times \labelSpace \to (0,\infty)$.

Let $\lossContribution_{\groupA}$ denote the total loss contribution from group $\groupA$

That is
 
\begin{equation}
    \lossContribution_{\evalutationData,\groupA} \definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)
\end{equation}

Similarly, we define the loss contribution from the group $\groupA$, label $\labelElement$ pair:

\begin{equation}
    \lossContribution_{\evalutationData,\groupA,\labelElement} \definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
\end{equation}

% \begin{theorem}\label{\thmOne}
%     Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
%     \begin{equation}
%         \Pr{\sum_{\labelElement \in \labelSpace}\abs{\lossContribution_{\evalutationData,\groupA,\labelElement} -\lossContribution_{\evalutationData,\groupB,\labelElement}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}}}}
%     \end{equation}
    
%     \end{theorem}


Our interest lies in bounding

\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder}
\end{equation}

Note that for all labels $\labelElement \in \labelSpace$, we have $0<\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}<1$. Furthermore, we know $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$
  
% In particular, for any $\labelElement \in \labelSpace$, we have $0 \leq \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} \leq 1$.  Furthermore, we have $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$.  These facts allow us to provide tight bounds on $ \Pr{\sum_{\labelElement \in \labelSpace}\abs{ \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} > \placeholder} $


\begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder}  
\end{align}

\begin{align}
    \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x=\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \cdot e^{tx} \differential x
\end{align}



Let us upper-bound the variance of such a random variable.

\begin{align}
    \variance\bracket*{X} &= \E{X^2} - \E{X}^2 \\
    &\leq  \E{X^2} \\
    &= \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x}} \cdot x^2 \differential x \\
    &\leq \E{X}
\end{align}

\begin{theorem}[Bhatia-Davis Inequality]
    Let $X$ be a random variable.  $X$ is bounded between $0$ and $1$, i.e. $X \in [0,1]$.  Then
    \begin{equation}
        \variance(X) \leq \paren*{1-\E{X}}\paren*{\E{X}}
    \end{equation}
\end{theorem}

\begin{theorem}[Bernstein Inequality]
    Suppose $
\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_\placeholderCount$ are i.i.d. random variables with zero mean.  If for all $i$, $\abs{\placeholderRandomVariable_i} < \scalarBound$, then for all $\placeholderCount > 0$

\begin{equation}
    \Pr{\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i > \placeholder} \leq \exp\paren*{-\frac{\placeholderCount\placeholder^2}{2\variance\paren*{\placeholderRandomVariable} + \frac{2\scalarBound \placeholder}{3} }}
\end{equation}

\end{theorem}

\begin{theorem}\label{thm:UnboundedLossFairnessUB}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
    \end{equation}
    where \begin{align}
        \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
        \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
    \end{align}
    \end{theorem}
\begin{proof}
Without loss of generality, we assume that $i \in \set{1,\dotsc,\abs{\labelSpace}}$, we have $ \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \geq \dotsc \geq  \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_{\abs{\labelSpace}}}}{\lossContribution_{\evalutationData,\groupA}}}$, then we know $\E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \leq \frac{1}{i}$


\begin{align}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder/2} + \Pr{\sum_{i = 1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder/2} \\
    &\leq \sum_{i = 1}^{\abs{\labelSpace}} \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\ 
    % \begin{split}\leq \sum_{\labelElement \in \labelSpace} \brparen*{\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
    %      \qquad \qquad+\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}}}
    % \end{split}\\
   &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}}\label{eq:theoremFollowsFromHere}
   \intertext{We now invoke the Bhatia-Davis Inequality in combination with \cref{lem:multinomialDistributionBound}}
   &\leq \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &< \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} + \frac{1}{6}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}  + \frac{1}{6}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} }}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}} \\
    \begin{split}\leq 2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
+2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
   \end{split}\\
%    \begin{split}\leq 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
%     +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
%        \end{split} \\
%        \begin{split}= 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
%         +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
%            \end{split} \\
           \begin{split}= 2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
            +2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
               \end{split} \\
               \intertext{Assume $\frac{1}{2}\geq\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}$}
              &\leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }\\
    \end{align}
\end{proof}

\begin{corollary}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } +  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
    \end{equation}
\end{corollary}




% On sub-Gaussianity of random variables:

% \begin{definition}
%     Let $\placeholderRandomVariable$ be a random variable with expectation $\E{\placeholderRandomVariable}$.  If $\placeholderRandomVariable \drawnFrom \subGaussian(\proxyStandardDeviation^2)$, then for any $t > 0$
%     \begin{align}
%         \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} > t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}} &\text{and}&& \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} < -   t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}}
%     \end{align}

% \end{definition}

% \subsection{Does the Bhatia-Davis bound on variance also a bound on proxy-variance?}

% Let $X$ be a random variable bounded between $0$ and $1$.

% \begin{align}
%     \Pr{\placeholderRandomVariable = 1} =  \Pr{\placeholderRandomVariable -\E{\placeholderRandomVariable} > 1-\E{\placeholderRandomVariable}} \leq \E{X}
% \end{align}

% Now we compare $\E{\placeholderRandomVariable}$ with $\exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}}$

% \begin{align}
%     \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}} &\leq \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\E{\placeholderRandomVariable}\paren*{1-\E{\placeholderRandomVariable}}}} \\
%     &= \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}}{2\E{\placeholderRandomVariable}}} \\
%     &= \exp\paren*{\frac{\E{\placeholderRandomVariable}-1}{2\E{\placeholderRandomVariable}}} \\
%     &=\exp\paren*{\frac{1}{2}}\exp\paren*{-\frac{1}{2\E{\placeholderRandomVariable}}}\\
% \end{align}     

==> aistats/src/old_stuff/7_lossFunctionDifference.tex <==
%!TeX root = ../note.tex
\section{The Weakness of Simple Ratios}

The ratio-type fairness bounds developed in the previous section are informative to fairness, their weakness is demonstrated in the following example:

\begin{example}
     Suppose for each $\labelElement \in \labelSpace$, $\lossContribution_{\evalutationData,\groupA,\labelElement}$ and $\lossContribution_{\evalutationData,\groupB,\labelElement}$ are positive-valued random variables, and $\placeholderScalar \neq 1$ is a positive-valued real number.  Given $\lossContribution_{\evalutationData,\groupA,\labelElement} = \placeholderScalar\lossContribution_{\evalutationData,\groupB,\labelElement}$, we see that $ 0=\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}$.  Our ratio based fairness metric suppresses the fact that when $\placeholderScalar > 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} > \lossContribution_{\evalutationData,\groupB,\labelElement}$, and when $\placeholderScalar < 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} < \lossContribution_{\evalutationData,\groupB,\labelElement}$.  We conclude that while a naive ratio-based fairness metric is informative, it suppresses differences between total loss contributions among groups.
\end{example} 

Hence, it is useful to capture in our fairness metric differences between total loss contributions among groups AND any discrepancy in ratios which the  naive ratio-based fairness metric captures.  Therefore, we consider the following fairness metric:


\begin{theorem}\label{thm:LossFunctionDifference}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
     \end{equation}
     where \begin{align}
         \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
         \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
     \end{align}
     \end{theorem}
\begin{proof}
\begin{align}
     \begin{split}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} 
     &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          & + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split} \\
     \begin{split}
          &\leq \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
          & + \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}}
     \end{split} \\
     \begin{split}
     &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}} \\
     &+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}}}
     \end{split}
\end{align}
Since $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$ and  $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$, the the rest of the proof is identical to the proof of \cref{thm:UnboundedLossFairnessUB} from equation \cref{eq:theoremFollowsFromHere} to end.
\end{proof}

\begin{corollary}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }+  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
     \end{equation}
 \end{corollary}

\hrule

Given the weakness of such naive ratio-based fairness metrics, we analyze a fairness metric which has utility in when loss is unbounded -- and avoids the pitfall of the fairness metric in the above example.  We consider 

\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}


We recognize that the above quantity is bounded by \begin{align}
     \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} &=  \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}} }
\end{align}

It is clear that both $\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}} \leq 1$ and $\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}}  \leq 1$ are true, but what can we say about $     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}}$ and $
\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}}$?

{\color{blue} The above function is not always easily interpretable}


\hrule
\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}

\begin{align}
     \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} &\leq \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }, \frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\lossContribution_{\evalutationData,\groupA} }},\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\lossContribution_{\evalutationData,\groupB} }}}
\end{align}

\begin{align}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} \leq 
     \begin{split}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split}
\end{align}



\hrule


Let us now consider $\max_{\labelElement_1,\labelElement_2 \in \labelSpace} \abs*{\log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupB,\labelElement_1}}} - \log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_2}}{\lossContribution_{\evalutationData,\groupB,\labelElement_2}}} }$

Suppose the distribution of losses is identical for both group $\groupA$ and group $\groupB$




==> aistats/src/old_stuff/__latexindent_temp.tex <==
!TeX root = ../note.tex
\section{Boosting and Fairness}

We now consider the multiclass boosting framework from Huang et al \cite{huang2018learning} in the context of fairness.
 

Trivial Bound[Bad]


\begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{theorem}

\begin{proof}
\begin{align}
\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
&\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{align}
\end{proof}

A better bound...

Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


\begin{lemma}
    Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
    \begin{equation}
        \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
    \end{equation}
\end{lemma}

Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  That is, we investigate 
\begin{equation}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\sample \in \unlabeledTrainingData \given \sampleProtected \in \groupA}\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} }{\groupWeight_{\groupA}}-\frac{\numSamples_{-,\labelElement}}{\groupWeight_{\groupB}}} > \placeholder}\end{equation}

where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$


\begin{align}
123
\end{align}
% \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> aistats/src/old_stuff/old_background.tex <==
% !TeX root = ../note.tex


\section{Background}


% \subsection{Notation and Definitions}

% Within thI is paper, we adopt the following notational conventions:

We consider a setting where we have an input set $\sampleSpace \subseteq \realNumbers^{\dimension}$ and a label set $\labelSpace$.  A sequence of examples is denoted as $\trainingData{} \subseteq \sampleSpace \times \labelSpace{}$ and contains the $\numSamples$ examples which constitute the population group.

Let $\Gamma_{\trainingData} = \set{\group_1,\dotsc,\group_{\abs{\Gamma}}}$ be a finite collection of subsets of $\trainingData$, heretoforth refered to as \emph{population subgroups}.  We follow the lead of existing multicalibration literature and assume population groups may be overlapping \cite{shabat2020sample,hebert2017calibration}.  $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  Our setting is that of binary classification: $\labelSpace = \left\{\pm 1\right\}$.  Since the labels in $\labelSpace$ are discrete, we also have $\Lambda = \left\{\pm 1\right\}$.


We now discuss our notation population subgroups: Given set of examples $\trainingData$ which will be clear from context, For each group $\group \in \Gamma_\trainingData$, $\left|\trainingData_{\group}\right|$ denotes the number of samples in $\trainingData$ within subgroup $\group$ and $\left|\trainingData_{(\group,\interval)}\right|$ denotes the number of samples in $\trainingData$ within category $(\group,\interval)$

% We now discuss the Poisson Process from which population groups are constructed:

% Samples belonging to each category $\interestingCategory \in \listInterestingCategories$ arrive in the population according to a Poisson Process with rate $\poissonRate_{\interestingCategory}$.  In this paper, we will assume $1 = \sum_{\interestingCategory \in \listInterestingCategories} \poissonRate_{\interestingCategory}$.  We denote by $\poissonRate_{\min}$, the minimum rate over over all categories, that is $\poissonRate_{\min} = \min_{\interestingCategory \in \listInterestingCategories}\poissonRate_{\interestingCategory}$

% We consider two stopping conditions:

% \begin{enumerate}
%     \item The Poisson process stops when there are exactly $\numSamples$ arrivals.
%     \item The Poisson process stops after running for $\period$ time.
% \end{enumerate}



% As necessary, subscripts will be used when enumerating training data; it may be expedient to write $\trainingData{}\definedAs \set{(\sample_1,\labelElement_1), \hdots, (\sample_{\numSamples},\labelElement_{\numSamples})}$. Let $\hypothesisClass$ be a hypothesis class from which a deterministic prediction rule, $\hyp : \sampleSpace \to \labelSpace$ is selected. For example, in a binary classification setting, a hypothesis class $\hypothesisClass$ which appears frequently in literature is the set of non-homogeneous linear classifiers in $\realNumbers^\dimension$, i.e. classifiers of the form $\hyp(\sample) = \sgn\set{\vec{w}^{\transpose}\sample + b}$ where $\vec{w} \in \realNumbers^{\dimension},b\in\realNumbers$. $\positiveIntegers$ denotes the set of positive integers.  

A \emph{protected} feature is defined to be a feature to which our learner is blind, but is of interest to a meta-learner.  Without loss of generality, we assume the population group, $\group$, is determined by the value of that protected feature. 
 
% Let $\Gamma = \set{U_1,\dotsc,U_{\abs{\Gamma}}}$ be a finite collection of population groups.  We break from a portion of multicalibration literature in which population groups may be overlapping \cite{shabat2020sample,hebert2017calibration} and instead follow the convention of Pleiss et al. \cite{pleiss2017fairness,kleinberg2016inherent}: we assume the groups to be mutually exclusive.   $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  The assumption of mutual exclusivity among population groups provides additional structure to the problem which we leverage when constructing our bounds. Namely, we know

% \begin{equation}
%    1 \geq \sum_{U \in \Gamma} \Pr[\sample \drawnFrom \sampleDist]{\sample \in U}
% \end{equation}






% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA}$ and $\numSamples_{\trainingData,\groupB}$ are calculated is clear from context, we instead write $\numSamples_{\groupA}$ and $\numSamples_{\groupB}$.

% Similarly, we denote by $\numSamples_{\trainingData,\groupA,\labelElement_i}$the number of samples in population with feature $\sampleProtected=\groupA$ and ground truth label $y=\labelElement_i \in \labelSpace$.  $\numSamples_{\trainingData,\groupB,\labelElement_i}$ denotes the number of samples in population with feature $\sampleProtected=\groupB$ and ground truth label $y=\labelElement_i$ where $\labelElement_i \in \labelSpace$.  That is, 

% \begin{align}
%     \numSamples_{\trainingData,\groupA,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupA}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}} &  \numSamples_{\trainingData,\groupB,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupB}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}}
% \end{align}

% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA,\labelElement_i}$ and $\numSamples_{\trainingData,\groupB,\labelElement_i}$ are calculated is clear from context, we instead write $\numSamples_{\groupA,\labelElement_i}$ and $\numSamples_{\groupB,\labelElement_i}$.

% % We abuse notation and take $\numSamples_{\marker,\placeholder}$ to mean $\numSamples_{\marker,\placeholder,\depth}$

% To characterize the performance of our classifiers, we will use both the emprical risk and the true risk:

% \begin{definition}
%   Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, training set $\trainingData{}$ and predictor $\hyp$, we denote the empirical risk as \begin{equation}
%       {\risk}_{\trainingData}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}} \loss\paren*{\hyp(\sample),\labelElement}
%   \end{equation}
% \end{definition}

% \begin{definition}
%     Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, sample distribution $\sampleDist$ and predictor $\hyp$, we denote the true risk as \begin{equation}
%         \risk_{\sampleDist}(\hyp) \definedAs \Ex_{(\sample,\labelElement)\drawnFrom \sampleDist}\left[{\loss\paren*{\hyp(\sample),\labelElement}}\right]
%     \end{equation}
%   \end{definition}

%   As true risk has a dependence on the unknown distribution $\sampleDist$, the exact value of the true risk is also unknown.  Hence, our characterization of classifier performance will be probabilistic bounds on the difference between true risk and empirical risk. That is, classifier performance will be characterized in the following manner:  Given a non-negative real number $\placeholder$, $\Pr{\abs{\risk_{\sampleDist}(\hyp)-\risk_{\trainingData}(\hyp)} \geq \placeholder} \leq \errorConfidence$ where $\errorConfidence$ is a real number between $0$ and $1$ which depends on $\placeholder$, the number of samples $\numSamples$ used to calculate the empirical risk, and other context dependent factors.

%   We will see that the the concentration of our fairness metric behaves in a manner similar to the way empirical risk concentrates about the true risk.

  We use several definitions from Shabat et al. \cite{shabat2020sample}, the first of which is the category:

  \begin{definition}[Category]
      A category is a pair $(\group,\interval)$ of a subgroup $\group \in \Gamma$ and an interval $I \in \Lambda$.  A category  $(\group,\interval)$ is interesting according to predictor $\hyp$ and parameters $\gamma, \psi \in (0,1]$ if $\PR_{\sample \drawnFrom \sampleDist}\left[{\sample \in \group} \right]\geq \gamma$ and  $\PR_{\sample \drawnFrom \sampleDist}\left[{\hyp\paren*{\sample} \in \interval \given \sample \in \group}\right] \geq \psi$.
  \end{definition}

%   \begin{remark}
%     Given an arrival occurs at time $t$, the probability it belongs to category $\interestingCategory$ is $\frac{\poissonRate_{\interestingCategory}}{\sum_{\interestingCategory'\in \listInterestingCategories} \poissonRate_{\interestingCategory'}}$
%   \end{remark}


We investigate how the empirical calibration error concentrates about the true multicalibration error:




  \begin{definition}[Calibration Error]
    Let $\sampleDist \subseteq \sampleSpace \times \labelSpace$ be a sample distribution and let  $(\group,\interval)$ be a category.  The calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to a category $(\group,\interval)$ is denoted $\calibrationError\paren*{\hyp,\group,\interval}$:
    \begin{dmath}
        \calibrationError\paren*{\hyp,\group,\interval} \definedAs \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[{\labelElement \given \sample \in \group, \hyp\paren*{\sample}\in \interval}\right] - \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[\hyp\paren*{\sample} \given \sample \in \group, \hyp\paren*{\sample}\in \interval\right]
    \end{dmath}


\end{definition}

Put in words, the calibration error is the difference between the expectations of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.


\begin{definition}[Empirical Calibration Error]
    Let $\trainingData\drawnFrom\sampleDist^{\numSamples}$ be a training set of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist\subseteq \sampleSpace \times \labelSpace$ and let $(\group,\interval)$ be a category.  The empirical calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to category $(\group,\interval)$ and sample $\trainingData$ is denoted $\empiricalCalibrationError\paren*{\hyp,\group,\interval,\trainingData}$
    \begin{dmath}
        \empiricalCalibrationError\paren*{\hyp,U,I,\trainingData} \definedAs \sum_{(\sample,\labelElement) \in \trainingData}\left\{\frac{\indicatorFunction\left[\sample \in \group, \hyp(\sample) \in \interval \right]}{\left|\trainingData_{(\group,\interval)}\right|}\times\left(\labelElement-\hyp(\sample)\right)\right\}
    \end{dmath}


\end{definition}

Intuitively, empirical calibration error captures the difference between the average, taken over samples in $\trainingData$, of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.



Lastly we define the Vapnik-Chervonenkis (VC) dimension \cite{vapnik1971uniform} and the Rademacher complexity \cite{bartlett2002rademacher}, two notions of function class expressiveness which are used in proving bounds multicalibration uniform convergence sample complexity bounds.

Existing state-of-the-art bounds on multicalibration uniform convergence depend on the VC dimension:

\begin{definition}[Vapnik-Chervonenkis (VC) dimension] Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A hypothesis class $\hypothesisClass$ shatters set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ if 
    \begin{dmath}
        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
    \end{dmath}

The VC-dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$
\end{definition}

While the VC-dimension represents a seminal contribution to theoretical machine learning, it does limitations.  Notably, VC-dimension does not capture the generalization properties of the Radial Basis Function (RBF) Kernel.  

The Rademacher complexity is a notion of function class expressiveness.  Our sample complexity bound for multicalibration uniform convergence will depend on the Rademacher complexity and will be applicable to the RBF kernel:



\begin{definition}[Rademacher Complexity]
    The Rademacher complexity of a hypothesis class class $\hypothesisClass$ with respect to a sample $\trainingData$ is
\begin{equation}
    \rademacherComplexity_{\trainingData}\left(\hypothesisClass\right) \definedAs \frac{1}{\numSamples}\Ex_{\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{\hypothesisClass}}\sum_{i=1}^{\numSamples}\rademacherRV_i \hyp(\sample_i)\right]
    \end{equation}
    where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$ and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$
    \end{definition}

    Our goal is to determine a bound on the sample complexity, $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorConfidence,\errorTolerance,\gamma,\psi)$, of uniform convergence guarantees on multicalibration error.  That is, we wish to determine a bound on the number of samples neeeded to yield guarantees of the form:

\begin{dmath}
    \PR\left\{\forall \hyp \hiderel{\in} \hypothesisClass,\forall \group \hiderel{\in} \Gamma, \forall \predictionValue \hiderel{\in} \labelSpace \hiderel{:} \\
    \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{dmath}

The state-of-the-art for such sample-complexity bounds was developed by Shabat et al. \cite{shabat2020sample}.  For a hypothesis class of VC-dimension $\graphDimension$ which we denote $\hypothesisClass_{\graphDimension}$, the authors claim the following multicalibration unfiform-convergence sample complexity bound:

\begin{dmath}
        \sampleComplexity_{\hypothesisClass_{\graphDimension}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

The VC-dimension is a notion of hypothesis class capacity which is independent from data.  As such, sample complexity bounds utilizing the VC dimension do not leverage any knowledge of the underlying data distribution.  On the other hand, Rademacher complexity does leverage information about the underlying data distribution, so we can surmise some sample complexity bounds which utilize Rademacher complexity will be more informative than those which leverage VC dimension.




% \begin{theorem}
%     Let $\placeholderFunction : [-1,\infty)$ be a function defined by $\placeholderFunction(\placeholder) \definedAs 2\frac{\paren*{1+\placeholder}\ln\paren*{1+\placeholder}-\placeholder}{\placeholder^2}$ and let $\placeholderRandomVariable \drawnFrom \PoissonDistribution\paren*{\poissonRate}$ for some parameter $\poissonRate > 0$.  Then for any $\placeholder > 0$, we have

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \geq \poissonRate + \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \leq \poissonRate - \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{-\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     Lastly, for any $\placeholder > 0$, we have 

%     \begin{equation}
%         \Pr{\abs{\placeholderRandomVariable - \poissonRate} \geq  \placeholder} \leq 2\exp^{-\frac{\placeholder^2}{2\paren*{\poissonRate + \placeholder}}}
%     \end{equation}


% \end{theorem}




% \begin{definition}
%   Let $\trainingData_{\marker}$ be a subset of $\trainingData{}$.  Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers^+$ and predictor $\hyp$,
%   We define the empirical risk contribution of $\trainingData_{\marker}$ (denoted by $\empiricalRisk_{\trainingData_{\marker},\trainingData{}}$, as the amount of empirical risk $\trainingData_{\marker}$ contributes to the total empirical risk over the training data:
%   \begin{equation}
%       \empiricalRisk_{\trainingData_{\marker},\trainingData{}}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}}\set*{ \loss\paren*{\hyp(\sample),\labelElement}\cdot\indicatorFunction\bracket*{(\sample,\labelElement) \in \trainingData_{\marker}}}
%   \end{equation}
% % \end{definition}

% We also define notation specially adapted to our use of residual networks:

% For the rest of note let $\depth \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $\depth$ feature transformations:

% \begin{equation}
%     \functionComposition(\sample) = (\function_{\depth} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1)(\sample),
% \end{equation}
% where $\function_t$ ($t \in \set{1,\dotsc,\depth}$) is some function. Note that $\function_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $\function_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically a convolutional neural network (CNN).
% The final binary classifier is determined by a size-conforming weight vector $\weights_T$,
% where the classification is determined as
% \begin{equation}
%     \sign(\weights_T^{\transpose}\functionComposition(\sample))
% \end{equation}
% We will use the notation $\function_{1:\depthIter}$ to mean the composition $\paren*{\function_{\depthIter} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1}(\sample)$.
% We further use the notation $g_\depthIter \definedAs G_{1:\depthIter}$ to mean the composition of the first $\depthIter$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
% Lastly, let $\BoostResNet{\boost}(\trainingData{},\depth)$ denote the $\depth$ residual network trained on training set $\trainingData{}$ as learned by the $\BoostResNet$ procedure given in Huang et al. \cite{huang2018learning}.

% \subsection{Related Results}

% The residual network, introduced in 2015 by He et al., captures the fundamental design principles underlying many of today's state-of-the-art image classifiers.  As is the case with many classes of deep networks, their performance in practice exceeds what theory is able to explain.  Furthermore, decisions made by deep networks are almost never human interpretable.  In an effort to close this gap between theory and practice while providing some degree of interpretability to deep networks, Huang et al. applied the framework of boosting to show that under certain mild conditions, the training error of a residual network exhibits exponential decay that has an explicit dependence on the depth of the network.

% todo: expand


% We begin our discussion of fairness with a motivational example.  Consider a  protected feature which has two possible values.  That is, $\sampleProtected \in \set{\groupA,\groupB}$ .  Assume the protected feature is probabilistically independent from both the label $\labelElement$ and the unprotected features $\sampleUnprotected$.  That is to say $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=+1}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=-1}$.  We do not require each protected group to be equally likely.  Suppose $\numSamples_+$ in training set $\trainingData$ are such that the value of their protected feature $\sampleProtected$  is $+1$. Given a classifier $\classifierPlaceholder \definedAs \BoostResNet(\depth,\protectedTrainingData)$, let us examine a particular choice of fairness metric, $\fairnessMetric\definedAs \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}(\hyp)-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}(\hyp)}$
% Because the protected feature is independent from both the label and the unprotected features, we have

% \begin{align}
%     \fairnessMetric = \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} &\leq \max \curlyBrace*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData},\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} \\ &=\max\curlyBrace*{\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = +1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2},\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}}\\
%     &= \frac{1}{\numSamples}\cdot \abs*{\max\set*{\abs*{\trainingData_{\curlyBrace{\sampleProtected = +1}}},\abs*{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% From this, we see the difference in size of each protected group has a direct impact on which group contributes the most to training error.  This result is entirely unsurprising, but it motivates that simple metrics, such as the difference in loss, may not be the best way to measure fairness.

% We can see, for a given training set $\trainingData$, the value of fairness metric $\fairnessMetric$ has a dependence on the imbalance in population between the protected group and unprotected group, yet the total empirical risk over the training data remains constant, regardless of how individuals are assigned to the protected or unprotected group.


% \begin{theorem}[Theorem 2.8 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffLowerBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a>b\geq 1$ and $\placeholderScalar \geq 2$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} > \frac{1}{\sqrt{2\pi}}\exp\paren*{b-\frac{1}{8\placeholderScalar}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\left(\placeholderScalar-1\right)+1 }}{(a-b)^{\paren*{a-b}\paren*{\placeholderScalar-1}-b+1}b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}


% \begin{theorem}[Theorem 2.6 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffUpperBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a\geq b\geq 1$ and $\placeholderScalar \geq 1$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} < \frac{1}{\sqrt{2\pi}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\placeholderScalar + \frac{1}{2}}}{\paren*{a-b}^{\paren*{a-b}\placeholderScalar + \frac{1}{2}} b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}

==> aistats/src/old_stuff/old_proofs_svm.tex <==
\section{Proof of \cref{thm:OurBoundSVM}}
\begin{proof}
\begin{dgroup}
   \begin{dmath}
   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
\begin{dmath}
=\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\begin{dmath}
   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp}\PR\left[ \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Substituting in $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, as per \cref{thm:CortesGeneralization}, we arrive at}:
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp} \errorConfidence'
\end{dmath}
\begin{dmath}
   =2\left|\Gamma\right|\left|\hypothesisClass\right| \errorConfidence'
\end{dmath}
\end{dgroup}




Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence'}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, where $\errorConfidence' = \frac{\errorConfidence}{2\left|\Gamma\right|\left|\hypothesisClass\right|}$ completes the proof.

\end{proof}

==> aistats/src/old_stuff/old_svm_study.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our tight multicalibration uniform convergence bounds on kernelized predictors which includes the Kernel SVM, and RELU networks with one hidden layer.



% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 

We take our description of Kernelized  classifiers from Cortes et al \cite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.

We focus on a particular class classifiers, $\hypothesisClass_{\placeholderCount}^{\q}$ the set of non-negative combinations of $\placeholderCount \geq 1$ kernels $\kernelFunction_1,\dotsc,\kernelFunction_{\placeholderCount}$ with the mixture weights obeying an $\ell_{\q}$ constraint:

\begin{equation}
   \hypothesisClass_{\placeholderCount}^{\q} \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^\placeholderCount \placeholderScalar_i\kernelFunction_i : \norm{\vec{\placeholderScalar}}_{\q} = 1, \vec{\placeholderScalar} \geq 0, \norm{\weights} \leq 1,}
\end{equation}

Cortes et al. \cite{cortes2010generalization} developed several generalization bounds for kernelized predictors.  We will utilize one such bound, \cref{thm:CortesGeneralization}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Theorem 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\placeholderCount > 1$ and assume that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and $i \in [1,\placeholderCount]$.  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis set $\hypothesisClass_\placeholderCount^1$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_\placeholderCount^1) \leq \sqrt{\frac{23e\lceil\log\placeholderCount\rceil\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

\begin{theorem}[Corollary 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:CortesGeneralization}
   Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
   \begin{equation}
      \trueRisk(\hyp) \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
   \end{equation}
   where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
\end{theorem}

The above bound requires our kernel be a non-negative combination of a fixed set of $\placeholderCount$ kernels where $\placeholderCount > 1$.  As such, our proofs will leverage a an all-zeros size-conforming `dummy'' kernel.

The last piece of the puzzle, in order to yield Rademacher complexity based sample complexity bounds for multicalibration uniform convergence, is to draw analogues of two  Graph-dimension based lemmas \cref{lem:shabat24,lem:shabat25} from Shabat et al.  We arrive at our analgoues of Shabat's lemmas by upon invokation of \cref{thm:shalevRademacherImproved}:
\begin{lemma}[Analogue of Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke \cref{thm:shalevRademacherImproved} to yield an expression for $\errorTolerance$ in terms of Rademacher complexity.  We perform algebraic manipulation:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance = 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
   
      \begin{dmath}
         \errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) = 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
      \begin{dmath}
         \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 = \frac{32c^2\log\left(4/\errorConfidence\right)}{\placeholderCount}
      \end{dmath}
      \begin{dmath}
         \numSamples_U = \frac{32c^2\ln\left(4/\errorConfidence\right)}{  \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 }
      \end{dmath}
      \intertext{Substituting in for rademacher Complexity of a kernelized classifier \cref{thm:cortesRademacher}, we see that the following inequality implies the previous inequality, we have}
      \begin{dmath}
         \numSamples_U \geq \frac{32\log\left(\frac{4}{\errorConfidence}\right)}{  \left(\epsilon - 2\sqrt{\frac{23e\scalarBound^2}{22\numSamples_U}}\right)^2 }
      \end{dmath}
     \intertext{And now algebra:}
      \begin{dmath}
         \left(\epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2 \geq 32\log\left(\frac{4}{\errorConfidence}\right)
      \end{dmath}
      \begin{dmath}
         \epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}} \geq \sqrt{32\log\left(\frac{4}{\errorConfidence}\right)}
      \end{dmath}
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{\left(\sqrt{32\log\left(\frac{4}{\errorConfidence}\right)} + 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2}{\epsilon^2}
      \end{dmath}
      \intertext{The last step is simplifying \eqref{eq:NUSampleComplexity}.  \Eqref{eq:NUSampleComplexity} holds true when   }
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}
      \end{dmath}
   \end{dgroup}
   which concludes the proof
\end{proof}


\begin{lemma}\label{lem:shabat25analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\dimension_{\graphDimension}(\hypothesisClass) \leq \dimension$ Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}


With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

\begin{theorem}
\label{thm:OurBoundSVM}
Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
\small{
   \begin{dmath}
      \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
   \end{dmath}
   }
\end{theorem}  
\begin{proof}[Proof Sketch]
The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
\end{proof}

Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  

\begin{corollary} The sample-complexity necessary for multicalibration uniform convergence in kernelized predictors is

\begin{dmath}
\numSamples\left({\errorConfidence,\errorTolerance,\gamma,\psi}\right) = \frac{1}{\errorTolerance^2 \gamma \psi}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2}}\right)^2 
=\bigOh\left(\frac{\frac{r\scalarBound^2}{\margin^2} + \log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\errorTolerance^2\gamma\psi}\right)
= \bigOh\left(\frac{{r\scalarBound^2}+ \margin^2\log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\margin^2\errorTolerance^2\gamma\psi}\right)
\end{dmath} 
\end{corollary}



This bound on the sample complexity exhibits a similar form as that of Shabat et al. The main differences, however, is that SVM-specific bound has direct dependency on the test-set margin and the kernel's sensitivity and does not depend on the graph dimension of the classifier. These differences imply that a classifier-agnostic bound for multi-calibration uniform convergence is unlikely to be effective in practice. Take for example the RBF kernel; this kernel has an infinite graph dimension but is bounded between 0 and 1. Our bound can provide a more meaningful sample complexity bound for group fairness.


Using this bound, we can present a bound on the sample complexity of two-layer RELU networks.



% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance' \right] 
% \end{dmath}

% \subsection{Failure of Multi-calibration uniform convergence}

% Inspired by the proof of failure for uniform convergence of Nagarajan et al. (Theorem 3.1 of \cite{nagarajan2019uniform}), we show the failure of multicalibration uniform convergence.   

% \begin{definition} 
%   The \emph{tightest algorithm-dependent multi-calibration uniform convergnce bound} with respect to loss $\loss$ is the smallest value $\errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$ for which there exists a set of sample sets $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ such that $\PR\left[\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}\right] \geq 1-\errorConfidence$ and if we define the space of hypotheses explored by $\learningAlgorithm$ on $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ as $\hypothesisClass_{\errorConfidence} \definedAs \union_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}} \hyp_{\trainingData} \subseteq \hypothesisClass$, the following holds: $\sup_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}}\sup_{\hyp \in \hypothesisClass_{\errorConfidence}} \leq \errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$
% \end{definition}



% \paragraph{Distribution $\placeholderDist$:} Each input $(\placeholder_1,\vec{\placeholder}_2,\vec{\placeholder}_3)$ is a $1+K+D$ dimensional vector where $\placeholder_1 \in \realNumbers$, $\vec{\placeholder}_2 \in \realNumbers^{K}$ and $\vec{\placeholder}_3 \in \realNumbers^{D}$.  $\vec{\mu} \in \realNumbers^{K}$ determines the centers of the classes.  THe label $\labelElement$ is drawn uniformly from $\left\{\pm 1\right\}$ and conditioned on $\labelElement$, we have $\vec{\placeholder}_1 = 2\labelElement\vec{\mu}$ while $\vec{\placeholder}_2$ is sampled independently from $\mathcal{N}(\vec{0}_{D},\frac{32}{D}\vec{I}_D)$


% \begin{theorem}
%   For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \left|\Gamma\right|\ln \sfrac{\numSamples}{\errorConfidence}, \left|\Gamma\right|\numSamples\ln\sfrac{1}{\errorTolerance}\right\}\right)$, there exists a category, $(U,I) \in \listInterestingCategories_{\hyp}$ for which $\errorTolerance_{\textrm{gen}}(\trainingData,U,I,\errorConfidence) \leq \errorTolerance$ while $\errorTolerance_{\unifalg}(\trainingData,U,I,\errorConfidence) \geq 1-\errorTolerance$. 
% \end{theorem}

% \begin{theorem}\label{thm:MansourFinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\gamma\psi}\right)
% \end{dmath}
% \end{theorem}


% \begin{theorem}\label{thm:MansourInfinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be an infinite predictor class from domain $\sampleSpace$ to a discrete prediction set $\labelSpace$ with finite graph-dimension $\dimension_G(\hypothesisClass) \leq \dimension$.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\dimension+ \log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\psi^2\gamma}\right)
% \end{dmath}
% \end{theorem}

% We now compare our bound (\cref{thm:kernelSampleComplexity}) which applies in the binary classification setting, to prior bounds on multicalibration uniform convergence (\cref{thm:MansourFinite,thm:MansourInfinite}) with $\lambda$, a parameter which serves as a proxy for $\left|\labelSpace\right|$, to $2$:

% Whereas 



% \begin{theorem} For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \ln \sfrac{\numSamples}{\errorConfidence}, \numSamples\ln\sfrac{2\abs{\Gamma}{\errorTolerance}}\right\}\right)$, $\greekScalar \in [0,1]$, the multi-calibration uniform convergence satisfies $\errorTolerance$
% \end{theorem}


% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\left|\left(\hat{\mu}_{\hyp}\left(\hyp,U,I,\trainingData \right)-\hat{\mu}_{\labelElement}\left(\hyp,U,I,\trainingData\right)\right)  \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right] =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \left(\hyp(\sample_i)-\labelElement_i  \right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       \leq \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \cdot \min\left(1,\left[1-\frac{\labelElement_i \hyp\left(\sample_i\right)}{\margin}\right]_+\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\hat{\risk}_{\margin,U,I}\left(\hyp\right) \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
% \end{dgroup}

% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\hat{\mu}_{\labelElement}\left(\hyp,U,I\right)-{\mu}_{\labelElement}\left(\hyp,U,I\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2}\right] 
%    \end{dmath}
% \end{dgroup}
% \begin{align}
%    \bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|{\calibrationError\left({\hyp,U,I}\right) - \empiricalCalibrationError\left({\hyp,U,I,\trainingData}\right)\right| \leq \errorTolerance}
% \end{align}

% \section{Boosting and Fairness}

% Let $\sampleInfNormUB \definedAs \E[\evaluationData \drawnFrom \sampleDist]{\max_{i}\norm{\sample_i}_\infty}$.  $\norm{\weights}_1 < \finalLinearClassifierOneNormUB  < \infty$

% \begin{theorem}[Generalization and Margin bound from Huang et al. \cite{huang2018learning}]
%    Given algorithm 1 from \cite{huang2018learning}, the fraction of training examples with margin at most $\margin$ is at most $\paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}$.  And the generalization error $\Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0}$ satisfies
%    \begin{align}
%     \Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0} &\leq \paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}\\ &+ \frac{4\finalLinearClassifierOneNormUB\sampleInfNormUB}{\margin}\sqrt{\frac{\log\paren*{2\dimension}}{2\numSamples}}\sum_{t=0}^{\depth}\weightsOneNormUB_t + \frac{2}{\margin}\sqrt{\frac{\log \depth}{\numSamples}} + \functionPlaceholder\paren*{\margin,\numSamples,\depth,\errorConfidence}
%    \end{align}
%    with probability at least $1-\errorConfidence$ for $\functionPlaceholder(\margin,\numSamples,\depth,\errorConfidence) \definedAs \sqrt{\ceil*{\frac{4}{\margin^2}\log\paren*{\frac{\margin^2 \numSamples}{\log \depth}}}\frac{\log \depth}{\numSamples} + \frac{\log \frac{2}{\errorConfidence}}{2\numSamples}}$
% \end{theorem}

% where $\weightsOneNormUB_t\definedAs \prod_{t'=0}^t2\weightsOneNormUB_{t',t'-1}$ and $\weightsOneNormUB_{t,t-1}$ is the upper bound on the $\ell_1$ norm of the weight vector connecting a neuron at layer $t$ with its preceding layer.

% THe above bound, of course, does not inform loss bounds similar to \cref{thm:LossFunctionDifference}.
 

% Trivial Bound[Bad]


% \begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
% Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
% \begin{equation}
%     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{equation}
% where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

% \end{theorem}

% \begin{proof}
% \begin{align}
% \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
% &\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% \end{proof}

% A better bound...

% Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


% % \begin{lemma}
% %     Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
% %     \begin{equation}
% %         \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
% %     \end{equation}
% % \end{lemma}

% Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  We assume  $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and proceed by bounding
% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}} \end{equation}
 
% where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$,$\indicatorFunctionInstance_{\labelElement}\paren*{\sample} \definedAs\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} $  and $\labelFunction$ is a function which returns some $\labelElement \in \labelSpace$.  

% This quantity is bounded above by

% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}}\end{equation}




% Hoeffding's inequality applies here, and yields a bound similar to the bound derived in \cref{\thmOne}.  Do sharper bounds apply?

% \begin{theorem}[Multiplicative Chernoff-Style Bound Distributions induced by Boosting]\label{thm:chernoffNice}
%     Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
%     \begin{align}
%         \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
%              \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
%     \end{align}
%     \end{theorem}
% % \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> facct/src/100_introduction.tex <==
% !TeX root = ../note.tex


\section{Introduction}


As machine learning (ML) systems have exhibited exemplary performance across a wide variety of tasks, the scope of their use has broadened to include decision-making in healthcare, education, financial, and legal settings. This intertwining of society and machine learning has surfaced the issue of fairness of such ML systems. ML fairness studies whether a given predictor achieves performance parity with respect to a sensitive attribute at the individual or group level~\cite{ind_group_fairness}. In this paper, we focus on characterizing fairness at the group level. Our focus is on understanding the performance of a predictor on different demographic groups. 


Among the most common characterizations of fairness are sample complexities for multicalibration error convergence. Multicalibration error is a notion of group fairness; it refers to the discrepancy, for a given population group, between the predicted label and the average of realized predicted labels of all samples within the group. Informally speaking, sample complexities are functions that return the number of samples necessary to achieve a specified performance guarantee associated with Empirical Risk Minimization (ERM). Sample complexity offers a probabilistic certificate on the difference between a predictor's true and empirical risk. Here, we study sample complexities for multicalibration error convergence: how many samples are needed to achieve an equitable performance of machine learning predictors over specified population groups.



Multicalibration error is a comprehensive framework that captures group fairness. Moreover, multicalibration error can be decoupled from specific training constraints and prediction accuracy. Since Hebert-Johnson et al. \cite{hebert2017calibration} introduced the notion of multicalibration error in ML, there has been much follow-up investigation about its relationship with fairness \cite{shabat2020sample,pmlr-v134-jung21a,liu2019implicit}. Thus far, multicalibration error sample complexity bounds require intensive mathematical analysis. Such analysis must take place for each notion of predictor class complexity, such as VC-dimension or Rademacher complexity. In some cases, this same analysis must be repeated for each predictor class; for example, sample complexity bounds for a Linear Support Vector Machine (SVM) may require a separate derivation from that of a two-layer Rectified Linear Unit (ReLU) network.  


This paper shows how to achieve sample complexity bounds for multicalibration uniform convergence through reparamterizing sample complexities for ERM learning, which frequently appear in the literature. We prove an explicit relationship between ERM learning sample complexity bounds and bounds for multicalibration error uniform convergence. This explicit relationship, \cref{thm:maintheorem}, grants ML practitioners a plug-and-play technique to capture the multicalibration error convergence behavior. For example, when applying our main theorem to VC dimension-based ERM bounds, we arrive at the multicalibration uniform convergence bounds by Shabat et al.~\cite{shabat2020sample}. Further, we apply our theorem to ERM sample complexity bounds based on Rademacher complexity for SVMs and two-layer ReLU networks.


Our main result implies a dependence on both dataset composition and choice of classifier architecture. Consequently, a simple classifier such as a linear SVM takes fewer samples to converge in multicalibration error than a more complicated model such as a deep neural network. Likewise, our results suggest dataset composition influences multicalibration error convergence. The least frequent group controls the sample complexity necessary to see multicalibration uniform convergence; balanced datasets lead to faster convergence. We experimentally validate our findings on tabular and image datasets. Our results in \cref{sec:evaluation} demonstrate, for each category, that when the number of samples increases, the empirical calibration error converges towards the true calibration error. Interestingly, we observe that the convergence behavior of the multicalibration error differs from that indicated by sample complexity bounds; our results suggest that calibration error may converge faster on neural network classifiers than on SVMs, which is counter to our theory. We attribute this discrepancy to ERM bounds which are known to be loose for ReLU networks.



 To summarize, we put forth a framework for ML practitioners to construct multicalibration uniform convergence bounds from sample complexities for ERM learning. As we will show, these bounds have an explicit dependence on the frequency of the least frequent protected group. This paper makes the following contributions:

\begin{enumerate}
    
    \item We show that sample complexities for state-of-the-art multicalibration uniform convergence are essentially re-parametrizations of sample complexities for ERM learning of hypothesis classes. As an example, we instantiate, via the Rademacher complexity, multicalibration bounds on small neural networks and Radial Basis Function (RBF) kernel SVMs (\cref{sec:our_bound}).
    
    \item We draw insights into dependencies of multicalibration error. We find that structural issues in both the dataset and the choice of classifier architecture induce a baseline of unfairness that cannot be overcome with any training regime.

    \item We perform empirical evaluation on several representative datasets: Adult from UCI \cite{Dua:2019}, COMPAS from ProPublica \cite{dressel2018accuracy,dieterich2016compas}, and CelebA from Chinese University of Hong Kong \cite{liu2015faceattributes} \footnote{Our codebase will be made public upon paper publication}. We study the tightness of the presented bounds and draw insights about the impact of both the data distribution and classifier regime on fairness. We show that bounds for multicalibration error convergence can be loose quite loose, especially for bounds on neural network classes.

\end{enumerate}







%this has to be tighter
% This notion of multicalibration error is similar to the colloquial use of calibration.  A predictor is multicalibrated for a population group very much like a scale at the grocery store is calibrated to consistently display the same weight for a given weight placed upon it.   




% Context typically influences the correct balance between utility and fairness.

% Often, machine learning fairness manifests itself as the implementation of so-called fairness constraints on the training of a predictive model so as to rigidly enforce fairness. The correct tradeoff between constraints  In this paper, we take a different approach: we evaluate the fairness of models after they have been trained in a standard, empirical risk minimization (ERM), training regime.

% Researchers have proposed different frameworks to formalize fairness notions. Recently, Hebert-Johnson et al applied the notion of multicalibration \cite{hebert2017calibration} error -- a comprehensive framework that captures group fairness and can be decoupled from specific from training constraints and prediction accuracy -- to machine learning.  After its introduction to the field of fairness in machine learning, multicalibration error has spurred further investigation into its relationship with fairness \cite{shabat2020sample,pmlr-v134-jung21a,liu2019implicit}. The notion of multicalibration is fairly intuitive.  When applied in the context of machine learning, multicalibration is very similar to the colloquial usage of calibration: a classifier is multicalibrated for a population group very much like a scale at the grocery store is calibrated to consistently display the same weight for a given weight placed upon it.  Thus, multicalibration error in the context of machine learning can be thought of as the discrepancy, for a fixed population group, between the predicted label and the average of realized predicted labels of all samples within the group.  Multicalibration is a notion of \emph{precision} and does not necessarily indicate accuracy: an untared scale is still calibrated as long as it consistently displays the gross weight (instead of net weight) of an intended purchase.

% In this paper, we show how multicalibration sample complexity bounds may be obtained from sample complexities for empirical risk minimization learning of hypothesis classes.  This has several implications: compared to previously existing bounds, our technique makes it easier to gain intuition regarding multicalibration uniform convergence.  Furthermore, our method shows that multicalibration uniform convergence shows a dependence on the choice of both hypothesis class and dataset.

% The ease with which we construct multicalibration uniform convergence sample complexity bounds is accomplished by a reparametrization of sample complexities for ERM.  As such, it is possible to obtain sample complexity bounds which depend on the amount and type of information available. If there is information about hypothesis architecture and dataset available, we may use a Rademacher complexity based ERM sample complexity bound, and if no such information is available, it is easy to devise a multicalibration uniform convergence bound based on the limited assumption of bounded losses.

% Our bounds also imply a dependence on both training dataset composition and choice of classifier architecture. Consequently, a simple classifier such as a linear SVM, takes fewer samples to converge in multicalibration error than does a more complicated model such as deep neural network. Likewise, our results suggest dataset composition influences multicalibration error convergence. It is the least frequent group which controls the sample complexity necessary to see multicalibration uniform convergence.  Hence, our technique suggests that balanced datasets lead to faster convergence.

% Because our technique allows the plug-and-play use of sample complexity bounds for ERM, our bounds may be applicable when current state-of-the-art multicalibration error sample-complexity bounds, as introduced by Shabat et al. \shortcite{shabat2020sample}, are not.  For example, our technique yields bounds which apply to the Radial Basis Function (RBF) Kernel SVM, whereas current state-of-the-art bounds are vacuous for such classifiers. 



% and the results apply to the general setting of calibration of measuring instruments such as pressure gauges and scales.


    % {\color{red} \textbf{Comment}: Not sure if we'll want to publish code upon project submission.  If we do submit code, we should submit it as a shortlink that we may redirect to the repository of our choosing post-submission}

==> facct/src/200_technical_background_and_motivation.tex <==
% !TeX root = ../note.tex


\section{Background}\label{sec:background}


Let us put forth the notation with which we will analyze multicalibration error: $\sampleSpace \subseteq \realNumbers^{\dimension}$ denotes the space of examples and $\labelSpace$ denotes the set of possible labels.  A sequence of examples is denoted as $\trainingData{} \subseteq \sampleSpace \times \labelSpace{}$ and contains the $\numSamples$ examples which constitute the population group.  $\trainingData$ is  $\left\{(\sample_1,\labelElement_1),\dotsc,(\sample_\numSamples,\labelElement_\numSamples)\right\}$.  Sometimes we abuse notation and use $\trainingData$ to represent an unlabeled set of training examples, i.e. $\trainingData \definedAs \left\{\sample_1,\dotsc,\sample_\numSamples \right\}$.  We may also refer to $\trainingData$ as a dataset.


The classifier architecture defines a predictor class $\hypothesisClass$, from which a predictor $\hyp : \sampleSpace \to \labelSpace$ is selected.  The terms hypothesis and predictor are used interchangably. This predictor selection process is known as \emph{training} and is performed by ERM, also known as loss minimization.  A loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$ is often used as a surrogate for accuracy.  Common examples of loss functions include logistic loss, hinge loss, and cross-entropy loss functions.  The \emph{risk} refers to the expected loss of a predictor $\hyp$.  More specifically, there two related varieties of risk to which we refer: the \emph{empirical risk} and the \emph{true risk}.  The empirical risk $\risk_{\trainingData}(\hyp)$ refers to the expected loss of a predictor $\hyp$ taken over a finite sample $\trainingData$ drawn from a data distribution $\sampleDist$:

\begin{equation}\label{eq:empiricalRisk}
    \risk_{\trainingData}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement)\in \trainingData} \loss\left(\hyp(\sample),\labelElement\right)
\end{equation}

The true risk $\risk_{\sampleDist}(\hyp)$ refers to the expected loss of a predictor taken over a typically unknown data distribution $\sampleDist$:

\begin{equation}\label{eq:trueRisk}
    \risk_{\sampleDist}(\hyp) \definedAs \E_{(\sample,\labelElement) \drawnFrom \trainingData} \loss\left(\hyp(\sample),\labelElement\right)
\end{equation}

Because $\trainingData$ is drawn i.i.d. from $\sampleDist$, $\risk_{\trainingData}(\hyp)$ is a consistent estimator of $ \risk_{\sampleDist}(\hyp)$.

The overall population $\trainingData$ breaks into potentially overlapping population groups denoted as $\group_i$.  The set of population groups is denoted $\groups$ and can be decomposed as $\set{\group_1,\dotsc,\group_{\abs{\groups}}}$. Each group $\group_i$ is associated with a frequency parameter $\gamma_i$.  That is, $\gamma_i = \Pr_{\sample \drawnFrom \sampleDist}\left[\sample \in \group_i\right]$.  Parameter $\gamma$ is defined to be the minimum of all group frequencies: $\gamma = \min_{i} \gamma_i$.  We follow the lead of existing multicalibration literature and assume population groups may be overlapping \shortcite{shabat2020sample,hebert2017calibration}.  When referring to a general population group, we may use $\group$ without subscript. 



% We now discuss our notation for population groups: given set of examples $\trainingData$, which will be clear from the context. 



A \emph{protected} feature is defined to be a feature to which our learner is blind. Though blind to the learner, such protected features may be of interest to society or an institution.  In this work, the population group $\group$ to which an example $\sample$ belongs is that example's protected feature.  That is to say, given an example $\sample$, the learner (i.e. trained classifier) is \emph{blind} to which population group $\group$ the example $\sample$ belongs, but the practitioner is \emph{aware} of the population group to which the example belongs.

Population groups are used within the definitions of category and calibration error.  More formally, 

\begin{definition}
    A category is a pair $(\group,\prediction)$ of population group $\group \in \groups$ and a predicted label $\prediction \in \labelSpace$.  

\end{definition}

% There are two parameters we use to characterize the behavior of categories. They are $\gamma$ and $\psi$.  Because $\gamma$ assume both  $(\group,\prediction)$, with respect to a predictor $\hyp$, is governed by two parameters $\gamma, \psi \in (0,1]$.   

The examples within training data which are members of category $(\group,\prediction)$ are denoted $\trainingData_{(\group,\prediction)}$.  That is

\begin{equation}
    \trainingData_{(\group,\prediction)} = \left\{\left(\sample,\labelElement\right) \in \trainingData \: :\: \sample \in \group, \labelElement=\prediction  \right\}
\end{equation}



The frequency with which a predictor $\hyp$ renders prediction $\prediction$ for each category $\group_i$ is denoted by $\psi_{\hyp,\prediction,i}$.  More precisely, $\psi_{\hyp,\prediction,i} = \Pr_{\sample \drawnFrom \sampleDist}\left[{\hyp\paren*{\sample} = \prediction \given \sample \in \group_i}\right]$. We denote by $\psi_{\hyp}$ the minimum such frequency over all such predictions: $\psi_{\hyp} = \min_{\prediction,\group} \psi_{\hyp,\prediction,i}$.  Thus, for a predictor $\hyp$, the frequency with which a category appears is $\gamma_i\psi_{\hyp,\prediction,i}$



Within the training regime, there are two losses with which we are concerned:  One is the training loss, which is typically a convex surrogate for accuracy such as cross-entropy loss or squared error.  The other is the calibration error which is the parity metric through which we understand fairness. In this work, we investigate how the empirical calibration error concentrates around the true multicalibration error.


  \begin{definition}[True Calibration Error]
    Let $\sampleDist \subseteq \sampleSpace \times \labelSpace$ be a sample distribution and let  $(\group,\prediction)$ be a category.  The calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to a category $(\group,\prediction)$ is denoted $\calibrationError\paren*{\hyp,\group,\prediction}$:
    \begin{equation}
        \calibrationError\paren*{\hyp,\group,\prediction} \definedAs \E_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[\hyp\paren*{\sample} \given \sample \in \group, \hyp\paren*{\sample}= \prediction\right] - \E_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[{\labelElement \given \sample \in \group, \hyp\paren*{\sample}= \prediction}\right]
    \end{equation}
\end{definition}

The calibration error is the difference between the expectations of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ and the hypothesis $\hyp$ rendering a prediction $\prediction$ for example $\sample$.  


\begin{definition}[Empirical Calibration Error]
\label{def:emp_cal_error}
    Let $\trainingData$ be a training set of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist\subseteq \sampleSpace \times \labelSpace$ and let $(\group,\prediction)$ be a category.  The empirical calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to category $(\group,\prediction)$ and sample $\trainingData$ is denoted $\empiricalCalibrationError\paren*{\hyp,\group,\prediction,\trainingData}$

    \begin{equation}
        \empiricalCalibrationError\paren*{\hyp,\group,\prediction,\trainingData} \definedAs \sum_{(\sample,\prediction) \in \trainingData}\left\{\frac{\indicatorFunction\left[\sample \in \group, \hyp(\sample) = \prediction \right]}{\left|\trainingData_{(\group,\labelElement)}\right|}\times\left(\hyp(\sample)-\labelElement\right)\right\}
    \end{equation}
    
\end{definition}

Unlike the true calibration error, an ML practitioner may compute the empirical calibration error without explicit access to the underling distribution $\sampleDist$.  Intuitively, the empirical calibration error captures the difference between the average, taken over samples in $\trainingData$, of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ on which predictor $\hyp$ maps an example $\sample$ to prediction $\prediction$. Within this paper, we abuse terminology and often use calibration error and multicalibration error interchangably.




% Informally, a predictor with group fairness guarantees should exhibit little discrepancy between its average classification error on any group and the error incurred by any example within the same group.  This discrepancy is denoted as the calibration error. The true calibration error establishes this notion over the data distribution $\sampleDist$, while the empirical calibration error establishes a similar notion over the training set $\trainingData$. 



We focus on how empirical calibration error concentrates around the true calibration error for each population group. In particular, we focus on sample-complexity bounds. In the context of ERM, sample-complexity bounds on a hypothesis $\hyp \in \hypothesisClass$ provide the number of i.i.d. samples drawn from a distribution $\sampleDist$ necessary to estimate, with a sufficiently small error $\errorTolerance$ and suitably high probability $1-\errorConfidence$, the true risk $\risk_{\sampleDist}(\hyp)$ of predictor $\hyp$ over that distribution $\sampleDist$. It is defined as follows.

\begin{definition}[Sample Complexity Bound]
Given a loss function, error tolerance $\errorTolerance \in [0,1)$ and confidence parameter $\errorConfidence \in (0,1]$, a sample complexity $\sampleComplexity_{\hypothesisClass}(\errorTolerance,\errorConfidence)$ is the minimum number of samples such that the following holds:


\begin{equation}
    \Pr\left\{
    \left|\risk_{\sampleDist}(\hyp) \hiderel{-} \risk_{\trainingData}(\hyp) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{equation}
\end{definition}



It is important to note that in some contexts, $\sampleComplexity_{\hypothesisClass}(\errorTolerance,\errorConfidence)$ is a \emph{distribution specific} bound. This means that it has a dependence on the data distribution, $\sampleDist$. 

For our purposes, it will also be useful to study the sample complexity for empirical risk convergence over a single population group, $\group \in \groups$. 

\begin{definition}[group sample complexity bound]\label{defn:group_complexity}
Let $\group \in \groups$ be a population group. Then given a loss function, error tolerance $\errorTolerance \in [0,1)$ and confidence parameter $\errorConfidence \in (0,1]$, a group sample complexity $\sampleComplexity_{\hypothesisClass, \group}(\errorTolerance,\errorConfidence)$ is the number of samples such that the following holds:


\begin{equation}
    \Pr\left\{
    \left|\risk_{\sampleDist_\group}(\hyp) \hiderel{-} \risk_{\trainingData_\group}(\hyp) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{equation}

Here $\sampleDist_\group$ denotes the data distribution conditioned on membership in group $\group$, and $S_\group$ denotes a sample drawn from this conditional distribution.
\end{definition}


Sample-complexity bounds for multicalibration uniform convergence capture how the difference between the true and empirical calibration errors relate to a number of context dependent factors including the size of the training set, the number of categories, and the frequency of the least common population group. Such sample-complexity bounds yield high-probability guarantees that the true calibration error is similar to the empirical calibration error for all specified categories within a dataset. Our goal is to determine a bound on that sample complexity, denoted as $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)$.  That is, we wish to determine a bound on the number of samples needed to yield guarantees of the form:

\begin{equation}\label{eq:multicalibrationUniformConvergence}
    \Pr\left[\left\{\forall \hyp \hiderel{\in} \hypothesisClass,\forall \group \hiderel{\in} \groups, \forall \predictionValue \hiderel{\in} \labelSpace \hiderel{:} \\
    \left|\calibrationError(\hyp,U,\prediction) \hiderel{-} \hat{\calibrationError}(\hyp,U,\prediction,\trainingData) \right| \hiderel{\leq} \errorTolerance \right\} \right]\geq 1-\errorConfidence
\end{equation}

where $\errorTolerance,\errorConfidence,\psi,\gamma \in (0,1]$.


Our method for doing so will be to bound the multicalibration complexity using the group sample complexity bound defined in Definition \ref{defn:group_complexity}. 



%Sample Complexity bounds are often derived utilizing a notion of predictor class capacity.  Two of the most prominent such notions are the Vapnik-Chervonenkis (VC) dimension \shortcite{vapnik1971uniform} and the Rademacher complexity \shortcite{bartlett2002rademacher} 
%%Existing state-of-the-art bounds on multicalibration uniform convergence depend on the VC dimension.
%
%\begin{definition}[VC dimension]\label{def:VCdimension} Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ shatters hypothesis class $\hypothesisClass$ if 
%    \begin{equation}
%        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
%    \end{equation}
%
%The VC dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$.
%\end{definition}
%
%{\color{red} Should we remark on multiclass generalizations of VC dimension? (graph dimension) Or would that add unnecessary complexity to the paper?}
%% The current state-of-the-art for the sample complexity bounds on uniform multicalibration convergence was developed by Shabat et al. \shortcite{shabat2020sample}.  For a hypothesis class of VC dimension $\graphDimension$ which we denote $\hypothesisClass_{\graphDimension}$, the multicalibration uniform-convergence sample complexity bound is given as:
%
%% \begin{equation}
%%         \sampleComplexity_{\hypothesisClass_{\graphDimension}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
%% \end{equation}
%
%
%% While the VC dimension represents a seminal contribution to theoretical machine learning, it has some limitations.  Notably, the VC dimension does not capture the generalization properties of kernel SVMs for which the kernel yields an infinite-dimensional feature mapping.  Examples of such kernels include the Laplace kernel and the RBF kernel. The second limitation of the VC dimension is its inability to capture the effect of the underlying data distribution on generalization (we further discuss this in Sec.~\ref{sec:evaluation}). As such, the VC dimension is a notion of hypothesis class capacity, which is independent of the underlying data distribution. 
%
%Rademacher complexity \cite{bartlett2002rademacher} is the notion of hypothesis class complexity through which we instantiate multicalibration uniform convergence bounds.  The Rademacher complexity measures hypothesis class complexity by leveraging information about the underlying data distribution. Hence, we can surmise some sample complexity bounds which utilize Rademacher complexity will be more informative than sample complexity bounds which leverage the VC dimension.
%
%
%
%\begin{definition}[Rademacher Complexity]\label{def:rademacherComplexity}
%    The Rademacher complexity of a hypothesis class  $\hypothesisClass$ with respect to a sample $\trainingData$ is
%\begin{equation}
%    \rademacherComplexity_{\trainingData}\left(\hypothesisClass\right) \definedAs \frac{1}{\numSamples}\E_{\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{\hypothesisClass}}\sum_{i=1}^{\numSamples}\rademacherRV_i \hyp(\sample_i)\right]
%    \end{equation}
%    where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$ and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{+1,-1\right\}$.
%    \end{definition}


==> facct/src/250_bounds_relationships.tex <==
%!TeX root = ../note.tex


\section{Relating Calibration and ERM Generalization}
\label{sec:our_bound}

With notation defined, we now focus on our contribution regarding multicalibration uniform convergence sample complexity bounds. The main contribution of this section is the ease with which such sample complexity bounds may be devised: \textit{Multicalibration uniform convergence sample complexity bounds are a reparametrization of ERM learning sample complexity bounds.} We begin with a theorem which formalizes the relationship between ERM and Multicalibration.  The theorem has implications on the relationship between multicalibration, hypothesis class complexity, and dataset balancing.


\begin{theorem}\label{thm:maintheorem}
   Let $\trainingData$ be an i.i.d. sample drawn from distribution $\sampleDist$, let $\groups$ be the set of groups, and let $\gamma,\psi$ be the frequency parameters described in \cref{sec:background}.  Then the multicalibration complexity can be bounded with the maximum group sample complexity. That is,  
   
  \begin{equation}
      \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) \leq \max_{\group \in \groups} \frac{2}{\gamma}\sampleComplexity_{\hypothesisClass, \group}\left(\frac{\psi\errorTolerance}{3},\frac{\errorConfidence}{4\abs{\groups}\abs{\labelSpace}}\right).
  \end{equation}
\end{theorem}



\textbf{Proof Ideas:} The main idea of proving Theorem \ref{thm:maintheorem} is to decompose the multicalibration problem into $\frac{1}{|\groups||\labelSpace|}$ separate instances. Each instances corresponds to a category $(\group, y)$. Then, for each category, we show that multicalibration for the category can be achieved by using standard ERM bounds \textit{for that category.} In particular, the category $(\group, \prediction)$ can be bounded in terms of $\sampleComplexity_{\hypothesisClass, \group}$. We then determine the number of samples needed so that each demographic group will have a sufficient number of samples to draw from (providing the $\frac{2}{\gamma}$ term). A full proof of this theorem appears in \cref{sec:ProveMainTheorem}.

% {\color{red} We may wish to make the above definition more abstract? The bounds may depend on training regime more broadly than just the hypothesis class and sample distribution, but also a myriad of factors we may wish to address. }

This theorem implies that group sample complexity is \textit{sufficient} for multicalibration. Note that these are two distinct tasks: group sample complexity is the amount of data needed to correctly estimate the loss of a given classifier whereas multicalibration is the amount of data needed to correctly estimate biases conditioned on \textit{category.} Furthermore, this theorem implies that any bounds that can be instantiated for empirical risk minimization will imply bounds on multicalibration. 



Demographic (im)balance within the dataset has been well discussed in fairness literature \cite{dwork2012fairness,buolamwini18a,barocas-hardt-narayanan}.  Interestingly, \cref{thm:maintheorem} bounds have implications in dataset balancing as well. Demographic balance manifests itself as $\gamma$. For fixed $\hypothesisClass,\errorTolerance,\errorConfidence,\psi$ and $\groups$, sample complexity for multicalibration uniform convergence $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)$ is minimized when $\gamma$ is maximized. This occurs when $\gamma = \frac{1}{\abs{\groups}}$, which is when the number of examples in each demographic is the same, i.e. when the dataset is demographically balanced.


The predictor class complexity factors into the multicalibration uniform convergence sample complexity bounds via the ERM group sample complexity bound $\sampleComplexity_{\hypothesisClass, \group}(\errorTolerance, \errorConfidence)$. The group sample complexity bound itself is a standard ERM sample complexity bound $\sampleComplexity_{\hypothesisClass}(\errorTolerance, \errorConfidence)$ conditioned on all samples being members of the specified group $\group$. In general it takes fewer samples to learn a less complicated predictor class than it does to learn a more complicated predictor class. Consider, for example, the sample complexity of a predictor class $\hypothesisClass$ with VC dimension $\graphDimension$. Shalev-Shwartz and Ben-David showed that $\sampleComplexity_{\hypothesisClass}(\errorTolerance, \errorConfidence) = \bigTheta\left(\frac{\graphDimension+\log\left(\sfrac{1}{\errorConfidence}\right)}{\errorTolerance^2}\right)$ \cite{shalev2014understanding}.  For fixed $\errorTolerance,\errorConfidence,\gamma,\psi$ and number of groups $\abs{\groups}$, as the Vapnik-Chervonenkis (VC) dimension \footnote{The definition of VC dimension is deferred to the appendix} \cite{vapnik1971uniform} of a hypothesis class increases, so does the multicalibration uniform convergence sample complexity $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)$.



\subsection{Illustrative Examples}

The choice of ERM sample complexity term also allows machine learning practitioners to loosen or tighten multicalibration uniform convergence bounds depending on how much information about the underlying classification scenario.  The more information a practitioner has, the sharper their bounds can be. For illustrative purposes, let us consider the following three scenarios. 

\begin{description}
	 \item[Scenario 1] The practitioner is aware of the predictor class $\hypothesisClass$, but has yet to receive any data.  
    \item[Scenario 2] The practitioner is aware of both the predictor class $\hypothesisClass$ and has received their labeled training dataset $\dataset$.
    \item[Scenario 3] The practitioner is aware of the predictor class, training sample $S$, and has additional knowledge of the data distribution.
\end{description}

These situations are ordered in increasing specificity -- each subsequent situation gives the practitioner more information which allows them to make tighter estimates on the amount of data needed for multicalibration. 

\subsubsection{Scenario 1: VC Dimension}

In this first setting, the practitioner has enough information to invoke the VC-dimension based ERM learning sample-complexity bounds. VC-dimension is the canonical distribution agnostic tool used to bound the sample complexity for learning a hypothesis class $\hypothesisClass.$ In particular, if $\hypothesisClass$ has VC-dimension $p$, then 
\begin{equation}
\sampleComplexity_{\hypothesisClass}(\errorTolerance, \errorConfidence) = \bigOh \left(\frac{p + \log\frac{1}{\delta}}{\epsilon^2} \right)
\end{equation}

As such, the practitioner can use \cref{thm:maintheorem} to recover the bounds of Shabat et al \cite{shabat2020sample}. That sample complexity bound is

\begin{equation}
    \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh \left(\frac{1}{\errorTolerance^2\psi^2\gamma}\left(\graphDimension+\log\left(\frac{\abs{\groups}\abs{\labelSpace}}{\errorConfidence}\right)\right)\right)
\end{equation}

\subsubsection{Scenario 2: Rademacher Complexity}

Because the practitioner now has access to both dataset $\dataset$ and the hypothesis class itself, a Rademacher-complexity based ERM learning sample-complexity bound may be invoked.  Some predictor classes have finite Rademacher complexity, but infinite or otherwise undefined VC-dimension.  The most notable such hypothesis class is the Radial Basis Function (RBF) kernel SVM. Hence, the ability to invoke a Rademacher complexity ERM learning bound may grant the ability to construct a multicalibration uniform convergence bound in a scenario for which a VC-dimension is uninformative.

We now illustrate this more precisely with two examples: Kernel SVM predictors, and ReLU activated neural networks. 


\paragraph{RBF Kernels:} Consider the Kernel SVM predictor class $\hypothesisClass_{\kernel}$:

\begin{equation}\label{eq:kernelHypClass}
 \hypothesisClass_{\kernel} \definedAs \left\{\sample \mapsto \sgn\left(\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right) : \abs{\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)} \geq 1\right\}   
\end{equation}

 where  $\kernelMapping : \realNumbers^\dimension \to \realNumbers^{\dimension'}$ is the kernel mapping function and $\dimension' \in \naturalNumbers \union \infty$.  Often, the dimension of the kernel $\dimension'$ is exceedingly large, so the \emph{kernel trick} is utilized to reduce the computational complexity of both the training of and prediction with a kernel predictor class. The kernel trick takes predictor classes of the form depicted in \cref{eq:kernelHypClass} and represents them as follows:
 
\begin{equation}\label{eq:kernelPredictor}
    \hyp(\sample) = \sum_{i=1}^\numSamples \weight_i\labelElement_i \kernelFunction\left(\sample_i,\sample \right)
\end{equation}
 
  Notably, for the RBF Kernel, $\dimension'$ is $\infty$.  Hence, the kernel trick is the only way to pragmatically deploy an RBF kernel.


By computing the Rademacher complexity (details are in section \ref{sec:boundsSec3} for this hypothesis class), we have that
\begin{equation}
\sampleComplexity_{\hypothesisClass_{\kernel}}(\errorTolerance, \errorConfidence) = \bigOh \left(\frac{B^2 + \log \frac{1}{\delta}}{\epsilon^2} \right),
\end{equation}

where $\scalarBound$ denotes the maximum value of $\kernel(\sample,\sample)$ over all $\sample$. This bound holds uniformly over all groups as the value of $\scalarBound$ is unchanged between groups. Substituting this into Theorem \ref{thm:maintheorem}, we find a multicalibration complexity of 

\begin{equation}
\sampleComplexity_{\hypothesisClass_{\kernel}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{1+ \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{equation}

\paragraph{ReLU Networks:} We can also devise a sample complexity bound for ReLU networks. Before providing the bound, we provide notational setup.  The predictor class, denoted by $\hypothesisClass_{\neuralNetwork}$, is parametrized by a sequence of matrices $\weightMatrix = (\weightMatrix_1,\dotsc,\weightMatrix_\depth)$, where $\weightMatrix_{i} \in \realNumbers^{\dimension_{i}\times\dimension_{i-1}}$ and $\dimension_0 = \dimension$. The depth of the network is $\depth$. In the binary classification setting, we have $\dimension_{\depth} = 1$, and in the multi-class setting, we have $\dimension_{\depth} = \abs{\labelSpace}$.  Let $\nonlinearity(\cdot)$ be the ReLU function.  $\nonlinearity(\vec{\placeholder})$ applies the ReLU to each coordinate in $\vec{\placeholder}$. Such networks are of the form
\begin{equation*}
    \weightMatrix_{\depth}\nonlinearity\left(\weightMatrix_{\depth-1}\nonlinearity\left(\cdots\nonlinearity\left(\weightMatrix_{1}\sample\right)\cdots\right)\right)
\end{equation*}

Thus, the ReLU predictor class is
\begin{equation}\label{eq:neuralNetworkHypothesisClass}
    \hypothesisClass_{\neuralNetwork} = \left\{\hyp_{\weightMatrix}(\sample) : \weightMatrix : \left(\weightMatrix_1,\dotsc,\weightMatrix_\depth\right), \norm{\weightMatrix_i}_2 \leq \placeholder_i, \norm{\weightMatrix_i^{\transpose}}_{2,1} \leq \placeholder'_{i}, i \in \left\{1,\dotsc,\depth\right\}\right\}
\end{equation}

By bounding the Rademacher complexity of this hypothesis class, under some mild assumptions we find a standard sample complexity (details in Appendix \ref{sec:boundsSec3}) satisfying
\begin{equation}
    \sampleComplexity_{\hypothesisClass_{\neuralNetwork}}(\errorTolerance, \errorConfidence) \leq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}
\end{equation}

This bound holds uniformly over all groups $g$ as the key parameter $\norm{\vec{X}}_{\Frobenius}^2$ upper bounds the corresponding quantity for all groups. Substituting this, the multicalibration uniform convergence sample complexity bound for this predictor class is
\begin{equation}
\sampleComplexity_{\hypothesisClass_{\neuralNetwork}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\log^2\left(\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + \log\left(\frac{\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right) 
\end{equation}

where $\vec{X}$ is the unlabeled portion of a dataset $\trainingData$, i.e. $\vec{X} = \left[\sample_1,\dotsc,\sample_N\right]$. 

\subsubsection{Scenario 3: Distribution specific bounds}

In this case, the practitioner is able to utilize their full knowledge of the distribution to obtain even tighter bounds. One important example of this is hard margin SVM classification. In this setting, let $\hypothesisClass$ be the set of all linear classifier, and let $\sampleDist$ be any distribution with hard margin $\rho$. The existence of a hard margin guarantees the existence of a linear classifier which achieves perfect accuracy on $\sampleDist$ with a margin of $\rho$, meaning that any point within distance $\gamma$ of the given point will also be classified the same. 

In this case, it is well known that $\sampleComplexity_{\hypothesisClass}(\epsilon, \delta) = O\left(\frac{D^2\log(\frac{1}{\delta})}{\rho^2 \epsilon}\right)$ where $D$ denotes the distance between the furthest two points in the data distribution. 

In our case, this bound will still hold for all groups, as the margin and diameter for each group must be at least $\rho$ and at most $D$ for each $\group \in \groups$. Applying the main theorem, we have that 

\begin{equation}
    \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh \left( \frac{D^2\log(\frac{4|\groups||\labelSpace|}{\delta})}{\rho^2 \gamma \psi \epsilon}\right).
\end{equation}

Observe that this bound is significantly tighter than the bounds in previous sections -- there is no dependence on any sample complexity measures outside of $\rho$ and $D$. Notably, $\rho$ and $D$ are both distances and have no dependence on the dimension of the data distribution. By contrast, both VC dimension and Rademacher complexity tend to include a term related to the dimensionality of the data. 


% derive our Rademacher complexity based multicalibration uniform convergence sample-complexity bounds for the kernel SVM. As indicated earlier, an advantage of this formulation is that it yields a sample-complexity of learning for nearly any classifier, even those with infinite VC-dimension.  This Rademacher complexity approach also has the added benefit of capturing the effect of the underlying data distribution on multicalibration uniform convergence.




% First, we take our description of kernels from Cortes et al. \shortcite{cortes2010generalization}.
% For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.  Since we are operating in the binary classification setting, we consider the set of kernel SVMs trained using hinge loss.


% We prescribe notation for the thresholded hypothesis class. For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernel}$:

% \begin{dmath}\label{eq:kernelHypothesisClass}
%   \hypothesisClass_{\kernel} \definedAs \left\{\sample \mapsto \sgn\left(\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right) \right\}
% \end{dmath}

% We also prescribe notation for the non-thresholded hypothesis class.  For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernelFunction}'$:

% \begin{equation}
%   \hypothesisClass_{\kernelFunction}' \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\:\bf{:}\:\lvert \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) \rvert \geq 1}
% \end{equation}

% Cortes et al. \shortcite{cortes2010generalization} developed several generalization bounds for such kernelized predictors.  We will utilize one such bound, \cref{thm:cortesRademacher}, to bound multicalibration gap over kernelized predictors.

% \begin{theorem}[Simplified version of Theorem 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:cortesRademacher}
%   Let $\kernelFunction$ be a kernel function and that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ .  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis class $\hypothesisClass_{\kernelFunction}'$ can be bounded as follows
%   \begin{dmath}
%       \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}') \leq \sqrt{\frac{23e\scalarBound^2}{22\numSamples}}
%   \end{dmath}
% \end{theorem}

% The simplification taken to yield this bound is discussed in the appendix.

% We will also need a two-sided Rademacher complexity generalization bound.




% \begin{theorem}[Two-sided Rademacher complexity based Generalization Bound]\label{thm:shalevRademacherImproved}
%   Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $\vec{\placeholder} \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp,\vec{\placeholder})\right| \leq c$. Then
%   with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
%   \begin{dgroup}
%   \begin{dmath}
%       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\placeholderCount}}
%   \end{dmath}
%   \begin{dmath}\label{eq:RademacherEmpiricalTwoSided}
%       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass)\\ + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
%   \end{dmath}
% \end{dgroup}
% \end{theorem}
% \Cref{thm:shalevRademacherImproved} represents a modification of Theorem 26.5 from Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding} as it establishes a two-sided Rademacher complexity bound for generalization. Ou proof of this theorem largely follows that of Shalev-Shwartz and Ben-David, and is deferred to the appendix.

% The last piece of the puzzle to yield Rademacher complexity based sample-complexity bounds for multicalibration uniform convergence is to draw analogues of two  graph dimension based lemmas from Shabat et al.  We arrive at our analogues of Shabat's lemmas by upon invocation of \cref{thm:shalevRademacherImproved}.  

% Before stating these lemmas, we must state the contraction lemma, which bounds the Rademacher complexity of a  function of known Lipschitz constant composed with a set of known Rademacher complexity:

% \begin{lemma}[Contraction Lemma, Theorem 7 from Meir and Zhang \shortcite{meir2003generalization}]\label{lem:contraction}
%   Let $\trainingData = \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ $\left\{\placeholderFunction\right\}_{i=1}^{\numSamples}$ be functions with Lipschitz constants $\placeholderScalar_i$, then
%   \begin{equation}
%       \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\rademacherRV_i\placeholderFunction_i(\hyp(\sample_i)) \right\} \leq \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\placeholderScalar_i\rademacherRV_i\hyp(\sample_i) \right\} 
%   \end{equation} where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$.
% \end{lemma} 

% We use the contraction lemma to determine a bound on the Rademacher complexity of $\hypothesisClass_{\kernel}$ when given both the Rademacher complexity of $\hypothesisClass_{\kernel}'$ and the value of $\min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$: 

% \begin{lemma}\label{lem:kernelHypothesisContraction}
%   Let $\hypothesisClass_{\kernel} : \sampleSpace \to \left\{\pm 1\right\}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and assume $\lambda > 0$, then we have

%   \begin{equation}
%       \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}) \leq \max\left\{\frac{1}{\lambda},1\right\}\rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}')
%   \end{equation}
% \end{lemma}

% \begin{proof}
%   Because $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$, exactly one of the following cases holds:

%   \begin{enumerate}
%       \item Case $\lambda \geq 1$:
      
%       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $1$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$

%       \item Case $0 < \lambda < 1$:
  
%       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $\frac{1}{\lambda}$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$


%   \end{enumerate}

   
%   Taking the $\max$ over both cases and applying the contraction lemma (\cref{lem:contraction}) yields the bound.
% \end{proof}
   

% The core theory underpinning our main result lies in \cref{lem:shabat24analogue,lem:shabat25analogue}.  Even though neither lemma on its own represents a bound on the sample complexity of multicalibration uniform convergence, when the statements in both \eqref{eq:statement24} and \eqref{eq:statement25}  are combined, we are able to provide the sample complexity bound on multicalibration uniform convergence, which is our main result.  Shabat et al. remark upon the difficulty of directly computing a bound on the sample complexity of multicalibration uniform convergence: uniform convergence guarantees over the infinite collection of distributions induced by the infinite hypothesis class $\hypothesisClass$ and the set of interesting categories $(\group,\interval)$ is challenging \shortcite{shabat2020sample}.



% \begin{lemma}[Analogue of Lemma 24 from \shortcite{shabat2020sample}]\label{lem:shabat24analogue}
%   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \subseteq \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
%   \begin{dmath}\label{eq:statement24}
%       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
%   \end{dmath}
% \end{lemma}

% \begin{proof}
% % \small 
%   Our proof strategy is to invoke our two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$ in terms of Rademacher complexity.  We accomplish this by setting $\errorTolerance$ to be less than or equal to the right side of \eqref{eq:RademacherEmpiricalTwoSided}.  Let $\numSamples_{\group}$ be the minimum number of samples necessary to satisfy the following inequality:
%   \begin{dgroup}
%       \begin{dmath}
%          \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
%       \end{dmath}
%       \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




%       % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

%       \begin{dmath}
%          \errorTolerance  \leq 23\max\left\{1,\frac{1}{\lambda^2}\right\} \frac{\scalarBound^2}{\numSamples_\group} + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
%       \end{dmath}


%       \intertext{Which gives us, after algebraic manipulation}

%       \begin{dmath}
%          \numSamples_{\group} < \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
%       \end{dmath}

%   \end{dgroup}
      
% Lastly, we know that if $\left|\trainingData_{\group}\right| > \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$, then $\left|\trainingData_{\group}\right| > \numSamples_{\group}$ which completes the proof.
% \end{proof}

% The proof technique for \cref{lem:shabat25analogue} is identical to that of \cref{lem:shabat24analogue}.

% \begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
%   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}'} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
%   \begin{dmath}\label{eq:statement25}
%       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
%   \end{dmath}
% \end{lemma}

% Now that we have the necessary lemmas stated, we may state our main result: a sample complexity bound for multicalibration uniform convergence, defined in~\eqref{eq:multicalibrationUniformConvergence}, which depends on the Rademacher complexity of hypothesis class $\hypothesisClass_{\kernel}$ with respect to sample $\trainingData$:

% \begin{theorem}[Main Result]\label{thm:OurBoundSVM}
%   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$,  $\hypothesisClass_{\kernel}$ has the multicalibration uniform convergence property with 

% {\small
% \begin{dmath}
%   \sampleComplexity_{\hypothesisClass_{\kernel}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2 + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
% \end{dmath}
% }
% \end{theorem}

% This bound on the sample complexity exhibits a similar form as that of Shabat et al.:

% \begin{dmath}\label{eq:shabatVCBound}
%   \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
% \end{dmath}

% where $\graphDimension$ is the graph dimension\footnote{The graph dimension is a multi-class generalization of the VC-dimension} of hypothesis class $\hypothesisClass$.

% The main difference, however, is that Rademacher complexity based bound has a direct dependence on the test-set margin and the kernel's sensitivity. Our bound has no explicit dependence on the VC dimension of the chosen hypothesis class, as we show in \cref{fig:adult_nn_bounds,fig:compas_nn_bounds}. These differences imply classifier-agnostic bounds for multi-calibration uniform convergence are unlikely to be effective in practice as notions of fairness are themselves data-dependent. Take for example the RBF kernel; this kernel has an infinite VC dimension, yet for all $\sample \in \sampleSpace$ we know $\kernelFunction(\sample,\sample) \leq \scalarBound^2 = 1$. Hence, our bound can provide a more meaningful sample complexity bound for group fairness. 

% While \cref{thm:OurBoundSVM} is fairly specific to the kernel SVM, it is possible to derive sample complexity bounds for multicalibration uniform convergence on other architectures by composing the relevant analogues to \cref{lem:shabat24analogue,lem:shabat25analogue} and replacing the Rademacher complexity of the kernel SVM with a (preferably tight) Rademacher complexity bound suitable for the choice of architecture. For instance,  one such family of classifiers is the feedforward ReLU network. An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al. \shortcite{bartlett2017spectrally}. This bound has a dependence on the number of samples, the norm of the input, and a couple varieties of matrix norm computed on the weight matrices.

% % Let us now illustrate the utility of our bound on the RBF kernel SVM.
% % \begin{example}[Example Instantiation of Bounds]. Consider the RBF kernel SVM, i.e. $\kernel_{\eta}(\sample,\sample')  = \exp\left(-\eta\norm{\sample'- \sample}_2^2\right)$ where $\eta$ is a positive real number and let $\gamma,\psi,\epsilon,\delta \in (0,1]$.  It is easy to see that $\scalarBound = 1=\max_{\sample} \kernel_{\eta}(\sample,\sample)$. which grants us a finite upper-bound on sample complexity by \cref{thm:OurBoundSVM}.  

% % Compare this to the bound of Shabat et al. (\eqref{eq:shabatVCBound}):  The RBF kernel SVM is known to have an infinite VC dimension. Hence the bound presents an upper bound of infinity on the sample complexity.

% % \end{example}







% % \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% % \end{definition}
 
% % \begin{theorem} 
% %   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
% %   \begin{equation}
% %       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
% %   \end{equation}
% % \end{theorem}
 






% % \begin{theorem}[Corollary 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:CortesGeneralization}
% %    Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
% %    \begin{equation}
% %       \risk_\hyp \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
% %    \end{equation}
% %    where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
% % \end{theorem}






% % With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

% % \begin{theorem}
% % \label{thm:OurBoundSVM}
% % Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
% % \small{
% %   \begin{dmath}
% %       \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
% %   \end{dmath}
% %   }
% % \end{theorem}  
% % \begin{proof}[Proof Sketch]
% % The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
% % \end{proof}

% % Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  








==> facct/src/300_SVMCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our Rademacher complexity based multicalibration uniform convergence sample-complexity bounds for the kernel SVM. As indicated earlier, an advantage of this formulation is that it yields a sample-complexity of learning for nearly any classifier, even those with infinite VC-dimension.  This Rademacher complexity approach also has the added benefit of capturing the effect of the underlying data distribution on multicalibration uniform convergence.




First, we take our description of kernels from Cortes et al. \shortcite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.  Since we are operating in the binary classification setting, we consider the set of kernel SVMs trained using hinge loss.


We prescribe notation for the thresholded hypothesis class. For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernel}$:

\begin{dmath}\label{eq:kernelHypothesisClass}
   \hypothesisClass_{\kernel} \definedAs \left\{\sample \mapsto \sgn\left(\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right) \right\}
\end{dmath}

We also prescribe notation for the non-thresholded hypothesis class.  For a given kernel function $\kernelFunction$ we denote this hypothesis class as $\hypothesisClass_{\kernelFunction}'$:

\begin{equation}
   \hypothesisClass_{\kernelFunction}' \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\:\bf{:}\:\lvert \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) \rvert \geq 1}
\end{equation}

Cortes et al. \shortcite{cortes2010generalization} developed several generalization bounds for such kernelized predictors.  We will utilize one such bound, \cref{thm:cortesRademacher}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Simplified version of Theorem 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\kernelFunction$ be a kernel function and that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ .  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis class $\hypothesisClass_{\kernelFunction}'$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}') \leq \sqrt{\frac{23e\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

The simplification taken to yield this bound is discussed in the appendix.

We will also need a two-sided Rademacher complexity generalization bound.




\begin{theorem}[Two-sided Rademacher complexity based Generalization Bound]\label{thm:shalevRademacherImproved}
   Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $\vec{\placeholder} \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp,\vec{\placeholder})\right| \leq c$. Then
   with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
   \begin{dgroup}
   \begin{dmath}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\placeholderCount}}
   \end{dmath}
   \begin{dmath}\label{eq:RademacherEmpiricalTwoSided}
       \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass)\\ + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
   \end{dmath}
\end{dgroup}
\end{theorem}
\Cref{thm:shalevRademacherImproved} represents a modification of Theorem 26.5 from Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding} as it establishes a two-sided Rademacher complexity bound for generalization. Ou proof of this theorem largely follows that of Shalev-Shwartz and Ben-David, and is deferred to the appendix.

The last piece of the puzzle to yield Rademacher complexity based sample-complexity bounds for multicalibration uniform convergence is to draw analogues of two  graph dimension based lemmas from Shabat et al.  We arrive at our analogues of Shabat's lemmas by upon invocation of \cref{thm:shalevRademacherImproved}.  

Before stating these lemmas, we must state the contraction lemma, which bounds the Rademacher complexity of a  function of known Lipschitz constant composed with a set of known Rademacher complexity:

\begin{lemma}[Contraction Lemma, Theorem 7 from Meir and Zhang \shortcite{meir2003generalization}]\label{lem:contraction}
  Let $\trainingData = \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ $\left\{\placeholderFunction\right\}_{i=1}^{\numSamples}$ be functions with Lipschitz constants $\placeholderScalar_i$, then
   \begin{equation}
      \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\rademacherRV_i\placeholderFunction_i(\hyp(\sample_i)) \right\} \leq \E_{\vec{\rademacherRV}}\left\{\sup_{\hyp \in \hypothesisClass} \sum_{i=1}^{\numSamples}\placeholderScalar_i\rademacherRV_i\hyp(\sample_i) \right\} 
   \end{equation} where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$.
\end{lemma} 

We use the contraction lemma to determine a bound on the Rademacher complexity of $\hypothesisClass_{\kernel}$ when given both the Rademacher complexity of $\hypothesisClass_{\kernel}'$ and the value of $\min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$: 

\begin{lemma}\label{lem:kernelHypothesisContraction}
   Let $\hypothesisClass_{\kernel} : \sampleSpace \to \left\{\pm 1\right\}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and assume $\lambda > 0$, then we have

   \begin{equation}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}) \leq \max\left\{\frac{1}{\lambda},1\right\}\rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}')
   \end{equation}
\end{lemma}

\begin{proof}
   Because $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample)\right|$, exactly one of the following cases holds:

   \begin{enumerate}
      \item Case $\lambda \geq 1$:
      
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $1$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$

       \item Case $0 < \lambda < 1$:
  
       Function $\sgn$ (in \eqref{eq:kernelHypothesisClass}) is $\frac{1}{\lambda}$-Lipschitz over $\left\{\weights^{\transpose}\kernelMapping_{\kernelFunction}(\sample) : \sample \in \sampleSpace\right \}$


   \end{enumerate}

   
   Taking the $\max$ over both cases and applying the contraction lemma (\cref{lem:contraction}) yields the bound.
\end{proof}
   

The core theory underpinning our main result lies in \cref{lem:shabat24analogue,lem:shabat25analogue}.  Even though neither lemma on its own represents a bound on the sample complexity of multicalibration uniform convergence, when the statements in both \eqref{eq:statement24} and \eqref{eq:statement25}  are combined, we are able to provide the sample complexity bound on multicalibration uniform convergence, which is our main result.  Shabat et al. remark upon the difficulty of directly computing a bound on the sample complexity of multicalibration uniform convergence: uniform convergence guarantees over the infinite collection of distributions induced by the infinite hypothesis class $\hypothesisClass$ and the set of interesting categories $(\group,\interval)$ is challenging \shortcite{shabat2020sample}.



\begin{lemma}[Analogue of Lemma 24 from \shortcite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \subseteq \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement24}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke our two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$ in terms of Rademacher complexity.  We accomplish this by setting $\errorTolerance$ to be less than or equal to the right side of \eqref{eq:RademacherEmpiricalTwoSided}.  Let $\numSamples_{\group}$ be the minimum number of samples necessary to satisfy the following inequality:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
      \end{dmath}
      \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




      % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

      \begin{dmath}
         \errorTolerance  \leq 23\max\left\{1,\frac{1}{\lambda^2}\right\} \frac{\scalarBound^2}{\numSamples_\group} + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
      \end{dmath}


      \intertext{Which gives us, after algebraic manipulation}

      \begin{dmath}
         \numSamples_{\group} < \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
      \end{dmath}

   \end{dgroup}
      
Lastly, we know that if $\left|\trainingData_{\group}\right| > \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$, then $\left|\trainingData_{\group}\right| > \numSamples_{\group}$ which completes the proof.
\end{proof}

The proof technique for \cref{lem:shabat25analogue} is identical to that of \cref{lem:shabat24analogue}.

\begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let  $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}'} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{\pm 1\right\}$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\left|\trainingData_\group\right| \geq \frac{23\max\left\{1,\frac{1}{\lambda^2}\right\} {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}\label{eq:statement25}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

Now that we have the necessary lemmas stated, we may state our main result: a sample complexity bound for multicalibration uniform convergence, defined in~\eqref{eq:multicalibrationUniformConvergence}, which depends on the Rademacher complexity of hypothesis class $\hypothesisClass_{\kernel}$ with respect to sample $\trainingData$:

\begin{theorem}[Main Result]\label{thm:OurBoundSVM}
   Let $\hypothesisClass_{\kernel}$ be a predictor class as defined in \eqref{eq:kernelHypothesisClass}. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a population subgroup.  Furthermore, let $\lambda = \min_{\hyp' \in \hypothesisClass_{\kernel}',\sample \in \sampleSpace} \left|\hyp'(\sample)\right|$ and let $\scalarBound^2 = \max_{\sample \in \sampleSpace}\kernelFunction(\sample,\sample)$.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$,  $\hypothesisClass_{\kernel}$ has the multicalibration uniform convergence property with 

{\small
\begin{dmath}
   \sampleComplexity_{\hypothesisClass_{\kernel}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2 + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}
}
\end{theorem}

This bound on the sample complexity exhibits a similar form as that of Shabat et al.:

\begin{dmath}\label{eq:shabatVCBound}
   \sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

where $\graphDimension$ is the graph dimension\footnote{The graph dimension is a multi-class generalization of the VC-dimension} of hypothesis class $\hypothesisClass$.

The main difference, however, is that Rademacher complexity based bound has a direct dependence on the test-set margin and the kernel's sensitivity. Our bound has no explicit dependence on the VC dimension of the chosen hypothesis class, as we show in \cref{fig:adult_nn_bounds,fig:compas_nn_bounds}. These differences imply classifier-agnostic bounds for multi-calibration uniform convergence are unlikely to be effective in practice as notions of fairness are themselves data-dependent. Take for example the RBF kernel; this kernel has an infinite VC dimension, yet for all $\sample \in \sampleSpace$ we know $\kernelFunction(\sample,\sample) \leq \scalarBound^2 = 1$. Hence, our bound can provide a more meaningful sample complexity bound for group fairness. 

While \cref{thm:OurBoundSVM} is fairly specific to the kernel SVM, it is possible to derive sample complexity bounds for multicalibration uniform convergence on other architectures by composing the relevant analogues to \cref{lem:shabat24analogue,lem:shabat25analogue} and replacing the Rademacher complexity of the kernel SVM with a (preferably tight) Rademacher complexity bound suitable for the choice of architecture. For instance,  one such family of classifiers is the feedforward ReLU network. An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al. \shortcite{bartlett2017spectrally}. This bound has a dependence on the number of samples, the norm of the input, and a couple varieties of matrix norm computed on the weight matrices.

% Let us now illustrate the utility of our bound on the RBF kernel SVM.
% \begin{example}[Example Instantiation of Bounds]. Consider the RBF kernel SVM, i.e. $\kernel_{\eta}(\sample,\sample')  = \exp\left(-\eta\norm{\sample'- \sample}_2^2\right)$ where $\eta$ is a positive real number and let $\gamma,\psi,\epsilon,\delta \in (0,1]$.  It is easy to see that $\scalarBound = 1=\max_{\sample} \kernel_{\eta}(\sample,\sample)$. which grants us a finite upper-bound on sample complexity by \cref{thm:OurBoundSVM}.  

% Compare this to the bound of Shabat et al. (\eqref{eq:shabatVCBound}):  The RBF kernel SVM is known to have an infinite VC dimension. Hence the bound presents an upper bound of infinity on the sample complexity.

% \end{example}







% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 






% \begin{theorem}[Corollary 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:CortesGeneralization}
%    Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
%    \begin{equation}
%       \risk_\hyp \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
%    \end{equation}
%    where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
% \end{theorem}






% With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

% \begin{theorem}
% \label{thm:OurBoundSVM}
% Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
% \small{
%   \begin{dmath}
%       \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
%   \end{dmath}
%   }
% \end{theorem}  
% \begin{proof}[Proof Sketch]
% The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
% \end{proof}

% Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  








==> facct/src/500_Experiments.tex <==
\section{Evaluation}
\label{sec:evaluation}

Our evaluation aims to show the convergence behavior of the multicalibration error. Towards that end, we leverage three popular datasets in ML experiments: the UCI Adult dataset, the Correctional Offender Management Profiling for Alternative Sanctions (COMPAS) from ProPublica, and the CelebA face recognition dataset from the Chinese University of Hong Kong. Three questions guide our evaluation:
\begin{description}

\item [{Q1.}] How does the data distribution affect the baseline multicalibration error dispersion?
    
\item [{Q2.}] Does the data distribution affect the convergence behavior of multicalibration error?

\item [{Q3.}] Does the choice of hypothesis class impact the convergence behavior of multicalibration error?
\end{description}

\input{facct/src/510_Experimental_Setup}
\input{facct/src/520_Experiment_Results}

   
   
   
   
   % plot $\empiricalCalibrationError(\hyp,\group,\prediction,\trainingData_{\test})$ where $\trainingData_{\test}$ is the 



% Given a dataset $\trainingData$, we divide i

    % \begin{enumerate}
    %     \item With respect to population demographics, how does multicalibration error dispersion behave across hypothesis classes?  Is convergence slower or otherwise less evident when hypothesis classes are more complicated? 
    %     \item Are there disparities in multicalibration error dispersion with respect to population category frequency, as indicated by our bounds?
    %     % \item With respect to the total number of examples in the training set, are there disparities in multicalibration error dispersion as indicated by our bounds?  Does the behavior match that which we calculated in our bounds? This question is evaluated on COMPAS, CelebA, and UCI Adult datasets.
    % \end{enumerate}

==> facct/src/510_Experimental_Setup.tex <==
\subsection{Experimental Setup}
\label{sec:experiment_setup}


The purpose of experiments is to study the impact of data distribution and hypothesis class on multicalibration uniform convergence behavior. In an ideal world, we would explicitly plot, for each classifier, the convergence of empirical multicalibration error to true multicalibration error, i.e., $\calibrationError(\hyp,\group,\prediction)-\empiricalCalibrationError(\hyp,\group,\prediction,\trainingData)$, as a function of category frequency $\gamma_i\psi_{\hyp,\prediction,i}$ and/or the number of examples in the dataset. Unfortunately, this requires access to the underlying data distribution, which we do not have.


Since we do not have access to the underlying data distribution, we simulate draws from it. This procedure is inspired by the seminal work of Zhang et al. \cite{zhang2016understanding}, in which randomness is applied to break the connection between examples and their labels. Instead of decoupling examples from their labels, we use randomness to decouple classifier performance from the explicit composition of training datasets. To do so, we generate many unique train-test splits, and we train classifiers on each such dataset split. 

Let $\left[\dataset_{\train}, \dataset_{\test}\right]$ by a partition of dataset $\trainingData$. Given the dataset $\dataset$, groups $\group_1$ and $\group_2$ (not necessarily the only groups in the dataset), and list of predictor classes, let $\placeholderSet_{\group_1},\placeholderSet_{\group_2}$ be sets denoting the number of examples in $\dataset_{\train}$ belonging to groups $\group_1$ and $\group_2$, respectively. Further, let $\placeholder_1,\placeholder_2$ denote elements of  $\placeholderSet_{\group_1}$ and $\placeholderSet_{\group_2}$, respectively. For each unique ordered pair $\placeholder_1,\placeholder_2$, we sample uniformly at random without replacement $\placeholder_1$ examples from $\group_1$ and $\placeholder_2$ examples from $\group_2$. $\dataset_{\train}$ consists of these randomly sampled examples along with all examples in $\dataset$ which are neither in group $\group_1$ nor in group $\group_2$. $\dataset_{\test}$ is the complement of $\dataset_{\train}$.  For each such train-test split, we train one classifier of each predictor class on training data $\dataset_{\train}$ and that classifier is evaluated on $\dataset_{\test}$.  We repeat this procedure 25 times for each such unique ordered pair $\placeholder_1,\placeholder_2$.

This procedure allows us to construct balanced datasets, and datasets that are imbalanced but with known demographic proportions. Because the test dataset $\dataset_{\test}$ is the complement of $\dataset_{\train}$, controlling the demographics of our training set means also means we are controlling that of our test set. Consequently, this procedure allows us to simulate, with finite data, the convergence behavior of empirical calibration error of each category.

\subsection{Datasets and Classifiers}

We discuss the evaluation datasets and their preparation. Categorical data are one-hot encoded, while numerical and ordinal data are left unmodified. The protected attributes for UCI Adult and COMPAS are race and sex, and the protected attribute for CelebA is sex. We plot, for each category, the empirical multicalibration error ($y$-axis) against the empirical category frequency ($x$-axis). For each train-test split and its associated classifier, the calibration error of each category is represented as a single dot on the associated scatterplot.







\subsubsection{Adult Dataset.}
\label{subsubsec:Adult_setup}
        
The Adult dataset, from the UCI machine learning repository, comprises 14 attributes and 48842 records. Entries in the dataset are extracted from the 1994 Census database. The label indicates if the income of a person exceeds \$50K. We assign an individual earning over \$50K the label $\labelElement = 1$, and if they do not, we assign them a label $\labelElement=0$.  Classifiers for the Adult dataset are trained on the following features: \texttt{Age}, \texttt{Workclass}, \texttt{fnlwgt}, \texttt{Education-Num}, \texttt{Martial Status},
        \texttt{Occupation}, \texttt{Relationship}, \texttt{Capital Gain}, \texttt{Capital Loss},
        \texttt{Hours per week}, and \texttt{Country}.  The sex and race features are withheld from training and are reserved as protected attributes.  
        
        When implementing the procedure previously defined, the two population groups, $\group_1$ and $\group_2$, correspond to male and female, respectively. Results pertaining to the race attribute may be found in \cref{sec:AdditionalFigures}. It is worth noting that the dataset contains 16192 entries representing females and 32650 entries representing males. We use $\placeholderSet_{\mathrm{male}} = \placeholderSet_{\mathrm{female}} = \left\{200,400,800,1600,3200,6400,12800\right\}$. When plotting, we only consider the classifiers trained using training sets of size between 4500 and 9000 examples. For each train-test split, we train a RBF Kernel SVM, Linear SVM, and a two-layer ReLU network consisting of 1000 hidden units.

\subsubsection{COMPAS Dataset.}
\label{subsubsec:Compas_setup}
        
The COMPAS dataset from ProPublica contains the features utilized by the COMPAS algorithm in assigning the risk of reoffending for defendants in Broward County, Florida. The dataset comprises roughly 7200 records and 28 features; the label indicates if a defendant re-offends within two years. If the defendant re-offends, we assign a label of $\labelElement = 1$, and if they do not, we assign a label of $\labelElement=0$. Classifiers on the COMPAS dataset are trained upon the following six features:  \texttt{age}, \texttt{juv_fel_count}, \texttt{juv_misd_count}, \texttt{priors_count}, \texttt{charge_id}, and \texttt{charge_degree (misd/fel)}. Sex and race features are withheld from training and are reserved as protected attributes.

The two population groups $\group_1$ and $\group_2$ correspond to male and female, respectively. Results pertaining to the race attribute may be found in \cref{sec:AdditionalFigures}. It worth noting that the dataset contains 1395 females and 5819 males. We use $\placeholderSet_{\mathrm{male}} = \placeholderSet_{\mathrm{female}} = \left\{20,40,80,160,320,640,1280\right\}$. 
When plotting, we only consider the classifiers trained using training sets of size between 800 and 1600 examples. For each train-test split,  we train an RBF Kernel SVM, Linear SVM, and a two-layer ReLU network consisting of 1000 hidden units.







\subsubsection{CelebA Dataset.}
\label{subsubsec:CelebA_setup}

The CelebA \cite{liu2015faceattributes} dataset consists of 202599 RGB face images from a total of 10177 identities.  There are 40 labeled binary attributes for each image, including sex, presence of mustache, presence of straight hair, and whether or not someone is smiling. If an attribute is present or otherwise holds true, we assign it a label $\labelElement=1$, and if not,  we assign it a label $\labelElement=0$. We use the sex attribute as a protected feature. We do not train classifiers on the CelebA data using raw images. Instead, we use 2048 dimensional embeddings of images obtained from a ResNet-152 \cite{he2016resnet} pretrained on the ImageNet \cite{Deng09imagenet} dataset.

Since we only have access to the sex attribute for examples in CelebA, we only construct train-test splits when conditioning on the sex attribute.  Plots are generated for 
classifiers trained using training sets of size between 27000 and 54000 images. When generating train-test splits, we have $\placeholderSet_{\mathrm{male}} = \placeholderSet_{\mathrm{female}} = \left\{200,400,800,1600,3200,6400,12800,25600,51200\right\}$. For each train-test split,  we train both a Linear SVM and a two-layer ReLU network consisting of 1000 hidden units.


Note that face recognition datasets, including CelebA, have become important benchmarks for machine learning practitioners. Such face recognition datasets have recently come under scrutiny due to ethics and privacy concerns. Many of these concerns relate to discrimination (racism, sexism, etc.) \cite{barocas2016big}. Consequently, dataset management procedures have been put forth to help the community become responsible dataset stewards \cite{hutchinson2021towards}. Given that CelebA is a widely disseminated dataset with strong precedent in existing literature, we feel our use of CelebA has benefit that outweighs any ethical or privacy concern. Furthermore, we do not make broad-scale conclusions regarding demographic groups: we only measure and characterize the convergence behavior of calibration error.


While there are multiple possible values for the race attribute, the Black and White groups are by far the most dominant groups in both UCI Adult and COMPAS. Hence, when conditioning on the race attribute, we augment the training set by including examples that are neither black nor white. Since there are only two sexes in the three datasets, such augmentation is unnecessary when conditioning by sex.  






==> facct/src/520_Experiment_Results.tex <==
 \subsection{Evaluation Results}

 


Each of \cref{fig:AdultSex,fig:CompasSex,fig:celeba} captures the multicalibration error of multiple predictor according to the procedure defined in \cref{sec:experiment_setup}. These plots represent scatterplots, where each point corresponds to the calibration error of a given classifier, category pair. The $x$-coordinate is the category's frequency $\gamma_i\psi_{\hyp,\prediction,i}$ in the given classifier's test set $\dataset_{\test}$, and the $y$-coordinate is that category's empirical calibration error. We can grasp the empirical distribution of multicalibration error by displaying all such points.  


The plots in \cref{fig:AdultSex,fig:CompasSex,fig:celeba} allow us to understand how the multicalibration error convergence rate relates to each dataset, its constituent demographics, and the predictor classes upon which learning occurs. This convergence rate is interpreted by visual inspection: A faster convergence rate means the vertical dispersion of calibration error, a proxy for $\errorTolerance$ (the difference between true calibration error $\calibrationError$ and empirical calibration error $\empiricalCalibrationError$), shrinks more quickly as category proportion increases. Existing ERM bounds provide the best lens of hypothesis class complexity through which we may examine the relationship between multicalibration error convergence and \cref{thm:maintheorem}.\\


 \begin{figure}[t]
    \centering
        \includegraphics[width=1.0\textwidth]{facct/src/figures/Sex_Adult.png}
    \caption{The multicalibration convergence behavior on the UCI Adult dataset, conditioned by sex.}
    \label{fig:AdultSex}
\end{figure}

\noindent
\textbf{Q1.} \textit{How does the data distribution affect the baseline multicalibration error dispersion?}

Understanding the baseline level of dispersion in multicalibration error is an important foundation for discussing its convergence behavior. This dispersion is directly related to the number of samples in each dataset. In the smallest dataset, COMPAS, we see the largest dispersion in calibration error. This is depicted in \cref{fig:CompasSex}.  At the other end of the spectrum is CelebA, our largest dataset, which is depicted in \cref{fig:celeba} has the least dispersion. When considering the dispersion properties of the Adult dataset, it is important to note the vast imbalances in category proportions. Such imbalances lead to vertical-appearing trends suggesting a large dispersion, but indeed the solution to a linear regression drawn through each category would have non-infinite slope. Consequently, the meaning the vertical dispersion is much less than a naive glance might suggest. We conclude that for a fixed category proportion, the larger the dataset, the less is the dispersion in calibration error. Indeed, if we fix all parameters in our main theorem with the exception of $\errorTolerance$, we see that decreases in $\errorTolerance$ necessitate an increased sample complexity $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)$. \\

\noindent
\textbf{Q2.} \textit{Does the data distribution affect the convergence behavior of multicalibration error?}

 The behavior we see in \cref{fig:AdultSex,fig:CompasSex,fig:celeba} captures that of ERM bounds upon which our main theorem is based.  With respect to the frequency in which a category appears in a dataset, our experiments confirm the convergence behavior of calibration error suggested by our theory (\cref{thm:maintheorem}). Furthermore, as the frequency of a category increases in a dataset, we observe the multicalibration error tends to converge. In a significant departure from the behavior suggested by ERM convergence, there is a mean shift when plotting the category-wise calibration error. Despite this mean shift, convergence behavior of multicalibration error is present as our bounds indicated would be the case. With respect to error convergence behavior, we observe different convergence rates for each dataset. This behavior is related to the number of samples in each dataset. COMPAS, our smallest dataset, as depicted in \cref{fig:CompasSex}, has some of the strongest convergence behavior among its categories. For this dataset, calibration error for each category appears as a thin line. Whereas, for the CelebA dataset as plotted in \cref{fig:celeba}, dispersion in calibration error is apparent. The dispersion of multicalibration error for the Adult dataset lies between the two. We attribute this to our sampling strategy, with less randomness in drawing training sets from a smaller dataset. However, the calibration error in COMPAS converges (faster) away from zero as evident in \cref{fig:CompasSex}, indicating a structural unfairness issue, attributed to the small dataset size. \\
 
 
 
    
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{facct/src/figures/Compas_Sex.png}
    \caption{The multicalibration convergence behavior on the COMPAS dataset, conditioned by sex. }
    \label{fig:CompasSex}
\end{figure}


\noindent
\textbf{Q3.} \textit{Does the choice of hypothesis class impact the convergence behavior of multicalibration error?}

The choice of predictor class appears to have an impact on the convergence behavior of multicalibration error, but not in the manner our bounds suggest. For all three datasets, neural networks appear to have the sharpest convergence behavior in multicalibration error. While the behavior of multicalibration error in our bounds suggests significant dispersion, this does not translate in our experiments. We attribute this discrepancy to the overparametrization of neural networks combined with the notoriously loose nature of neural network information capacity bounds. Consequently, sample complexity bounds for multicalibration error convergence in neural networks are pessimistic. The behavior of multicalibration error on SVM predictor classes is sharper than that of the neural network. Linear SVMs are less expressive than RBF SVMs, and this behavior is best captured in the plots for COMPAS \cref{fig:CompasSex}. The convergence behavior of the Linear SVM is stronger than that of the RBF SVM. In the Adult dataset, the number of examples in the least frequent categories is insufficient to draw any substantive conclusions.
    
    


    
\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{facct/src/figures/celeba_sex_attr.png}
    \caption{The convergence behavior of calibration error for the CelebA dataset, conditioned by sex. Note that the clusters for each category can overlap, obscuring the true shape of the background cluster. 
    For both the linear SVM and the neural network, the cluster in which males are predicted to have straight hair overlaps the cluster representing females also predicted to have straight hair. Also, for both the linear SVM and the neural network, the cluster representing females predicted not to be smiling obscures the cluster representing males predicted not to be smiling. }
    \label{fig:celeba}
\end{figure}


==> facct/src/600_Related_Work.tex <==
\section{Related Work}
The following discusses the related works to sample complexity measures in ERM, multicalibration error, and other fairness notions. Further, we highlight our contributions relative to these related works.

\subsection{ERM Learning}

Our results demonstrate how sample complexity bounds for ERM learning translate into multicalibration convergence bounds. ERM bounds are common in literature, including bounds on decision trees, neural networks, and other families of classifiers. Given the prevalence of machine learning classifiers and associated bounds, our main theorem (\cref{thm:maintheorem}) makes the rendering of multicalibration sample complexity bounds accessible for any ML practitioner who uses ERM bounds.

Much of modern ML fairness literature is focused on an application of constrained ERM known as learning fair classifiers. This is accomplished by performing ERM, or some variant thereof, subject to what is known as a fairness constraint. A fairness constraint is often formulated as an optimization constraint and is dependent on population group $\group$, or another protected attribute.   Examples of fairness constraints include \emph{statistical parity} (also referred to as \emph{demographic parity}) introduced by Dwork et al. \shortcite{dwork2012fairness} and \emph{equality of opportunity} introduced by Hardt et al. \shortcite{hardt2016equality}.  These works differ from ours in that a learner is assumed to have access to protected attributes: they assume the fairness constraint(s) can be enforced during training.

\subsection{Multicalibration Error}

Multicalibration error is a well-studied quantity measuring group-wise performance parity. This notion is useful when classifiers do not have access to group information; Hebert-Johnson et al. were the first to develop and study the notion of multicalibration \shortcite{hebert2017calibration} in the context of machine learning. They develop several algorithms for learning multicalibrated predictors and analyze their sample complexity. 

Liu et al. consider a two-protected group binary decision problem. The learner aims to identify the selection policy, which maximizes utility subject to a fairness constraint. Samples are assumed to have a score that serves as a proxy for selecting the utility. The authors relate the multicalibration of a learned selection policy subject to a fairness constraint to the prediction utility \shortcite{liu2018delayed}.

Liu et al. also study the relationship between multicalibration and unconstrained machine learning \shortcite{liu2019implicit}. They show that for a large class of loss functions, if a learned classifier has a small excess risk over the Bayes risk when conditioning on the protected attribute(s), the learned classifier will also be well-calibrated.

More recently, Shabat et al. utilize the graph dimension \shortcite{daniely2011multiclass}, a multi-class generalization of the VC dimension, to determine the sample-complexity necessary for uniform convergence guarantees on multicalibration error \shortcite{shabat2020sample}. Their results have no dependence on the underlying learning algorithm. Jung et al. \cite{pmlr-v134-jung21a} design algorithms which yield predictors that have guarantees on higher central moments of multicalibration error. This provides information on the geometry of the multicalibration error beyond what is given by standard mean estimates.

In this work, we showed that multicalibration error sample complexity bounds are reparametrizations of existing ERM learning sample complexity bounds. We also put forth new Rademacher-complexity based multicalibration uniform convergence sample complexity bounds.

\subsection{Other Fairness Notions}

Related to the multicalibration error is the notion of Outcome Indistinguishability. Outcome Indistinguishability, as introduced by Dwork et al. \cite{dwork2021outcome}, measures the degree to which a set of examples as labeled by nature differs from the same set of examples labeled as a synthetic or trained classifier. Furthermore, Dwork et al. demonstrate that enforcing outcome indistinguishability transitively enforces multicalibration and vice-versa. Kearns et al. utilized the VC dimension \shortcite{vapnik1971uniform}  in their study of auditing algorithms for the prevention of fairness gerrymandering \shortcite{kearns2018preventing}. Another closely related paper is Rothblum and Yona's \cite{rothblum2021multi} study of Multi-group Probably Approximately Correct (PAC) Learnability. For a fixed loss function, the authors provide an algorithm that produces a classifier that guarantees that each population group has a similar average loss. The authors also provide sample complexity bounds for Multi-group PAC learning.



==> facct/src/700_conclusion.tex <==
%!TeX root = ../note.tex

\section{Conclusion and Future Work}

This paper explored machine learning fairness from the perspective of sample complexities for multicalibration uniform convergence. We proved that multicalibration uniform convergence bounds are reparametrizations of ERM learning sample complexity bounds. This reparametrization subsumes existing state-of-the-art sample complexity bounds for multicalibration error uniform convergence. Furthermore, utilizing our main theorem, we put forth a novel Rademacher complexity style bound on multicalibration uniform convergence. Beyond these theoretical contributions, we explored our bounds and the overarching concept of multicalibration uniform convergence with experimentation using a two-layer ReLU network, linear SVM, and RBF SVM. Our results provide ML practitioners, equipped with ERM learning bounds, a plug-and-play technique that yields sample complexity bounds for multicalibration uniform convergence. 

In future work, we will explore the empirical behavior of multicalibration error convergence in larger datasets and machine learning applications such as voice recognition and image recognition. As machine learning fairness is intrinsically a human-centered problem, we will focus on how the existing theory for fair classifiers matches the performance of such classifiers in these more human-focused settings. In a more theoretical vein, sharp sample complexity lower bounds for multicalibration error also present an interesting research direction.

==> facct/src/A050_Additional_Figures.tex <==
   \section{Additional Figures}\label{sec:AdditionalFigures}
   
   In this section we discuss the preparation of datasets for plotting the race attribute.
   
   \subsubsection*{Adult dataset}
        

The Adult dataset from the UCI machine learning repository comprises 14 attributes and 48842 records.  Entries in the dataset are extracted from the 1994 Census database. The label indicates if the income of a person exceeds \$50K. With respect to race, there are 470 entries with American Indian and Eskimo as the race attribute, 1519 entries with Asian and Pacific-Islander as the race attribute, 4685 entries with Black as the race attribute, 41762 entries with White as the race attribute, and 406 with Other as the race attribute.

        
For the race attribute, when implementing the procedure previously defined in \cref{sec:evaluation},  the two population groups, $\group_1$ and $\group_2$ correspond to Black and White, respectively. We use $\placeholderSet_{\mathrm{White}} = \placeholderSet_{\mathrm{Black}} = \left\{20,40,80,160,320,640,1280,2560\right\}$. When plotting the race attribute, only considered are classifiers trained on between 2500 and 5000 examples.
        

        % $\vec{\placeholder}_{\mathrm{white}} = \left\{20,40,80,160,320,640,1280,2560\right\}$
        
        For each train-test split,  we train  a Radial Basis Function (RBF) Kernel Support Vector Machine (SVM), Linear SVM,  and a two-layer ReLU network consisting of 1000 hidden units.

\subsubsection*{COMPAS dataset.}
        
The COMPAS dataset from ProPublica. This dataset contains the features utilized by the COMPAS algorithm in assigning the risk of reoffending for defendants in Broward County, Florida. With respect to race, there are 3175 individuals with Black as the race attribute, 2103 individuals with White as the race attribute, 509 with Hispanic as the race attribute, 31 with Asian as the race attribute, 11 with Native American as the race attribute, and 343 individuals with a race attribute listed as Other. the The dataset comprises roughly 7200 records and 28 features; the label indicates if a defendant re-offends within two years. For the race attribute, the two population groups, $\group_1$ and $\group_2$ correspond to Black and White, respectively. We use $\placeholderSet_{\mathrm{White}} = \placeholderSet_{\mathrm{Black}} = \left\{20,40,80,160,320,640,1280\right\}$.

 For both the race attributes, plots are generated for classifiers trained on between 800 and 1600 examples. For each train-test split,  we train a RBF Kernel SVM, Linear SVM, and a two-layer ReLU network consisting of 1000 hidden units.


\begin{figure}[b]
    \centering
        \includegraphics[width=1.0\textwidth]{facct/src/figures/Race_Adult.png}
    \caption{The multicalibration convergence behavior on the UCI Adult dataset, conditioned by race.}
     \label{fig:AdultRace}
\end{figure}


\begin{figure}[b]
    \centering
        \includegraphics[width=1.0\textwidth]{facct/src/figures/Compas_Race.png}
    \caption{The multicalibration convergence behavior on the COMPAS dataset, conditioned by race.  }
    \label{fig:CompasRace}
\end{figure}



==> facct/src/A100_proofs.tex <==
%!TeX root = ../note.tex
\section{Existing Lemmas and Definitions}

In this section we re-state, for completeness, several lemmas which appear in the paper by Shabat et al.  In our main paper, for the lemmas stated here which have a dependence on VC dimension and/or graph dimension of an underlying hypothesis class, we developed analogues with dependence on the class's Rademacher complexity.

\begin{lemma}[Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.   Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 25 from \cite{shabat2020sample}]\label{lem:shabat25}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\graphDimension_{\mathcal{G}}(\hypothesisClass) \leq \graphDimension$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let ${\group} \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is the induced distribution on $\group \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\numSamples}$ is a random sample of $\numSamples \geq C\frac{\graphDimension + \log\left(\frac{1}{\errorConfidence}\right)}{\errorTolerance^2}$ examples drawn i.i.d. according to $\sampleDist_{\group}$, then with probability at least $1-\errorConfidence$:
    \begin{dmath}
        \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
    \end{dmath}
\end{lemma}

\begin{lemma}[Lemma 26 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat26}
   Let $p_1,p_2,\tilde{p}_1,\tilde{p}_2,\epsilon,\psi \in [0,1]$ such that $p_1,\psi \leq p_2$ and $\left|p_1-\tilde{p}_1\right|,\left|p_2-\tilde{p}_2\right| \leq \psi\epsilon/3$.  Then,

   \begin{equation}
      \left|\frac{p_1}{p_2} - \frac{\tilde{p}_1}{\tilde{p}_2}\right| \leq \epsilon
   \end{equation}

\end{lemma}

\begin{lemma}[Lemma 27 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat27}
   Let $\gamma \in (0,1)$ and let $\Gamma_\gamma = \left\{\group \in \Gamma \given \Pr_{\sample \drawnFrom \sampleDist}\left[\sample \in \group\right] \geq \gamma\right\}$ be the collection of subpopulations from $\Gamma$ that has probability at least $\gamma$ according to $\sampleDist$.  Let $\errorConfidence \in (0,1)$ and let $\trainingData$ be a random sample of $\numSamples$ drawn i.i.d. from $\sampleDist$.  Then with probability at least $1-\errorConfidence$, if $\numSamples \geq \frac{8\log\left(\frac{\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$,

   \begin{dmath}
      \forall \group \in \Gamma_{\gamma} \hiderel{:} \left|\trainingData \intersection \group\right| \hiderel{>} \frac{\gamma \numSamples}{2}
   \end{dmath}

\end{lemma}

\begin{remark}[Remark on Theorem 1]
Firstly, we expand on the simplification from Theorem 2 by Cortes et al. taken to yield \cref{thm:cortesRademacher}.  Our \cref{thm:cortesRademacher}, which is a simplification of theorem 2 as by given Cortes et al. \cite{cortes2010generalization}, is a bound on the hypothesis class consisting of a non-negative combinations of at least two kernels. Given a set $\placeholderCount \geq 2$,  The authors' theorem 2 applies to the hypothesis class denoted $\hypothesisClass_{\placeholderCount}^1$ where

\begin{dmath}
\hypothesisClass_{\placeholderCount}^1 \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^{\placeholderCount}\alpha_i\kernelFunction_i, \norm{\weights} \leq 1, \vec{\alpha} \geq 0, 1= \sum_{i=1}^{\placeholderCount}\alpha_i \right\}
\end{dmath}

Our non-thresholded hypothesis class $\hypothesisClass_{\kernel}'$, on the other hand, consists of only one kernel:

\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :   \norm{\weights} \leq 1\right\}
\end{dmath}

 



Hence, when invoking the bounds from Cortes et al., we implicitly consider our hypothesis class to be non-negative combinations of our kernel and a dummy kernel $\kernelFunction_{\mathrm{dummy}}$.  The dummy kernel is assumed to always have weight $0$.  We accomplish this by re-writing $\hypothesisClass_{\kernel}'$ as
\begin{dmath}
\hypothesisClass_{\kernel}' \definedAs \left\{\sample \mapsto \weights \cdot \kernelMapping_{\kernelFunction}(\sample) :  \kernelFunction = 1\cdot \kernelFunction + 0\cdot\kernelFunction_{\mathrm{dummy}}, \norm{\weights} \leq 1\right\}
\end{dmath}


\end{remark}



==> facct/src/A200_rademacher_two_sided.tex <==
%!TeX root = ../note.tex


\section{Two-sided Rademacher Complexity Bounds}\label{sec:rad_appendix}



In this section, we discuss the motivation behind the one-sided Rademacher complexity based generalization bounds of Shalev-Shwartz and Ben-David \shortcite{shalev2014understanding}, and we show how to transform these bounds into two-sided generalization bounds.  Notation and proof techniques in this section largely follow that of Shalev-Shwartz and Ben-David.  Furthermore, the notation is also largely consistent with notation of Shabat et al \cite{shabat2020sample}.  Using the Rademacher random variable, Bartlett et al. \cite{bartlett2002rademacher} were able to develop a notion of expressiveness for a given function class.  This measure of expressiveness is known as the Rademacher Complexity:

\begin{definition}[Rademacher Complexity]\label{def:rademacherComplexity}
The Rademacher complexity of a function class $\mathcal{H}$ with respect to a sample $\trainingData$ is
\begin{equation}
\rademacherComplexity\left(\mathcal{H} \circ \trainingData \right) \definedAs \frac{1}{\numSamples}\E_{\vec{\rademacherRV}\drawnFrom\left\{\pm 1\right\}}\left[\sup_{f \in \mathcal{H}}\sum_{i=1}^{\numSamples}\rademacherRV_i f(\vec{\placeholder}_i)\right]
\end{equation}
where sample $\trainingData \definedAs \left\{\vec{\placeholder}_1,\dotsc,\vec{\placeholder}_\numSamples \right\}$ is a set of of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$.
and $\mathcal{H} \circ \trainingData$ denotes the set of all possible evaluations a function $f \in \mathcal{H}$ can achieve on a sample $\trainingData$, i.e.
\begin{equation}
    \mathcal{H} \circ \trainingData \definedAs \left\{(f(\vec{\placeholder}_1),\dotsc,f(\vec{\placeholder}_\numSamples)) : f \in \mathcal{H}\right\}
\end{equation}
\end{definition}

The Rademacher complexity (\cref{def:rademacherComplexity}) is a useful notion of function class expressiveness because it can be used to bound the \emph{representativeness} of a sample $\trainingData$ with respect to $\loss \circ \mathcal{H}$ as the largest gap between the true risk of a function $\hyp$ and its empirical risk.



\begin{definition}
    The \emph{representativeness} of $\trainingData$, a sample drawn from distribution $\sampleDist$, with respect to $\mathcal{H}$, denoted $\Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData)$, is the largest gap between the true risk of a hypothesis $\hyp$ in hypothesis class $\hypothesisClass$ and its empirical risk.
\begin{equation}
    \Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData) \definedAs \sup_{\hyp \in \mathcal{H}} \left(L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right)
\end{equation}
\end{definition}

The following lemma, from Shalev-Shwartz and Ben-David  describes the relationship between expected representativeness and expected Rademacher complexity:

\begin{lemma}[Lemma 26.2 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{lem:representativeness}
    \begin{equation}
\E_{\trainingData \drawnFrom \sampleDist} \Representativeness_{\sampleDist}(\loss \circ \mathcal{H},\trainingData) \leq 2 \E_{\trainingData \drawnFrom \sampleDist} \rademacherComplexity_{\trainingData}\left(\loss\circ\mathcal{H} \right) 
    \end{equation}
\end{lemma}

Inspired by this bound, it is possible to construct generalization bounds based on empirical Rademacher complexity:

\begin{theorem}[Theorem 26.5 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{thm:shalevRademacher}
    Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be an i.i.d. sample of size $\numSamples$. Assume that for all $(\sample,\labelElement) \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp(\sample),\labelElement)\right| \leq c$. Then
    with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
    \begin{align}
        L_\sampleDist(\hyp) - L_{\trainingData}(\hyp) &\leq 2\E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\numSamples}} \\
        L_\sampleDist(\hyp) - L_{\trainingData}(\hyp) &\leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
\end{align}
\end{theorem}



Note that \cref{thm:shalevRademacher} contains only one-sided bounds on $L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)$, yet we would like two-sided bounds, i.e. bounds on the probability $\left|L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right|$ is small.  Let us now pursue such bounds $\left|L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp)\right|$ using the Rademacher complexity.  Our proof follows the style of the proof of lemma 26.2 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}.  

\begin{lemma}[Two-sided version of \cref{lem:representativeness}]\label{lem:improvedRepresentativeness}
    \begin{equation}
    \E_{\trainingData \drawnFrom \sampleDist^\numSamples} \sup_{\hyp \in \mathcal{H}} \left|L_{\sampleDist}(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2 \E_{\trainingData \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData}\left(\loss \circ \mathcal{H} \right) 
    \end{equation}
\end{lemma}
\begin{proof}
Let us now provide a proof of  \cref{lem:improvedRepresentativeness}:

\begin{align}
    \sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right| &= \sup_{\hyp \in \mathcal{H}} \E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right| \\
    \intertext{Because expectation of supremum is larger than supremum of expectation, we have:}
        \sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right| &\leq \E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \sup_{\hyp \in \mathcal{H}} \left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right|
    \end{align}
    Taking expectation over $\trainingData$ on both sides, we have
    \begin{align}
        \E_{\trainingData \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}} \left| L_{\sampleDist}(\hyp)-L_{\trainingData}(\hyp) \right|\right] &\leq \E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}} \left|L_{\trainingData'}(\hyp)-L_{\trainingData}(\hyp)\right|\right] \\
            &=\frac{1}{\numSamples} \E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left| \sum_{i=1}^\numSamples \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] \\
        \end{align}
        For each $j$, $(\sample_j',\labelElement_j')$ and $(\sample_j,\labelElement_j)$ are i.i.d. variables, which allows us to make the following statement:
        \begin{align}
            \underbrace{\frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_j'),\labelElement_j') - \loss(\hyp(\sample_j),\labelElement_j) +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]}_{A}\\
            = \underbrace{\frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_j),\labelElement_j) - \loss(\hyp(\sample_j'),\labelElement_j') +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]}_{B} \\
        \end{align}
        \begin{align}
        \intertext{Let $\rademacherRV_j$ be a Rademacher random variable (i.e. a draw from the uniform distribution over $\left\{+1,-1\right\}$).  Then we have:}
            \frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\rademacherRV_j(\loss(\hyp(\sample_j'),\labelElement_j') - \loss(\hyp(\sample_j),\labelElement_j)) +\sum_{i\neq j} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] &= \frac{1}{2}\left(A + B\right) \\
            &= \frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right]
        \end{align}
        \begin{align}
        \intertext{Let $\vec{\rademacherRV} = \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^{\transpose}$ be a vector consisting of $\numSamples$ i.i.d. samples from the Rademacher distribution.  Repeating this procedure for all $j$, we have}
            \frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\sum_{i=1}^{\numSamples} \loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] &=  \frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left|\sum_{i=1}^{\numSamples} \rademacherRV_i(\loss(\hyp(\sample_i'),\labelElement_i') - \loss(\hyp(\sample_i),\labelElement_i)\right|\right] \\
            &= \frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i'),\labelElement_i') \right) - \inf_{\hyp \in \mathcal{H}}\left(\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right)\right] \\
        \intertext{We know the distribution of $\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i)$ to be symmetric, hence}
            &=\frac{1}{\numSamples}\E_{\trainingData,\trainingData' \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i'),\labelElement_i') \right) + \sup_{\hyp \in \mathcal{H}}\left(\sum_{i=1}^{\numSamples}  \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right)\right] \\
            &=\frac{2}{\numSamples}\E_{\trainingData \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\sup_{f \in \mathcal{H}}  \left(\sum_{i=1}^{\numSamples} \rademacherRV_i\loss(\hyp(\sample_i),\labelElement_i) \right) \right] \\
            &=2\E_{\trainingData \drawnFrom \sampleDist^{\numSamples},\vec{\rademacherRV}}\left[\rademacherComplexity_{\trainingData}(\loss \circ \mathcal{H})\right]
\end{align}
\end{proof}

Upon replacing \cref{lem:representativeness} with \Cref{lem:improvedRepresentativeness}, \cref{thm:ShalevImproved} naturally follows from the proof of \cref{thm:shalevRademacher}.  Hence, we arrive at the following two-sided bound:

\begin{theorem}[Two-sided version of Theorem 26.5 from Shalev-Shwartz and Ben-David \cite{shalev2014understanding}]\label{thm:ShalevImproved}
    Let $\trainingData \drawnFrom \sampleDist^{\numSamples}$ be a sample of size $\numSamples$. Assume that for all $(\sample,\labelElement) \in \trainingData$ and $\hyp \in \hypothesisClass$, we have that $\left|\loss(\hyp(\sample),\labelElement)\right| \leq c$. Then
    with probability of at least $1-\errorConfidence$, for all $\hyp \in \hypothesisClass$:
    \begin{dgroup}
    \begin{dmath}
        \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\E_{\trainingData' \drawnFrom \sampleDist^{\numSamples}} \rademacherComplexity_{\trainingData'}(\loss \circ \hypothesisClass) + c\sqrt{\frac{2\ln\left(2/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
    \begin{dmath}\label{eq:rademacherEmpiricalTwoSided}
        \left|L_\sampleDist(\hyp) - L_{\trainingData}(\hyp)\right| \leq 2\rademacherComplexity_{\trainingData}(\loss \circ \hypothesisClass \circ \trainingData) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\numSamples}}
    \end{dmath}
\end{dgroup}
\end{theorem}


==> facct/src/A250_Important_Bounds.tex <==

\section{Bounds, Theorems, and Algebra for Section 3}\label{sec:boundsSec3}

\subsection{VC Dimension Definition}


\begin{definition}[VC dimension]\label{def:VCdimension} Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ shatters hypothesis class $\hypothesisClass$ if 
    \begin{dmath}
        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
    \end{dmath}

The VC dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$.
\end{definition}

\subsection{Sample Complexities for RBF Kernels}
\begin{theorem}[Simplified version of Theorem 2 from Cortes et al. \shortcite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\kernelFunction$ be a kernel function and that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ .  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis class $\hypothesisClass_{\kernelFunction}'$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_{\kernel}) \leq \sqrt{\frac{23e\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}


\begin{lemma}[RBF Kernel SVM Sample Complexity Bound]
   Let $\hypothesisClass_{\kernel}$ be an RBF kernel SVM predictor class. Let $\predictionValue \in \labelSpace$ be a prediction value.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\trainingData$ is a random sample of at least $\numSamples$ samples where
   
   \begin{equation*}
       \numSamples \geq \frac{23 {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
   \end{equation*} 
   examples drawn i.i.d. according to $\sampleDist$, then with probability at least $1-\errorConfidence$:
  \begin{equation}
      \forall \hyp \hiderel{\in} \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]\right| \hiderel{\leq} \errorTolerance
  \end{equation}
\end{lemma}




\begin{proof}
Fix $\hyp ,\group, \prediction$ and $\trainingData$. We take $\risk_{\trainingData}(\hyp)$ as $\empiricalCalibrationError(\hyp,\group,\prediction,\trainingData)$ and  $\risk_{\sampleDist}(\hyp)$ as $\calibrationError(\hyp,\group,\prediction)$  for convenience,

Invoking \cref{thm:ShalevImproved}, and solving for $\numSamples$:

 \begin{align}
      \abs{\risk_{\sampleDist}(\hyp) - \risk_{\trainingData}(\hyp)} &\hiderel{\leq} 2\rademacherComplexity_{\trainingData}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples}}
      \intertext{Because the absolute value of empirical calibration error is bounded by $1$, we set $c=1$, to yield}
         \abs{\risk_{\sampleDist}(\hyp) - \risk_{\trainingData}(\hyp)}  &\leq 23 \frac{\scalarBound^2}{\numSamples} + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples}
      \intertext{To guarantee this is smaller the right hand side of the inequality is less than $\epsilon$, we need}
         \numSamples &\geq\frac{23 {\scalarBound^2}+ 64\log\left(4/\errorConfidence\right)}{\errorTolerance^2}
   \end{align}
   
   Thus arriving at the sample complexity bound
\end{proof}

\subsection{Sample Complexities for ReLU Networks}





\begin{lemma}[Two layer ReLU Sample Complexity Bound]


Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$ Hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\weightMatrix = (\weightMatrix_1,\dotsc,\weightMatrix_\depth)$, where $\weightMatrix_{i} \in \realNumbers^{\dimension_{i}\times\dimension_{i-1}}$ where $\dimension = \dimension_0$. In the binary classification setting, we have $\dimension_{\depth} = 1$, and in the multi-class setting, we have $\dimension_{\depth} = \abs{\labelSpace}$.  Let $\nonlinearity(\cdot)$ be the ReLU function.  $\nonlinearity(\vec{\placeholder})$ applies the ReLU to each coordinate in $\vec{\placeholder}$. Such networks are of the form
\begin{equation*}
    \weightMatrix_{\depth}\nonlinearity\left(\weightMatrix_{\depth-1}\nonlinearity\left(\cdots\nonlinearity\left(\weightMatrix_{1}\sample\right)\cdots\right)\right)
\end{equation*}

The following is a Rademacher complexity bound on ReLU networks.  The bound is originally attributed to Bartlett et al.\cite{bartlett2017spectrally}, but we find the manner it is expressed in Theorem 5 from Yin et al. \cite{yin2019rademacher} to be more amenable to our results.
\begin{theorem}[Rademacher Complexity bound for ReLU Networks, \cite{bartlett2017spectrally,yin2019rademacher}]
Consider the neural network hypothesis class
\begin{equation}
    \hypothesisClass_{\neuralNetwork} = \left\{\hyp_{\weightMatrix}(\sample) : \weightMatrix : \left(\weightMatrix_1,\dotsc,\weightMatrix_\depth\right), \norm{\weightMatrix_i}_2 \leq \placeholder_i, \norm{\weightMatrix_i^{\transpose}}_{2,1} \leq \placeholder'_{i}, i \in \left\{1,\dotsc,\depth\right\}\right\}
\end{equation}
Then we have 
\begin{equation*}
    \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{\sfrac{3}{2}}} + \frac{26\log(\numSamples)\log(2\dimension_{\max})}{\numSamples}\norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}
\end{equation*}
where $\vec{X}$ are the unlabeled training data $\trainingData$, i.e. $\vec{X} = \left[\sample_1,\dotsc,\sample_N\right]$
\end{theorem}

   Let $\hypothesisClass_{\neuralNetwork}$ be a ReLU neural network predictor class defined above. Let $\predictionValue \in \labelSpace$ be a prediction value and assume 
   
   \begin{equation*}1 \leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \end{equation*}  
   
 Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\trainingData$ is a random sample of at least $\numSamples$ samples where
   
   \begin{equation*}
       \numSamples \geq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}
   \end{equation*} 
   examples drawn i.i.d. according to $\sampleDist$, then with probability at least $1-\errorConfidence$:
  \begin{equation}
      \forall \hyp \hiderel{\in} \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]\right| \hiderel{\leq} \errorTolerance
  \end{equation}
\end{lemma}

\begin{proof} Our proof strategy is to invoke a two-sided Rademacher complexity bound (\cref{thm:ShalevImproved}) to yield a sample complexity bound:
Fix $\hyp ,\group, \prediction$ and $\trainingData$. We take $\risk_{\trainingData}(\hyp)$ as $\empiricalCalibrationError(\hyp,\group,\prediction,\trainingData)$ and  $\risk_{\sampleDist}(\hyp)$ as $\calibrationError(\hyp,\group,\prediction)$ 
     \begin{align}
          \abs{\risk_{\sampleDist}(\hyp) - \risk_{\trainingData}(\hyp)} &\hiderel{\leq} 2\rademacherComplexity_{\trainingData}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples}}
      \intertext{Because the absolute value of empirical calibration error is bounded by $1$, we set $c=1$ and substitute the Rademacher complexity of ReLU networks, to yield}
           \abs{\risk_{\sampleDist}(\hyp) - \risk_{\trainingData}(\hyp)}  &\hiderel{\leq} \frac{8}{\numSamples^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples)\log(2\dimension_{\max})}{\numSamples}\norm{\vec{X}}_{\Frobenius}\hiderel{\cdot}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \hiderel{+} 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples}} \\
         &\leq \frac{8}{\numSamples^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples)\log(2\dimension_{\max})}{\numSamples^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples}} \\
      \intertext{Let us now assume that }
        1 &\leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}
    \intertext{Which gives us}
           \abs{\risk_{\sampleDist}(\hyp) - \risk_{\trainingData}(\hyp)} &\leq  \frac{60 \log(2\dimension_{\max})}{\numSamples^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples}} \\
      \intertext{To guarantee this is smaller the right hand side of the inequality is less than $\epsilon$, we need}\\
 \numSamples &\geq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}      
\end{align}
   Thus arriving at the sample complexity bound

\end{proof}
   
   


==> facct/src/A300_proof_thm_3.tex <==
\section{Proof of \Cref{thm:OurBoundSVM}}

Our proof of \cref{thm:OurBoundSVM} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize Rademacher complexity instead of VC dimension.


\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to subpopulation ${\group}$. Let $\hypothesisClass_{\kernel}$ denote the hypothesis class defined in \eqref{eq:kernelHypothesisClass}. Let $\Gamma_\gamma$ denote the set of all subpopulations $\group \in \Gamma$ which have probability at least $\gamma$:
   \begin{dmath}
      \Gamma_{\gamma} \definedAs \left\{{\group} \in \Gamma \given \Pr_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
   \end{dmath}

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
   \begin{dmath}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{dmath}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\interval)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
   \end{align}

   By \cref{lem:shabat24analogue}, we know  for any $\predictionValue \in \labelSpace$ and any ${\group} \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{dgroup}
   \begin{dmath}
      \numSamples_1 \geq \frac{64\log\left(\frac{4}{\errorConfidence'}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{(\epsilon')^2}
   \end{dmath}
   \begin{dmath}
      = \frac{64\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + \max\left\{1,\frac{1}{\lambda^2}\right\}23\scalarBound^2}{\left(\frac{\psi\errorTolerance}{3}\right)^2}
   \end{dmath}
   \begin{dmath}
      = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
   \end{dmath}
\end{dgroup}
   then we have

   
\begin{dmath}
   \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{dmath}
By \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any subpopulation ${\group} \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \left\{-1,1\right\}$, where

\begin{dmath} 
   \numSamples_2 \geq\frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2}
\end{dmath}

then we also have 

   \begin{dmath}
         \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{dmath}
   Set $\numSamples^\marker$ such that 
   \begin{dmath}
    \numSamples^\marker = \frac{576\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 207\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
   \end{dmath}
   Then, if for all subpopulations ${\group} \in \Gamma_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

   \begin{dgroup}
      \begin{dmath}\label{eq:calibrationClosenessA}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}\label{eq:calibrationClosenessB}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  = \frac{1152\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right) + 414\max\left\{1,\frac{1}{\lambda^2}\right\}\scalarBound^2}{\gamma\errorTolerance^2\psi^2} 
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \Gamma_\gamma$. Recall there are at most $\left|\Gamma \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \Gamma_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{dgroup}
      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{dgroup}
   \begin{dmath}
      p_1(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      p_2(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_1(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_2(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
   \end{dmath}
\end{dgroup}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$:

\begin{dmath}
   {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \Pr\left[\sample \in {\group}\right] \hiderel{\geq} \gamma,  \Pr\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi \implies
   \left|\calibrationError(\hyp,{\group},\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
\end{dmath}

which completes the proof.


\end{proof}




% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to subpopulation $U$.  Let $\Gamma_\gamma$ denote the set of all subpopulations $U \in \Gamma$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \Gamma_{\gamma} \definedAs \left\{U \in \Gamma \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \Gamma_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\Gamma\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \Gamma_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all subpopulations $U \in \Gamma_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\Gamma\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \Gamma_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \Gamma_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \Gamma, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\Gamma}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\Gamma}} = \frac{1}{2\abs{\hypothesisClass}\abs{\Gamma}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.


==> facct/src/A400_proof_NN.tex <==
\section{Proof of \Cref{thm:OurBoundSVM}}


Let us consider multicalibration uniform convergence bounds on depth $\depth$ ReLU networks.  Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$ Hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\weightMatrix = (\weightMatrix_1,\dotsc,\weightMatrix_\depth)$, where $\weightMatrix_{i} \in \realNumbers^{\dimension_{i}\times\dimension_{i-1}}$ where $\dimension = \dimension_0$. In the binary classification setting, we have $\dimension_{\depth} = 1$, and in the multi-class setting, we have $\dimension_{\depth} = \abs{\labelSpace}$.  Let $\nonlinearity(\cdot)$ be the ReLU function.  $\nonlinearity(\vec{\placeholder})$ applies the ReLU to each coordinate in $\vec{\placeholder}$. Such networks are of the form
\begin{equation*}
    \weightMatrix_{\depth}\nonlinearity\left(\weightMatrix_{\depth-1}\nonlinearity\left(\cdots\nonlinearity\left(\weightMatrix_{1}\sample\right)\cdots\right)\right)
\end{equation*}
\begin{theorem}[\cite{bartlett2017spectrally}]
Consider the neural network hypothesis class
\begin{equation}\label{eq:neuralNetworkHypothesisClass}
    \hypothesisClass_{\neuralNetwork} = \left\{\hyp_{\weightMatrix}(\sample) : \weightMatrix : \left(\weightMatrix_1,\dotsc,\weightMatrix_\depth\right), \norm{\weightMatrix_i}_2 \leq \placeholder_i, \norm{\weightMatrix_i^{\transpose}}_{2,1} \leq \placeholder'_{i}, i \in \left\{1,\dotsc,\depth\right\}\right\}
\end{equation}
Then we have 
\begin{equation*}
    \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{\sfrac{3}{2}}} + \frac{26\log(\numSamples)\log(2\dimension_{\max})}{\numSamples}\norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}
\end{equation*}
where $\vec{X}$ are the unlabeled training data $\trainingData$, i.e. $\vec{X} = \left[\sample_1,\dotsc,\sample_N\right]$
\end{theorem}
Our proof of \cref{thm:OurBoundSVM} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize Rademacher complexity instead of VC dimension.


% \left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}}

Let us begin by proving a lemma that will be helpful for proving a multicalibration uniform convergence bound.

\begin{lemma}[Analogue of Lemma 25 from \shortcite{shabat2020sample} ]\label{lem:shabat25analogue}
   Let $\hypothesisClass_{\neuralNetwork}$ be a ReLU neural network predictor class. Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \groups$ be a population group, and assume 
   
   \begin{equation*}1 \leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \end{equation*}  
   
   Furthermore, let   Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{\pm 1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_{\group}$ is $\sampleDist$ conditioned on examples being members of group $\group$ and $\trainingData_{\group} = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of 
   
   \begin{equation*}
       \left|\trainingData_\group\right| \geq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}
   \end{equation*} 
   examples drawn i.i.d. according to $\sampleDist_\group$, then with probability at least $1-\errorConfidence$:
  \begin{dmath}
      \forall \hyp \hiderel{\in} \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}\predictionValue\right]\right| \hiderel{\leq} \errorTolerance
  \end{dmath}
\end{lemma}

\begin{proof} Our proof strategy is to invoke a two-sided Rademacher complexity bound (\cref{thm:shalevRademacherImproved}) to yield a bound on $\errorTolerance$:
     \begin{dgroup}
      \begin{dmath}
         \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
      \end{dmath}
      \intertext{By \cref{lem:kernelHypothesisContraction} and because $\empiricalCalibrationError$ is $1$-Lipschitz with respect to $\frac{1}{\numSamples}\sum_{\sample \in \trainingData}\hyp(\sample)$, we are able upper bound the Rademacher complexity term.  Furthermore, because the empirical calibration loss is bounded by $1$, we set $c=1$}




      % \intertext{Our Rademacher complexity bound is on $\hypothesisClass_{\kernel}'$ but we need a bound on \RademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\kernel})}
      

      \begin{dmath}
         \errorTolerance  \hiderel{\leq} \frac{8}{\numSamples_\group^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples_{\group})\log(2\dimension_{\max})}{\numSamples_{\group}}\norm{\vec{X}}_{\Frobenius}\hiderel{\cdot}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \hiderel{+} 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}
            \begin{dmath}
         \leq \frac{8}{\numSamples_\group^{\sfrac{3}{2}}} + \frac{52 \log(\numSamples_{\group})\log(2\dimension_{\max})}{\numSamples_{\group}^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}
      
      \intertext{Let us now assume that }
         \begin{dmath*}1 \leq\log\left(2\dimension_{\max}\right)\vec{X}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} \end{dmath*}  
    \intertext{Which gives us}
       \begin{dmath}
         \errorTolerance \leq  \frac{60 \log(2\dimension_{\max})}{\numSamples_{\group}^{\sfrac{1}{2}}} \norm{\vec{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\placeholder_i\right)\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{\sfrac{3}{2}} + 4\sqrt{\frac{2\log\left(\sfrac{4}{\errorTolerance}\right)}{\numSamples_{\group}}}
      \end{dmath}


      \intertext{Which gives us, after algebraic manipulation}

      \begin{dmath}
 \numSamples_{\group} \leq \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence}\right)}{\errorTolerance^2}      
 \end{dmath}

   \end{dgroup}
   
\end{proof}


\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to group ${\group}$. Let $\hypothesisClass_{\neuralNetwork}$ denote the hypothesis class defined in \eqref{eq:neuralNetworkHypothesisClass}.  Recall that $\gamma$ is the lowest frequency amongst groups $\group \in \groups$ present in the training data $\trainingData$:
   

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups$:
   \begin{dmath}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{dmath}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\interval)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
   \end{align}

   By \cref{lem:shabat24analogue}, we know  for any $\predictionValue \in \labelSpace$ and any ${\group} \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{dgroup}
   \begin{dmath}
      \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\sfrac{4}{\errorConfidence'}\right)}{(\errorTolerance')^2} 
   \end{dmath}
   \begin{dmath}
      =       \frac{7200\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 64\log\left(\frac{4}{\frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}}\right)}{(\frac{\psi\errorTolerance}{3})^2} 
   \end{dmath}
   \begin{dmath}
      =       \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2} 
   \end{dmath}
\end{dgroup}
   then we have

   
\begin{dmath}
   \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{dmath}
By \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any group ${\group} \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \labelSpace$, where

\begin{dmath} 
     \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2} 
\end{dmath}

then we also have 

   \begin{dmath}
         \forall \hyp \in \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{dmath}
   Set $\numSamples^\marker$ such that 
   \begin{dmath}
    \numSamples^\marker = \frac{64800\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 576\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\psi^2\errorTolerance^2}  \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
   \end{dmath}
   Then, if for all groups ${\group} \in \groups_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

   \begin{dgroup}
      \begin{dmath}\label{eq:calibrationClosenessA}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}\label{eq:calibrationClosenessB}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs   \frac{129600\log^2\left(2\dimension_{\max}\right)\norm{\vec{X}}_{\Frobenius}^2\left(\prod_{i=1}^{\depth}\placeholder_i\right)^2\left(\sum_{j=1}^{\depth}\left(\frac{\placeholder_j'}{\placeholder_j}\right)^{\sfrac{2}{3}}\right)^{3} + 1152\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\gamma\psi^2\errorTolerance^2} 
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \groups_\gamma$. Recall there are at most $\left|\groups \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \groups_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{dgroup}
      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}

      \begin{dmath}
         {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{dmath}
   \end{dgroup}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{dgroup}
   \begin{dmath}
      p_1(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      p_2(\hyp,{\group},\predictionValue) \definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_1(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
   \end{dmath}
   \begin{dmath}
      \tilde{p}_2(\hyp,{\group},\predictionValue) \definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
   \end{dmath}
\end{dgroup}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$:

\begin{dmath}
   {\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\  \Pr\left[\sample \in {\group}\right] \hiderel{\geq} \gamma,  \Pr\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi \implies
   \left|\calibrationError(\hyp,{\group},\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
\end{dmath}

which completes the proof.


\end{proof}

% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to group $U$.  Let $\groups_\gamma$ denote the set of all groups $U \in \groups$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \groups_{\gamma} \definedAs \left\{U \in \groups \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all groups $U \in \groups_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \groups_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\groups}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\groups}} = \frac{1}{2\abs{\hypothesisClass}\abs{\groups}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.


==> facct/src/A500_proof_general.tex <==
\section{Proof of Main Theorem}\label{sec:ProveMainTheorem}


Our proof of \cref{thm:maintheorem} follows the proof technique of theorem 15 from Shabat et al \cite{shabat2020sample}.  The principal difference is that we utilize general sample complexities for ERM learning instead of devising an VC dimension specific bound. Let us begin by assuming a group-wise sample complexity exists for each group, that is:

A function $\sampleComplexity_{\group,\hypothesisClass} : (0,1)^2 \to \naturalNumbers$ such that for every $\errorTolerance,\errorConfidence \in (0,1)$ and every probability distribution in group $\group$, $\sampleDist_{\group}$, if $\numSamples_\group \geq \sampleComplexity_{\group,\hypothesisClass}(\errorTolerance,\errorConfidence)$, we have

\begin{equation}
\Pr\left[\abs{\risk_{\trainingData_{\group}}(\hyp) - \risk_{\sampleDist_{\group}}(\hyp)} \leq \errorTolerance \right] \geq 1-\errorConfidence
\end{equation}

Indeed, this formulation allows use any sort of concentration bound, including those based upon Rademacher complexity and VC dimension.  Once we have a general concentration bound on calibration error for a demographic group, we leverage the frequency of each group to yield an overall bound for multicalibration uniform convergence .

To make our proof, we will also need the following lemmas:

\begin{lemma}[Lemma 26 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat26}
   Let $p_1,p_2,\tilde{p}_1,\tilde{p}_2,\epsilon,\psi \in [0,1]$ such that $p_1,\psi \leq p_2$ and $\left|p_1-\tilde{p}_1\right|,\left|p_2-\tilde{p}_2\right| \leq \psi\epsilon/3$.  Then,

   \begin{equation}
      \left|\frac{p_1}{p_2} - \frac{\tilde{p}_1}{\tilde{p}_2}\right| \leq \epsilon
   \end{equation}

\end{lemma}


\begin{lemma}[Lemma 27 from Shabat et al. \cite{shabat2020sample}]\label{lem:shabat27}
  Let $\gamma \in (0,1)$ and let $\Gamma_\gamma = \left\{\group \in \Gamma \given \Pr_{\sample \drawnFrom \sampleDist}\left[\sample \in \group\right] \geq \gamma\right\}$ be the collection of subpopulations from $\Gamma$ that has probability at least $\gamma$ according to $\sampleDist$.  Let $\errorConfidence \in (0,1)$ and let $\trainingData$ be a random sample of $\numSamples$ drawn i.i.d. from $\sampleDist$.  Then with probability at least $1-\errorConfidence$, if $\numSamples \geq \frac{8\log\left(\frac{\left|\Gamma\right|}{\errorConfidence}\right)}{\gamma}$,

  \begin{equation}
      \forall \group \in \groups \hiderel{:} \left|\trainingData \intersection \group\right| \hiderel{>} \frac{\gamma \numSamples}{2}
  \end{equation}

\end{lemma}

The proof of \cref{thm:maintheorem} follows:



\begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_{\group} \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in {\group} \right\}$ be the samples in $\trainingData$ belonging to group ${\group}$. Let $\hypothesisClass$ denote a fixed hypothesis class and assume $\sampleComplexity_{\group,\hypothesisClass}(\errorTolerance,\errorConfidence)$ exists.  Recall that $\gamma$ is the lowest frequency amongst groups $\group \in \groups$ present in the training data $\trainingData$:
   

   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  This assumption allows us to invoke \cref{lem:shabat27}, which tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups$:
   \begin{equation}\label{eq:minSampleSize}
      \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
   \end{equation}

   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ yields an accurate estimate of the calibration error for an interesting category $(\group,\prediction)$.  For this purpose, we define
   \begin{align}
      \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
   \end{align}

   Given the existence of $\sampleComplexity_{\group,\hypothesisClass}(\errorTolerance,\errorConfidence)$, we know for any $\predictionValue \in \labelSpace$ and any ${\group} \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_1$ examples from ${\group}$ where   
   \begin{align}
      \numSamples_1 &\hiderel{=} \sampleComplexity_{\group,\hypothesisClass}\left(\errorTolerance',\errorConfidence'\right) \\
      &=  \sampleComplexity_{\group,\hypothesisClass}\left(\frac{\psi\errorTolerance}{3}, \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}\right)
\end{align}
   then we have

   
\begin{equation}
   \forall \hyp \hiderel{\in} \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
\end{equation}
 Given the existence of $\sampleComplexity_{\group,\hypothesisClass}(\errorTolerance,\errorConfidence)$ we also know that for any $\predictionValue \in \labelSpace$ and any group ${\group} \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, for a random sample of $\numSamples_2$ labeled examples from ${\group} \times \labelSpace$, where

\begin{align}
      \numSamples_2 &\hiderel{=} \sampleComplexity_{\group,\hypothesisClass}\left(\frac{\psi\errorTolerance}{3}, \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}\right)
\end{align}

then we also have 

   \begin{equation}
         \forall \hyp \hiderel{\in} \hypothesisClass_{\kernel} \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  \hiderel{-}\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
   \end{equation}
   Set $\numSamples^\marker$ such that upper-bounds $\max\left\{\numSamples_1, \numSamples_2\right\}$
   \begin{equation}
    \numSamples^\marker =  2\sampleComplexity_{\group,\hypothesisClass}\left(\frac{\psi\errorTolerance}{3}, \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}\right)
   \end{equation}
   Then, if for all groups ${\group} \in \groups_\gamma$, $\left|\trainingData_{\group}\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$:
   
   \begin{align} 
        \begin{split} \label{eq:calibrationClosenessA}
       &\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace : \\
       &\left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
       \end{split}\\
       \shortintertext{and we also have}
       \begin{split} \label{eq:calibrationClosenessB}
            &\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :\\
            & \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
       \end{split}
   \end{align}
   
   Let us now choose the following overall sample size :
   \begin{dmath}
      \numSamples \definedAs   2\sampleComplexity_{\group,\hypothesisClass}\left(\frac{\psi\errorTolerance}{3}, \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}\right)
   \end{dmath}
Recall our use of \cref{lem:shabat27} at the beginning of this proof.  Given a sample of size at least $\numSamples$, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every ${\group} \in \groups_\gamma$. Recall there are at most $\left|\groups \right|$ such population subgroups, and with probability at least $1-\errorConfidence/2$, for every $\group \in \groups_{\gamma}$:
\begin{dmath}
   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} \hiderel{=}\numSamples^{\marker}
\end{dmath}
   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
   \begin{align}
      \begin{split}
         &{\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ &\left|\frac{1}{\numSamples_{\group}}\sum_{\sample' \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{split} \\
      \shortintertext{and we also have}
      \begin{split}
         &{\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   &\left|\frac{1}{\numSamples_\group}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\Pr_{\sample \drawnFrom \sampleDist_{\group}}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
      \end{split}
   \end{align}
To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
\begin{align}
      p_1(\hyp,{\group},\predictionValue) &\definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} {\group}\right] \\
      p_2(\hyp,{\group},\predictionValue) &\definedAs \Pr\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} {\group}\right] \\
      \tilde{p}_1(\hyp,{\group},\predictionValue) &\definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right] \\
      \tilde{p}_2(\hyp,{\group},\predictionValue) &\definedAs \frac{1}{\left|\trainingData_{\group}\right|}\sum_{\sample'\hiderel{\in} \trainingData_{\group}} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
\end{align}

Then, upon invoking \cref{lem:shabat26}, we have for all $\hyp \in \hypothesisClass_{\kernel}, {\group} \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

\begin{equation}
   \left|\frac{p_1(\hyp,{\group},\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,{\group},\predictionValue)}{\tilde{p}_2(\hyp,{\group},\predictionValue)}\right| \leq \epsilon
\end{equation}

Thus, with probability at least $1-\errorConfidence$, we have


\begin{align}
   &{\forall \hyp \hiderel{\in} \hypothesisClass_{\kernel}, \forall {\group}\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\ & \Pr\left[\sample \in {\group}\right] \hiderel{\geq} \gamma \text{ and }  \Pr\left[\hyp(\sample)=\predictionValue \given \sample \in {\group} \right] \hiderel{\geq} \psi
\end{align}

which implies 
   $\left|\calibrationError(\hyp,{\group},\predictionValue) \hiderel{-} \hat{\calibrationError}(\hyp,{\group},\predictionValue,\trainingData) \right| \hiderel{\leq} \errorTolerance$
which completes the proof.


\end{proof}





% \section{Proof of NN theorem}



% \begin{proof} Let $\trainingData \definedAs \left\{(\sample_i,\labelElement_i)\right\}_{i=1}^{\numSamples}$ be a sample of $\numSamples$ labeled examples drawn i.i.d. from $\sampleDist$, and let $\trainingData_U \definedAs \left\{(\sample,\labelElement) \in \trainingData : \sample \in U \right\}$ be the samples in $\trainingData$ belonging to group $U$.  Let $\groups_\gamma$ denote the set of all groups $U \in \groups$ which have probability at least $\gamma$:
%   \begin{dmath}
%       \groups_{\gamma} \definedAs \left\{U \in \groups \given \PR_{\sample \drawnFrom \sampleDist} \geq \gamma\right\}
%   \end{dmath}

%   Let us assume $\numSamples \geq \frac{8\log\left(\frac{2\left|\groups\right|}{\errorConfidence}\right)}{\gamma}$.  By making this assumption, \cref{lem:shabat27}, tells that with probability $1-\frac{\errorConfidence}{2}$, for every $\group \in \groups_\gamma$:
%   \begin{dmath}\label{eq:minSampleSize}
%       \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2}
%   \end{dmath}

%   Next, we show that, with high probability, having a large number of examples in $\trainingData_\group$ suggests an accurate estimate of the calibration error for an interesting category $(U,I)$.  For this purpose, we define
%   \begin{align}
%       \errorTolerance' &\definedAs \frac{\psi\errorTolerance}{3} & \errorConfidence' &\definedAs \frac{\errorConfidence}{4\left|\groups\right|\left|\labelSpace\right|}
%   \end{align}

%   Using {\color{red} insert lemma} we know  for any $\predictionValue \in \labelSpace$ and any $U \in \groups_{\gamma}$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_1$ examples from $U$ where   
%   \begin{dgroup}
%   \begin{dmath}
%       \numSamples_1 \geq  \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{(\errorTolerance')^2} + \frac{64{\log\left(4/(\errorConfidence')\right)}}{(\errorTolerance')^2}
%   \end{dmath}
%   \begin{dmath}
%       = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% \end{dgroup}
%   then we have

   
% \begin{dmath}
%   \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
% \end{dmath}
% Using \cref{lem:shabat25analogue} ,we know that for any $\predictionValue \in \labelSpace$ and any $U \in \groups_\gamma$, with probability at least $1-\errorConfidence'$, a random sample of $\numSamples_2$ labeled examples from $U \times \left\{0,1\right\}$, where

% \begin{dmath} 
%   \numSamples_2 \geq\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
% \end{dmath}


%   \begin{dmath}
%          \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%   \end{dmath}
%   Set $\numSamples^\marker$ such that 
%   \begin{dmath}
%     \numSamples^\marker = \frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2} \hiderel{\geq} \max\left\{\numSamples_1, \numSamples_2\right\}
%   \end{dmath}
%   Then, if for all groups $U \in \groups_\gamma$, $\left|\trainingData_U\right| \geq \numSamples^\marker$, we have with probability at least $1-2\left|\groups\right|\left|\labelSpace\right|\errorConfidence' = 1 - \frac{\errorConfidence}{2}$

%   \begin{dgroup}
%       \begin{dmath}\label{eq:calibrationClosenessA}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}\label{eq:calibrationClosenessB}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_\group}\sum_{(\sample,\labelElement) \in \trainingData_{\group}}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
%   Choosing sample size 
%   \begin{dmath}
%       \numSamples \definedAs \frac{2\numSamples^\marker}{\gamma}  =\frac{48672\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2\psi^2} + \frac{576{\log\left(\frac{16\left|\groups\right|\left|\labelSpace\right|}{\errorConfidence}\right)}}{\errorTolerance^2\psi^2}
%   \end{dmath}
% Given this sample size, we know with probability at least $1-\frac{\errorConfidence}{2}$, for every $U \in \groups_\gamma$:
% \begin{dmath}
%   \left|\trainingData_{\group}\right| \geq \frac{\gamma \numSamples}{2} =\numSamples^{\marker}
% \end{dmath}
%   By making the assumptions in \eqref{eq:minSampleSize}, \eqref{eq:calibrationClosenessA},  \eqref{eq:calibrationClosenessB}, and invoking the union bound again, we have, with probability at least $1-\errorConfidence$
%   \begin{dgroup}
%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace :}\\ \left|\frac{1}{\numSamples_U}\sum_{\sample' \in \trainingData_U}\indicatorFunction\left[\hyp(\sample') \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}

%       \begin{dmath}
%          {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:}\\   \left|\frac{1}{\numSamples_1'}\sum_{i=1}^{\numSamples}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \frac{\psi\errorTolerance}{3}
%       \end{dmath}
%   \end{dgroup}
% To conclude the proof, we will invoke \cref{lem:shabat26}.  For notational convenience, we denote the following:
% \begin{dgroup}
%   \begin{dmath}
%       p_1(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       p_2(\hyp,U,\predictionValue) \definedAs \PR\left[\hyp(\sample)\hiderel{=}\predictionValue, \given \sample \hiderel{\in} U\right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_1(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{(\sample',\labelElement')\hiderel{\in} \trainingData_U}\indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue, \labelElement\hiderel{=}1 \right]
%   \end{dmath}
%   \begin{dmath}
%       \tilde{p}_2(\hyp,U,\predictionValue) \definedAs \frac{1}{\left|\trainingData_U\right|}\sum_{\sample'\hiderel{\in} \trainingData_U} \indicatorFunction\left[\hyp(\sample)\hiderel{=}\predictionValue\right]
%   \end{dmath}
% \end{dgroup}

% Then, upon invoking the lemma, we have for all $\hyp \in \hypothesisClass, U \in \groups_{\gamma}$ and $\predictionValue \in \labelSpace$, if $p_2(\hyp,\group,\predictionValue) \geq \psi$:

% \begin{equation}
%   \left|\frac{p_1(\hyp,U,\predictionValue)}{p_2(\hyp,\group,\predictionValue)} - \frac{\tilde{p}_1(\hyp,U,\predictionValue)}{\tilde{p}_2(\hyp,U,\predictionValue)}\right| \leq \epsilon
% \end{equation}

% Thus, with probability at least $1-\errorConfidence$:

% \begin{dmath}
%   {\forall \hyp \hiderel{\in} \hypothesisClass, \forall U\hiderel{\in} \groups, \forall \predictionValue \in \labelSpace:} \\  \PR\left[\sample \in U\right] \hiderel{\geq} \gamma,  \PR\left[\hyp(\sample)=\predictionValue \given \sample \in U \right] \hiderel{\geq} \psi \implies
%   \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance
% \end{dmath}

% \end{proof}

% \begin{proof}


% Let $\trainingData$ be a sample of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist$. We begin by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ will not be too large:

% \begin{dgroup}
%   \begin{dmath}
%   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
% \begin{dmath}
% =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
% \end{dmath}
% \begin{dmath}
%   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
% \end{dmath}
% \end{dgroup}

% \end{proof}




% Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance =  \frac{\errorTolerance}{\abs{I}\abs{\hypothesisClass}\abs{\groups}} = \frac{\errorTolerance}{2\abs{\hypothesisClass}\abs{\groups}} = \frac{1}{2\abs{\hypothesisClass}\abs{\groups}}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$ and taking a union bound completes the proof.

==> facct/src/B1_Inequalities_and_facts.tex <==
% !TeX root = ../note.tex

\section{Important Inequalities and Facts}

We begin by stating facts and inequalities necessary for our proofs:

\begin{lemma}[From \url{https://math.stackexchange.com/questions/171241/approximations-for-the-partial-sums-of-exponential-series}]\label{lem:expPartialSum}

    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}

\end{lemma}

\begin{lemma}[Frech\'et Inequality]\label{lem:frechet}
    Let $\event_1,\dotsc,\event_{\placeholderCount}$ be probabilistic events.  The following is true:
    
    \begin{equation}
        \Pr{\bigIntersection_{i=1}^{\placeholderCount} \event_i} \leq \min_{i} \Pr{\event_i}
    \end{equation}
    
    \end{lemma}



    \begin{theorem}[Hoeffding's Inequality \cite{hoeffding1963probability}]\label{\hoeffding}. Let $\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_{\placeholderCount}$ independent random variables strictly bounded by the intervals $\bracket{a_i,b_i}$, then

        \begin{equation}
            \Pr{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i - \sum_{i=1}^{\placeholderCount}\E{\placeholderRandomVariable_i}} \geq \placeholder} \leq \exp\paren*{-\frac{2\placeholderCount^2\placeholder^2}{\sum_{i=1}^{\placeholderCount}\paren*{b_i-a_i}^2}}
        \end{equation}
        
        \end{theorem}

        \begin{definition}
            The $\ell_1$ distance between any two distributions $\placeholderDist_1,\placeholderDist_2$ is defined as 
            \begin{equation}
                \norm{\placeholderDist_1-\placeholderDist_2}_1 \definedAs \sum_{\placeholder \in \support\paren*{\placeholderDist_1} \union \support\paren*{\placeholderDist_2}} \abs{\placeholderDist_1(\placeholder)-\placeholderDist_2(\placeholder)}
            \end{equation}
            \end{definition}

            \begin{lemma}[Lemma from Thomas and Cover \cite{coverthomas1991elements}]\label{lem:pinsker}
                \begin{equation}
                \infdiv{\placeholderDist_1}{\placeholderDist_2} \geq \frac{1}{2 \ln 2}\norm{\placeholderDist_1-\placeholderDist_2}_1^2
                \end{equation}
                \end{lemma}

                \begin{theorem}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{thm:chernoffNice}
                    Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
                    \begin{align}
                        \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
                             \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
                    \end{align}
                    \end{theorem}
                    
                    \begin{corollary}[Multiplicative Chernoff Bound for Bernoulli Random Variables]\label{cor:chernoffNice}
                        Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\errorConfidence > 0$ then
                        \begin{align}
                            \Pr{\paren*{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}} && 0 \leq \frac{\errorTolerance}{\E{\randomVariable}}\leq 1
                        \end{align} 
                        \end{corollary}
                    
                        \begin{proof}
                            \begin{align}
                            \Pr{{\frac{1}{\placeholderCount}\abs*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} &\leq \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \errorTolerance} + \Pr{{\frac{1}{\placeholderCount}\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\errorTolerance} \\
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \placeholderCount\errorTolerance} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\placeholderCount\errorTolerance}
                            \intertext{Putting $\errorTolerance$ in terms of the parameters in \cref{thm:chernoffNice}, we see that $\errorTolerance = \relativeErrorTolerance \E{\randomVariable}$}
                            &= \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \geq \frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} + \Pr{{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i - \E{\randomVariable}}} \leq -\frac{\errorTolerance}{\E{\randomVariable}} \cdot \E{\randomVariable}\cdot \placeholderCount} \\
                            &\leq 2\exp\paren*{-\frac{\errorTolerance^2\placeholderCount}{3\E{\randomVariable}}}
                            \end{align}
                        \end{proof}


\begin{lemma}\label{lem:multinomialDistributionBound}
    Let $\vec{\placeholder} \in \realNumbers^{\dimension}$ be a vector of probabilities.  That is, for $i \in \set{1,\dotsc,\dimension}$, we have $0 \leq \placeholder_i \leq 1$ and $1=\sum_{i=1}^{\dimension}\placeholder_{i}$.  Furthermore, the entries of $\vec{\placeholder}$ are ordered such that $\placeholder_1 \geq \placeholder_2 \geq \dotsc \geq \placeholder_{\dimension}$.  Then for all $i \in \set{1,\dotsc,\dimension}$, we have
    
    \begin{equation}
        \placeholder_i \leq \frac{1}{i}
    \end{equation}
    \end{lemma}
    \begin{proof}
        todo
    \end{proof}
    
                    

==> facct/src/essential/macros.tex <==
\usepackage{bm}
\usepackage{mathtools}
\usepackage{xfrac}
\usepackage{bbm}
\usepackage{cleveref}
\usepackage{tikz}
\usepackage{breqn}

\renewcommand{\vec}{\bm}
\newcommand{\randomVariable}{X}
\newcommand{\randomVariableInstance}{x}
\newcommand{\bernoulliParameter}{p}
\newcommand{\placeholderCount}{m}
\newcommand{\errorTolerance}{\epsilon}
\newcommand{\relativeErrorTolerance}{\eta}
\newcommand{\errorConfidence}{\delta}
\newcommand{\martingaleDifference}{c}
\newcommand{\BernoulliDistribution}{\mathrm{Bernoulli}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2
}
\newcommand{\infdiv}{D\infdivx}
\newcommand{\scratchVariable}{q}
\newcommand{\event}{A}
\newcommand{\decisionFunction}{\sigma}
\newcommand{\hoeffding}{thm:hoeffding}
\newcommand{\placeholderSample}{Q}
\newcommand{\sampleElement}{x}
\newcommand{\labelElement}{y}
\newcommand{\prediction}{\hat{y}}
\newcommand{\weightsElement}{w}
\newcommand{\weight}{\weightsElement}

\newcommand*\rect[1]{
    \tikz[baseline=(char.base)]{
        \node[inner sep=8pt, minimum size=1cm] (char) {#1};
        \draw (char.north west) -- (char.south west) -| (char.north east);
        }
}
\newcommand{\poissonRate}{\lambda}
\newcommand{\PoissonDistribution}{\mathrm{Poisson}}
\newcommand{\bigOh}{O}
\newcommand{\bigOmega}{\Omega}

\newcommand{\unifalg}{\mathrm{unif-alg}}

\newcommand{\loss}{\ell}
\newcommand{\regularizedGammaFunction}{Q}
\newcommand{\GammaFunction}{\Gamma}
\newcommand{\lossContribution}{L}

\newcommand{\labelFunction}{\hat{\sigma}}
\newcommand{\indicatorFunctionInstance}{\zeta}
\newcommand{\period}{T}

\newcommand{\sampleSpace}{\mathcal{X}}
\newcommand{\labelSpace}{\mathcal{Y}}
\newcommand{\sampleDist}{\mathcal{D}}
\newcommand{\drawnFrom}{\sim}
\newcommand{\fairnessMetric}{\mathcal{F}}
\newcommand{\multicalibration}{\mathrm{mc}}

\newcommand{\calibrationError}{\mathrm{c}}
\newcommand{\empiricalCalibrationError}{\hat{\mathrm{c}}}
\newcommand{\Frobenius}{\mathrm{F}}

\newcommand{\moduleClassifier}{h}
\newcommand{\hypothesisModule}{\moduleClassifier}
\newcommand{\classifierPlaceholder}{\psi}
\newcommand{\scalarBound}{B}
\newcommand{\spectralBound}{s}
\newcommand{\normBound}{b}

\newcommand{\opt}{*}
\newcommand{\svm}{\mathrm{SVM}}

\newcommand{\moduleScalar}{\alpha}
\newcommand{\blockScalar}{\moduleScalar}
\newcommand{\convexHullOperator}{\mathrm{conv}}
\newcommand{\composeOperator}{\circ}
\newcommand{\greekScalar}{\lambda}
\newcommand{\placeholderScalar}{\alpha}
\newcommand{\metricEntropy}{\Phi}

\newcommand{\zeroVector}{\vec{0}}
\newcommand{\sampleComplexity}{m}
\newcommand{\metric}{\rho}
\newcommand{\setVar}{Y}
\newcommand{\setVarElement}{y}
\newcommand{\protectedTrainingData}{\trainingData_{\mathrm{pro}}}
\newcommand{\rademacherRV}{\sigma}
\newcommand{\variance}{\mathrm{Var}}
\newcommand{\openBall}{B}

\newcommand{\learningAlgorithm}{\mathcal{A}}
\newcommand{\boost}{\textrm{boost}}

\newcommand{\probabilityDensityFunction}{f}
\newcommand{\differential}{\mathrm{d}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\probabilityVar}{q}
\newcommand{\badGroups}{\mathtt{badGroups}}
\newcommand{\goodGroups}{\mathtt{goodGroups}}

\newcommand{\powerSet}{{P}}

\newcommand{\E}{\mathop{\mathbb{E}}}
% \newcommand{\E}[2][]{\ifthenelse{\equal{#1}{}}{{\mathbb{E}}\left[#2 \right]}{\underset{#1}{ {\mathbb{E}}}\left[#2 \right]}}
% \renewcommand{\Pr}[2][]{\ifthenelse{\equal{#1}{}}{\mathbb{P}\left[#2 \right]}{\underset{#1}{\mathbb{P}}\left[#2 \right]}}
% \newcommand{\PrEmpirical}[2][]{\ifthenelse{\equal{#1}{}}{\hat{\mathbb{P}}\left[#2 \right]}{\underset{#1}{\hat{\mathbb{P}}}\left[#2 \right]}}
\renewcommand{\Pr}{\mathop{\mathbb{P}}}
\newcommand{\thmOne}{thm:one}
\newcommand{\thmTwo}{thm:Two}
\newcommand{\corThmTwo}{cor:two}
\newcommand{\intersection}{\cap}

\newcommand{\functionPlaceholder}{\beta}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\numInterestingCategories}{C}
\newcommand{\interestingCategory}{c}
\newcommand{\listInterestingCategories}{\mathcal{C}}

\newcommand{\weightMatrix}{\vec{W}}

\newcommand{\given}{\mid}

\newcommand{\metricEntropyRadius}{\epsilon}
\newcommand{\q}{q}
\newcommand{\qDual}{r}
\newcommand{\functionComposition}{F}
\newcommand{\function}{G}
\newcommand{\sampleInfNormUB}{r_{\infty}}
\newcommand{\weightsOneNormUB}{\Lambda}
\newcommand{\finalLinearClassifierOneNormUB}{C_{0}}
\newcommand{\rademacherComplexity}{\mathcal{R}}

\newcommand{\blockOutput}{o}
\newcommand{\blockIter}{t}
\newcommand{\blockFunction}{f}
\newcommand{\moduleIter}{\blockIter}
\newcommand{\placeholderInt}{n}
\newcommand{\depth}{T}
\newcommand{\depthIter}{t}
\newcommand{\indicatorFunction}{\mathbbm{1}}
\newcommand{\entropy}{H}
\newcommand{\kernel}{\kernelFunction}
\newcommand{\threshold}{\tau}
\newcommand{\blockError}{\gamma}
\newcommand{\learningCondition}{\eta}
\crefname{fact}{fact}{facts}

\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\curlyBrace}{\{}{\}}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\innerProduct}{\langle}{\rangle}

\newcommand{\BoostResNet}{\mathrm{BoostResNet}}
\newcommand{\groupDist}{\vec{\pi}}
\newcommand{\minNumSamples}[1]{N_{\min,#1}}
\newcommand{\sample}{\vec{\sampleElement}}

\newcommand{\sampleProtected}{\sampleElement_{\protectedIndex}}
\newcommand{\sampleUnprotected}{\sample_{\unprotectedIndices}}
\newcommand{\hypothesisModuleSum}[2]{s_{#1:#2}}

\newcommand{\bigTheta}{\Theta}
\newcommand{\costMatrix}{\vec{C}}
\newcommand{\fairnessCostMatrix}{\vec{F}}

\newcommand{\weights}{\vec{\weightsElement}}
\newcommand{\sumHypothesisModules}{H}

\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\naturalNumbers}{\mathbb{N}}

\newcommand{\integers}{\mathbb{Z}}
\newcommand{\positiveIntegers}{\mathbb{Z}^+}

\newcommand{\dimension}{d}
\newcommand{\trainingData}{S}
\newcommand{\dataset}{S}

\newcommand{\train}{\mathrm{train}}
\newcommand{\test}{\mathrm{test}}

\newcommand{\evalutationData}{\evaluationData}
\newcommand{\evaluationData}{T}
\newcommand{\margin}{\theta}
\newcommand{\placeholderConstant}{\alpha}
\newcommand{\Representativeness}{\mathrm{Rep}}

\newcommand{\unlabeledTrainingData}{Q}
\newcommand{\marker}{\dagger}
\newcommand{\bigIntersection}{\bigcap}
\newcommand{\bigUnion}{\bigcup}
%\newcommand{\risk}{R}
\newcommand{\numSamples}{N}
\newcommand{\numSamplesComplement}{N^c}
\newcommand{\placeholderSet}{\mathcal{Z}}
\newcommand{\placeholderDist}{\mathcal{Q}}
\newcommand{\placeholderRandomVariable}{X}
\newcommand{\placeholderRandomVariableInstance}{x}
\newcommand{\boostDist}{D}
\newcommand{\placeholder}{z}
\newcommand{\protectedIndex}{1}
\newcommand{\unprotectedIndices}{2:\dimension}
\newcommand{\dimensionUnprotected}{\dimension-1}
\newcommand{\risk}{L}
\newcommand{\hyp}{\mathrm{h}}
\newcommand{\hypMultiClass}{H}
\newcommand{\hypothesisClass}{\mathcal{H}}
\newcommand{\definedAs}{\triangleq}
\newcommand{\placeholderFunction}{f}
\newcommand{\rademacherSamplesComponentFunction}{\mathrm{N}}
\newcommand{\rademacherOtherComponentFunction}{\mathrm{q}}
\newcommand{\rademacherOtherComponent}{\mathrm{q}(\hat{\calibrationError}\circ \hypothesisClass \circ \trainingData)}
\newcommand{\rademacherSamplesComponent}{\rademacherSamplesComponentFunction(\hat{\calibrationError}\circ \hypothesisClass \circ \trainingData)}
\newcommand{\rademacherSamplesExponent}{\nu}


\newcommand{\kernelFunction}{K}
\newcommand{\kernelMapping}{\Phi}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\union}{\cup}
\newcommand{\support}{\mathrm{supp}}
\newcommand{\hilbertSpace}{\mathbb{H}}
\newcommand{\graphDimension}{\mathrm{p}}
\newcommand{\groupA}{a}
\newcommand{\groupB}{b}
\newcommand{\predictionValue}{\prediction}
\newcommand{\groupWeight}{\alpha}
\newcommand{\group}{\mathsf{g}}
\newcommand{\groups}{\mathsf{G}}

\newcommand{\transpose}{\mathsf{T}}


\newcommand{\interval}{\mathrm{I}}
\newcommand{\mat}{\bm}
\newcommand{\neuralNetwork}{\mathrm{NN}}
\newcommand{\nonlinearity}{\sigma}

\newcommand{\subGaussian}{\mathsf{subG}}
\newcommand{\proxyStandardDeviation}{\sigma}
\newcommand\MTkillspecial[1]{% helper macro
\bgroup
\catcode`\&=9
\let\\\relax%
\scantokens{#1}%
\egroup
}
\DeclarePairedDelimiter\brparen
\lparen\rparen
\reDeclarePairedDelimiterInnerWrapper\brparen{star}{
\mathopen{#1\vphantom{\MTkillspecial{#2}}\kern-\nulldelimiterspace\right.}
#2
\mathclose{\left.\kern-\nulldelimiterspace\vphantom{\MTkillspecial{#2}}#3}}
\DeclarePairedDelimiter{\angleBracket}{\langle}{\rangle}
\newcommand{\dotProduct}[2]{\angleBracket{#1,#2}}



==> facct/src/essential/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}

% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
%\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> facct/src/img/tex/binsForLearner.tex <==
%!TeX root = ../../../note.tex
 

\begin{tikzpicture}
\foreach \x in {0,...,5}{
\draw (\x*2,0) rectangle (\x*2+1, 1);};
\node  at (6*2+0.5,0.5) {$\ldots$}  ;
\draw (7*2,0) rectangle (7*2+1, 1);
\draw[black,fill=black] (0.5, 0.5) circle (0.1);
\end{tikzpicture}

==> facct/src/old_stuff/2_related_work.tex <==
\section{Background}



% As machine learning systems have exhibited exemplary performance across a wide variety of tasks, the scope of their use has broadened.  Impactful life decisions which in the past have been rendered exclusively by humans, such as college admission and mortgage approval, are now using machine learning systems to supplement, or even outright replace, humans in the decision making process.  This shift in how such important decisions are made has sparked a new field of machine learning research: \emph{fairness}. 

% Much of modern ML fairness literature is concerned with the implications of learning classifiers via empirical risk minimization (ERM), or some variant thereof, subject to what is known as a fairness constraint.  A fairness constraint is typically formulated as a constraint on the optimization objective which is dependent on the value of a so-called \emph{protected attribute} (also referred to as a \emph{sensitive attribute}). Examples include the fairness constraints known as \emph{statsitical parity} (also referred to as \emph{demographic parity}) introduced by Dwork et al. \citep{dwork2012fairness} and \emph{equality of opportunity} introduced by Hardt et al. \citep{hardt2016equality}.  Most importantly, these works assume access to a fairness constraint which can be enforced during ERM, which is to say, it is known precisely which constraints are required to make the resulting trained classifier fair.  We refer to the setting in which the protected attribute is available to the learner as \emph{learner assessable fairness}.

% When the protected attribute is not available to the learner, the learner is unable to evaluate the fairness of classifier.  In such situations, fairness of the learned classifier is assessed by a meta-learner which \emph{does} have access to the protected attribute.  This setting we refer to as \emph{learner remitted fairness}. In learner remitted fairness, a learner only has access to information about the underlying data distribution.  Examples of such information include, but are not limited to the number of protected groups, and the frequency of each protected group.  The exact information to which a learner has access is often context dependent.

% Multicalibration is a well studied quantity which captures the fairness of a classifier in the learner remitted fairness setting: Hebert-Johnson et al. were the first to develop and study the notion of multicalibration \cite{hebert2017calibration}.  In particular, the authors develop algorithms for learning multicalibrated predictors 
 

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% {\color{blue} Fairness constraints have been heavily studied in recent years, but several limitations exist in current literature:
% one of the most important limitations appearing in modern theoretical fairness literature is the implicit focus on samples of infinite size.   Two examples of an implicit focus on populations of infinite size follow:
  
% \begin{enumerate}
% \item Liu et al. assume the existence of two mutually exclusive population groups, in which each group occupies a known proportion of the population, denoted as $g_\groupA$ and $g_\groupB$ where $g_\groupA = 1-g_{\groupB}$, of the entire population \cite{liu2018delayed} we shall denote as $P$.The exact proportion of each population group is  not always known, but this knowledge is frequently assumed in literature either as an explicit population proportion \cite{MouzannarFairness,kearns2018preventing}, or as a rate parameter in a Poisson Process which generates population $P$ \cite{hashimoto2018fairness}.  

% % whether Hashimoto et al. consider a data generation model which introduces elements of randomness: the authors consider data drawn from a Poisson process in which each each population group $i$ has an associated Poisson rate $\placeholderScalar_i$ \cite{hashimoto2018fairness}, yet their bounds still have an explicit dependence on the Poisson rates.

% \item  The definition of \emph{individual fairness} as given by Dwork et al. can be stated, informally, as a Lipschitz condition \cite{dwork2012fairness}, yet how to validate individual fairness on a deep neural network is not clear: to our knowledge, there is no procedure which can exactly compute the Lipschitz constant of a deep network.  Such Lipschitz-based fairness constraints occur frequently in literature \cite{KimFairness,GillenFairness}

% % Such Lipschitz-condition-based notions of fairness are common in literature: Gillen et al. investigate Lipschitz-based fairness constraints in the context of online learning \cite{GillenFairness}. Kim et al. analyze a bevy of Lipschitz-based fairness constraints, in a setting termed multi-fairness \cite{KimFairness}.
% \end{enumerate}

 

% Therein lies the problem: Datasets used for training and testing machine learning algorithms are of finite size.  We show the finite nature of a dataset impacts the utility of many existing fairness constraints.  In particular, we show that, in the mutli-class classification setting when there are two mutually exclusive population groups, the finite nature of datasets suggests the existence of a baseline level of unfairness which cannot be overcome.  This baseline level of unfairness depends on both the imbalance among population groups and the number of samples in the dataset.  We conclude that when datasets are of finite size, strict notions of fairness may not have much utility, and should instead be replaced by those which tolerate approximate fairness.
% }

% We identify three veins of related work in the fairness in ML domain.  They are: 
% \begin{enumerate}
%     \item Lower bounds for fairness in online learning
%     \item Machine Learning Fairness Problems with finite data
%     \item Impossibility results for Machine Learning Fairness Problems
% \end{enumerate}

% Lower bounds for machine learning fairness exist in the space of online learning:  Joseph et al. consider fairness in the context of multi-armed bandits (MABs) \cite{FairBandits}.  Let $k$ be the number of arms in a MAB problem.  The authors of show that any MAB algorithm with a fairness constraint will experience constant per-round regret--online learning's analogue to loss-- for $\bigOmega\paren*{k^3}$ rounds. The authors compare to a standard MAB algorithm,  Upper Confidence Bound (UCB) \cite{auer2002using}, which experiences constant per-round regret for the first $\bigOh(k)$ rounds.   This work suggests that MAB algorithms with fairness constraints are indeed more expensive than MAB algorithms without fairness constraints. 

% Lower bounds on approximation ratios for fair clustering have been are discussed by Chierichetti et al. \cite{chierichetti2017fair}.  The authors also show fairness constraints can introduce a ``computational bottleneck''.

%  There exists literature which connects fairness to the number of samples in a finite dataset: Kearns et al. show that both false positive subgroup fairness and statistical parity each uniformly converge which suggests the finite nature of datasets used in machine learning does affect fairness.  Such proofs; however, only require upper-bounds on fairness.  Furthermore, the authors also suggest that finite training time can induce some level of unfairness in a trained classifier. \cite{kearns2018preventing}, but their work focuses on the binary classification setting when populations consist of two or more mutually exclusive groups. Donini et al. consider $\epsilon$-fairness, in which $\epsilon$ is a parameter which governs how much unfairness a learner is willing to tolerate \cite{NIPS2018_7544}.

%  Impossibility results for machine learning fairness problems represent the largest vein of related work. Kleinberg et al. demonstrate develop three fairness conditions, and show that with the exception of constrained special cases, no solution can satisfy the three conditions simultaneously \cite{kleinberg2016inherent}.  This suggests certain notions of fairness may be incompatible with each other.  The conclusion supports observations made in earlier papers: Dwork et al identify that when group-wise fairness constraints are satisfied, individuals may deem the solution ``blatantly unfair'' \citep{dwork2012fairness}.

% % In the real world, such constraints are not always available or apparent.  Taking a statistical-learning theoretic lens, we investigate the conditions under which standard empirical risk minimization is likely to yield a fair, according to several of our criterion, classifier. Informally, we see that if the distribution of data is independent from a sensitive feature, then classifiers are fair with respect to our criteria.





==> facct/src/old_stuff/3_5_calibration_concentration.tex <==
%!TeX root = ../note.tex
\section{Concentration Inequalities for Multi-calibration}

We begin this section by stating a sample-complexity bound for multi-calibration uniform convergence from Shabat et al. \cite{shabat2020sample}

\begin{theorem}
    Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Furthermore assume that groups $\set{U_1,\dotsc,U_{\abs{\Gamma}}}$ may overlap.Then $\hypothesisClass$ has the uniform multicalibration convergence property with
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\gamma,\psi} = \bigOh\paren*{\frac{\log\paren*{\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}}{\errorTolerance^2\gamma\psi}}
    \end{equation}

\end{theorem}

We will improve upon this bound by utilizing the structure which the assumption of mutually exclusive groups provides:

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    The ``bad'' event $B^{\trainingData}$ is the event in which denotes the existence of an interesting category for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$:

    \begin{equation}
        B^{\trainingData} \definedAs \set*{\trainingData : \exists \hyp \in \hypothesisClass, \exists (U,I) \in C_{\hyp} : \abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance}
    \end{equation}

    We also define the ``good'' event $G^{\trainingData,\placeholder}$, which is the event that each interesting category in $\trainingData$  contains at least $\placeholder$ samples:

    \begin{equation}
        G^{\trainingData,\placeholder} \definedAs \set*{\trainingData : \forall \hyp \in \hypothesisClass, \forall (U,I) \in C_{\hyp} : \abs{(U_{\trainingData},I)} \geq \placeholder }
    \end{equation}

    Note that the ``bad'' event and the ``good'' event are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    \begin{equation}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}
    \end{equation}

    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,U,I} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Now, we upper-bound this quantity:

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    % \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\
        &\leq  \sum_{\hyp \in \hypothesisClass}\sum_{(U,I)\in C_{\hyp}} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}\\
        &\leq 4\frac{\abs{\Gamma}\abs{\hypothesisClass}}{\lambda}\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}



   \begin{equation}
    \Pr{\trainingData \in B^{\trainingData} \given \trainingData \in G^{\trainingData,\placeholder}}  \iff \placeholder \geq \frac{2}{\errorTolerance^2}\log\paren*{\frac{8\abs*{\Gamma}\abs{\hypothesisClass}}{\errorConfidence\lambda}}
   \end{equation}

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   
   \begin{align}
    \Pr{\abs{\paren*{U_\trainingData,I}} \leq \placeholder} &\leq Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
    &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
    &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
   \end{align}
\end{proof}



With only lower bounds on the frequency of an ``interesting'' category, our bounds are remarkably similar to those
Let's now analyze the case of the finite hypothesis class but in the leave $k$ out setting.  That is, given $k$, a non-negative integer less than $\abs{\Gamma}$, what is the sample complexity necessary for at least $\abs{\listInterestingCategories_{\hyp}} -k$ groups to satisfy the fairness criteria?


\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  

 

    We also define the ``good'' event $G^{\trainingData,\placeholder,m}$, which is the event that at least $\abs{C}-m$ interesting categories in $\trainingData$  contain at least $\placeholder$ samples.

    Note again the ``bad'' events and the ``good'' events are not mutually exclusive. 

    Using this notation, our goal is to upper-bound

    We now define a new ``bad'' event, distinct from the event defined in the previous proof.  Let $B^{\trainingData,\listInterestingCategories}$ be the event which denotes the existence of at least $1$ interesting category in set $\listInterestingCategories$ for which the difference between its true calibration error and empirical calibration error is larger than $\errorTolerance$.  Suppose we have a function $\goodGroups$ which takes in, as an argument, the event $G^{\trainingData,\placeholder,m}$ and returns the powerset of exactly $\numInterestingCategories-k$ distinct categories $(U,I)$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$ holds true. That is to say, for any integer $k$, $\goodGroups\paren*{G^{\trainingData,\placeholder,k}}$ $\numInterestingCategories - m$ categories which satisfy this condition.

    WE further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\listInterestingCategories} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.
    
    Event $B^{\trainingData,l,\listInterestingCategories}$ occurs when at least $l$ categories $(U,I)$ in list $\listInterestingCategories$ for which $\abs{\empiricalCalibrationError\paren*{\hyp,U,I,\trainingData}-\calibrationError\paren*{\hyp,U,I}} > \errorTolerance$

    Let $\listInterestingCategories^k$ denote the list of all possible combinations of $k$ interesting categories.  In order to have leave-$k$-out fairness, we bound 
    
    \begin{align}\Pr{\bigIntersection_{i=1}^{\abs{\listInterestingCategories}} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \sum_{\listInterestingCategories' \in \listInterestingCategories^k}\prod_{i=1}^k \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder} \given \bigIntersection_{j=1}^{i-1}\curlyBrace*{B_{\interestingCategory_j}^{\trainingData} \union \lnot G_{\interestingCategory_j}^{\trainingData,\placeholder}} }\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k} \subseteq \listInterestingCategories} \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    &\leq \prod_{\set{\interestingCategory_i}_{i=1}^{k}} \errorConfidence\\
    &= \errorConfidence^{k}
    \end{align}



 
    For notational convenience, we define the following:

    \begin{align}
        \mu_y\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\labelElement \given \sample \in U, \hyp\paren*{\sample}\in I}  \\
        \mu_\hyp\paren*{\hyp,\interestingCategory} &\definedAs \E[\paren*{\sample,\labelElement}\in \sampleDist]{\hyp\paren*{\sample} \given \sample \in U, \hyp\paren*{\sample}\in I}  
    \end{align}

    Suppose we wish to have leave-$k$-out fairness.  Then must we have $l+m\geq k$
    
    Then the event we are interested upper-bounding is:

    
    \begin{align}
        \Pr{B^{\trainingData,\listInterestingCategories_\hyp^{\marker},l} \given G^{\trainingData,\placeholder,m}} &\leq \sum_{\hyp \in \hypothesisClass} \Pr{B_{\interestingCategory_1}^{\trainingData,\listInterestingCategories_\hyp^{\marker} \setminus \set*{}} \intersection B_{\interestingCategory_2}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_1}} \intersection \hdots \intersection  B_{\interestingCategory_l}^{\trainingData,\listInterestingCategories_\hyp^{\marker}\setminus \set{\interestingCategory_i}_{i=1}^{l-1}}} \\
        &\leq \sum_{\hyp \in \hypothesisClass} \binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}\\
        &\leq \abs{\hypothesisClass}\binom{\abs*{\listInterestingCategories_\hyp}-m}{l}\paren*{4 \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^{l}
    \end{align}

    where $\listInterestingCategories_{\hyp}^{\marker}\definedAs \goodGroups\paren*{G^{\trainingData,\placeholder,m}}$

    which suggests

    \begin{equation}
        \frac{\errorConfidence}{2} \geq \abs{\hypothesisClass}\binom{\listInterestingCategories_{\hyp}-m}{l}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}}^l \iff \placeholder \geq \frac{2}{\errorTolerance^2}\ln\paren*{4\sqrt[l]{\binom{\abs{\listInterestingCategories_{\hyp}}-m}{l}\frac{2\abs*{\hypothesisClass}}{\errorConfidence}}}
    \end{equation}

    Let us now bound $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}}$ 

    In order to compute this bound, we further decompose the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    We upper-bound the complement of the good event, $\Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,m}}}$, by translating it into the language of category-wise good events,$G^{\trainingData,\placeholder,\listInterestingCategories}_{\interestingCategory}$ , into it's category-wise good events:

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{}}_{\interestingCategory_1} \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_1}}_{\interestingCategory_2} \intersection \hdots \intersection \lnot G^{\trainingData,\placeholder,\listInterestingCategories \setminus \set{\interestingCategory_i}_{i=1}^{m-1}}_{\interestingCategory_m}}\\
        &\prod_{i=1}^m
    \end{align}



    In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$, hence we have

    \begin{align}
        \Pr{\lnot \curlyBrace*{\trainingData \in G^{\trainingData,\placeholder,k}}} &\leq \Pr{\abs{\paren*{U_\trainingData,I}} \leq \frac{\E{\abs{\paren*{U_\trainingData,I}}}}{2}  } \\
        &\leq \exp\paren*{-\frac{\E{\abs{\paren*{U_\trainingData,I}}}}{8}} \\
        &\leq \frac{\lambda\errorConfidence}{2\abs{\Gamma}\abs{\hypothesisClass}}
       \end{align}


    % \Pr{\set*{\bigcup_{\listInterestingCategories \in \goodGroups\paren*{G^{\trainingData,\placeholder,k}}}\trainingData \in B^{\trainingData,l,\listInterestingCategories}} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq \sum_{\hyp \in \hypothesisClass}\sum_{B^{\trainingData,k} \in \powerSet_{\trainingData,k}}\sum_{(U,I)\in C_{\hyp}\setminus \badGroups\paren*{B^{\trainingData,k}}}\bracket*{\Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} } \\

    \begin{align}
        \Pr{\trainingData \in B^{\trainingData,l,\listInterestingCategories} \given \trainingData \in G^{\trainingData,\placeholder,k}} &\leq 4\binom{\abs{\listInterestingCategories}}{l}\abs{\hypothesisClass} \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}

The bad event is not so simple.  If we are considering leave 

   In order to invoke the relative Chernoff bound in a convenient manner, we will set $\sampleComplexity_\hypothesisClass\paren*{\errorTolerance,\errorConfidence,\psi,\gamma,\lambda}$ such that $\E{\abs{\paren*{U_\trainingData,I}}} \geq 2\placeholder$

   Hence, we have 
   

\end{proof}

==> facct/src/old_stuff/3_7_calibration_concentration.tex <==
%!TeX root = ../note.tex

\subsection{Multi-calibration uniform convergence in the Poisson Model.}

\begin{theorem}  Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then, for the Poisson model, we have the following sample-complexity for leave $k$ out fairness:
    \begin{equation}
        \sampleComplexity_{\hypothesisClass}^{\multicalibration}\paren*{\errorTolerance,\errorConfidence,\poissonRate_{\interestingCategory},k} = \bigOh\paren*{\frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\poissonRate_\interestingCategory\errorTolerance^2}}
    \end{equation}
\end{theorem}

\begin{proof} We will follow notation of Shabat et al.
    Let $C_\hyp$ denote the collection of all interesting categories according to predictor $\hyp$:
    \begin{equation}
        C_{\hyp} \definedAs \curlyBrace*{(U,I): U \in \Gamma, I \in \Lambda, \Pr[\sample \drawnFrom \sampleDist]{\sample \in U} \geq \gamma, \Pr[\sample \drawnFrom \sampleDist]{\hyp\paren*{\sample} \in \Lambda} \geq \psi},
    \end{equation}

    To analyze leave $k$ out fairness, we further decompose both the good and bad events into category-wise good and and bad events.
  
    We further specify the bad event where, for a given hypothesis $\hyp \in \hypothesisClass$, and a given category $\interestingCategory \in \listInterestingCategories$:

    \begin{align}
        B_{\interestingCategory}^{\trainingData,\hyp} &\definedAs \set*{\trainingData :  \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}} \union \curlyBrace*{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,\interestingCategory}}\geq \sfrac{\errorTolerance}{2}}}
    \end{align}

    In order to compute this bound, we also further specify  the good event by defining category-wise good events: Given a category $\interestingCategory \in \listInterestingCategories_\hyp$ all hypotheses $\hyp$:

    \begin{equation}
        G_{\interestingCategory}^{\trainingData,\placeholder,\hyp} \definedAs \curlyBrace*{\trainingData : \forall \hyp \in \hypothesisClass:  \abs{\interestingCategory} \geq \placeholder }
    \end{equation}

    Utilizing this definition of $\goodGroups$, we may now define the bad event $B^{\trainingData,l}$.

    In order to have leave-$k$-out fairness, there must be at least $k$ distinct categories $\interestingCategory$ for which at least one of the following is true:

    \begin{enumerate}
        \item Good event $G_{\interestingCategory}^{\trainingData,\placeholder}$ does \emph{not} occur
        \item Bad event $B_{\interestingCategory}^{\trainingData,\listInterestingCategories}$ does occur
    \end{enumerate}

    \begin{align}
        \Pr{\lnot G_{\interestingCategory}^{\trainingData,\placeholder}} &= \Pr{\abs{\interestingCategory} \leq \placeholder} \\
        &\leq \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}
        % &= \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}
    \end{align}

    where $\regularizedGammaFunction$ is the regularized gamma function:

    \begin{equation}
        \regularizedGammaFunction(\placeholder_1,\placeholder_2) \definedAs \frac{\GammaFunction\paren*{\placeholder_1,\placeholder_2}}{\GammaFunction\paren*{\placeholder_1}} = \frac{\int_{\placeholder_2}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}{\int_{0}^{\infty}t^{\placeholder_1-1}e^{-t}\mathrm{d}t}
    \end{equation}

    Let us now bound $\Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}}$:

    \begin{align}
        \Pr{B_{\interestingCategory}^{\trainingData,\hyp} \given G_{\interestingCategory}^{\trainingData,\placeholder}} &\leq \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\labelElement-\mu_{\hyp}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}} + \Pr{\abs*{\frac{1}{\placeholder}\sum_{\paren*{\sample,\labelElement} \in \trainingData}\hyp\paren*{\sample}-\mu_{\labelElement}\paren*{\hyp,U,I}}\geq \sfrac{\errorTolerance}{2}}  \\
        &\leq 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}
    \end{align}


    Let $\listInterestingCategories^{k}$ denote the set of all combinations of $k$ categories in $\listInterestingCategories$.  All together, we have:

    \begin{align}
\Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} +\exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}\\
            &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\poissonRate_\interestingCategory}^2}{2\poissonRate_{\interestingCategory}-\placeholder}}}^k\\
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\paren*{\placeholder-\placeholder_{\interestingCategory}}^2}{2\poissonRate_{\interestingCategory}}}}}^k 
            \intertext{assume $\placeholder \leq \poissonRate_{\interestingCategory}/2$}
            &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}}}^k  \label{eq:PoissonUnionBound}\\
    \end{align}

    % \begin{align}
    %     \Pr{\bigIntersection_{\listInterestingCategories' \in \listInterestingCategories^k} \curlyBrace*{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}} &= \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} \Pr{B_{\interestingCategory_i}^{\trainingData} \union \lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories}  \curlyBrace*{\Pr{B_{\interestingCategory_i}^{\trainingData}\given G_{\interestingCategory_i}^{\trainingData,\placeholder}} + \Pr{\lnot G_{\interestingCategory_i}^{\trainingData,\placeholder}}}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\prod_{\set{\interestingCategory_1,\dotsc,\interestingCategory_k} \subseteq \listInterestingCategories} 4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}\\
    %                 &\leq \binom{\abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}^k\\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \regularizedGammaFunction\paren*{\placeholder+1,\poissonRate_\interestingCategory}}}^k \\
    %                 &= \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\sum_{i=0}^{\placeholder}\frac{\poissonRate_{\interestingCategory}^i}{i!}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + e^{-\poissonRate_{\interestingCategory}}\paren*{e^{\poissonRate_{\interestingCategory}}-\frac{\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &\leq \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate}\poissonRate_\interestingCategory^{\placeholder+1}}{\paren*{\placeholder+1}!}}}}^k \\
    %                 &< \paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{e^{-\poissonRate_{\interestingCategory}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}\exp\paren*{-\paren*{\placeholder+1}+\frac{1}{12\placeholder + 13}}}}}}^k \\
    %                 &=\paren*{\frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}} + \paren*{1-\frac{\exp\paren*{-\poissonRate_{\interestingCategory}+\placeholder+1-\frac{1}{12\placeholder+13}}\poissonRate_\interestingCategory^{\placeholder+1}}{\sqrt{2\pi}\paren*{\placeholder+1}^{\placeholder + \frac{3}{2}}}}}}^k \label{eq:PoissonUnionBound}\\
    %         \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the left-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\paren*{4\exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}} & \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder\errorTolerance^2}{2}}& \leq \frac{k\errorConfidence^{\frac{1}{k}}}{8 e \abs{\listInterestingCategories}} \\ 
        \placeholder &\geq \frac{2\ln\paren*{\frac{8 e \abs{\listInterestingCategories}}{k\errorConfidence^{\frac{1}{k}}}}}{\errorTolerance^2}
    \end{align}

    WE now determine a lower-bound for $\placeholder$ based on the right-hand term in \cref{eq:PoissonUnionBound}:

    \begin{align}
        \frac{e \cdot \abs{\listInterestingCategories}}{k}\exp\paren*{-\frac{\paren*{\placeholder}^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{\errorConfidence^{\frac{1}{k}}}{2} \\
        \exp\paren*{-\frac{\placeholder^2}{2\poissonRate_{\interestingCategory}}}& \leq \frac{ k\errorConfidence^{\frac{1}{k}}}{2e\abs{\listInterestingCategories}} \\
       \placeholder& \geq \sqrt{2\poissonRate_{\interestingCategory}\ln\paren*{\frac{2e\abs{\listInterestingCategories}}{ k\errorConfidence^{\frac{1}{k}}}}} \\
    \end{align}

\end{proof}



    Let $\placeholderScalar$ be a positive integer and let $\poissonRate$ be real number.  Then the following holds:
\begin{equation}
    \frac{\poissonRate^{\placeholderScalar+1}}{\paren*{\placeholderScalar+1}!} \leq e^{\poissonRate} - \sum_{i=0}^{\placeholderScalar}\frac{\poissonRate^{i}}{i!}
\end{equation}




\begin{lemma}
    \begin{align}
      \binom{\abs{\listInterestingCategories}}{k}^{\frac{1}{k}} < \paren*{\frac{1}{\sqrt{2\pi}}\frac{\abs{\listInterestingCategories}^{\paren*{\abs*{\listInterestingCategories}+\frac{1}{2} }}}{\paren*{\abs*{\listInterestingCategories}-k}^{\abs*{\listInterestingCategories}-k + \frac{1}{2}}k^{k+\frac{1}{2}} }}^{\frac{1}{k}}
    \end{align}

\end{lemma}

\begin{lemma} Let $a,b$ be integers such that $a \geq b \geq 1$ (from wiki)
    THe following are true:
    \begin{equation}
        \frac{a^b}{b^b} \leq \binom{a}{b} \leq \frac{a^b}{b!} \leq \paren*{\frac{e\cdot a}{b}}^{b}
    \end{equation}
\end{lemma}

==> facct/src/old_stuff/3_RevisitingResidualHypothesisBoosting.tex <==
\section{Revisiting Residual Hypothesis Boosting}
% In this note we present a boosting framework for any sequential composition of functions.
% For the rest of note let $T \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $T$ feature transformations:
% $$F(\sample) = (G_T \circ G_{T-1} \circ \cdots \circ G_1)(\sample),$$
% where $G_t$ ($t \in [T]$) is some function. Note that $G_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $G_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically say a CNN.
% The final binary classifier is determined by another weight vector $\weights_T$ of appropriate shape,
% where the classification is determined as
% $$\sign(\weights_T^{\transpose}F(\sample))$$
% We will use the notation $G_{1:t}$ to mean the composition $G_t \circ G_{t-1} \circ \cdots \circ G_1$.
% We further use the notation $g_t \definedAs G_{1:t}$ to mean the composition of the first $t$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
The weight vectors $\weights_1, \dots, \weights_{T-1}$ will not appear in the final classifier, but they are used to
guide training. Specifically, the following proposition is straightforward:
\begin{proposition}[Final hypothesis is sum of residuals]
  The final hypothesis is the \emph{sum of residual hypotheses} scaled by $1/\alpha_T$:
  \begin{align*}
    \weights_T^{\transpose}F(\sample) = \frac{1}{\alpha_T}\sum_{t=0}^{T-1}h_t(\sample)
  \end{align*}
\end{proposition}
Therefore we can focus on training $\sum_{t=1}^Th_t$, and we can do it simply by AdaBoost.
In fact, let us see what is going on there: Let $K \in [T]$, and suppose that $h_1, \dots, h_{K-1}$
have been trained (when $K=1$, we have $0$ to start with), and our goal is to train a hypothesis
$\sum_{t=1}^Kh_t$ to minimize the training error. That is
\begin{align}
  \minimize_{h_0,\dots,h_{K-1}} \sum_{i=1}^\numSamples \exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right)
\end{align}
where we have been using exponential loss. We note that:
\begin{align}
  &\exp\left(-y_i\left(\sum_{t=0}^{K-1}h_t(\sample_i)\right)\right) \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right) + (-y_ih_{K-1}(\sample_i))\right) && \text{($h_0, \dotsc, h_{K-2}$ have been trained)} \\
  = &\exp\left(-y_i\left(\sum_{t=0}^{K-2}h_t(\sample_i)\right)\right) \exp(-y_ih_{K-1}(\sample_i)) \\
  = &\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))\exp(-y_ih_{K-1}(\sample_i)) \\
\end{align}
Here the term $\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i)$ is viewed as a ``weight'' we assigned to each training point.
In AdaBoost there is a specific iterative weighting procedure to turn these weights into a proper probability distribution.
That probability distribution will be important for the theory, so we repeat that derivation here:
\begin{itemize}
\item The end goal is to turn these terms into
  \begin{align}
    D_{K}(i) = \frac{\exp(-y_i\alpha_{K-1}o_{K-1}(\sample_i))}{\sum_{j=1}^\numSamples\exp(-y_j\alpha_{K-1}o_{K-1}(\sample_j))}
  \end{align}
\item Note that we know that
  \begin{align}
    \alpha_{K-1}o_{K-1} \definedAs \sum_{t=1}^{K-1}h_t
  \end{align}
  It turns out that such a distribution can be constructed recursively as follows:
  \begin{enumerate}
  \item Start with a uniform distribution on all the training points: $D_0(i) = \frac{1}{N}$.
  \item Then for $t = 1, 2, \dots$,
    \begin{align}
      \label{def:recursive-weighting}
      D_t(i) = \frac{D_{t-1}(i)\exp(-y_ih_t(\sample_i))}{\sum_{j=1}^\numSamples D_{t-1}(j)\exp(-y_jh_t(\sample_j))}.
    \end{align}
  \end{enumerate}
\end{itemize}
Therefore at the stage $K$ of AdaBoost, the minimization problem is equivalent to:
\begin{align}
  \label{def:stage-K-objective}
  \minimize_{h_K}\sum_{i=1}^\numSamples D_{K-1}(i)\exp(-y_ih_K(\sample_i))
\end{align}
Let us now open $h_K$ a little, by definition
\begin{align*}
  h_{K-1}(\sample) &= \alpha_Ko_K(\sample) - \alpha_{K-1}o_{K-1}(\sample) \\
         &= \alpha_K\weights_K^{\transpose}G_K(g_{K-1}(\sample)) - \alpha_{K-1}o_{K-1}(\sample)
\end{align*}
The unknowns here are only $\alpha_K, \weights_K$, and $G_K$ (the feature transformation at step $K$),
and therefore the minimization problem at boosting stage $K$ can be rewritten as:
\begin{align*}
  (\alpha_K, \weights_K, G_K) = \argmin_{\alpha, w, G} \sum_{i=1}^\numSamples D_{K-1}(\sample_i)\exp\left(
  -y_i \left(\alpha \cdot w^{\transpose} \cdot G(g_{K-1}(\sample_i)) - \alpha_{K-1}o_{K-1}(\sample_i)\right)\right)
\end{align*}
\begin{remark}
  If one plugs in the ResNet where $G_K(g_{K-1}(\sample_i)) = f_K(g_{K-1}(\sample_i)) + g_{K-1}(\sample_i)$,
  then the goal is to identify $f_K$. This recovers BoostResNet!
\end{remark}

\section{On proving that training error will vanish}

We now give a key observation of why this general residual hypothesis boosting can quickly make
the training error vanish. The argument here is really already in the proof of AdaBoost.
We want to repeat it here because it demonstrates again that there is nothing special in BoostResNet about ResNet!
Here is the key argument: In binary classification we eventually want to bound the following:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\exp\left(-y_i\left(\sum_{t=0}^{T-1}h_t(\sample_i)\right)\right)
\end{align}
This can be turned into a sum of product:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp\left(-y_ih_t(\sample_i)\right)
\end{align}
Basically, this recursive nature of $D_K$ allows us to turn this \emph{sum of product} into \emph{product of sum}.
That is:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i))
  &= \sum_{i=1}^{\numSamples}\Big\{D_0(i)\exp(-y_ih_0(\sample_i))\Big\}\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples} \left\{D_1(i)\left(\sum_{j=1}^mD_0(j)\exp(-y_jh_0(\sample_j))\right)\right\} \prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i)) \\
  &= \sum_{i=1}^{\numSamples}D_1(i)Z_1\prod_{t=1}^{T-1}\exp(-y_ih_t(\sample_i))
\end{align}
where we define $Z_1 \definedAs \sum_{j=1}^mD_0(j)\exp(-y_jh_1(\sample_j))$,
which measures the quality of residual hypothesis $h_1$. Continue doing this we have:
\begin{align}
  \sum_{i=1}^{\numSamples}D_0(i)\prod_{t=0}^{T-1}\exp(-y_ih_t(\sample_i)) = \prod_{t=0}^{T-1}Z_t
\end{align}
where
$$Z_t \definedAs \sum_{j=1}^\numSamples D_{t}(j)\exp(-y_jh_t(\sample_j)).$$
This is the key why we can bound training error!

==> facct/src/old_stuff/4_NNCaseStudy.tex <==
%!TeX root = ../note.tex

\section{Neural Networks and Fairness}

Our technique for deriving sample complexity bounds is not just limited to the kernelized classifier, but we are able to compute multicalibration uniform convergence bounds any hypothesis class for which the Rademacher complexity is defined.  One such family of classifiers is the feedforward neural network:

Each hypothesis $\hyp_{\neuralNetwork}$ in the hypothesis class $\hypothesisClass_{\neuralNetwork}$ is parametrized by a sequence of matrices $\mat{W} \definedAs \left(\mat{W}_1,\mat{W}_2,\dotsc,\mat{W}_\depth\right)$.  For $i \in \left\{1,\dotsc,\depth\right\}$, we assume $\mat{W}_i \in \realNumbers^{\dimension_i \times \dimension_{i-1}}$ where $\dimension_0$ is the dimension of the input vector $\sample$ and $\dimension_{\depth} = 1$.  We let $\nonlinearity(\cdot)$ denote the rectified linear unit (ReLU), i.e. for $\vec{\placeholder} \in \realNumbers^{\dimension}$, $\nonlinearity(\vec{\placeholder}) \definedAs \max\left\{\vec{\placeholder},\vec{0}_\dimension\right\}$ and is applied element-wise to $\vec{\placeholder}$. The neural network is formulated as:



\begin{dmath}
    \hyp_{\mat{W}}'(\sample) \definedAs \mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))
\end{dmath}

and the decision version of the neural network is formulated as:

\begin{dmath}\label{eq:NNHypothesisClass}
        \hyp_{\mat{W}}(\sample) \definedAs \sgn\left(\mat{W}_{\depth}\nonlinearity(\mat{W}_{\depth-1}\nonlinearity(\hdots \nonlinearity(\mat{W}_1\sample) \hdots ))\right)
\end{dmath}
An upper-bound on the Rademacher complexity of such a neural network was given by Bartlett et al \cite{bartlett2017spectrally}.  We use the ``nice'' formulation of the bound from Yin et al. \cite{yin2019rademacher}.

\begin{theorem}[Theorem 5 from Yin et al.]
    Consider the neural network hypothesis class \begin{dmath}\hypothesisClass_{\neuralNetwork} \definedAs \left\{\hyp_{\neuralNetwork} : \mat{W} = (\mat{W}_1,\dotsc,\mat{W}), \\ \forall i \in \left\{1,\dotsc,\depth\right\}: \norm{\mat{W}_i}_{\sigma} \leq \spectralBound_i, \norm{\mat{W}_i}_{2,1} \leq \normBound_i\right\} \end{dmath}

    Then we have 

    \begin{dmath}
        \rademacherComplexity_{\trainingData}(\hypothesisClass_{\neuralNetwork}) \leq \frac{4}{\numSamples^{3/2}} + \frac{26\log\left(\numSamples\right)\log\left(2\dimension_{\max}\right)}{\numSamples}A
    \end{dmath}
    where $A=\norm{\mat{X}}_{\Frobenius}\left(\prod_{i=1}^{\depth}\spectralBound_i \right)\left(\sum_{j=1}^{\depth} \left(\frac{\normBound_j}{\spectralBound_j}\right)^{2/3}\right)^{3/2}$
\end{theorem}

Using techniques similar to those of the previous section, we are able to determine sample complexity bounds for multicalibration uniform convergence in feedforward ReLU networks.  In particular, we develop lemmas similar to \cref{lem:shabat24analogue,lem:shabat25analogue}, but for feedforward ReLU networks:

\begin{lemma} Let $\hypothesisClass_{\neuralNetwork}$ be as defined in \cref{eq:NNHypothesisClass}.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $\group \in \Gamma$ be a subpopulation.  Furthermore, let $\lambda = \min_{\hyp'\in \hypothesisClass_{\neuralNetwork}',\sample \in \sampleSpace}\left\{\hyp'(\sample)\right\}$

\end{lemma}
Scratch:
\begin{dgroup}
    \begin{dmath}
        \errorTolerance \hiderel{\leq} 2\rademacherComplexity_{\trainingData_{\group}}(\empiricalCalibrationError \circ \hypothesisClass_{\neuralNetwork}) + 4c\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{4}{\numSamples_{\group}^{3/2}} + \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Assume for some $\alpha \in \realNumbers_+$, $\frac{4}{\numSamples_{\group}^{3/2}} \leq \alpha \frac{26\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A $}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(\numSamples_{\group}\right)\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation}
         \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\frac{\sqrt{\numSamples_\group-1}}{\numSamples_\group}\log\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \begin{dmath}
                \leq 2\max\left\{1,\frac{1}{\lambda}\right\}\left(\frac{26(1+\alpha)\log\left(2\dimension_{\max}\right)}{\sqrt{\numSamples_{\group}}}A\right) + 4\sqrt{\frac{2\log\left(4/\errorConfidence\right)}{\numSamples_\group}}
        \end{dmath}
        \intertext{Algebraic Manipulation:}
        \begin{dmath}
                \errorTolerance^2 \leq 8\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{26^2(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
            \begin{dmath}
                = 5408\max\left\{1,\frac{1}{\lambda^2}\right\}\left(\frac{(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)}{\numSamples_{\group}}A\right) + 64\frac{\log\left(4/\errorConfidence\right)}{\numSamples_\group}
        \end{dmath}
        \intertext{Algebraic Manipulation}
        \begin{dmath}
                \numSamples_{\group} \leq \frac{5408\max\left\{1,\frac{1}{\lambda^2}\right\}(1+\alpha)^2\log^2\left(2\dimension_{\max}\right)A}{\errorTolerance^2} + \frac{64{\log\left(4/\errorConfidence\right)}}{\errorTolerance^2}
        \end{dmath}
\end{dgroup}
 

==> facct/src/old_stuff/4_ballsandbins.tex <==
%!TeX root = ../note.tex

\section{Balls and Bins}\label{sec:ballsAndBins}


Before investigating the behavior of our fairness on general loss function, we seek to develop intuition via a ``balls-and-bins'' perspective: We imagine the learner, blind to protected feature $\sampleProtected$, must classify each sample (the ball) in $\trainingData$ with exactly one of $\abs{\labelSpace}$  labels (the bins).  After all examples in $\trainingData$ have been classified, a meta-learner which has access to all features of any sample, including the protected feature $\sampleProtected$.

\begin{figure}
    \input{src/img/tex/binsForLearner.tex}
\end{figure}


We may view fairness with a balls and bins perspective.  Within the two group setting in which the elements of $\labelSpace$ are discrete, we examine $\numSamples_+$ and $\numSamples_-$ impact an empirical fairness metric.  We again consider the setting in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$, however the protected groups are not always balanced: $\Pr{\sampleProtected = \groupA}$ is not necessarily equal to $\Pr{\sampleProtected = \groupB}$.

We now share our first bound on our fairness metric, which arises from two invokations of the union bound.  We utilize the following fact in our to construct our bounds: we utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$.  Note the dependence on number of labels $\abs{\labelSpace}$ appears both inside and outside the exponential. 

\begin{theorem}\label{\thmOne}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}
\end{equation}

\end{theorem}





\begin{proof}
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
    &\leq \sum_{\labelElement \in \labelSpace}\exp\paren*{-\frac{\numSamples_{+,\labelElement}\placeholder^2}{\abs*{\labelSpace}}} + \exp\paren*{-\frac{\numSamples_{-,\labelElement}\placeholder^2}{\abs*{\labelSpace}^2}}\label{eq:applyHoeffdingInequality}\\
        &\leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}^2}}}\label{eq:applySimplification}
\end{align}
\end{proof}

\Cref{\thmOne} does gives us some intuition about our machine learning fairness. Namely, our fairness metric has no explicit dependence on the accuracy of our classifier.  Furthermore, this bound is broadly applicable as it is agnostic to underlying classification architecture: The bound has dependence only on the sample distribution $\sampleDist$.  This upper-bound on fairness has a dependence on the number of labels $\abs{\labelSpace}$ and the number of the lowest number of samples assigned to a (label $\labelElement$, group $\sampleProtected$) pair.

The  dependence on $\abs{\labelSpace}$ is in fact suboptimal -- the above bound is na\"vely constructed.  Whereas we only used the fact that probabilities are bounded between $0$ and $1$, we may use knowledge that the sum of all probabalistic events is $1$ to tighten our bound and yield \cref{thm:Two}.  More formally, we know:

\begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i} \end{equation} 




We will show in \cref{\thmTwo} that we can indeed eliminate the dependence on $\abs{\labelSpace}$  outside the exponential by utilizing the fact: \begin{equation}1 = \sum_{i=1}^{\abs{\labelSpace}} \Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \sampleDist]{\labelElement = \labelElement_i}\end{equation}



The bound presented in $\cref{\thmOne}$ is also loose: We applied a union bound several times to arrive at $\cref{eq:applyUnionBound}$ which is an upper-bound on the left side of $\cref{eq:triangleInequality}$. By using Hoeffding's inequality, we only utilize the fact that, for any label $\placeholder$ and any group $\marker$, $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ is bounded between $0$ and $1$, hence our bounds implicitly assume that the random variable $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has the maximum variance of a random variable bounded over such an interval, yet it cannot be the case, that when $\abs*{\labelSpace}\neq 2$ $\frac{\numSamples_{\marker,\placeholder}}{\numSamples_{\marker}}$ has maximum variance for each $\placeholder, \marker$ pair, as we know 

\begin{equation}
    1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}
\end{equation}

Lastly, we compare \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification}:  if the number of samples assigned to each label $\labelElement \in \labelSpace$ is balanced, then \cref{eq:applyHoeffdingInequality} and \cref{eq:applySimplification} evaluate to similar quantities.  On the other hand, if there exists a label $\labelElement$ in label space $\labelSpace$ such that the number of samples assigned to that label is a small, positive rational number, then it is not hard to see  \cref{eq:applySimplification} is a very loose upper bound on \cref{eq:applyHoeffdingInequality}.  Naturally, the question which follows is, can we do better?  Indeed, we can do better, as we prove in \cref{\thmTwo}

\begin{theorem}\label{\thmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \frac{\numSamples_{ \sampleProtected,\labelElement}}{1}$

\end{theorem}


\begin{proof}
    
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq   \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} + \sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} >  \placeholder} \label{eq:triangleInequality}\\
    &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \placeholder/2} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \placeholder/2} \\
    & \leq \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}} > \frac{\placeholder}{2\abs{\labelSpace}}} + \sum_{\labelElement \in \labelSpace}\Pr{ \abs*{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}-\E{\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}} > \frac{\placeholder}{2\abs{\labelSpace}}} \label{eq:applyUnionBound}\\
        \shortintertext{Utilizing \cref{cor:chernoffNice} with $\errorTolerance = \frac{\placeholder}{2\abs{\labelSpace}}$:}
    % &\leq \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{+,\labelElement}}{3}} +  \sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{\paren*{\frac{\placeholder}{2\abs{\labelSpace}\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}^2\cdot\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}} \cdot \numSamples_{-,\labelElement}}{3}}\\
    &\leq\sum_{\labelElement \in \labelSpace} 2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{+,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} +  \sum_{\labelElement \in \labelSpace}2\exp\paren*{-\frac{ \placeholder^2 \numSamples_{-,\labelElement}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}}\\
    &\leq \sum_{\labelElement \in \labelSpace} 4\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2\E{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}}}} \\
    \intertext{We invoke \cref{lem:multinomialDistributionBound} to yield the right-hand-sum:}
        &\leq 16\sum_{i=2}^{\abs{\labelSpace}} \exp\paren*{-\frac{ i\placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}} \\
        \intertext{We utilize \cref{fact:geometricSeriesFinite}, which gives a closed-form expression for a finite geometric series}
    % &=  8\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}-8 - 8\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}\\
    &<  16\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}-1} \\
    %  &=  8\paren*{\frac{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}^{\abs{\labelSpace}+1}-1+\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}}}}\\
          &<  16\paren*{\frac{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}+1}}{1-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}}}
          \shortintertext{Assume $\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}}} < \sfrac{1}{2}$}
          & <  32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}-\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}^{\abs{\labelSpace}^2+1}} \\
          &<32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} 
\end{align}
\end{proof}

Let us now discuss \cref{\thmTwo}.  Much like in \cref{\thmOne}, the bound we present here shows that our choice of fairness metric has no dependence on the accuracy of the underlying classifier.  The bound in $\cref{\thmTwo}$ exhibits a tighter dependence on $\abs{\labelSpace}$. Indeed the discrepancy between the bounds presented in \cref{\thmOne} and \cref{\thmTwo} becomes more significant as the number of labels $\abs{\labelSpace}$ increases.  

While the implications of both \cref{\thmOne,\thmTwo} are similar, the proof of $\cref{\thmTwo}$ is more intricate: we utilize the fact that $1=\sum_{\placeholder \in \labelSpace}\frac{\numSamples_{\marker,\placeholder}}{\numSamples_+}$ by invoking lemma \cref{lem:multinomialDistributionBound}.  We also invoke the Chernoff bound, \cref{thm:chernoffNice}, which can be far tighter than Hoeffding's Inequality.

Let us now devise a bound for the case that $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$. The bound follows from \cref{\thmTwo} and \cref{lem:pinsker}

\begin{corollary} \label{\corThmTwo}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} <32\paren*{\exp\paren*{-\frac{ \placeholder^2 \numSamples_{\min}}{12\abs{\labelSpace}^2}}} + \sqrt{2\ln\paren{2}\infdiv{\sampleDist_a}{\sampleDist_b}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{corollary}

Compared to the bounds presented in \cref{\thmOne} and \cref{\thmTwo}, the bound presented in \cref{\corThmTwo} provides a bound on our fairness metric when the distribution of labels depends on the group.




==> facct/src/old_stuff/5_lowerBounds.tex <==
!TeX root = ../note.tex

\section{Lower Bound}
Let us now develop a lower bound on $    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder}$. 

\begin{theorem}\label{thm:lowerBound}
Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  If $\placeholder > \sqrt{\frac{12\abs{\labelSpace}\ln\paren*{2}}{\numSamples_{\min}}}$, then we  have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
\end{theorem}


\begin{proof}  
\begin{align}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
    &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
        &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
        &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
                &\geq 1- \paren*{1-\exp\paren*{-2\placeholder^2\numSamples_{\min}}}\label{eq:postAbsIntersection}\\
                &= \exp\paren*{-2\placeholder^2\numSamples_{\min}}
\end{align}

Where to relate \cref{eq:preAbsIntersection} to \cref{eq:postAbsIntersection}, we used both Hoeffding's inequality (\cref{\hoeffding}) that for any non-negative $\placeholder$:
\begin{equation}
    \Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}} \leq \min \curlyBrace*{\Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}, \Pr{ \curlyBrace*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}>-\placeholder}}
\end{equation}
\end{proof}
Indeed, this lower bound is similar to that which is presented in \cref{\thmTwo}.  Notably, no $\abs{\labelSpace}$ term appears in the exponent. Note this lower bound is tightest when $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  A sharper bound for the case in which $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq \Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$ has not been developed.

{\color{blue}
CURRENTLY IN PROGRESS
\begin{theorem}\label{thm:lowerBound}
    Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$.  Furthermore, for all $\labelElement^{\marker} \in \labelSpace$ assume $\Pr[(\sampleProtected,\sampleUnprotected,\labelElement) \drawnFrom \labelElement]{\labelElement = \labelElement^{\marker}} \geq \placeholderScalar$ where $0 < \placeholderScalar < \frac{1}{\abs{\labelSpace}}$:
    \begin{equation}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \geq ??
    \end{equation}
    where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$
    \end{theorem}

    \begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &= 1-\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}\\
        &\geq 1-\Pr{\bigIntersection_{\labelElement \in \labelSpace} \curlyBrace*{\abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}}<\placeholder}}\\
            &\geq 1-\Pr{\bigIntersection_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}} \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}\\
            &\geq 1- \min_{\paren*{\sampleProtected,\labelElement} \in \paren*{\sampleSpace_{\protectedIndex},\labelSpace}}\curlyBrace*{\Pr{ \curlyBrace*{\abs*{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}-\E{\frac{\numSamples_{\sampleProtected,\labelElement}}{\numSamples_{\sampleProtected}}}}<\placeholder}}}\label{eq:preAbsIntersection}\\
            &\geq 1- \paren*{1-\exp\paren*{-\frac{\numSamples\placeholder^2}{2\paren*{1-\placeholderScalar\paren*{\abs{\labelSpace}-1}}\paren*{\placeholderScalar\paren*{\abs{\labelSpace}-1}} + \frac{2\placeholder}{3}}}}\\
    \end{align}
}

==> facct/src/old_stuff/6_LossFunctions.tex <==
%!TeX root = ../note.tex
\section{Fairness and (Un-)Bounded Loss Functions}

In \cref{sec:ballsAndBins}, we examined fairness in the context of counting.  Let us now compare examine fairness in the context of positive-valued loss functions.  Let $\loss$ be a  positive-valued loss function, that is $\loss : \sampleSpace \times \labelSpace \to (0,\infty)$.

Let $\lossContribution_{\groupA}$ denote the total loss contribution from group $\groupA$

That is
 
\begin{equation}
    \lossContribution_{\evalutationData,\groupA} \definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)
\end{equation}

Similarly, we define the loss contribution from the group $\groupA$, label $\labelElement$ pair:

\begin{equation}
    \lossContribution_{\evalutationData,\groupA,\labelElement} \definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
\end{equation}

% \begin{theorem}\label{\thmOne}
%     Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, we have:
%     \begin{equation}
%         \Pr{\sum_{\labelElement \in \labelSpace}\abs{\lossContribution_{\evalutationData,\groupA,\labelElement} -\lossContribution_{\evalutationData,\groupB,\labelElement}} > \placeholder} \leq 2\abs{\labelSpace}\exp\paren*{-\min_{\labelElement,\in \labelSpace} \curlyBrace*{\min_{\marker \in \set{+,-}} \frac{\numSamples_{\marker,\labelElement}\placeholder^2}{\abs{\labelSpace}}}}
%     \end{equation}
    
%     \end{theorem}


Our interest lies in bounding

\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder}
\end{equation}

Note that for all labels $\labelElement \in \labelSpace$, we have $0<\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}<1$. Furthermore, we know $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$
  
% In particular, for any $\labelElement \in \labelSpace$, we have $0 \leq \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} \leq 1$.  Furthermore, we have $1=\sum_{\labelElement \in \labelSpace}\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}$.  These facts allow us to provide tight bounds on $ \Pr{\sum_{\labelElement \in \labelSpace}\abs{ \frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\labelElement}} > \placeholder} $


\begin{align}
        \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder} + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder}  
\end{align}

\begin{align}
    \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x=\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \cdot e^{tx} \differential x
\end{align}



Let us upper-bound the variance of such a random variable.

\begin{align}
    \variance\bracket*{X} &= \E{X^2} - \E{X}^2 \\
    &\leq  \E{X^2} \\
    &= \int_{0}^{1}\probabilityDensityFunction_X\paren*{{x}} \cdot x^2 \differential x \\
    &\leq \E{X}
\end{align}

\begin{theorem}[Bhatia-Davis Inequality]
    Let $X$ be a random variable.  $X$ is bounded between $0$ and $1$, i.e. $X \in [0,1]$.  Then
    \begin{equation}
        \variance(X) \leq \paren*{1-\E{X}}\paren*{\E{X}}
    \end{equation}
\end{theorem}

\begin{theorem}[Bernstein Inequality]
    Suppose $
\placeholderRandomVariable_1,\dotsc,\placeholderRandomVariable_\placeholderCount$ are i.i.d. random variables with zero mean.  If for all $i$, $\abs{\placeholderRandomVariable_i} < \scalarBound$, then for all $\placeholderCount > 0$

\begin{equation}
    \Pr{\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\placeholderRandomVariable_i > \placeholder} \leq \exp\paren*{-\frac{\placeholderCount\placeholder^2}{2\variance\paren*{\placeholderRandomVariable} + \frac{2\scalarBound \placeholder}{3} }}
\end{equation}

\end{theorem}

\begin{theorem}\label{thm:UnboundedLossFairnessUB}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
    \end{equation}
    where \begin{align}
        \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
        \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
    \end{align}
    \end{theorem}
\begin{proof}
Without loss of generality, we assume that $i \in \set{1,\dotsc,\abs{\labelSpace}}$, we have $ \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \geq \dotsc \geq  \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_{\abs{\labelSpace}}}}{\lossContribution_{\evalutationData,\groupA}}}$, then we know $\E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupA}}} \leq \frac{1}{i}$


\begin{align}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} &\leq \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \placeholder/2} + \Pr{\sum_{i = 1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \placeholder/2} \\
    &\leq \sum_{i = 1}^{\abs{\labelSpace}} \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{\abs*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\ 
    % \begin{split}\leq \sum_{\labelElement \in \labelSpace} \brparen*{\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
    %      \qquad \qquad+\Pr{{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \E{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}} + \Pr{{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}} - \E{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}} \leq -\frac{\placeholder}{2\abs{\labelSpace}}}}
    % \end{split}\\
   &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} + \frac{\placeholder}{6\abs{\labelSpace}}}}}\label{eq:theoremFollowsFromHere}
   \intertext{We now invoke the Bhatia-Davis Inequality in combination with \cref{lem:multinomialDistributionBound}}
   &\leq \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}-\frac{1}{i^2}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &< \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}} + \frac{\placeholder}{6\abs{\labelSpace}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\paren*{\frac{1}{i}}  + \frac{\placeholder}{6\abs{\labelSpace}}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} + \frac{1}{6}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}  + \frac{1}{6}}}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}}}}+ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder}{8\abs*{\labelSpace}}}{2\frac{\abs{\labelSpace}}{\placeholder}\paren*{\frac{1}{i}} }}} \\
   &= \sum_{i = 2}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot i\cdot\placeholder^2}{16\abs*{\labelSpace}^2}}} \\
    \begin{split}\leq 2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
+2\paren*{\frac{1}{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i} \cdot \frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
   \end{split}\\
%    \begin{split}\leq 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }\\
%     +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} -\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}} }
%        \end{split} \\
%        \begin{split}= 2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
%         +2\paren*{\frac{\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}\paren*{1-1 + \exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}} }{1-\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
%            \end{split} \\
           \begin{split}= 2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i} \cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}\\
            +2\paren*{\frac{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }{1-\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}}}
               \end{split} \\
               \intertext{Assume $\frac{1}{2}\geq\exp\paren*{-\frac{\placeholder^2}{16\abs*{\labelSpace}^2}}$}
              &\leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }\\
    \end{align}
\end{proof}

\begin{corollary}
    Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
    \begin{equation}
    \Pr{\sum_{i=1}^{\abs{\labelSpace}} \abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_i}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}} \geq \placeholder} \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } +  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
    \end{equation}
\end{corollary}




% On sub-Gaussianity of random variables:

% \begin{definition}
%     Let $\placeholderRandomVariable$ be a random variable with expectation $\E{\placeholderRandomVariable}$.  If $\placeholderRandomVariable \drawnFrom \subGaussian(\proxyStandardDeviation^2)$, then for any $t > 0$
%     \begin{align}
%         \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} > t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}} &\text{and}&& \Pr{\placeholderRandomVariable-\E{\placeholderRandomVariable} < -   t} &\leq \exp\paren*{-\frac{t^2}{2\proxyStandardDeviation^2}}
%     \end{align}

% \end{definition}

% \subsection{Does the Bhatia-Davis bound on variance also a bound on proxy-variance?}

% Let $X$ be a random variable bounded between $0$ and $1$.

% \begin{align}
%     \Pr{\placeholderRandomVariable = 1} =  \Pr{\placeholderRandomVariable -\E{\placeholderRandomVariable} > 1-\E{\placeholderRandomVariable}} \leq \E{X}
% \end{align}

% Now we compare $\E{\placeholderRandomVariable}$ with $\exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}}$

% \begin{align}
%     \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\proxyStandardDeviation^2}} &\leq \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}^2}{2\E{\placeholderRandomVariable}\paren*{1-\E{\placeholderRandomVariable}}}} \\
%     &= \exp\paren*{-\frac{\paren*{1-\E{\placeholderRandomVariable}}}{2\E{\placeholderRandomVariable}}} \\
%     &= \exp\paren*{\frac{\E{\placeholderRandomVariable}-1}{2\E{\placeholderRandomVariable}}} \\
%     &=\exp\paren*{\frac{1}{2}}\exp\paren*{-\frac{1}{2\E{\placeholderRandomVariable}}}\\
% \end{align}     

==> facct/src/old_stuff/7_lossFunctionDifference.tex <==
%!TeX root = ../note.tex
\section{The Weakness of Simple Ratios}

The ratio-type fairness bounds developed in the previous section are informative to fairness, their weakness is demonstrated in the following example:

\begin{example}
     Suppose for each $\labelElement \in \labelSpace$, $\lossContribution_{\evalutationData,\groupA,\labelElement}$ and $\lossContribution_{\evalutationData,\groupB,\labelElement}$ are positive-valued random variables, and $\placeholderScalar \neq 1$ is a positive-valued real number.  Given $\lossContribution_{\evalutationData,\groupA,\labelElement} = \placeholderScalar\lossContribution_{\evalutationData,\groupB,\labelElement}$, we see that $ 0=\abs*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{\lossContribution_{\evalutationData,\groupA}} - \frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{\lossContribution_{\evalutationData,\groupB}}}$.  Our ratio based fairness metric suppresses the fact that when $\placeholderScalar > 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} > \lossContribution_{\evalutationData,\groupB,\labelElement}$, and when $\placeholderScalar < 1$, $\lossContribution_{\evalutationData,\groupA,\labelElement} < \lossContribution_{\evalutationData,\groupB,\labelElement}$.  We conclude that while a naive ratio-based fairness metric is informative, it suppresses differences between total loss contributions among groups.
\end{example} 

Hence, it is useful to capture in our fairness metric differences between total loss contributions among groups AND any discrepancy in ratios which the  naive ratio-based fairness metric captures.  Therefore, we consider the following fairness metric:


\begin{theorem}\label{thm:LossFunctionDifference}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=a}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and loss function positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }
     \end{equation}
     where \begin{align}
         \lossContribution_{\evalutationData,\groupA} &\definedAs \sum_{\paren*{\sample,\labelElement} \in \evalutationData \given \sampleProtected = \groupA} \loss(\sample,\labelElement)& \text{and}&&
         \lossContribution_{\evalutationData,\groupA,\labelElement} &\definedAs \sum_{\paren*{\sample,\labelElement^{\marker}} \in \evalutationData \given \sampleProtected = \groupA, \labelElement^{\marker} = \labelElement} \loss(\sample,\labelElement^{\marker})
     \end{align}
     \end{theorem}
\begin{proof}
\begin{align}
     \begin{split}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} 
     &\leq \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          & + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split} \\
     \begin{split}
          &\leq \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}} \\
          & + \sum_{\labelElement \in \labelSpace} \Pr{\abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2\abs{\labelSpace}}}
     \end{split} \\
     \begin{split}
     &\leq \sum_{i = 1}^{\abs{\labelSpace}} \brparen*{ 2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}} \\
     &+2\exp\paren*{-\frac{\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}}{\cdot\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} + \frac{\placeholder}{6\abs{\labelSpace}}}}}
     \end{split}
\end{align}
Since $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$ and  $\variance\paren*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \leq \variance\paren*{\frac{\lossContribution_{\evalutationData,\groupB,\labelElement_i}}{\lossContribution_{\evalutationData,\groupB}}}$, the the rest of the proof is identical to the proof of \cref{thm:UnboundedLossFairnessUB} from equation \cref{eq:theoremFollowsFromHere} to end.
\end{proof}

\begin{corollary}
     Given a training set $\evaluationData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{a,b}$ , $\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=a}\neq\Pr{\loss(\sampleUnprotected,\labelElement) \given \sampleProtected=b}$, and positive-valued loss function $\loss$, we have:
     \begin{equation}
          \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}  \leq 4{\exp\paren*{-\numSamples_{\evalutationData,\groupA,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} } + 4{\exp\paren*{-\numSamples_{\evalutationData,\groupB,\labelElement_i}\cdot\frac{\placeholder^2}{8\abs*{\labelSpace}^2}} }+  \sqrt{2\ln\paren{2}\infdiv{\sampleDist_{\loss_\groupA}}{\sampleDist_{\loss_\groupB}}}
     \end{equation}
 \end{corollary}

\hrule

Given the weakness of such naive ratio-based fairness metrics, we analyze a fairness metric which has utility in when loss is unbounded -- and avoids the pitfall of the fairness metric in the above example.  We consider 

\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}


We recognize that the above quantity is bounded by \begin{align}
     \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} &=  \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}}},\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{\paren*{\frac{1}{\numSamples_{\groupA,\labelElement}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB,\labelElement}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}},
     \frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}} }
\end{align}

It is clear that both $\frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupA}} \leq 1$ and $\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupB}}  \leq 1$ are true, but what can we say about $     \frac{\numSamples_{\groupA,\labelElement}\cdot\lossContribution_{\evalutationData,\groupB,\labelElement}}{\numSamples_{\groupB}\cdot\lossContribution_{\evalutationData,\groupA}}$ and $
\frac{\numSamples_{\groupB,\labelElement}\cdot\lossContribution_{\evalutationData,\groupA,\labelElement}}{\numSamples_{\groupA}\cdot\lossContribution_{\evalutationData,\groupB}}$?

{\color{blue} The above function is not always easily interpretable}


\hrule
\begin{equation}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder}
\end{equation}

\begin{align}
     \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} &\leq \max\curlyBrace*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }, \frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \\
     &\leq \max\curlyBrace*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\lossContribution_{\evalutationData,\groupA} }},\frac{\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\lossContribution_{\evalutationData,\groupB} }}}
\end{align}

\begin{align}
     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}-\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }} \geq \placeholder} \leq 
     \begin{split}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}} \\
          + \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} } - \E{\frac{\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB,\labelElement}}{{\frac{1}{\numSamples_{\groupA}}\lossContribution_{\evalutationData,\groupA}+\frac{1}{\numSamples_{\groupB}}\lossContribution_{\evalutationData,\groupB}} }}}  \geq \frac{\placeholder}{2}}
     \end{split}
\end{align}



\hrule


Let us now consider $\max_{\labelElement_1,\labelElement_2 \in \labelSpace} \abs*{\log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_1}}{\lossContribution_{\evalutationData,\groupB,\labelElement_1}}} - \log\paren*{\frac{\lossContribution_{\evalutationData,\groupA,\labelElement_2}}{\lossContribution_{\evalutationData,\groupB,\labelElement_2}}} }$

Suppose the distribution of losses is identical for both group $\groupA$ and group $\groupB$




==> facct/src/old_stuff/__latexindent_temp.tex <==
!TeX root = ../note.tex
\section{Boosting and Fairness}

We now consider the multiclass boosting framework from Huang et al \cite{huang2018learning} in the context of fairness.
 

Trivial Bound[Bad]


\begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
\begin{equation}
    \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{equation}
where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

\end{theorem}

\begin{proof}
\begin{align}
\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
&\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
\end{align}
\end{proof}

A better bound...

Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


\begin{lemma}
    Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
    \begin{equation}
        \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
    \end{equation}
\end{lemma}

Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  That is, we investigate 
\begin{equation}\Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\sample \in \unlabeledTrainingData \given \sampleProtected \in \groupA}\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} }{\groupWeight_{\groupA}}-\frac{\numSamples_{-,\labelElement}}{\groupWeight_{\groupB}}} > \placeholder}\end{equation}

where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$


\begin{align}
123
\end{align}
% \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> facct/src/old_stuff/old_background.tex <==
% !TeX root = ../note.tex


\section{Background}


% \subsection{Notation and Definitions}

% Within thI is paper, we adopt the following notational conventions:

We consider a setting where we have an input set $\sampleSpace \subseteq \realNumbers^{\dimension}$ and a label set $\labelSpace$.  A sequence of examples is denoted as $\trainingData{} \subseteq \sampleSpace \times \labelSpace{}$ and contains the $\numSamples$ examples which constitute the population group.

Let $\Gamma_{\trainingData} = \set{\group_1,\dotsc,\group_{\abs{\Gamma}}}$ be a finite collection of subsets of $\trainingData$, heretoforth refered to as \emph{population subgroups}.  We follow the lead of existing multicalibration literature and assume population groups may be overlapping \cite{shabat2020sample,hebert2017calibration}.  $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  Our setting is that of binary classification: $\labelSpace = \left\{\pm 1\right\}$.  Since the labels in $\labelSpace$ are discrete, we also have $\Lambda = \left\{\pm 1\right\}$.


We now discuss our notation population subgroups: Given set of examples $\trainingData$ which will be clear from context, For each group $\group \in \Gamma_\trainingData$, $\left|\trainingData_{\group}\right|$ denotes the number of samples in $\trainingData$ within subgroup $\group$ and $\left|\trainingData_{(\group,\interval)}\right|$ denotes the number of samples in $\trainingData$ within category $(\group,\interval)$

% We now discuss the Poisson Process from which population groups are constructed:

% Samples belonging to each category $\interestingCategory \in \listInterestingCategories$ arrive in the population according to a Poisson Process with rate $\poissonRate_{\interestingCategory}$.  In this paper, we will assume $1 = \sum_{\interestingCategory \in \listInterestingCategories} \poissonRate_{\interestingCategory}$.  We denote by $\poissonRate_{\min}$, the minimum rate over over all categories, that is $\poissonRate_{\min} = \min_{\interestingCategory \in \listInterestingCategories}\poissonRate_{\interestingCategory}$

% We consider two stopping conditions:

% \begin{enumerate}
%     \item The Poisson process stops when there are exactly $\numSamples$ arrivals.
%     \item The Poisson process stops after running for $\period$ time.
% \end{enumerate}



% As necessary, subscripts will be used when enumerating training data; it may be expedient to write $\trainingData{}\definedAs \set{(\sample_1,\labelElement_1), \hdots, (\sample_{\numSamples},\labelElement_{\numSamples})}$. Let $\hypothesisClass$ be a hypothesis class from which a deterministic prediction rule, $\hyp : \sampleSpace \to \labelSpace$ is selected. For example, in a binary classification setting, a hypothesis class $\hypothesisClass$ which appears frequently in literature is the set of non-homogeneous linear classifiers in $\realNumbers^\dimension$, i.e. classifiers of the form $\hyp(\sample) = \sgn\set{\vec{w}^{\transpose}\sample + b}$ where $\vec{w} \in \realNumbers^{\dimension},b\in\realNumbers$. $\positiveIntegers$ denotes the set of positive integers.  

A \emph{protected} feature is defined to be a feature to which our learner is blind, but is of interest to a meta-learner.  Without loss of generality, we assume the population group, $\group$, is determined by the value of that protected feature. 
 
% Let $\Gamma = \set{U_1,\dotsc,U_{\abs{\Gamma}}}$ be a finite collection of population groups.  We break from a portion of multicalibration literature in which population groups may be overlapping \cite{shabat2020sample,hebert2017calibration} and instead follow the convention of Pleiss et al. \cite{pleiss2017fairness,kleinberg2016inherent}: we assume the groups to be mutually exclusive.   $\Lambda$ is a partition of $\labelSpace$ into a finite number of disjoint subsets.  The assumption of mutual exclusivity among population groups provides additional structure to the problem which we leverage when constructing our bounds. Namely, we know

% \begin{equation}
%    1 \geq \sum_{U \in \Gamma} \Pr[\sample \drawnFrom \sampleDist]{\sample \in U}
% \end{equation}






% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA}$ and $\numSamples_{\trainingData,\groupB}$ are calculated is clear from context, we instead write $\numSamples_{\groupA}$ and $\numSamples_{\groupB}$.

% Similarly, we denote by $\numSamples_{\trainingData,\groupA,\labelElement_i}$the number of samples in population with feature $\sampleProtected=\groupA$ and ground truth label $y=\labelElement_i \in \labelSpace$.  $\numSamples_{\trainingData,\groupB,\labelElement_i}$ denotes the number of samples in population with feature $\sampleProtected=\groupB$ and ground truth label $y=\labelElement_i$ where $\labelElement_i \in \labelSpace$.  That is, 

% \begin{align}
%     \numSamples_{\trainingData,\groupA,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupA}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}} &  \numSamples_{\trainingData,\groupB,\labelElement_i} &\definedAs \sum_{\paren{\sampleElement_{\protectedIndex},\sampleElement_{\unprotectedIndices},\labelElement} \in \trainingData{}} \indicatorFunction\bracket*{{\sampleProtected=\groupB}} \cdot  \indicatorFunction\bracket*{{\labelElement = \labelElement_i}}
% \end{align}

% When the i.i.d. sample from which $\numSamples_{\trainingData,\groupA,\labelElement_i}$ and $\numSamples_{\trainingData,\groupB,\labelElement_i}$ are calculated is clear from context, we instead write $\numSamples_{\groupA,\labelElement_i}$ and $\numSamples_{\groupB,\labelElement_i}$.

% % We abuse notation and take $\numSamples_{\marker,\placeholder}$ to mean $\numSamples_{\marker,\placeholder,\depth}$

% To characterize the performance of our classifiers, we will use both the emprical risk and the true risk:

% \begin{definition}
%   Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, training set $\trainingData{}$ and predictor $\hyp$, we denote the empirical risk as \begin{equation}
%       {\risk}_{\trainingData}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}} \loss\paren*{\hyp(\sample),\labelElement}
%   \end{equation}
% \end{definition}

% \begin{definition}
%     Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers$, sample distribution $\sampleDist$ and predictor $\hyp$, we denote the true risk as \begin{equation}
%         \risk_{\sampleDist}(\hyp) \definedAs \Ex_{(\sample,\labelElement)\drawnFrom \sampleDist}\left[{\loss\paren*{\hyp(\sample),\labelElement}}\right]
%     \end{equation}
%   \end{definition}

%   As true risk has a dependence on the unknown distribution $\sampleDist$, the exact value of the true risk is also unknown.  Hence, our characterization of classifier performance will be probabilistic bounds on the difference between true risk and empirical risk. That is, classifier performance will be characterized in the following manner:  Given a non-negative real number $\placeholder$, $\Pr{\abs{\risk_{\sampleDist}(\hyp)-\risk_{\trainingData}(\hyp)} \geq \placeholder} \leq \errorConfidence$ where $\errorConfidence$ is a real number between $0$ and $1$ which depends on $\placeholder$, the number of samples $\numSamples$ used to calculate the empirical risk, and other context dependent factors.

%   We will see that the the concentration of our fairness metric behaves in a manner similar to the way empirical risk concentrates about the true risk.

  We use several definitions from Shabat et al. \cite{shabat2020sample}, the first of which is the category:

  \begin{definition}[Category]
      A category is a pair $(\group,\interval)$ of a subgroup $\group \in \Gamma$ and an interval $I \in \Lambda$.  A category  $(\group,\interval)$ is interesting according to predictor $\hyp$ and parameters $\gamma, \psi \in (0,1]$ if $\PR_{\sample \drawnFrom \sampleDist}\left[{\sample \in \group} \right]\geq \gamma$ and  $\PR_{\sample \drawnFrom \sampleDist}\left[{\hyp\paren*{\sample} \in \interval \given \sample \in \group}\right] \geq \psi$.
  \end{definition}

%   \begin{remark}
%     Given an arrival occurs at time $t$, the probability it belongs to category $\interestingCategory$ is $\frac{\poissonRate_{\interestingCategory}}{\sum_{\interestingCategory'\in \listInterestingCategories} \poissonRate_{\interestingCategory'}}$
%   \end{remark}


We investigate how the empirical calibration error concentrates about the true multicalibration error:




  \begin{definition}[Calibration Error]
    Let $\sampleDist \subseteq \sampleSpace \times \labelSpace$ be a sample distribution and let  $(\group,\interval)$ be a category.  The calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to a category $(\group,\interval)$ is denoted $\calibrationError\paren*{\hyp,\group,\interval}$:
    \begin{dmath}
        \calibrationError\paren*{\hyp,\group,\interval} \definedAs \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[{\labelElement \given \sample \in \group, \hyp\paren*{\sample}\in \interval}\right] - \Ex_{\paren*{\sample,\labelElement}\drawnFrom\sampleDist}\left[\hyp\paren*{\sample} \given \sample \in \group, \hyp\paren*{\sample}\in \interval\right]
    \end{dmath}


\end{definition}

Put in words, the calibration error is the difference between the expectations of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.


\begin{definition}[Empirical Calibration Error]
    Let $\trainingData\drawnFrom\sampleDist^{\numSamples}$ be a training set of $\numSamples$ examples drawn i.i.d. from sample distribution $\sampleDist\subseteq \sampleSpace \times \labelSpace$ and let $(\group,\interval)$ be a category.  The empirical calibration error of a predictor $\hyp \in \hypothesisClass$ with respect to category $(\group,\interval)$ and sample $\trainingData$ is denoted $\empiricalCalibrationError\paren*{\hyp,\group,\interval,\trainingData}$
    \begin{dmath}
        \empiricalCalibrationError\paren*{\hyp,U,I,\trainingData} \definedAs \sum_{(\sample,\labelElement) \in \trainingData}\left\{\frac{\indicatorFunction\left[\sample \in \group, \hyp(\sample) \in \interval \right]}{\left|\trainingData_{(\group,\interval)}\right|}\times\left(\labelElement-\hyp(\sample)\right)\right\}
    \end{dmath}


\end{definition}

Intuitively, empirical calibration error captures the difference between the average, taken over samples in $\trainingData$, of $\labelElement$ and $\hyp\paren*{\sample}$, conditioned on samples from population group $\group$ which hypothesis $\hyp$ maps to values in $\interval$.



Lastly we define the Vapnik-Chervonenkis (VC) dimension \cite{vapnik1971uniform} and the Rademacher complexity \cite{bartlett2002rademacher}, two notions of function class expressiveness which are used in proving bounds multicalibration uniform convergence sample complexity bounds.

Existing state-of-the-art bounds on multicalibration uniform convergence depend on the VC dimension:

\begin{definition}[Vapnik-Chervonenkis (VC) dimension] Let $\hypothesisClass \subseteq \left\{0, 1\right\}^{\sampleSpace}$ be a binary hypothesis class.  A hypothesis class $\hypothesisClass$ shatters set $\placeholderSet = \left\{\sample_1,\dotsc,\sample_\numSamples\right\} \subseteq \sampleSpace$ if 
    \begin{dmath}
        \left|\left\{\hyp(\sample_1),\dotsc,\hyp(\sample_{\numSamples})\right\} : \hyp \in \hypothesisClass\right| = 2^\numSamples
    \end{dmath}

The VC-dimension of $\hypothesisClass$ is the maximal size of $\placeholderSet$ which shatters $\hypothesisClass$
\end{definition}

While the VC-dimension represents a seminal contribution to theoretical machine learning, it does limitations.  Notably, VC-dimension does not capture the generalization properties of the Radial Basis Function (RBF) Kernel.  

The Rademacher complexity is a notion of function class expressiveness.  Our sample complexity bound for multicalibration uniform convergence will depend on the Rademacher complexity and will be applicable to the RBF kernel:



\begin{definition}[Rademacher Complexity]
    The Rademacher complexity of a hypothesis class class $\hypothesisClass$ with respect to a sample $\trainingData$ is
\begin{equation}
    \rademacherComplexity_{\trainingData}\left(\hypothesisClass\right) \definedAs \frac{1}{\numSamples}\Ex_{\vec{\rademacherRV}}\left[\sup_{\hyp \in \mathcal{\hypothesisClass}}\sum_{i=1}^{\numSamples}\rademacherRV_i \hyp(\sample_i)\right]
    \end{equation}
    where sample $\trainingData \drawnFrom \sampleDist^{\numSamples}$ is a set of $\numSamples$ i.i.d. samples drawn from distribution $\sampleDist$ and $\vec{\rademacherRV} \definedAs \left[\rademacherRV_1,\dotsc,\rademacherRV_{\numSamples}\right]^\transpose$ is a vector of $\numSamples$ samples drawn i.i.d. from the uniform distribution over $\left\{\pm 1\right\}$
    \end{definition}

    Our goal is to determine a bound on the sample complexity, $\sampleComplexity_{\hypothesisClass}^{\multicalibration}(\errorConfidence,\errorTolerance,\gamma,\psi)$, of uniform convergence guarantees on multicalibration error.  That is, we wish to determine a bound on the number of samples neeeded to yield guarantees of the form:

\begin{dmath}
    \PR\left\{\forall \hyp \hiderel{\in} \hypothesisClass,\forall \group \hiderel{\in} \Gamma, \forall \predictionValue \hiderel{\in} \labelSpace \hiderel{:} \\
    \left|\calibrationError(\hyp,U,\left\{v\right\}) \hiderel{-} \hat{\calibrationError}(\hyp,U,\left\{v\right\},\trainingData) \right| \hiderel{\leq} \errorTolerance \right\} \geq 1-\errorConfidence
\end{dmath}

The state-of-the-art for such sample-complexity bounds was developed by Shabat et al. \cite{shabat2020sample}.  For a hypothesis class of VC-dimension $\graphDimension$ which we denote $\hypothesisClass_{\graphDimension}$, the authors claim the following multicalibration unfiform-convergence sample complexity bound:

\begin{dmath}
        \sampleComplexity_{\hypothesisClass_{\graphDimension}}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi) = \bigOh\left(\frac{\graphDimension + \log\left(\frac{\left|\Gamma\right|\left|\labelSpace\right|}{\errorConfidence}\right)}{\errorTolerance^2\psi^2\gamma}\right)
\end{dmath}

The VC-dimension is a notion of hypothesis class capacity which is independent from data.  As such, sample complexity bounds utilizing the VC dimension do not leverage any knowledge of the underlying data distribution.  On the other hand, Rademacher complexity does leverage information about the underlying data distribution, so we can surmise some sample complexity bounds which utilize Rademacher complexity will be more informative than those which leverage VC dimension.




% \begin{theorem}
%     Let $\placeholderFunction : [-1,\infty)$ be a function defined by $\placeholderFunction(\placeholder) \definedAs 2\frac{\paren*{1+\placeholder}\ln\paren*{1+\placeholder}-\placeholder}{\placeholder^2}$ and let $\placeholderRandomVariable \drawnFrom \PoissonDistribution\paren*{\poissonRate}$ for some parameter $\poissonRate > 0$.  Then for any $\placeholder > 0$, we have

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \geq \poissonRate + \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     \begin{equation}
%         \Pr{\placeholderRandomVariable \leq \poissonRate - \placeholder} \leq \exp\paren*{-\frac{\placeholder^2}{2\poissonRate}\placeholderFunction\paren*{-\frac{\placeholder}{\poissonRate}}}
%     \end{equation}

%     Lastly, for any $\placeholder > 0$, we have 

%     \begin{equation}
%         \Pr{\abs{\placeholderRandomVariable - \poissonRate} \geq  \placeholder} \leq 2\exp^{-\frac{\placeholder^2}{2\paren*{\poissonRate + \placeholder}}}
%     \end{equation}


% \end{theorem}




% \begin{definition}
%   Let $\trainingData_{\marker}$ be a subset of $\trainingData{}$.  Given a loss function $\loss: \labelSpace \times \labelSpace \to \realNumbers^+$ and predictor $\hyp$,
%   We define the empirical risk contribution of $\trainingData_{\marker}$ (denoted by $\empiricalRisk_{\trainingData_{\marker},\trainingData{}}$, as the amount of empirical risk $\trainingData_{\marker}$ contributes to the total empirical risk over the training data:
%   \begin{equation}
%       \empiricalRisk_{\trainingData_{\marker},\trainingData{}}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{(\sample,\labelElement) \in \trainingData{}}\set*{ \loss\paren*{\hyp(\sample),\labelElement}\cdot\indicatorFunction\bracket*{(\sample,\labelElement) \in \trainingData_{\marker}}}
%   \end{equation}
% % \end{definition}

% We also define notation specially adapted to our use of residual networks:

% For the rest of note let $\depth \ge 1$ be some integer. We consider binary classification
% where label is in $\{\pm 1\}$. We will consider a feature function that is a \emph{sequential composition}
% of $\depth$ feature transformations:

% \begin{equation}
%     \functionComposition(\sample) = (\function_{\depth} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1)(\sample),
% \end{equation}
% where $\function_t$ ($t \in \set{1,\dotsc,\depth}$) is some function. Note that $\function_t$ may not be a layer, but it can
% be a group of layers, or even some function over a group of layers. For example, in ResNet,
% $\function_t(z) = f_t(z) + z$ where $f_t$ is called a \emph{module} in ResNet, which is typically a convolutional neural network (CNN).
% The final binary classifier is determined by a size-conforming weight vector $\weights_T$,
% where the classification is determined as
% \begin{equation}
%     \sign(\weights_T^{\transpose}\functionComposition(\sample))
% \end{equation}
% We will use the notation $\function_{1:\depthIter}$ to mean the composition $\paren*{\function_{\depthIter} \composeOperator \function_{\depth-1}   \composeOperator \cdots  \composeOperator \function_1}(\sample)$.
% We further use the notation $g_\depthIter \definedAs G_{1:\depthIter}$ to mean the composition of the first $\depthIter$ feature transformations.
% We have now the following definitions.
% \begin{definition}[Weak Hypothesis]
%   Let $t \in [T]$. For a weight vector $\weights_t$, the \emph{weak hypothesis} at step $t$ is defined as
%   $$o_t(\sample) = \weights_t^{\transpose} g_t(\sample) = \weights_t^{\transpose} G_{1:t}(\sample).$$
%   Therefore $o_T$ is simply the final hypothesis $\weights_T^{\transpose}g_T(\sample) = \weights_T^{\transpose}F(\sample)$.
%   Define $o_0 \equiv 0$.
% \end{definition}
% \begin{definition}[Residual Hypothesis]
%   Let $t \in [T]$. For two fixed scalar $\alpha_t$ and $\alpha_{t+1}$,
%   we define \emph{residual hypothesis} between step $t$ and step $t+1$ as:
%   $$h_t(\sample) = \alpha_{\blockIter+1}\blockOutput_{\blockIter+1}(\sample) -  \alpha_{\blockIter}\blockOutput_{\blockIter}(\sample)$$
% \end{definition}
% Lastly, let $\BoostResNet{\boost}(\trainingData{},\depth)$ denote the $\depth$ residual network trained on training set $\trainingData{}$ as learned by the $\BoostResNet$ procedure given in Huang et al. \cite{huang2018learning}.

% \subsection{Related Results}

% The residual network, introduced in 2015 by He et al., captures the fundamental design principles underlying many of today's state-of-the-art image classifiers.  As is the case with many classes of deep networks, their performance in practice exceeds what theory is able to explain.  Furthermore, decisions made by deep networks are almost never human interpretable.  In an effort to close this gap between theory and practice while providing some degree of interpretability to deep networks, Huang et al. applied the framework of boosting to show that under certain mild conditions, the training error of a residual network exhibits exponential decay that has an explicit dependence on the depth of the network.

% todo: expand


% We begin our discussion of fairness with a motivational example.  Consider a  protected feature which has two possible values.  That is, $\sampleProtected \in \set{\groupA,\groupB}$ .  Assume the protected feature is probabilistically independent from both the label $\labelElement$ and the unprotected features $\sampleUnprotected$.  That is to say $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=+1}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=-1}$.  We do not require each protected group to be equally likely.  Suppose $\numSamples_+$ in training set $\trainingData$ are such that the value of their protected feature $\sampleProtected$  is $+1$. Given a classifier $\classifierPlaceholder \definedAs \BoostResNet(\depth,\protectedTrainingData)$, let us examine a particular choice of fairness metric, $\fairnessMetric\definedAs \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}(\hyp)-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}(\hyp)}$
% Because the protected feature is independent from both the label and the unprotected features, we have

% \begin{align}
%     \fairnessMetric = \abs*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData}-\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} &\leq \max \curlyBrace*{\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = +1}},\trainingData},\empiricalRisk_{\trainingData_{\curlyBrace{\sampleProtected = -1}},\trainingData}} \\ &=\max\curlyBrace*{\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = +1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2},\frac{\abs{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}{\numSamples}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}}\\
%     &= \frac{1}{\numSamples}\cdot \abs*{\max\set*{\abs*{\trainingData_{\curlyBrace{\sampleProtected = +1}}},\abs*{\trainingData_{\curlyBrace{\sampleProtected = -1}}}}}\exp\paren{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% From this, we see the difference in size of each protected group has a direct impact on which group contributes the most to training error.  This result is entirely unsurprising, but it motivates that simple metrics, such as the difference in loss, may not be the best way to measure fairness.

% We can see, for a given training set $\trainingData$, the value of fairness metric $\fairnessMetric$ has a dependence on the imbalance in population between the protected group and unprotected group, yet the total empirical risk over the training data remains constant, regardless of how individuals are assigned to the protected or unprotected group.


% \begin{theorem}[Theorem 2.8 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffLowerBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a>b\geq 1$ and $\placeholderScalar \geq 2$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} > \frac{1}{\sqrt{2\pi}}\exp\paren*{b-\frac{1}{8\placeholderScalar}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\left(\placeholderScalar-1\right)+1 }}{(a-b)^{\paren*{a-b}\paren*{\placeholderScalar-1}-b+1}b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}


% \begin{theorem}[Theorem 2.6 from Stanica \cite{stanica2001good}]\label{thm:Stanica_binomialCoeffUpperBound}
%     Let $a,b,\placeholderScalar$ be positive integers such that $a\geq b\geq 1$ and $\placeholderScalar \geq 1$.  Then the following is true:
%     \begin{equation}
%         \binom{a\placeholderScalar}{b\placeholderScalar} < \frac{1}{\sqrt{2\pi}}\placeholderScalar^{-\frac{1}{2}}\frac{a^{a\placeholderScalar + \frac{1}{2}}}{\paren*{a-b}^{\paren*{a-b}\placeholderScalar + \frac{1}{2}} b^{b\placeholderScalar + \frac{1}{2}}}
%     \end{equation}
% \end{theorem}

==> facct/src/old_stuff/old_proofs_svm.tex <==
\section{Proof of \cref{thm:OurBoundSVM}}
\begin{proof}
\begin{dgroup}
   \begin{dmath}
   \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \geq \errorTolerance \right] = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\labelElement -\hyp\left(\sample\right) \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\left(\labelElement_i-\hyp(\sample_i)\right)\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{When $\labelElement \in [0,1]$, we know the following about 0-1 loss: $\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right] \geq \labelElement - \hyp(\sample)$:}
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right) \right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Furthermore, the empirical margin loss is an upper-bound on the 0-1 loss: }
\begin{dmath}
   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| +  \underbrace{\left|\left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) - \sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\indicatorFunction\left[ \labelElement_i \hiderel{\neq} \hyp(\sample_i)\right]\right\}\right|}_{=0} \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\intertext{The margin $\margin$ is selected such that either $\labelElement_i\hyp(\sample_i) \geq \margin$ or $\labelElement_i\hyp(\sample_i) < 0$  }
\begin{dmath}
=\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance\right]
\end{dmath}
\begin{dmath}
   =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp}\PR\left[ \left|\risk_{U,I}\left(\hyp\right) - \hat{\risk}_{U,I}^{\margin}\left(\hyp\right)\right| \hiderel{\geq} \errorTolerance \right] 
\end{dmath}
\intertext{Substituting in $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, as per \cref{thm:CortesGeneralization}, we arrive at}:
\begin{dmath}
   \leq\sum_{\hyp \in \hypothesisClass}\sum_{(U,I) \in \listInterestingCategories_\hyp} \errorConfidence'
\end{dmath}
\begin{dmath}
   =2\left|\Gamma\right|\left|\hypothesisClass\right| \errorConfidence'
\end{dmath}
\end{dgroup}




Invoking \cref{thm:CortesGeneralization} with  $\errorTolerance = \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\frac{2}{\errorConfidence'}}{2\numSamples(\hyp,I,U,\trainingData)}}\right)$, where $\errorConfidence' = \frac{\errorConfidence}{2\left|\Gamma\right|\left|\hypothesisClass\right|}$ completes the proof.

\end{proof}

==> facct/src/old_stuff/old_svm_study.tex <==
%!TeX root = ../note.tex

\section{Kernels and Fairness}
With notation defined, we now derive our tight multicalibration uniform convergence bounds on kernelized predictors which includes the Kernel SVM, and RELU networks with one hidden layer.



% \begin{definition} Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$.  We say that $\sampleDist$ is separable with $\paren*{\margin,\scalarBound}$-margin if there exists $\paren*{\weights^{\opt},\placeholderScalar^{\opt}}$ such that $\norm{\weights^{\opt}}=1$ and such that with probability $1$ over the choice of $\paren*{\sample,\labelElement}\drawnFrom \sampleDist$, we have that $\labelElement\paren*{\dotProduct{\weights^{\opt}}{\sample}+\placeholderScalar^{\opt}} \geq \margin$ and $\norm{\sample}\leq \scalarBound$.  Similarly, we say that $\sampleDist$ is separable with a $(\margin,\scalarBound)$-margin using a homogenous halfspace if the preceding holds with a halfspace of the form $\paren*{\weights^{\opt},0}$
% \end{definition}
 
% \begin{theorem} 
%   Let $\sampleDist$ be a distribution of $\realNumbers^{\dimension} \times \set{\pm 1}$ that satisfies the $\paren*{\margin,\scalarBound}$ separability with margin assumption using a homogenous halfspace.  Then with probability of at least $1-\errorConfidence$ over the choice of a training set of size $\numSamples$, the zero-one error of the output of a Hard-SVM is at most 
%   \begin{equation}
%       \sqrt{\frac{4 \paren*{\scalarBound/\margin}^2}{\numSamples}} + \sqrt{\frac{2\log \paren*{2/\errorConfidence}}{\numSamples}}
%   \end{equation}
% \end{theorem}
 

We take our description of Kernelized  classifiers from Cortes et al \cite{cortes2010generalization}.
For any kernel function $\kernelFunction$, we denote by $\kernelMapping_{\kernelFunction} : \sampleSpace \to \hilbertSpace_{\kernelFunction}$ the feature mapping $\sampleSpace$ to the reproducing kernel Hilbert space $\hilbertSpace_{\kernelFunction}$ induced by $\kernelFunction$.

We focus on a particular class classifiers, $\hypothesisClass_{\placeholderCount}^{\q}$ the set of non-negative combinations of $\placeholderCount \geq 1$ kernels $\kernelFunction_1,\dotsc,\kernelFunction_{\placeholderCount}$ with the mixture weights obeying an $\ell_{\q}$ constraint:

\begin{equation}
   \hypothesisClass_{\placeholderCount}^{\q} \definedAs \set*{\sample \mapsto \weights^{\transpose}{}\kernelMapping_{\kernelFunction}(\sample) : \kernelFunction = \sum_{i=1}^\placeholderCount \placeholderScalar_i\kernelFunction_i : \norm{\vec{\placeholderScalar}}_{\q} = 1, \vec{\placeholderScalar} \geq 0, \norm{\weights} \leq 1,}
\end{equation}

Cortes et al. \cite{cortes2010generalization} developed several generalization bounds for kernelized predictors.  We will utilize one such bound, \cref{thm:CortesGeneralization}, to bound multicalibration gap over kernelized predictors.

\begin{theorem}[Theorem 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:cortesRademacher}
   Let $\placeholderCount > 1$ and assume that $\kernelFunction(\sample,\sample)\leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and $i \in [1,\placeholderCount]$.  Then for any sample $\trainingData$ of size $\numSamples$, the Rademacher complexity of the hypothesis set $\hypothesisClass_\placeholderCount^1$ can be bounded as follows
   \begin{dmath}
      \rademacherComplexity_{\trainingData}(\hypothesisClass_\placeholderCount^1) \leq \sqrt{\frac{23e\lceil\log\placeholderCount\rceil\scalarBound^2}{22\numSamples}}
   \end{dmath}
\end{theorem}

\begin{theorem}[Corollary 2 from Cortes et al. \cite{cortes2010generalization}]\label{thm:CortesGeneralization}
   Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction_i\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$ and for all $i \in \set{1,\dotsc,\placeholderCount}$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$ and any $\hyp \in \hypothesisClass_{\placeholderCount}^{\q}$,, we have
   \begin{equation}
      \trueRisk(\hyp) \leq \empiricalRisk_{\margin}(\hyp) + 4\sqrt{\frac{23 \qDual \scalarBound^2}{22\margin^2\numSamples}} + 3\sqrt{\frac{\log\paren*{\frac{2}{\errorConfidence}}}{2\numSamples}}
   \end{equation}
   where $\empiricalRisk_{\margin}(\hyp) \definedAs \frac{1}{\numSamples}\sum_{i=1}^{\numSamples}\min\curlyBrace*{1,\bracket*{1-\labelElement_i\hyp\paren*{\sample_i}/\margin}_{+}}$ is the empirical margin loss.
\end{theorem}

The above bound requires our kernel be a non-negative combination of a fixed set of $\placeholderCount$ kernels where $\placeholderCount > 1$.  As such, our proofs will leverage a an all-zeros size-conforming `dummy'' kernel.

The last piece of the puzzle, in order to yield Rademacher complexity based sample complexity bounds for multicalibration uniform convergence, is to draw analogues of two  Graph-dimension based lemmas \cref{lem:shabat24,lem:shabat25} from Shabat et al.  We arrive at our analgoues of Shabat's lemmas by upon invokation of \cref{thm:shalevRademacherImproved}:
\begin{lemma}[Analogue of Lemma 24 from \cite{shabat2020sample}]\label{lem:shabat24analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\kernelFunction(\sample,\sample) \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}

\begin{proof}
% \small 
   Our proof strategy is to invoke \cref{thm:shalevRademacherImproved} to yield an expression for $\errorTolerance$ in terms of Rademacher complexity.  We perform algebraic manipulation:
   \begin{dgroup}
      \begin{dmath}
         \errorTolerance = 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) + 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
   
      \begin{dmath}
         \errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData) = 4c\sqrt{\frac{2\ln\left(4/\errorConfidence\right)}{\placeholderCount}}
      \end{dmath}
      \begin{dmath}
         \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 = \frac{32c^2\log\left(4/\errorConfidence\right)}{\placeholderCount}
      \end{dmath}
      \begin{dmath}
         \numSamples_U = \frac{32c^2\ln\left(4/\errorConfidence\right)}{  \left(\errorTolerance - 2\rademacherComplexity(\loss \circ \hypothesisClass \circ \trainingData)\right)^2 }
      \end{dmath}
      \intertext{Substituting in for rademacher Complexity of a kernelized classifier \cref{thm:cortesRademacher}, we see that the following inequality implies the previous inequality, we have}
      \begin{dmath}
         \numSamples_U \geq \frac{32\log\left(\frac{4}{\errorConfidence}\right)}{  \left(\epsilon - 2\sqrt{\frac{23e\scalarBound^2}{22\numSamples_U}}\right)^2 }
      \end{dmath}
     \intertext{And now algebra:}
      \begin{dmath}
         \left(\epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2 \geq 32\log\left(\frac{4}{\errorConfidence}\right)
      \end{dmath}
      \begin{dmath}
         \epsilon\sqrt{\numSamples_U} - 2\sqrt{\frac{23e\scalarBound^2}{22}} \geq \sqrt{32\log\left(\frac{4}{\errorConfidence}\right)}
      \end{dmath}
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{\left(\sqrt{32\log\left(\frac{4}{\errorConfidence}\right)} + 2\sqrt{\frac{23e\scalarBound^2}{22}}\right)^2}{\epsilon^2}
      \end{dmath}
      \intertext{The last step is simplifying \eqref{eq:NUSampleComplexity}.  \Eqref{eq:NUSampleComplexity} holds true when   }
      \begin{dmath}\label{eq:NUSampleComplexity}
         \numSamples_U  \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}
      \end{dmath}
   \end{dgroup}
   which concludes the proof
\end{proof}


\begin{lemma}\label{lem:shabat25analogue}
   Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a predictor class with $\dimension_{\graphDimension}(\hypothesisClass) \leq \dimension$ Let $\predictionValue \in \labelSpace$ be a prediction value and let $U \in \sampleSpace$ be a subpopulation.  Then there exists some constant $C \in \realNumbers$ such that, for any distribution $\sampleDist$ over $\sampleSpace \times \left\{0,1\right\}$ and any $\errorTolerance,\errorConfidence \in (0,1)$, if $\sampleDist_U$ is the induced distribution on $U \times \left\{0,1\right\}$ and $\trainingData = \left\{\sample_i,\labelElement_i\right\}_{i=1}^{\placeholderCount}$ is a random sample of $\numSamples_U \geq \frac{64\log\left(\frac{4}{\errorConfidence}\right) + 23\scalarBound^2}{\epsilon^2}$ examples drawn i.i.d. according to $\sampleDist_U$, then with probability at least $1-\errorConfidence$:
   \begin{dmath}
       \forall \hyp \in \hypothesisClass \hiderel{:} \left|\frac{1}{\placeholderCount}\sum_{i=1}^{\placeholderCount}\indicatorFunction\left[\hyp(\sample_i) \hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]  -\PR_{\sample \drawnFrom \sampleDist_U}\left[\hyp(\sample)\hiderel{=} \predictionValue,\labelElement\hiderel{=}1\right]\right| \hiderel{\leq} \errorTolerance
   \end{dmath}
\end{lemma}


With the above generalization bound for kernelized predictors in place, we will now bound their multicalibration gap with the following theorem:

\begin{theorem}
\label{thm:OurBoundSVM}
Let $\q,\qDual \geq 1$ with $\frac{1}{\q} + \frac{1}{\qDual} = 1$ and assume that $\qDual$ is an integer. Fix $\margin > 0$.  If $\kernelFunction\paren*{\sample,\sample} \leq \scalarBound^2$ for all $\sample \in \sampleSpace$.  Then for $\placeholderCount > 1$,  and any $\errorConfidence > 0$,  we have 
\small{
   \begin{dmath}
      \PR\left[\bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|\calibrationError\left(\hyp,U,I \right) - \empiricalCalibrationError\left(\hyp,U,I,\trainingData \right) \right| \leq \left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2\numSamples(\hyp,I,U,\trainingData)}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2\numSamples(\hyp,I,U,\trainingData)}}\right) \right] \hiderel{\geq} 1-\errorConfidence
   \end{dmath}
   }
\end{theorem}  
\begin{proof}[Proof Sketch]
The proof begins by bounding the probability that the calibration gap for any category $(U,I) \in \listInterestingCategories$ is not too large. Then, we take a bound over the 0-1 loss from the true calibration and empirical calibration, which gives a bound on difference between the true risk and marginal empirical risk.   The full proof is available in Appendix A.
\end{proof}

Using the bound on the multicalibration uniform convergence in \cref{thm:OurBoundSVM}, we can derive an upper bound on the sample complexity.  

\begin{corollary} The sample-complexity necessary for multicalibration uniform convergence in kernelized predictors is

\begin{dmath}
\numSamples\left({\errorConfidence,\errorTolerance,\gamma,\psi}\right) = \frac{1}{\errorTolerance^2 \gamma \psi}\left(4\sqrt{\frac{23\qDual\scalarBound^2}{22\margin^2}} + 3\sqrt{\frac{\log\left(\frac{4\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{2}}\right)^2 
=\bigOh\left(\frac{\frac{r\scalarBound^2}{\margin^2} + \log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\errorTolerance^2\gamma\psi}\right)
= \bigOh\left(\frac{{r\scalarBound^2}+ \margin^2\log\left(\frac{\left|\Gamma\right|\left|\hypothesisClass\right|}{\errorConfidence}\right)}{\margin^2\errorTolerance^2\gamma\psi}\right)
\end{dmath} 
\end{corollary}



This bound on the sample complexity exhibits a similar form as that of Shabat et al. The main differences, however, is that SVM-specific bound has direct dependency on the test-set margin and the kernel's sensitivity and does not depend on the graph dimension of the classifier. These differences imply that a classifier-agnostic bound for multi-calibration uniform convergence is unlikely to be effective in practice. Take for example the RBF kernel; this kernel has an infinite graph dimension but is bounded between 0 and 1. Our bound can provide a more meaningful sample complexity bound for group fairness.


Using this bound, we can present a bound on the sample complexity of two-layer RELU networks.



% \begin{dmath}
%   \leq\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\Ex_{\sampleDist}\left[\indicatorFunction\left[ \labelElement \hiderel{\neq} \hyp(\sample)\right] \hiderel{\given} \sample \hiderel{\in} U, \hyp(\sample) \hiderel{\in} I \right] - \left(\sum_{i=1}^{N}\left\{\frac{\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp(\sample_i) \hiderel{\in} I\right]}{\numSamples(\hyp,I,U,\trainingData)}\min\left\{1,\left[1-\frac{\labelElement_i \hyp(\sample_i)}{\margin}\right]_+ \right\}\right\}\right) \right| \hiderel{\geq} \errorTolerance' \right] 
% \end{dmath}

% \subsection{Failure of Multi-calibration uniform convergence}

% Inspired by the proof of failure for uniform convergence of Nagarajan et al. (Theorem 3.1 of \cite{nagarajan2019uniform}), we show the failure of multicalibration uniform convergence.   

% \begin{definition} 
%   The \emph{tightest algorithm-dependent multi-calibration uniform convergnce bound} with respect to loss $\loss$ is the smallest value $\errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$ for which there exists a set of sample sets $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ such that $\PR\left[\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}\right] \geq 1-\errorConfidence$ and if we define the space of hypotheses explored by $\learningAlgorithm$ on $\mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}$ as $\hypothesisClass_{\errorConfidence} \definedAs \union_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}} \hyp_{\trainingData} \subseteq \hypothesisClass$, the following holds: $\sup_{\trainingData \in \mathcal{S}_{\errorConfidence,\listInterestingCategories_{\hyp}}}\sup_{\hyp \in \hypothesisClass_{\errorConfidence}} \leq \errorTolerance_{\unifalg}(\numSamples,\errorConfidence,\listInterestingCategories)$
% \end{definition}



% \paragraph{Distribution $\placeholderDist$:} Each input $(\placeholder_1,\vec{\placeholder}_2,\vec{\placeholder}_3)$ is a $1+K+D$ dimensional vector where $\placeholder_1 \in \realNumbers$, $\vec{\placeholder}_2 \in \realNumbers^{K}$ and $\vec{\placeholder}_3 \in \realNumbers^{D}$.  $\vec{\mu} \in \realNumbers^{K}$ determines the centers of the classes.  THe label $\labelElement$ is drawn uniformly from $\left\{\pm 1\right\}$ and conditioned on $\labelElement$, we have $\vec{\placeholder}_1 = 2\labelElement\vec{\mu}$ while $\vec{\placeholder}_2$ is sampled independently from $\mathcal{N}(\vec{0}_{D},\frac{32}{D}\vec{I}_D)$


% \begin{theorem}
%   For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \left|\Gamma\right|\ln \sfrac{\numSamples}{\errorConfidence}, \left|\Gamma\right|\numSamples\ln\sfrac{1}{\errorTolerance}\right\}\right)$, there exists a category, $(U,I) \in \listInterestingCategories_{\hyp}$ for which $\errorTolerance_{\textrm{gen}}(\trainingData,U,I,\errorConfidence) \leq \errorTolerance$ while $\errorTolerance_{\unifalg}(\trainingData,U,I,\errorConfidence) \geq 1-\errorTolerance$. 
% \end{theorem}

% \begin{theorem}\label{thm:MansourFinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be a finite predictor class.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\gamma\psi}\right)
% \end{dmath}
% \end{theorem}


% \begin{theorem}\label{thm:MansourInfinite}
% Let $\hypothesisClass \subseteq \labelSpace^{\sampleSpace}$ be an infinite predictor class from domain $\sampleSpace$ to a discrete prediction set $\labelSpace$ with finite graph-dimension $\dimension_G(\hypothesisClass) \leq \dimension$.  Then $\hypothesisClass$ has the  multicalibration uniform convergence property with
% \begin{dmath}
% \numSamples_{\hypothesisClass}^{\multicalibration}(\errorTolerance,\errorConfidence,\gamma,\psi)= \bigOh\left(\frac{\dimension+ \log\left(\frac{\left|\Gamma \right|\left|\hypothesisClass \right|}{\errorConfidence\lambda}\right)}{\errorTolerance^2\psi^2\gamma}\right)
% \end{dmath}
% \end{theorem}

% We now compare our bound (\cref{thm:kernelSampleComplexity}) which applies in the binary classification setting, to prior bounds on multicalibration uniform convergence (\cref{thm:MansourFinite,thm:MansourInfinite}) with $\lambda$, a parameter which serves as a proxy for $\left|\labelSpace\right|$, to $2$:

% Whereas 



% \begin{theorem} For any $\errorTolerance,\errorConfidence > 0,\errorConfidence < \sfrac{1}{4}$, when $D = \bigOmega\left(\max\left\{\numSamples \ln \sfrac{\numSamples}{\errorConfidence}, \numSamples\ln\sfrac{2\abs{\Gamma}{\errorTolerance}}\right\}\right)$, $\greekScalar \in [0,1]$, the multi-calibration uniform convergence satisfies $\errorTolerance$
% \end{theorem}


% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\left|\left(\hat{\mu}_{\hyp}\left(\hyp,U,I,\trainingData \right)-\hat{\mu}_{\labelElement}\left(\hyp,U,I,\trainingData\right)\right)  \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right] =\PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \left(\hyp(\sample_i)-\labelElement_i  \right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       \leq \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\frac{1}{\numSamples(\hyp,I,U,\trainingData)}\left|\sum_{i=1}^{\numSamples}\indicatorFunction\left[\sample_i \hiderel{\in} U, \hyp\left( \sample_i \right) \hiderel{\in} I \right] \cdot \min\left(1,\left[1-\frac{\labelElement_i \hyp\left(\sample_i\right)}{\margin}\right]_+\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
%    \begin{dmath}
%       = \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp}\hat{\risk}_{\margin,U,I}\left(\hyp\right) \hiderel{\geq} \sfrac{\errorTolerance}{2} \right]
%    \end{dmath}
% \end{dgroup}

% \begin{dgroup}
%    \begin{dmath}
%       \PR\left[\bigUnion_{\hyp \in \hypothesisClass}\bigUnion_{(U,I) \in \listInterestingCategories_\hyp} \left|\hat{\mu}_{\labelElement}\left(\hyp,U,I\right)-{\mu}_{\labelElement}\left(\hyp,U,I\right) \right| \hiderel{\geq} \sfrac{\errorTolerance}{2}\right] 
%    \end{dmath}
% \end{dgroup}
% \begin{align}
%    \bigIntersection_{\hyp \in \hypothesisClass}\bigIntersection_{(U,I) \in \listInterestingCategories_\hyp} \left|{\calibrationError\left({\hyp,U,I}\right) - \empiricalCalibrationError\left({\hyp,U,I,\trainingData}\right)\right| \leq \errorTolerance}
% \end{align}

% \section{Boosting and Fairness}

% Let $\sampleInfNormUB \definedAs \E[\evaluationData \drawnFrom \sampleDist]{\max_{i}\norm{\sample_i}_\infty}$.  $\norm{\weights}_1 < \finalLinearClassifierOneNormUB  < \infty$

% \begin{theorem}[Generalization and Margin bound from Huang et al. \cite{huang2018learning}]
%    Given algorithm 1 from \cite{huang2018learning}, the fraction of training examples with margin at most $\margin$ is at most $\paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}$.  And the generalization error $\Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0}$ satisfies
%    \begin{align}
%     \Pr[\sampleDist]{\labelElement\functionComposition\paren{\sample} \leq 0} &\leq \paren*{1+\frac{2}{\frac{1}{\sqrt{\blockError_{\depth+1}}}-1}}^{\frac{\margin}{2}}\exp\paren*{-\frac{1}{2}\learningCondition^2\depth}\\ &+ \frac{4\finalLinearClassifierOneNormUB\sampleInfNormUB}{\margin}\sqrt{\frac{\log\paren*{2\dimension}}{2\numSamples}}\sum_{t=0}^{\depth}\weightsOneNormUB_t + \frac{2}{\margin}\sqrt{\frac{\log \depth}{\numSamples}} + \functionPlaceholder\paren*{\margin,\numSamples,\depth,\errorConfidence}
%    \end{align}
%    with probability at least $1-\errorConfidence$ for $\functionPlaceholder(\margin,\numSamples,\depth,\errorConfidence) \definedAs \sqrt{\ceil*{\frac{4}{\margin^2}\log\paren*{\frac{\margin^2 \numSamples}{\log \depth}}}\frac{\log \depth}{\numSamples} + \frac{\log \frac{2}{\errorConfidence}}{2\numSamples}}$
% \end{theorem}

% where $\weightsOneNormUB_t\definedAs \prod_{t'=0}^t2\weightsOneNormUB_{t',t'-1}$ and $\weightsOneNormUB_{t,t-1}$ is the upper bound on the $\ell_1$ norm of the weight vector connecting a neuron at layer $t$ with its preceding layer.

% THe above bound, of course, does not inform loss bounds similar to \cref{thm:LossFunctionDifference}.
 

% Trivial Bound[Bad]


% \begin{theorem}[Trivial Bound] \label{BoostingAndFairness}
% Consider a $\depth$-module telescoping sum boosting framework using algorithms 1 and 2 of $\cite{huang2018learning}$.  Given a training set $\trainingData{}$ over $\sampleSpace \times \labelSpace$ such that $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and $\labelSpace=\set{\labelElement_1,\labelElement_2}$. If the $\learningCondition$-learning condition holds, we have:
% \begin{equation}
%     \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} \leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{equation}
% where $\numSamples_{\min} = \min_{\labelElement \in \labelSpace, \sampleProtected \in \sampleSpace_1} \numSamples_{ \sampleProtected,\labelElement}$

% \end{theorem}

% \begin{proof}
% \begin{align}
% \Pr{\sum_{\labelElement \in \labelSpace} \abs*{\frac{\numSamples_{+,\labelElement}}{\numSamples_+}-\frac{\numSamples_{-,\labelElement}}{\numSamples_-}} > \placeholder} &\leq \sum_{g \in \set{\groupA,\groupB}} \Pr{\indicatorFunction\bracket*{\sum_{i=1}^{\numSamples_{\groupA}}\decisionFunction\paren*{\sum_{\blockIter} \hypothesisModule_{\blockIter}(\sampleUnprotected)} \neq \labelElement \given \sampleProtected = g} > \placeholder} \\
% &\leq \numSamples\exp\paren*{-\frac{1}{2}\depth\learningCondition^2}
% \end{align}
% \end{proof}

% A better bound...

% Suppose that for all $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$


% % \begin{lemma}
% %     Suppose that for all $\sample \in \trainingData$, $t \in \set{0,\dotsc,\depth}$, $\hypothesisModule_{\blockIter} \in \bracket*{-\scalarBound,\scalarBound}$, we have
% %     \begin{equation}
% %         \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{2\scalarBound}}\leq \boostDist_1(\sample) \leq  \frac{1}{1+ \paren*{\numSamples-1}\exp\paren*{-2\scalarBound}}
% %     \end{equation}
% % \end{lemma}

% Let us now consider the analogue of \cref{\thmOne}, but in the context of Boosting.  We assume  $\sampleSpace_1 = \set{\groupA,\groupB}$ and $\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupA}=\Pr{(\sampleUnprotected,\labelElement) \given \sampleProtected=\groupB}$ and proceed by bounding
% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{1-\indicatorFunctionInstance_{\labelElement^{\marker}}(\sample)}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}} \end{equation}
 
% where $\groupWeight_{\groupA} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupA} \boostDist_1\paren*{\sample}$ and $\groupWeight_{\groupB} \definedAs \sum_{\sample \in \trainingData \given \sampleProtected = \groupB} \boostDist_1\paren*{\sample}$,$\indicatorFunctionInstance_{\labelElement}\paren*{\sample} \definedAs\indicatorFunction\bracket*{\labelElement = \labelFunction\paren*{\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}} $  and $\labelFunction$ is a function which returns some $\labelElement \in \labelSpace$.  

% This quantity is bounded above by

% \begin{equation}\sum_{\labelElement \in \labelSpace} \abs*{\frac{\sum_{\paren*{\sample,\labelElement^{\marker}} \in \trainingData \given \sampleProtected= \groupA}\indicatorFunctionInstance_{\labelElement}(\sample)\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1(\sample)}{\groupWeight_{\groupA}}-\frac{\sum_{\paren*{\sample,\labelElement^{\marker}}\in \trainingData \given \sampleProtected = \groupB}\indicatorFunctionInstance_{\labelElement}\paren*{\sample}\paren*{\exp\paren*{-\labelElement^{\marker}\sum_{\blockIter}^{\depth}\hypothesisModule_{\blockIter}(\sample)}}\boostDist_1\paren*{\sample}}{\groupWeight_{\groupB}}}\end{equation}




% Hoeffding's inequality applies here, and yields a bound similar to the bound derived in \cref{\thmOne}.  Do sharper bounds apply?

% \begin{theorem}[Multiplicative Chernoff-Style Bound Distributions induced by Boosting]\label{thm:chernoffNice}
%     Suppose $\randomVariable_1,\dotsc,\randomVariable_{\placeholderCount}$ are i.i.d. random variables taking in values $\set{0,1}$.  Let $\bernoulliParameter = \E{\randomVariable}$ and $\relativeErrorTolerance > 0$ then
%     \begin{align}
%         \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \geq \paren{1+\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance\\
%              \Pr{\paren*{\sum_{i=1}^{\placeholderCount}\randomVariable_i} \leq \paren{1-\relativeErrorTolerance}\bernoulliParameter\placeholderCount} &\leq \exp\paren*{-\frac{\relativeErrorTolerance^2\bernoulliParameter\placeholderCount}{3}} && 0 \leq \relativeErrorTolerance \leq 1
%     \end{align}
%     \end{theorem}
% % \begin{align}
    
% \end{align}

   


% \begin{lemma}\label{lem:langfordCost}
% Consider a sample $\paren{\sample,\labelElement} \in \trainingData$. The optimal cost function under the exponential loss is \begin{equation}
%     \costMatrix^{\blockIter}_{\sample,\placeholder} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{lemma}

% The cost function described in \cref{lem:langfordCost} applies to individual samples in training data $\trainingData$--Our fairness metric on the other hand, relies on the label distribution of all samples in training data $\trainingData$, hence we consider the following cost function:

% \begin{definition}\label{lem:fairnessCost}
% Consider a sample $\paren{\sampleProtected,\sampleUnprotected, \labelElement} \in \trainingData$. Furthermore, let $\sampleSpace_1 = \set{a,b}$ We consider a fairness Cost Matrix \begin{equation}
%     \fairnessCostMatrix^{\blockIter}_{\labelElement,\labelElement^{\marker}} \definedAs \begin{cases}
%     \exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement}}  &\mbox{if } \labelElement \neq \placeholder\\
%     -\sum_{\labelElement^{\marker} \neq \labelElement}\exp\paren*{\hypothesisModuleSum{1}{\blockIter}\paren*{\sample}_{\placeholder}-\hypothesisModuleSum{1}{\blockIter}(\sample)_{\labelElement^{\marker}}}  &\mbox{if } \labelElement = \placeholder
%     \end{cases}
% \end{equation}
% where $\hypothesisModuleSum{i}{j}(\sample) \definedAs \sum_{\tau=i}^{j}\hyp_{\tau}(\sample)$
% \end{definition}

==> outline/essential/macros.tex <==
\usepackage{bm}
\usepackage{mathtools}
\usepackage{xfrac}
\usepackage{bbm}
\usepackage{cleveref}
\usepackage{tikz}
% \usepackage{breqn}
\usepackage{amsmath,amsfonts,bm,amssymb}

\newcommand{\partition}{\mathrm{I}}
% \newcommand{\subgroup}{\mathrm{U}}
\newcommand{\subgroupProbability}{\gamma}
%\newcommand{\subgroupLabelProbability}{\psi}
\newcommand{\transpose}{\mathsf{T}}
\newcommand{\empirical}{\mathrm{emp}}
\newcommand{\distributionBound}{A}
\newcommand{\graph}{G}
\newcommand{\vertexSet}{V}
\newcommand{\vertex}{v}
\newcommand{\vertexCount}{k}
\newcommand{\edgeSet}{E}
\newcommand{\cost}{c}
\newcommand{\stateSpace}{\mathcal{S}}

\newcommand{\encoding}{\vec{y}}

\renewcommand{\vec}{\bm}
\newcommand{\randomVariable}{X}
\newcommand{\randomVariableInstance}{x}
\newcommand{\bernoulliParameter}{p}
\newcommand{\placeholderCount}{m}
\newcommand{\errorTolerance}{\epsilon}
\newcommand{\relativeErrorTolerance}{\eta}
\newcommand{\errorConfidence}{\delta}
\newcommand{\martingaleDifference}{c}
\newcommand{\BernoulliDistribution}{\mathrm{Bernoulli}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2
}
\newcommand{\infdiv}{D\infdivx}
\newcommand{\scratchVariable}{q}
\newcommand{\event}{A}
\newcommand{\decisionFunction}{\sigma}
\newcommand{\hoeffding}{thm:hoeffding}
\newcommand{\placeholderSample}{Q}
\newcommand{\sampleElement}{x}
\newcommand{\labelElement}{y}
\newcommand{\weightsElement}{w}

\newcommand*\rect[1]{
    \tikz[baseline=(char.base)]{
        \node[inner sep=8pt, minimum size=1cm] (char) {#1};
        \draw (char.north west) -- (char.south west) -| (char.north east);
        }
}
\newcommand{\poissonRate}{\lambda}
\newcommand{\PoissonDistribution}{\mathrm{Poisson}}
\newcommand{\bigOh}{O}
\newcommand{\bigOmega}{\Omega}

\newcommand{\unifalg}{\mathrm{unif-alg}}

\newcommand{\loss}{\ell}
\newcommand{\regularizedGammaFunction}{Q}
\newcommand{\GammaFunction}{\Gamma}
\newcommand{\lossContribution}{L}

\newcommand{\labelFunction}{\hat{\sigma}}
\newcommand{\indicatorFunctionInstance}{\zeta}
\newcommand{\period}{T}

\newcommand{\sampleSpace}{\mathcal{X}}
\newcommand{\labelSpace}{\mathcal{Y}}
\newcommand{\sampleDist}{\mathcal{D}}
\newcommand{\drawnFrom}{\sim}
\newcommand{\fairnessMetric}{\mathcal{F}}
\newcommand{\multicalibration}{\mathrm{mc}}
\newcommand{\metricEmbeddingNetwork}{\mathrm{f}}
\newcommand{\nearestNeighborClassifier}{\mathrm{H}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\centroid}{\vec{c}}

\newcommand{\MLE}{\psi}
\newcommand{\PDF}{p}
\newcommand{\calibrationError}{\mathrm{c}}
\newcommand{\empiricalCalibrationError}{\hat{\mathrm{c}}}
\newcommand{\Frobenius}{F}
\newcommand{\classifier}{\mathrm{f}}
\newcommand{\hypothesisModule}{\moduleClassifier}
\newcommand{\classifierPlaceholder}{\psi}
\newcommand{\scalarBound}{B}
\newcommand{\spectralBound}{s}
\newcommand{\normBound}{b}
\newcommand{\normalDist}{\mathcal{N}}

\newcommand{\opt}{*}
\newcommand{\svm}{\mathrm{SVM}}

\newcommand{\moduleScalar}{\alpha}
\newcommand{\blockScalar}{\moduleScalar}
\newcommand{\convexHullOperator}{\mathrm{conv}}
\newcommand{\composeOperator}{\circ}
\newcommand{\greekScalar}{\lambda}
\newcommand{\placeholderScalar}{\alpha}
\newcommand{\metricEntropy}{\Phi}

\newcommand{\rp}{\mathrm{rp}}

\newcommand{\zeroVector}{\vec{0}}
\newcommand{\sampleComplexity}{m}
\newcommand{\metric}{\rho}
\newcommand{\setVar}{Y}
\newcommand{\setVarElement}{y}
\newcommand{\protectedTrainingData}{\trainingData_{\mathrm{pro}}}
\newcommand{\rademacherRV}{\sigma}
\newcommand{\variance}{\mathrm{Var}}
\newcommand{\covariance}{\mathrm{cov}}
\newcommand{\openBall}{B}

\newcommand{\learningAlgorithm}{\mathcal{A}}
\newcommand{\boost}{\textrm{boost}}

\newcommand{\probabilityDensityFunction}{f}
\newcommand{\differential}{\mathrm{d}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\probabilityVar}{q}
\newcommand{\badGroups}{\mathtt{badGroups}}
\newcommand{\goodGroups}{\mathtt{goodGroups}}

\newcommand{\powerSet}{{P}}
% \DeclareMathOperator{\E}{\mathbb{E}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\E}{\mathop{\mathbb{E}}}

\renewcommand{\Pr}{\mathop{\mathbb{P}}}
\newcommand{\thmOne}{thm:one}
\newcommand{\thmTwo}{thm:Two}
\newcommand{\corThmTwo}{cor:two}
\newcommand{\intersection}{\cap}

\newcommand{\functionPlaceholder}{\beta}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\numInterestingCategories}{C}
\newcommand{\interestingCategory}{c}
\newcommand{\listInterestingCategories}{\mathcal{C}}

\newcommand{\given}{\mid}

\newcommand{\metricEntropyRadius}{\epsilon}
\newcommand{\q}{q}
\newcommand{\qDual}{r}
\newcommand{\functionComposition}{F}
\newcommand{\function}{G}
\newcommand{\sampleInfNormUB}{r_{\infty}}
\newcommand{\weightsOneNormUB}{\Lambda}
\newcommand{\finalLinearClassifierOneNormUB}{C_{0}}
\newcommand{\rademacherComplexity}{\mathcal{R}}

\newcommand{\blockOutput}{o}
\newcommand{\blockIter}{t}
\newcommand{\blockFunction}{f}
\newcommand{\moduleIter}{\blockIter}
\newcommand{\placeholderInt}{n}
\newcommand{\depth}{T}
\newcommand{\depthIter}{t}
\newcommand{\indicatorFunction}{\mathbbm{1}}
\newcommand{\entropy}{H}
\newcommand{\kernel}{\kernelFunction}
\newcommand{\threshold}{\tau}
\newcommand{\blockError}{\gamma}
\newcommand{\learningCondition}{\eta}
\crefname{fact}{fact}{facts}

\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\curlyBrace}{\{}{\}}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\innerProduct}{\langle}{\rangle}

\newcommand{\BoostResNet}{\mathrm{BoostResNet}}
\newcommand{\groupDist}{\vec{\pi}}
\newcommand{\minNumSamples}[1]{N_{\min,#1}}
\newcommand{\sample}{\vec{\sampleElement}}


\newcommand{\sampleProtected}{\sampleElement_{\protectedIndex}}
\newcommand{\sampleUnprotected}{\sample_{\unprotectedIndices}}
\newcommand{\hypothesisModuleSum}[2]{s_{#1:#2}}

\newcommand{\bigTheta}{\Theta}
\newcommand{\costMatrix}{\vec{C}}
\newcommand{\fairnessCostMatrix}{\vec{F}}

\newcommand{\weights}{\vec{\weightsElement}}
\newcommand{\sumHypothesisModules}{H}

\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\positiveIntegers}{\mathbb{Z}^+}

\newcommand{\mutualInformation}{\mathrm{I}}

\newcommand{\faithfulParameter}{\phi}

\newcommand{\dimension}{d}
\newcommand{\trainingData}{S}
\newcommand{\evalutationData}{\evaluationData}
\newcommand{\evaluationData}{T}
\newcommand{\margin}{\theta}
\newcommand{\placeholderConstant}{\alpha}
\newcommand{\Representativeness}{\mathrm{Rep}}

\newcommand{\unlabeledTrainingData}{Q}
\newcommand{\marker}{\dagger}
\newcommand{\bigIntersection}{\bigcap}
\newcommand{\bigUnion}{\bigcup}
%\newcommand{\risk}{R}
\newcommand{\numSamples}{N}
\newcommand{\numSamplesComplement}{N^c}
\newcommand{\placeholderSet}{\mathcal{V}}
\newcommand{\placeholderDist}{\mathcal{Q}}
\newcommand{\placeholderRandomVariable}{X}
\newcommand{\placeholderRandomVariableInstance}{x}
\newcommand{\boostDist}{D}
\newcommand{\placeholder}{z}
\newcommand{\protectedIndex}{1}
\newcommand{\unprotectedIndices}{2:\dimension}
\newcommand{\dimensionUnprotected}{\dimension-1}
\newcommand{\risk}{\mathcal{L}}
\newcommand{\hyp}{\mathrm{h}}
\newcommand{\hypMultiClass}{H}
\newcommand{\hypothesisClass}{\mathcal{H}}
\newcommand{\definedAs}{\triangleq}
\newcommand{\placeholderFunction}{f}
\newcommand{\kernelFunction}{K}
\newcommand{\kernelMapping}{\Phi}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\union}{\cup}
\newcommand{\support}{\mathrm{supp}}
\newcommand{\hilbertSpace}{\mathbb{H}}
\newcommand{\graphDimension}{\mathrm{d}}
\newcommand{\groupA}{\mathsf{a}}
\newcommand{\groupB}{\mathsf{b}}
\newcommand{\predictionValue}{v}
\newcommand{\groupWeight}{\alpha}
\newcommand{\group}{\mathsf{g}}
\newcommand{\groups}{\mathsf{G}}
\newcommand{\placeholderGroup}{\mathsf{g}}
\newcommand{\interval}{\mathrm{I}}
\newcommand{\mat}{\bm}
\newcommand{\faceRecognitionSystem}{\mathrm{G}}
\newcommand{\frs}{\faceRecognitionSystem}
\newcommand{\neuralNetwork}{\mathrm{NN}}
\newcommand{\nonlinearity}{\sigma}
\newcommand{\pca}{\mathrm{f}}
\newcommand{\subGaussian}{\mathsf{subG}}
\newcommand{\proxyStandardDeviation}{\sigma}
\newcommand{\tcavScore}{T}
\newcommand\MTkillspecial[1]{% helper macro
\bgroup
\catcode`\&=9
\let\\\relax%
\scantokens{#1}%
\egroup
}
\DeclarePairedDelimiter\brparen
\lparen\rparen
\reDeclarePairedDelimiterInnerWrapper\brparen{star}{
\mathopen{#1\vphantom{\MTkillspecial{#2}}\kern-\nulldelimiterspace\right.}
#2
\mathclose{\left.\kern-\nulldelimiterspace\vphantom{\MTkillspecial{#2}}#3}}
\DeclarePairedDelimiter{\angleBracket}{\langle}{\rangle}
\newcommand{\dotProduct}[2]{\angleBracket{#1,#2}}
\newcommand{\perturbedExample}{\Delta}
\newcommand{\getPerturbation}{\Delta}
\newcommand{\embeddingFunc}{\mathrm{f}} 
\newcommand{\perturbation}{\vec{\delta}}
\newcommand{\likelihood}{L}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\standardDev}{\sigma}
\newcommand{\hinge}{\mathrm{G}}
\newcommand{\covarianceContribution}{\mathrm{C}}
